Xiezhi: An Ever-Updating Benchmark for Holistic Domain Knowledge Evaluation

New Natural Langauge Process~(NLP) benchmarks are urgently needed to align with the rapid development of large language models (LLMs). We present Xiezhi, the most comprehensive evaluation suite designed to assess holistic domain knowledge. Xiezhi comprises multiple-choice questions across 516 diverse disciplines ranging from 13 different subjects with 249,587 questions and accompanied by Xiezhi-Specialty and Xiezhi-Interdiscipline, both with 15k questions. We conduct evaluation of the 47 cutting-edge LLMs on Xiezhi. Results indicate that LLMs exceed average performance of humans in science, engineering, agronomy, medicine, and art, but fall short in economics, jurisprudence, pedagogy, literature, history, and management. We anticipate Xiezhi will help analyze important strengths and shortcomings of LLMs, and the benchmark is released in~\url{https://github.com/MikeGu721/XiezhiBenchmark}.

==> 00CoverLetter.tex <==


\clearpage



\section*{To Reviewer \#1:}

\noindent \myblue{\textbf{[R1-W1] Is your use of ChatGPT legal?}}

\noindent \textbf{[Response]} 

\textbf{It is legal}.
Usage of the data entirely generated by ChatGPT or GPT-4 for commercial purposes is not permitted.
However, the following actions are permissible:
\begin{enumerate}
\item Utilizing data generated by GPT to train models and then open-sourcing these models. 
Examples of such work include 
``RefGPT: Reference-$\rightarrow$ Truthful \& Customized Dialogues Generation by GPTs and for GPTs'',
``Baize: An Open-Source Chat Model with Parameter-Efficient Tuning on Self-Chat Data'',
and ``\url{https://github.com/LianjiaTech/BELLE}''.
\item Employing GPT to assist in data filtering and annotation. Examples of such work include:
``RoleLLM: Benchmarking, Eliciting, and Enhancing Role-Playing Abilities of Large Language Models'',
``Character-LLM: A Trainable Agent for Role-Playing'' or
``Does Role-Playing Chatbots Capture the Character Personalities? Assessing Personality Traits for Role-Playing Chatbots''
\end{enumerate}
We have open-sourced the complete dataset of Xiezhi and commit to open-sourcing the annotation model trained by Xiezhi-Meta (it is not currently open-sourced due to its effective performance, which still requires substantial human annotation).
Therefore, we have not only open-sourced the model but also utilized GPT solely for data annotation. 
Both the data collection and post-processing were conducted manually.


% 完全使用GPT生成的数据是不被允许用于商业用途的训练。
% 但下列行为都是可以的：
% 1. 使用GPT生成的数据，训练模型，并将模型开源。类似的工作有：``RefGPT: Reference-> Truthful \& Customized Dialogues Generation by GPTs and for GPTs'', ``Baize: An Open-Source Chat Model with Parameter-Efficient Tuning on Self-Chat Data'' or ``https://github.com/LianjiaTech/BELLE''.
% 2. 使用GPT协助数据过滤、标注。

% 在Xiezhi的工作中，我们将Xiezhi完整的数据集已经开源，并且承诺会将Xiezhi-Meta训练的标注模型开源（现在未开源，是因为效果还比较有效，依然需要大量的人力参与标注）

\noindent \myblue{\textbf{[R1-W2] How can you ensure your results are reproducible in the long term?}}

\noindent \textbf{[Response]} 

It is easy to reproduce the evaluation results obtained in our experiment using Xiezhi.
We have included the relevant code with all the random seed in it in our submission, which ensure that the reproducible results of our experiments.

Upon reviewing the Weakness written by the reviewer, we think reviewer may have concern in how to reproduce the labeling process of Xiezhi, which we use GPT-API mainly.
All works utilizing GPT-API currently suffer from irreproducibility, including the labeling process of Xiezhi.
We have upload all data of Xiezhi to the submission to ensure the reproducibility.
Nevertheless, we believe that by following the methodology outlined in our paper, we can still provide high-quality labeling for disciplinary data.



\noindent \myblue{\textbf{[R1-W3] Xiezhi is not suitable for AAAI-2024}}

\noindent \textbf{[Response]} 

We regret that you this conclusion.
We believe that Xiezhi not only encompasses a significant amount of engineering work but primarily explores how to effectively evaluate large language models.
The main research in this paper include (1) which type of benchmark do we need, and (2) what kind of metrics do we need.

Similar benchmark construction papers accepted by AAAI-2023 include: 
``RGBD1K: A Large-Scale Dataset and Benchmark for RGB-D Object Tracking'' and ``FakeSV: A Multimodal Benchmark with Rich Social Context for Fake News Detection on Short Video Platforms''. 
We are puzzled as to why ``RGB Object Tracking'' and ``Fake News Detection'' can be considered scientific questions, while our exploration of ``how to effectively evaluate LLM'', a great concern in the era of LLMs, is thought not a research proposal but merely engineering work.

We hope the reviewer note that while we have indeed undertaken a substantial amount of engineering work, it is all centered around a meaningful scientific question.
Xiezhi, focusing on the scientific question of ``how to effectively evaluate LLM'', has constructed a high-quality benchmark, proposed new evaluation metrics, and detailed the differences between traditional evaluation methods and current ones.
This provides a fresh perspective on LLM evaluation and conducts an extremely detailed evaluation and analysis of current mainstream models.

\section*{To Reviewer \#2:}

\noindent \myblue{\textbf{[R2-W1] Chinese Bias}}

\noindent \textbf{[Response]} 

We have devoted substantial time, manual efforts, and financial investment to eliminate all ethical or bias concerns, including Chinese Bias. 

In terms of the Chinese Bias, we believe that there is no bias issue between Chinese and English for most of the questions since they are most knowledge-based, such as those related to ship design, finance, and so forth. 
Regarding the issue of Chinese idioms raised by the reviewer, we initially utilized a Chinese translation API, which understand Chinese idioms well, to translate all the questions into English, while also mobilizing a significant amount of manual effort to inspect any potential Chinese Bias.

The reason for not labeling ``Chinese Centric'' in title is because the goal of Xiezhi is to become a comprehensive, unbiased knowledge assessment benchmark that covers all fields.
It would be unjust to think Xiezhi is Chinese bias simply because we adopted Chinese academic classification standards and questions.
MMLU, which is also a well-known benchmark in the world, has adopted a large number of American exam questions, yet the academic community still don't regards it is American bias.

We are highly confident in our handling of potential bias issues in our benchmark, which is why we have submitted it.
If you have objections to our bench, you should, like the reviewers in NeurIPS-2023, directly point out the issues in our benchmark, rather than making speculations.

\noindent \myblue{\textbf{[R2-W2] Will there be updates in terms of tasks ? Or domains ? That is not clear. But in due course that will be something that would be helpful.}}

\noindent \textbf{[Response]} 

We will continuously update the tasks and domains within the Xiezhi benchmark to ensure that the questions encapsulated in Xiezhi remains ahead of the training data used by LLMs.



% 我们对两位审稿人的意见表示震惊。
% 所以给SPC写下以下confidential comments。

% Reviewer #1的审稿意见相对稍好一些，但他对大模型研究的现状不清楚，以至于会写出一些不符合现状的weakness。
% 1. Reviewer认为，构建的benchmark应当具有可复现性。而几乎所有构建benchmark的工作，都不会考虑benchmark的可复现性，而正是因为构建benchmark的不可复现性，所以构建benchmark才会有巨大的价值。
% 2. Reviewer认为我们的工作不具有research proposal。我不清楚reviewer是为什么会说，但我们的工作有着非常明确的科研目标——探究怎样才能准确地评估LLM的能力。
% 关于Reviewer #1的其他concern，如使用ChatGPT是否合法的问题，我们都在response PDF里进行了解释。

% 而我们认为，Rivewer #2的审稿意见简直不可理喻。
% 我们认为Reviewer #2的审稿意见有着很强的歧视意味，因为他仅仅是因为我们使用了中国教育部颁布的学科分类体系来构建benchmark而认为我们的benchmark具有很强的bias。
% 审稿人的原话如下：
% ``The paper is highly biased by a national educational taxonomy... While the discipline based taxonomy is based in China, it is not a widely accepted practice.''
% 事实上，我们考虑到可能会存在的Chinese Bias问题，我们组织了大量的人力来消除包括Chinese Bias在内的所有可能的Ethical Problem和偏见。
% 我们对Xiezhi Benchmark非常自信，因此我们将所有的代码、数据集上传。
% 希望审稿人如果有意见，能够像NeurIPS-2023的审稿人一样，指出我们数据集中具体哪里存在什么样的偏见。
% 我们认为Reviewer #2的无端猜想和污蔑是不可接受的，Xiezhi是许多人一起努力的心血，他这样的评论是对我们工作的一种诋毁。


% We are astonishing at the comments made by the two reviewers, especially Reviewer #2, and thus, we are writing the following confidential comments to the SPC.

% Reviewer #1 may lack of understanding of the current state of LLM research, which has led to some glaring errors made in his comments:
% 1. The reviewer suggests that the constructed benchmark should be reproducible. However, almost all benchmark construction work does not consider the reproducibility of the benchmark. And irreproducibility is one of the reason why benchmark works are valuable.
% 2. The reviewer believes our work lacks a research proposal, so our work is only a great engineer work. However, we are unclear why the reviewer would make such a statement, but our work has a very clear research objective: how to accurately assess the capabilities of LLMs. 
% As for other comments, such as the legality of using ChatGPT, we have made further explanations in the feedback PDF file.

% As for Reviewer #2, we think his/her comments is utterly unreasonable.
% We perceive a strong discriminatory undertone in Reviewer #2's comments, as he/she seems to suggest that our benchmark is highly biased simply because we construct the benchmark based on the subject classification system raised by the Chinese Ministry of Education. 
% The reviewer's comments were: ``The paper is highly biased by a national educational taxonomy... While the discipline based taxonomy is based in China, it is not a widely accepted practice.''
% In fact, we anticipated potential issues of Chinese Bias and organized a significant amount of manpower to eliminate all possible ethical problems and biases, including Chinese Bias.
% We have great confidence in the Xiezhi Benchmark, which is why we have submitted all the code and datasets.
% If the reviewer has any objections, he/she should point them out in our dataset, just like the reviewers of NeurIPS-2023, rather than making speculation only based on the source of our data.
% Xiezhi is the result of the hard work from many individuals, and such comments are a denigration of our work.


==> 075BiasEthical.chn.tex <==
尽管我们努力地避免所有可能的道德问题，但作为目前世界上规模最大，学科标签数最多的知识性评估benchmark，且极大程度地从单一语种中收集并构建起来的数据集，我们还是很难保证所有的道德问题都被解决。
我们在这一章节将就我们数据集中可能存在的所有道德问题，以及我们是如何解决的进行详细描述。

\subsection{Bias From Multilingual Dataset Curation}
作为从中文数据源构建起来的数据集，以及邀请的标注者都为中国人，这样的数据集或多或少都会存在中文倾向。
其中，我们花费了大量的精力来尽可能地消除数据集中的中文倾向性。
具体包含以下一些方法：
\begin{itemize}
    \item 从Xiezhi-All中尽可能地选择涉及各个国家各个地区的题目，而不是选择中文倾向的题目。
    \item 尽可能地保证中文和英文风格的虚拟人名分布平均，如中文中的Li Hua，英文中的Mike。
    \item 将涉及政治立场的问题删除。
    \item 涉及中国人常见的价值观的问题中，我们加上诸如“In Chinese”之类的修饰定语。
\end{itemize}
但即便我们做了很多的工作来缓解数据的中文Bias，我们认为可能还有一种Chinese Bias的问题存在。
尽管我们在涉及中文价值观的题目中加上了修饰定语，并且在构建Xiezhi-Speciality和Xiezhi-Interdisciplinary的时候尽可能选择包含世界各地区不同价值观的题目，但包含中国特有价值观题目的总体数量依然偏多。

\subsection{Translation Version of Xiezhi}
在本文中，我们使用了Google Translate的API将Xiezhi-Speciality和Xiezhi-Interdisciplinary翻译为了英语。
而后进行了大量的人工后验，主要检验内容包括以下几个方面：
\begin{itemize}
    \item 修正翻译错误
    \item 修正表达不流畅的语句
    \item 修正对于特定术语的表达
\end{itemize}
我们邀请了在小节~\ref{a3}详述的10位标注者参与Xiezhi英语版的修订，这10为标注者都是研究生，且都在读研时候发表了英文论文，因此我们认为他们对于专业知识和英语能力都有较高的水平。
我们对翻译版具有很高的要求，但即便如此，我们依然认为当前版本的Xiezhi中可能存在以下问题。
\begin{itemize}
    \item 标注者并非在英语国家生活的native speaker，因此在表达上可能依然不够地道。
    \item 因为数据集涉及了512个不同领域的学科，虽然标注者都为具有英文写作经验的研究生，但依然对于领域术语的翻译会不够精准。
\end{itemize}


\subsection{Human Performance}
我们在正文中详述了人类得分的统计方式。
值得一提的是，这种算分方法是一种妥协。
主要原因是单纯只获取某一个来源的学科数据数量过少，且极其有偏。
而且因为各个数据集所包含的领域内容差别太大，因此我们也难以邀请来自全部512个领域的专业人士提供人类baseline结果。
我们认为，目前我们提供的human performance分数能一定程度上体现了人类在Xiezhi-Speciality和Xiezhi-Interdisciplinary上的表现，但也希望真实的社会决策者们不要依赖这个分数做出决策。


\subsection{Gender, Race, Religion, National Discrimination or Prejudice}
考虑到benchmark的提出将会在一段时间内为大模型的训练效果提供度量指标。
如果benchmark本身包含有歧视、偏见内容，将会诱导大模型向着非常不好的方向发展。
因此，我们严格遵从NeurIPS的数据集审核标准，在Xiezhi-Specility和Xiezhi-Interdisciplinary的后验过程中尽可能地消除了所有和性别、种族、宗教、国家歧视或偏见相关的内容。
从我们在表~\ref{tab:example_in_annotation}中列出的要求可以见到我们对于消除偏见和歧视所做出的努力。

尽管如此，考虑到我们的大量的题目都是从中文考试题中获取的，以及少量的题目是从英文论文中生成来的，并且我们的标注团队都是中国的研究生，因此，Xiezhi数据集依然可能存在以下一些道德隐患。
\begin{itemize}
    \item 由于我们的题目来源于中文考试题和英文论文，而我们的标注者也是中国的研究生，这可能会使得标注的数据偏向于东方的或者西方的一种文化观念而标注者没有发觉。
    \item 考虑到各个性别、种族、信仰、国家在能够获取的题目中的分布极其不均匀而导致的有偏，我们在Xiezhi
    -Speciality和Xiezhi-Interdisciplinay中努力解决了不同性别的分布问题。而种族、信仰、国家所带来的隐含的偏见可能比性别更严重，我们尽可能地保证我们已有的题目不会在题目描述和答案中出现偏见内容，但对于整体的题目分布而言却无能为力。
\end{itemize}








==> 078XiezhiTrain.tex <==
Xiezhi-Train内包含了Xiezhi-Interdiscipline和Xiezhi-Speciality两种构建方法所得来的题目。
具体而言Xiezhi-Train包含了一道题目只有一个标签的共




==> different_models_performance_table.tex <==

\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|cccccccccccc}
        \toprule
        Method & \#ift& phi. & eco. & law & edu. & lit. & his. & sci. & eng. & agr. & med. & man. & arts \\
        \hline
        % &\multicolumn{13}{c}{Bloomz-7B} \\
        Bloomz-7b1-mt & 65M & 0.127 & 0.189 & 0.194 & 0.222 & 0.124 & 0.180 & 0.218 & 0.189 & 0.215 & 0.214 & 0.159 & 0.073   \\
        Bloomz-7b1 & 79M & 0.255 & \textbf{0.308} & 0.247 & 0.382 & \textbf{0.290} & \textbf{0.277} & 0.239 & 0.157 & 0.167 & 0.357 & 0.232 & 0.304  \\
        Belle-0.2M & 65.2M & 0.240 & 0.266 & 0.245 & 0.308 & 0.259 & 0.257 & 0.296 & 0.301 & 0.063 & 0.273 & 0.208 & \textbf{0.417}    \\
        Belle-0.6M & 65.6M & 0.259 & 0.258 & 0.248 & 0.289 & 0.271 & 0.245 & 0.255 & 0.218 & 0.037 & 0.242 & 0.200 & 0.316 \\
        Belle-1M & 66M & 0.018 & 0.063 & 0.080 & 0.055 & 0.066 & 0.092 & 0.123 & 0.090 & 0.132 & 0.097 & 0.068 & 0.048  \\
        Belle-2M & 67M & 0.018 & 0.032 & 0.040 & 0.042 & 0.025 & 0.070 & 0.064 & 0.067 & 0.099 & 0.068 & 0.045 & 0.049  \\
        \hline
        % &\multicolumn{13}{|c}{LLaMA-7B} \\
        Llama-7B & - & 0.364 & 0.232 & 0.239 & 0.300 & 0.198 & 0.237 & 0.261 & 0.185 & 0.467 & 0.192 & 0.310 & 0.238 \\
        Luotuo & 0.15M & - & - & - & - & - & - & - & - & - & - & - & -   \\
        Alpaca & 0.05M  & - & - & - & - & - & - & - & - & - & - & - & -  \\
        Vicuna & 0.07M & - & - & - & - & - & - & - & - & - & - & - & - \\
        Baize & 0.16M & 0.036 & 0.011 & 0.032 & 0.097 & 0.057 & 0.045 & 0.017 & 0.041 & 0.066 & 0.039 & 0.045 & 0.098  \\
        Baize-Health & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        \hline
        % &\multicolumn{13}{|c}{LLaMA-7B} \\
        Llama-13B & - & 0.111 & 0.071 & 0.073 & 0.105 & 0.045 & 0.064 & 0.056 & 0.118 & 0.067 & 0.077 & 0.020 & 0.025  \\
        Koala & 0.47M & - & - & - & - & - & - & - & - & - & - & - & -  \\
        Alpaca & 0.05M & - & - & - & - & - & - & - & - & - & - & - & - \\
        Vicuna & 0.07M & - & - & - & - & - & - & - & - & - & - & - & - \\
        Baize & 0.16M &  \\
        \hline
        Moss-16B & -    \\
        Moss-SFT &  1.1M & 0.015 & 0.050 & 0.032 & 0.056 & 0.033 & 0.019 & 0.030 & 0.026 & 0.017 & 0.030 & 0.023 & 0.024  \\
        \hline
        % &\multicolumn{13}{|c}{Others} \\
        Pythia-6.9B & - & \textbf{0.027} & \textbf{0.023} & \textbf{0.052} & 0.029 & 0.044 & 0.046 & \textbf{0.027} & \textbf{0.020} & \textbf{0.031} & \textbf{0.016} & \textbf{0.015} & \textbf{0.083}  \\
        H2Ogpt & 0.26M & 0.020 & 0.021 & 0.028 & \textbf{0.038} & \textbf{0.089} & \textbf{0.067} & 0.013 & 0.014 & 0.024 & 0.011 & 0.010 & 0.025  \\
        \hline
        ChatGLM-6B & 0.26M & 0.239 & 0.206 & 0.195 & 0.158 & 0.202 & 0.221 & 0.235 & 0.127 & 0.182 & 0.278 & 0.250 & 0.188  \\
        ChatGLM-Med & 0.26M & - & - & - & - & - & - & - & - & - & - & - & - \\
        DoctorGLM & 0.26M & 0.163 & 0.164 & 0.206 & 0.341 & 0.218 & 0.233 & 0.239 & 0.141 & 0.364 & 0.308 & 0.305 & 0.130  \\
        \hline
        Students-Average~\footnote{Results come from \url{https://zhuanlan.zhihu.com/p/430201117}} & - & 0.397 & 0.461 & 0.428 & 0.438 & 0.516 & 0.423 & 0.379 & 0.354 & 0.323 & 0.400 & 0.390 & 0.361   \\
        Students-High~\footnote{Results come from \url{https://www.dxsbb.com/news/67598.html}} & - & 0.453 & 0.520 & 0.460 & 0.510 & 0.560 & 0.460 & 0.394 & 0.380 & 0.333 & 0.430 & 0.513 & 0.400   \\
        Students-Top~\footnote{Results are sampled from the highest scores of the enrolled students of top 2 universities in China} & - & 0.856 & 0.871 & 0.761 & 0.854 & 0.825 & 0.854 & 0.926 & 0.928 & 0.902 & 0.805 & 0.857 & 0.821   \\
        \bottomrule
    \end{tabular}
    }
    \caption{Result on Xiezhi-Easy}
    \label{tab:detailedModelsPerformance}
\end{table*}

% 哲学 {'mean': 0.0, 'std': 0.0, 'num': 55}
% 经济学 {'mean': 0.05263157894736842, 'std': 0.22329687826943603, 'num': 95}
% 法学 {'mean': 0.03225806451612903, 'std': 0.17668469596940847, 'num': 124}
% 教育学 {'mean': 0.05555555555555555, 'std': 0.2290614236454256, 'num': 72}
% 文学 {'mean': 0.03305785123966942, 'std': 0.17878766655193337, 'num': 121}
% 历史学 {'mean': 0.01893939393939394, 'std': 0.13631101678368623, 'num': 528}
% 理学 {'mean': 0.029914529914529916, 'std': 0.1703515506666218, 'num': 234}
% 工学 {'mean': 0.025906735751295335, 'std': 0.15885709551042373, 'num': 386}
% 农学 {'mean': 0.01652892561983471, 'std': 0.12749792248381414, 'num': 121}
% 医学 {'mean': 0.02912621359223301, 'std': 0.1681602725795026, 'num': 103}
% 管理学 {'mean': 0.022727272727272728, 'std': 0.14903269373413638, 'num': 44}
% 艺术学 {'mean': 0.024390243902439025, 'std': 0.1542574468374819, 'num': 41}


% \begin{table*}
%     \small
%     \centering
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
%         \hline
%         \multirow{2}{*}{Model} & \multicolumn{5}{c|}{GLUE} & \multicolumn{5}{c|}{CLUE}\\
%         & \textbf{SST-2} & \textbf{MRPC} & \textbf{QQP} & \textbf{MNLI-mm} & \textbf{RTE} & \textbf{AFQMC} & \textbf{TNEWS} & \textbf{IFLYTEK} & \textbf{CMNLI} & \textbf{CSL}\\
%         \hline
%         Bert-base & \cellcolor{lime}89.36 & 85.14 & 67.33 & \cellcolor{green}\textbf{83.10} & 62.85 & \cellcolor{lime}71.59 & 54.74 & 56.48 & \cellcolor{green}\textbf{78.43} & 78.73\\

%         \cellcolor{yellow} -BT & \cellcolor{yellow} 93.5 & \cellcolor{yellow} 88.9 & \cellcolor{yellow} 71.2 & \cellcolor{yellow} 83.4 & \cellcolor{yellow} 66.4 & \cellcolor{yellow} 73.70 & \cellcolor{yellow} 56.58 & \cellcolor{yellow} 60.29 & \cellcolor{yellow} 79.69 & \cellcolor{yellow} 80.36 \\
        
%         +EDA &89.14&84.16&65.68&80.47&62.71&70.17&52.42&55.14&75.65&76.74\\
        
%         +LIBERT &86.48&\cellcolor{lime}85.29$\uparrow$&\cellcolor{lime}69.71$\uparrow$&81.12&\cellcolor{lime}64.51$\uparrow$&70.29&53.27&\cellcolor{lime}56.74$\uparrow$&74.33&77.49\\
        
%         % +SAPBERT & 16.42 & 83.91 & 80.23 & 80.17 & 76.54 & 49.37 & 64.96 & 50.83 & 53.78 & 68.91 & 70.18\\
        
%         +PICSO &88.47&84.69&\cellcolor{green}\textbf{70.34}$\uparrow$&82.11&63.56$\uparrow$&71.43&\cellcolor{lime}55.48$\uparrow$&55.40&74.19&\cellcolor{lime}79.16$\uparrow$\\
        
%         +Sem4SAP $\uparrow$ & \cellcolor{green}\textbf{92.89}$\uparrow$ & \cellcolor{green}\textbf{88.41}$\uparrow$ & 69.15$\uparrow$ & \cellcolor{lime}83.08 & \cellcolor{green}\textbf{65.16}$\uparrow$ &
%         \cellcolor{green}\textbf{73.54}$\uparrow$ & \cellcolor{green}\textbf{\underline{\underline{56.82}}}$\uparrow$ & \cellcolor{green}\textbf{\underline{\underline{60.38}}}$\uparrow$ & \cellcolor{lime}78.41 & \cellcolor{green}\textbf{\underline{\underline{81.22}}}$\uparrow$\\
       
        
%         \hline
%         Roberta-base & \cellcolor{lime}92.36 & \cellcolor{lime}86.41 & 68.45 & \cellcolor{lime}84.78 & \cellcolor{lime}64.37 & \cellcolor{lime}70.87 & 55.53 & 56.52 & \cellcolor{lime}79.45 & 78.20\\

%         \cellcolor{yellow} -BT & \cellcolor{yellow} 94.6 & \cellcolor{yellow} 89.8 & \cellcolor{yellow} 71.5 & \cellcolor{yellow} 85.2 & \cellcolor{yellow} 67.3 & \cellcolor{yellow} 74.45 & \cellcolor{yellow} 57.12 & \cellcolor{yellow} 60.88 & \cellcolor{yellow} 80.17 & \cellcolor{yellow} 80.59 \\
        
%         +EDA &91.78&86.04&67.14&83.45&62.51&69.43&53.48&55.67&76.64&76.31\\
        
%         +LIBERT &86.91&86.13&69.38$\uparrow$&82.47&63.35&70.05&53.44&\cellcolor{lime}56.91$\uparrow$&74.46&74.84\\
        
%         % +SAPBERT & 16.42 & 83.91 & 80.23 & 80.17 & 76.54 & 49.37 & 64.96 & 50.83 & 53.78 & 68.91 & 70.18\\
        
%         +PICSO &91.56&85.43&\cellcolor{green}\textbf{72.22}$\uparrow$&82.35&62.19&68.51&\cellcolor{lime}56.41$\uparrow$&56.17&75.43&\cellcolor{lime}79.14$\uparrow$\\
        
%         +Sem4SAP& \cellcolor{green}\textbf{93.13}$\uparrow$ & \cellcolor{green}\textbf{87.17}$\uparrow$ & \cellcolor{lime}71.48$\uparrow$ & \cellcolor{green}\textbf{84.96}$\uparrow$ & \cellcolor{green}\textbf{66.35}$\uparrow$ &
%         \cellcolor{green}\textbf{73.51}$\uparrow$ & \cellcolor{green}\textbf{\underline{\underline{57.34}}}$\uparrow$ & \cellcolor{green}\textbf{60.70}$\uparrow$ & \cellcolor{green}\textbf{\underline{\underline{80.35}}}$\uparrow$ & \cellcolor{green}\textbf{\underline{\underline{81.28}}}$\uparrow$\\


        
%         \hline
%         Roberta-large & 93.17 & \cellcolor{lime}90.54 & 87.60 &\cellcolor{green}\textbf{ 89.45} & \cellcolor{lime}86.34 &72.84 & 57.15 & \cellcolor{lime}59.79 & \cellcolor{green}\textbf{81.11} & 80.10\\

%         \cellcolor{yellow} -BT & \cellcolor{yellow} 96.7 & \cellcolor{yellow} 92.3 & \cellcolor{yellow} 90.2 & \cellcolor{yellow} 90.2 & \cellcolor{yellow} 88.2 & \cellcolor{yellow} 74.02 & \cellcolor{yellow} 57.86 & \cellcolor{yellow} 62.55 & \cellcolor{yellow} 81.70 & \cellcolor{yellow} 81.36 \\
        
%         +EDA &\cellcolor{lime}93.25$\uparrow$&88.37&86.51&\cellcolor{lime}89.22&85.48&\cellcolor{lime}73.10$\uparrow$&55.42&59.64&80.32&78.61\\
        
%         +LIBERT &89.64&87.14&85.79&86.97&85.29&71.26&56.43&58.32&78.44&79.71\\
        
%         % +SAPBERT & 16.42 & 83.91 & 80.23 & 80.17 & 76.54 & 49.37 & 64.96 & 50.83 & 53.78 & 68.91 & 70.18\\
        
%         +PICSO $\uparrow$&92.48&90.04&89.17$\uparrow$&83.56&85.46&72.43&\cellcolor{lime}57.32$\uparrow$&58.25&76.42&\cellcolor{lime}80.56$\uparrow$\\
        
%         +Sem4SAP & \cellcolor{green}\textbf{96.14}$\uparrow$ & \cellcolor{green}\textbf{91.47}$\uparrow$ & \cellcolor{green}\textbf{89.02}$\uparrow$ & 89.17 & \cellcolor{green}\textbf{87.77}$\uparrow$ & 
%         \cellcolor{green}\textbf{74.25}$\uparrow$ & \cellcolor{green}\textbf{\underline{\underline{57.64}}}$\uparrow$ & \cellcolor{green}\textbf{62.46}$\uparrow$ & \cellcolor{lime}81.04 & \cellcolor{green}\textbf{\underline{\underline{82.41}}}$\uparrow$\\
%         \hline
%     \end{tabular}
%     }
%     \vspace{-2mm}
%     \caption{Overall Experiments on GLUE and CLUE datasets}
%     \label{tab:overallExperiemnt}
    
%     \vspace{-5mm}
% \end{table*}

==> old_version/01Introduction.0.tex <==

\subsection{Background}
领域知识是对于世界的深入的理解，理解领域知识需要抽象能力、推理能力、想象力等诸多能力。
在过去很长的一段时间里，人类在自然语言上对于领域知识的掌握程度要远超任何机器学习模型的能力。
但是近年来，Large Language Models~(LLMs), such as Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}，Gopher~\cite{rae2021gopher}, UL2~\cite{tay2022ul2}, Bard~\cite{pichai2023important} and GPT4~\cite{openai2023gpt4, bubeck2023sparks}在自然语言处理方面表现出了惊人的能力。
这些LLMs在许多涉及领域知识的文本理解上似乎已经达到了人类专家的水平~\cite{wei2022emergent}。
但要让人们相信LLMs在各个领域中能够提供准确的信息，全面且深度地评估模型对于领域知识的掌握程度便尤为重要。


\subsection{Motivation}
无论是在LLMs到来前还是之后，都有许多学者提出过不少用于语言模型评估的benchmark。
诸如GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}，MMLU~\cite{hendrycks2021measuring}在过去很长一段时间为模型在领域上的表现提供了很好的标准，但是现在的LLM在这些benchmark上已经有了远超人类的表现。
近年来提出的BIG-Bench~\cite{srivastava2022bigbench}，HELM~\cite{liang2022holistic}正在成为全新的语言模型评估标准，但是这些benchmark的目标并不是专门针对领域知识进行评估，所以他们只涉及了非常有限的若干个领域维度。
最近，GPT4~\cite{openai2023gpt4, bubeck2023sparks}在两篇论文里为交叉领域的评估提出了一些思路，比如用JavaScript画一头独角兽，或者是用莎士比亚的语言风格证明数学公式，但是这些评估都太过开放，以至于只能使用人工进行结果校验。

除此之外，随着LLMs输出方式的改变，以及所使用的数据规模越来越大，也使得之前的Benchmarks不再适合用来评估最新的LLMs工作。
近年来新出的LLMs多为text-to-text类型的模型，这类模型takes text and generates text probabilistically，所以难以直接生成和ground truth一样的答案，因此如何评估LLMs的输出成为了一个问题。
另外，大模型所使用的语料越来越庞大，最前沿的LLMs，比如GPT-4，所使用的语料几乎已经涵盖了互联网上所有能够找到的开源信息，因此如何保证评估样本不会出现在模型的训练数据中也成为了一个问题。


根据上面所述，我们将前人工作的不足总结如下：
1. 专业领域有限：涵盖的领域知识非常有限，维度不够全面。
2. 没有区分知识深度：没有对领域知识的深度做很好的区分，难以判断模型对于具体领域知识掌握到了什么程度。
3. 存在开放问题：有很多评估是开放性的评估，需要较大的人力开销去检验模型的输出结果。
4. 难以校验模型输出：目前所有的Benchmarks都不适合评估现在text-to-text类型的模型，因为这些模型难以生成和ground truth一模一样的答案。
5. 评估数据集污染：随着各个LLMs所使用的语料越来越庞大，评估用到的数据很可能已经作为LLMs的训练数据，因此便缺少了评估的公平性。


\subsection{Our Works}
因此在本文，我们提出了FS-Benchmark，这是一个目前对于领域知识覆盖面最广、数据量最大、数据内容不断更新的适合LLMs评估的Domain Benchmarks。

为了涵盖尽可能多的专业领域，我们借鉴了中国学科分类中所有的112个一级学科的分类方法来构建我们的benchmark。
这些学科涵盖了14个学科门类，包括哲学、经济学、法学、教育学、文学、历史学、理学、工学、农学、医学、军事学、管理学、艺术学、交叉学科。
我们收集了大量的中国高校的研究生入学考试题目和本科生期中期末考试题目，我们用一级学科的类别标签对这些题目进行分类，并进行了人工筛选、过滤以保证数据的质量。
同时为了保证我们的数据能够深入地评估模型，我们还使用了尽可能多的二级学科和三级学科来对每道题目打上标签，这些学科标签相较于一级学科而言是更加细分的领域，我们认为这可以有效地为我们的benchmark做出一些深度上的规划。

为了能够有效地进行自动化评估，我们只使用了有明确ground truth的题目。
这些题目主要包含填空题、选择题、判断题。
考虑到不同LLMs对于prompt的敏感程度不同，我们为FS-Benchmark中的每道题目都设置了至少5种完全不同的提问方式。
并且我们针对模型的回答结果设计了一种算法来判断模型是因为不理解具体的知识而导致的回答错误，还是因为不理解提问方式而导致的回答错误。

为了能够有效地校验模型的输出，我们设计了一个Pipeline式的评估方法进行评估。
首先我们会将所有的题目构建成多选题，以保证模型如果知道某题的答案，则该模型的输出会尽量和ground truth保持一致。
但即便如此，也会有不少语言模型输出一些冗余的信息。
所以第二步，我们设计了一种加权字符相似度的方式来计算模型输出和ground truth的相似程度，最后根据相似度判断模型是否答对一道题。

为了缓解评估数据集污染的问题，我们将持续不断地获取每年最新的中国各高校研究生入学考试的题目，以及各大高校合法的期中期末考试题来更新我们的数据集。
同时，我们也会持续获取各个专业程度不同的人类在不同题目上的答题准确率，以建立具有分级参考意义的人工评估结果。




==> old_version/01Introduction.1.tex <==

\subsection{Background}
Domain knowledge refers to a deep understanding of the world, which requires various abilities such as abstraction, reasoning, and imagination to acquire. 
For an extended period, humans have far surpassed the capabilities of any machine learning models in mastering domain knowledge through natural language. 
However, in recent years, Large Language Models (LLMs), such as Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, Gopher~\cite{rae2021gopher}, UL2~\cite{tay2022ul2}, Bard~\cite{pichai2023important}, and GPT4~\cite{openai2023gpt4, bubeck2023sparks}, have demonstrated astonishing capabilities in natural language processing. 
These LLMs seem to have achieved human expert-level performance in understanding texts involving domain knowledge~\cite{wei2022emergent}. 
To convince people that LLMs can provide accurate information across various domains, it is paramount to thoroughly and in-depth assess the models' mastery of domain knowledge.

\subsection{Motivation}
Both before and after the advent of LLMs, numerous benchmarks for language model evaluation have been proposed by scholars. Benchmarks such as GLUE (Wang et al., 2018), SuperGLUE (Wang et al., 2019), and MMLU (Hendrycks et al., 2021) have been excellent standards for a long time in measuring model performance in various domains. Still, now LLMs have far surpassed human performance on these benchmarks. Recently introduced BIG-Bench (Srivastava et al., 2022) and HELM (Liang et al., 2022) are becoming new evaluation standards for language models. However, these benchmarks do not specifically target domain knowledge evaluation, and thus only cover a few limited domain dimensions.

Recently, GPT-4 (OpenAI et al., 2023; Bubeck et al., 2023) proposed some ideas for cross-domain evaluation in two articles, such as using JavaScript to draw a unicorn or proving mathematical formulas in Shakespeare's language style. However, these evaluations are too open-ended that they can only be verified using human intervention.

Moreover, with advancements in LLMs' output mechanisms and the increasing scale of data used, previous benchmarks are no longer suitable for evaluating the latest LLMs. Recently emerging LLMs are mostly text-to-text models, which take text input and generate text probabilistically making it difficult to directly generate answers identical to the ground truth. Consequently, evaluating LLM outputs becomes an issue. Furthermore, the corpora used by large models are becoming increasingly vast. For cutting-edge LLMs, such as GPT-4, the data used almost covers all open-source information that can be found on the internet. Hence, ensuring the evaluation samples do not appear in the model's training data is another challenge.

Based on the above, we summarize the limitations of previous work as follows:

Limited professional domains: The covered domain knowledge is extremely limited, and the dimensions are not comprehensive.
Lack of depth discrimination: They have not adequately distinguished the depth of domain knowledge, making it challenging to determine how well the models have grasped specific domain knowledge.
Open-ended questions: Many evaluations are open-ended, requiring considerable human effort to verify the model's output results.
Difficulty in verifying model outputs: None of the current benchmarks are suitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
Evaluation dataset contamination: As LLMs use increasingly vast corpora, the data used for evaluation may already be part of the LLMs' training data, thereby compromising the fairness of the evaluation.

\subsection{Our Work}
In this paper, we propose FS-Benchmark, a domain benchmark currently offering the most extensive coverage of domain knowledge, the largest data volume, and continually updated content suitable for LLM evaluation.

To cover as many professional domains as possible, we refer to the classification method of China's 112 first-level disciplines to construct our benchmark. These disciplines span 14 categories, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields. We collected a considerable number of graduate entrance examination questions and undergraduate midterm and final exam questions from Chinese universities, and we categorized these questions using the first-level discipline labels, performing manual screening and filtering to ensure data quality.

To ensure a comprehensive evaluation of our dataset, we used as many secondary and tertiary disciplines as possible to label each question. These discipline labels are more detailed compared to primary disciplines, and we believe they can effectively outline some depth for our benchmark.

For effective automated evaluation, we used only questions with a definite ground truth. These questions mainly include fill-in-the-blank, multiple-choice, and true-or-false questions. Considering the varying sensitivity of different LLMs to prompts, we provided at least five completely different questioning methods for each question in FS-Benchmark. Additionally, we designed an algorithm to determine whether the answer errors are due to inadequate understanding of the specific knowledge or misunderstanding the question format.

To effectively verify the model's output, we designed a pipeline-style evaluation method. First, we construct all questions as multiple-choice questions to ensure that if a model knows the answer, its output remains as consistent as possible with the ground truth. However, even with this approach, some language models still generate redundant information. Therefore, as a second step, we designed a method to calculate the similarity between the model's output and the ground truth based on a weighted character similarity, and finally, judge whether the model answers a question correctly based on its similarity score.

To mitigate the issue of evaluation dataset contamination, we continually obtain the latest Chinese graduate entrance examination questions and legally available midterm and final exam questions from major universities to update our dataset. Concurrently, we will also continuously gather the accuracy of people with different professional levels on various questions to establish human evaluation results with graded reference significance.


==> old_version/01Introduction.10.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as memorization, abstraction, logical thinking, reasoning and imagination. 
Human has exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, have shown remarkable capabilities in domain text understanding~\cite{wei2022emergent}.
It is time to propose more comprehensive and more prospective evaluations than before to explore whehter language models~(LMs) have actually acquired knowledge, or just acquired a better imitation ability~\cite{srivastava2022bigbench}.

Constructing benchmarks is crucial for automatic evaluation as benchmarks facilitate efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they exhibit outstanding performance across a wide range of domain-specific tasks.
This makes even the newly released benchmarks like MMLU~\cite{hendrycks2021measuring}, BIG-bench~\cite{srivastava2022bigbench} or HELM~\cite{liang2022holistic} all lag behind the capabilities of the LMs quickily~\cite{suzgun2022big-bench-hard}.


Considering LMs' performance today, we conclude that the benchmark used to evaluate LMs should meet the following needs:
(1) \textit{Needs to cover more tasks~\cite{srivastava2022bigbench}}: 
现在的语言模型都集合了许多能力于一身。
所以对于LMs的评估应更加聚焦于多任务的能力。
\red{The previous benchmarks have limited coverage towards domain aspects, even the most comprehensive domain benchmark cover no more than 70 domain-specific knowledge areas, which prevent these benchmarks serving as a comprehensive criterion for domain mastery evaluation.}
(2) \textit{Needs to cover more difficulties~\cite{huang2023ceval}}: 
Considering the emergent capacity of the models~\cite{wei2022emergent}, it is likely that the SoTA LLMs now have a certain level of performance in all domains. 
Benchmark therefore needs to split the evaluation dimensions more detailed so that it can assess exactly how well the model performs.
(3) \textit{Needs to go ahead of the training set~\cite{wei2022emergent}}: 
As LLMs trained on increasingly extensive corpora, newly released benchmark may become part of the LLMs' training data much sooner than before.
Frequently updated benchmarks are needed to keep the evaluation samples fresher than the training data used by LLMs.



\begin{figure}[t]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{SubjectClassification.pdf}
}
\end{center}
\caption{Caption}
\label{fig:subjectclassification}
\end{figure}

In the light of the aforementioned needs, we propose Xiezhi-Benchmark, a comprehensive, multi-disciplinary, auto-updating benchmark for domain knowledge evaluation.
Xiezhi consists of 118 different disciplinary questions, ranging from 13 different categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management and arts.
In addition to these 118 disciplines, \red{Xiezhi labels samples with a more refined set of 396 sub-disciplinary tags.} 
The disciplinary taxonomy used by Xiezhi, comprising over 500 disciplines in total, is derived from the \red{参考C-eval里的说法Chinese Disciplinary Classification System}, which is utilized by all Chinese universities and is highly recognized.
We manually post-checked 50,000 natural annotated questions from Chinese postgraduate entrance examination,
and train an automatic annotation model based on these questions and to annotate an additional 150,000 questions collected from various examinations, such as exams from primary, secondary schools, college entrance exams, as well as professional examination.
Based on these 200,000 questions obtained through the aforementioned method, we further proposed Xiezhi-Easy and Xiezhi-Hard, two datasets with 15,000 more balanced, less sensitive, less Chinese-centric questions.
\red{Both of datasets are released an Chinese version and English version.}
Xiezhi-Easy is a good indicator for small size LLMs, with it containing only the most fundamental knowledge from each domain.
Xiezhi-Hard is specifically tailored for large size models, even GPT-4 can only achieve a 40\% accuracy rate under a 3-shot setting.

Compared to previous evaluation works target at generative models, we have made some changes in evaluation process.
We set 50 options for each multiple-choice question, as previous researchers use only 4 options, result in significantly reducing the accuracy of random guessing and thus better revealed model's real capabilities. 
We use the generation probability to calculate the probability of each model choosing all options, thereby avoiding inaccurate evaluations due to the model's inabilities in answering multiple-choice questions or errors in the generated content extraction.
Furthermore, as our method calculate the probability of the model choosing each option, some other metrics, like hit@k or mrr, can be used to reflect the model's performance in finer detail.

We conducted experiments on 48 LLMs among nearly released 4 benchmarks which targets at domain knowledge evaluation. 
All models were tested on both Chinese Xiezhi and English Xiezhi, and analyzed based the best results.
We found that although GPT-4 achieved the best results in all domain categories, it did not reach even the average level of domain practitioners in any field. 
Furthermore, although LLMs are believed to possess emergent capabilities in unseen tasks~\cite{wei2022emergent}, their performance in some domains with limited corpora is even worse than in tasks that require complex reasoning.
Simultaneously, we discovered that LLMs' understanding in domain knowledge is not related to the volume of finetuning data. 
In fact, the performance may drastically decrease for many LLMs after finetuning. 
In addition to this, we tested the recently proposed domain benchmarks in our evaluation settings.
\blue{从所有模型的hit@k变化图来看，不同模型在Xiezhi-Easy上的变化差异最大。}
This demonstrates that Xiezhi, covering the most comprehensive domains, containing the most volume of questions, is best at discerning the capability differences between various LLMs, and hence is benchmark most suitable for the evaluation of LLMs with various abilities.





==> old_version/01Introduction.11.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as memorization, abstraction, logical thinking, reasoning and imagination. 
Human has exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, have shown remarkable capabilities in domain text understanding~\cite{wei2022emergent}.
It is time to propose more comprehensive and more prospective evaluations than before to explore whehter language models~(LMs) have actually acquired knowledge, or just acquired a better imitation ability~\cite{srivastava2022bigbench}.

Constructing benchmarks is crucial for automatic evaluation as benchmarks facilitate efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they exhibit outstanding performance across a wide range of domain-specific tasks.
This makes even the newly released benchmarks like MMLU~\cite{hendrycks2021measuring}, BIG-bench~\cite{srivastava2022bigbench} or HELM~\cite{liang2022holistic} all lag behind the capabilities of the LMs quickily~\cite{suzgun2022big-bench-hard}.


Considering LMs' performance today, we conclude that the benchmark used to evaluate LMs should meet the following needs:
(1) \textit{Needs to cover more tasks~\cite{srivastava2022bigbench}}: 
Cutting-edge LMs have integrated multiple capabilities into a unified Text-to-Text transformer models~\cite{raffel2020t5}.
Therefore, the evaluation of LMs should focused on abilities in multiple tasks processing.
(2) \textit{Needs to cover more difficulties~\cite{huang2023ceval}}: 
Considering the emergent capacity of the models~\cite{wei2022emergent}, it is likely that the SoTA LLMs now have a certain level of performance in all domains. 
Benchmark therefore needs to split the evaluation dimensions more detailed so that it can assess exactly how well the models with different capacities perform.
(3) \textit{Needs to go ahead of the training set~\cite{bubeck2023sparks}}: 
As LLMs trained on increasingly extensive corpora, newly released benchmark may become part of the LLMs' training data much sooner than before.
A prerequisite for effective evaluation is to ensure that the benchmarks are fresher than the training data used by LMs.



\begin{figure}[t]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{SubjectClassification.pdf}
}
\end{center}
\caption{
In Chinese mythology, the Xiezhi is a legendary creature known for its ability to discern right from wrong and uphold justice. 
Xiezhi Benchmark encompasses 13 distinct disciplinary categories, 118 sub-disciplines, and 385 further fine-grained disciplines, aiming to provide a extensive domain taxonomy and benchmark for fair, effective and comprehensive domain evaluation.
% Xiezhi是中国的一个有着辨别是非，公正不阿的本性的一个传说神兽。
% Xiezhi Benchmark包含了13个不同的学科门类，516个细分学科，以及385个更加细分的学科，旨在为领域评估提供一个全面的分类体系和基准。
}
\label{fig:subjectclassification}
\vspace{-5mm}
\end{figure}

In the light of the aforementioned needs, we propose a comprehensive, multi-disciplinary, auto-updating benchmark for domain knowledge evaluation.
We name this benchmark Xiezhi, a mythical animal that symbolizes fairness.
Xiezhi consists of 200,000 questions with 516 disciplines, ranging from 13 different categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management and arts.
These 516 disciplines comes from Chinese Disciplinary Taxonomy, which is proposed by the Chinese Ministry of Education and is highly recognized in China as a comprehensive hierarchical classification to domain knowledge.
We manually post-checked 20,000 natural annotated questions from Chinese postgraduate entrance examination,
and train an automatic annotation model based on these questions and to annotate an additional 180,000 questions collected from various examinations, such as exams from primary, secondary schools, college entrance exams, as well as professional examination.
Based on these 200,000 questions, we further proposed Xiezhi-Specialty and Xiezhi-Interdisciplinary, two datasets with 15,000 more balanced, less sensitive, less Chinese-centric questions.
Xiezhi-Specialty is a good indicator for small size LLMs, with it containing only the most fundamental knowledge from each domain.
Xiezhi-Interdisciplinary is specifically tailored for large size models, even GPT-4 can only achieve a 40\% accuracy rate under a 3-shot setting.
We also translate the both dataset into English, and manually checked the quality before experiments and released.

Compared to previous evaluation works target at generative models, we have made some changes in evaluation process.
We set 50 options for each multiple-choice question, as previous researchers use only 4 options, result in significantly reducing the accuracy of random guessing and thus better revealed model's real capabilities. 
We use the generation probability to calculate the probability of each model choosing all options, thereby avoiding inaccurate evaluations due to the model's inabilities in answering multiple-choice questions or errors in the generated content extraction.
Furthermore, as our method calculate the probability of the model choosing each option, some other metrics, like hit@k or mrr, can be used to reflect the model's performance in finer detail.

We conducted experiments on 48 LLMs on 4 nearly released benchmarks which targets at domain knowledge evaluation. 
All models were tested on both Chinese Xiezhi and English Xiezhi, and analyzed based on the best results.
We found that although GPT-4 achieved the best results in all domain categories, it did not reach even the average level of domain practitioners in any field. 
Furthermore, although LLMs are believed to possess emergent capabilities in unseen tasks~\cite{wei2022emergent}, their performance in some domains with limited corpora is even worse than in tasks that require complex reasoning.
Simultaneously, we discovered that LLMs' understanding in domain knowledge is not related to the volume of finetuning data. 
In fact, the performance may drastically decrease for many LLMs after finetuning. 
In addition to this, we tested the recently proposed domain benchmarks in our evaluation settings.
Our experiments demonstrate that Xiezhi, covering the most comprehensive domains, containing the most volume of questions, is also best at discerning the capability differences between various LLMs, ranging from GPT-4 to LMs with only 560M parameters, and hence is the benchmark most suitable for the evaluation of LLMs with various abilities.





==> old_version/01Introduction.2.tex <==

% \subsection{Background}
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, Gopher~\cite{rae2021gopher}, UL2~\cite{tay2022ul2}, Bard~\cite{pichai2023important}, and GPT4~\cite{openai2023gpt4, bubeck2023sparks} have shown remarkable capabilities in domain understanding~\cite{wei2022emergent}.
We cannot help but raise the following questions, and hope to quantify these doubts through experiments:

\begin{center}
    
\textit{In which domains do LLMs perform well?
To what degree can LLMs perform?
How do LLMs compare to human experts?}
\end{center}


For a long period, language understanding benchmarks served as excellent standards for measuring model performance across various domains~\cite{wang2018glue,wang2019superglue,hu2020xtreme,mishra2021cross}. 
However, LLMs' performance on benchmarks such as GLUE~\cite{wang2018glue} or SuperGLUE~\cite{wang2019superglue} have already surpassed human experts', which show that these benchmarks are not suitable for evaluating the latest powerful language models. 
Recently introduced benchmarks, such as BIG-Bench~\cite{srivastava2022bigbench} or HELM~\cite{liang2022holistic}, are emerging as new evaluation standards for LLMs. 
These benchmarks have developed many evaluation dimensions, which are very challenging for language models, but these benchmarks do not have more detailed designs or annotate more data for the dimensions they proposed.
Therefore, they can only roughly evaluate whether models have a certain ability.
% \red{Nevertheless, these benchmarks do not specifically target domain knowledge evaluation and thus only limited domain knowledge is covered.}
% In addition to the evaluation works in these benchmarks, GPT-4~\cite{openai2023gpt4, bubeck2023sparks} proposed ideas for cross-domain evaluation, involving tasks such as using JavaScript to draw a unicorn or proving mathematical formulas in the style of Shakespearean language. 
% These evaluations, however, are highly open-ended, necessitating human intervention for verification.

In addition to the benchmakrs, there have more problems than before in how to effectively evaluate LLMs.
Recently emerging LLMs are predominantly text-to-text models, which take text input and generate text probabilistically, \red{making it challenging to generate answers identical to the ground truth directly.
As a result, evaluating LLM outputs becomes problematic.}
Furthermore, the corpora used by large models are becoming increasingly extensive, and cutting-edge LLMs, like GPT-4, use data covering almost all open-source information found on the internet. 
Ensuring that evaluation samples are not part of the model's training data, therefore, poses another challenge.

Based on the aforementioned points, we summarize the limitations of previous works as follows:

1. Limited domain coverage: The previous benchmarks covered only limited domain knowledge, \red{and lack of some domain classification}.
2. Lack of depth design: They have not adequately distinguished the depth of domain knowledge, making it challenging to determine the extent of models' understanding to specific domain knowledge.
\red{3. 缺少不同水平的人类baseline。}
3. Open-ended questions: Many evaluations are open-ended, necessitating substantial human efforts to verify the model's output results.
4. Difficulty in verifying model outputs: Current benchmarks are unsuitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
5. Evaluation dataset contamination: As LLMs use increasingly extensive corpora, evaluation data may already be part of the LLMs' training data, thereby jeopardizing the fairness of the evaluation.

% \subsection{Our Work}The dataset is meticulously crafted to assess the degree of domain knowledge understanding in large-scale language models.
In this work, we present \textbf{DomMa}, a \textbf{Dom}ain \textbf{Ma}stery Benchmark designed to assess the proficiency of LLMs in comprehending domain knowledge. The benchmark is characterized by its extensive coverage of domain-specific knowledge, substantial data volume, and continuously auto update.

To cover as many domains as possible, we refer to the classification of 112 first-level subjects in Chinese University Education System to construct our benchmark. 
These subjects span 14 categories: philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields.
And we used as many second-level subjects as possible to label each question. 
These second-level subject labels provide greater detail compared to first-level, which give the benchmark a detail design of domain depth.

{To ensure the data quality and volume,}
we collected a significant number of graduate entrance examination questions and undergraduate midterm and final exam questions from Chinese universities. 
We categorized the questions from graduate entrance examination into seed benchmarks using the first-level subject labels, and keep collecting final exams from undergraduate exams and do auto-annotation based on the seed benchmarks and subject information of the exams.

To effectively verify the model's output, we selected questions with definite ground truth, primarily comprising fill-in-the-blank, multiple-choice, and true-or-false questions.
During model prediction, we use five different instructions to test every samples since models are sensitive to prompts~\cite{jiang2020can} .
And we design instruction to encourage the model to provide responses that are completely the same to one of the given options, thereby reducing the difficulty of evaluation.
Considering that we have no access to all models' parameters, and not all models have the ability to give the response exactly as we want.
Three distinct evaluation methods have been developed to address these scenarios, with the goal of accurately assessing a model's capabilities in the most precise manner possible.

% a white-box evaluation method, a grey-box evaluation method, and a black-box evaluation method for situations where models generate redundant information.
% If we can obtain the model's parameters, we use the white-box evaluation method to directly access the probability generated by the model for each option. If we cannot obtain the model's parameters, we can still use the grey-box prompt to induce the model to generate the probabilities for each option.
% If the model's performance is poor, we can use the black-box prompt to require the model to make predictions directly and determine the model's choice based on the semantic similarity between the generated content and each option.

% 模型预测时，我们使用五种不同的prompt去针对一个question进行提问来降低模型对于prompt敏感的问题~\cite{jiang2020can}，并通过设计prompt来诱导模型给出和选项完全一致的回复，来降低评估的难度
% 考虑到不是所有的模型都有能力完全理解指令，所以针对模型会生成冗余信息的情况，我们设计了一种白盒评估方法、一种灰盒评估方法，和一种黑盒评估方法。
% 如果我们可以拿到模型的参数，则我们可以使用白盒评估方法，直接获取模型生成各个选项的概率。
% 如果我们拿不到模型的参数，我们依然可以通过灰盒prompt来诱导出模型生成各个选项的概率。
% 如果模型能力很差，则我们可以通过黑盒prompt来要求模型直接进行预测，并根据模型生成内容和各个选项的语义相似度来判断模型选择的选项。

% To effectively verify the model's output, we designed a pipeline-style evaluation method. Firstly, we reformatted all questions as multiple-choice questions to encourage model outputs that closely align with the ground truth. However, given that some language models still generate redundant information, we implemented a second step: calculating the similarity between the model's output and the ground truth based on weighted character similarity. Finally, we determined whether the model answered a question correctly by comparing its similarity score with a designated threshold.

% To address the issue of evaluation dataset contamination, we continuously acquire the latest Chinese graduate entrance examination questions and legally available midterm and final exam questions from major universities to update our dataset. Simultaneously, we gather accuracy data from individuals with diverse professional levels on various questions, establishing human evaluation results with graded reference significance.

In summary, our contributions can be summarized as follows:

1. We construct DomMa Benchmark, which aims at providing a metric to evaluate the extent to which models can manage domain-specific knowledge.
2. The DomMa Benchmark caters particularly to LLMs, and we propose three distinct evaluation methods tailored to assess the outputs generated by the models.
% 3. Future work entails conducting a thorough analysis of existing LLMs to identify their strengths and weaknesses, culminating in the generation of a detailed analytical report.


% 1. We have construct DomMa Benchmark, which aims at providing a metric of how models can handle domain knowledge.
% 2. DomMa Benchmark is LLMs friendly, and we have propose three distinct evaluation methods to assess the models' outputs.
% 3. We are about to do a comprehensive analysis to the existing LLMs, summarize their strength and weakness, and propose a deliberate analysis report.


% 1. 我们搞了个benchmark。
% 2. 我们搞了个适合LLMs评估的方法。
% 3. 我们针对大多数已有的模型，进行了评估，并给出了详细的分析报告。

==> old_version/01Introduction.3.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, Gopher~\cite{rae2021gopher}, UL2~\cite{tay2022ul2}, Bard~\cite{pichai2023important}, and GPT4~\cite{openai2023gpt4, bubeck2023sparks} have shown remarkable capabilities in domain understanding~\cite{wei2022emergent}.
We cannot help but raise the following questions, and hope to quantify these doubts through experiments:

\begin{center}
    
\textit{In which domains do LLMs perform well?
To what degree can LLMs perform?
How do LLMs compare to human experts?}
\end{center}


For a long period, language understanding benchmarks served as excellent standards for measuring model performance across various domains~\cite{wang2018glue,wang2019superglue,hu2020xtreme,mishra2021cross}. 
However, many classic language understanding benchmarks, such as GLUE~\cite{wang2018glue} or SuperGLUE~\cite{wang2019superglue}, do not target at domain text understanding at all, and only covered evaluation dimensions which are too simple for LLMs nowadays, so they are no longer suitable for assessing the ability of the cutting-edge language models.
Recently introduced benchmarks are emerging as new evaluation standards for LLMs.
Many of these benchmarks, such as BIG-Bench or HELM, focus on the functional evaluation of models, making it difficult to assess the extent to which models grasp knowledge. 
Others, such as MMLU, MATH, or APPS, concentrate on the knowledge-based evaluation of models.
However, the prevailing language models have surpassed human performance in these benchmarks these days.
These benchmarks also suffer from limited data amount (e.g., MMLU covers only over 15k evaluation data points), and and lack of deeper designs for each subject, which making it challenging to assess the extent to which language models specifically master a particular category of knowledge.
% However, none of these works construct the relationship between different subjects, which we think can better describe the abilities of a language model.

% Many of these benchmarks, such as BIG-Bench or HELM, 聚焦于模型的功能性评估，所以难以评估模型对于知识的掌握程度.
% Others, such as MMLU, MATH or APPS, 聚焦于模型的知识性评估，但是他们将所有的知识维度离散化，没有对知识之间进行有效地建模。这些benchmarks所涵盖的数据量非常有限（如MMLU只涵盖了15k多条评估数据），还缺少了对于每种知识更深层次的设计，所以难以评估语言模型对于一类知识具体掌握到什么程度。

In addition to the benchmarks, how to effectively and fairly evaluate LLMs become problematic.
Recently emerging LLMs are predominantly text-to-text models, which take text input and generate text probabilistically, making it difficult to determine whether the output of models have the same semantic with ground-truth.
Furthermore, the corpora used by large models are becoming increasingly extensive, and cutting-edge LLMs, like GPT-4, use data covering almost all open-source information found on the internet. 
Ensuring that evaluation samples are not part of the model's training data, therefore, poses another challenge.

Based on the aforementioned points, we summarize the limitations of previous works as follows:

1. Limited subjects or tasks coverage: The previous benchmarks covered only limited domain knowledge.
2. Lack of depth design: They have not adequately distinguished the depth of domain knowledge, making it challenging to determine the extent of models' understanding to specific domain knowledge.
3. Have open-ended questions: Many evaluations are open-ended, necessitating substantial human efforts to verify the model's output results, which introduces uncertainty and potential unfairness in the assessment of models.
4. Difficulty in verifying LLMs' outputs: Current benchmarks are unsuitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
This will make models to fit the benchmarks in order to achieve the best performance, potentially compromising their generalizability.
5. Evaluation dataset contamination: As LLMs use increasingly extensive corpora, evaluation data may already be part of the LLMs' training data, thereby jeopardizing the fairness of the evaluation.


In this work, we present \textbf{DomMa}, a \textbf{Dom}ain \textbf{Ma}stery Benchmark designed to assess the proficiency of LLMs in comprehending domain knowledge. 
The benchmark is characterized by its extensive coverage of domain-specific knowledge, substantial data volume, and continuously auto update.


DomMa draws inspiration from the subject classification system of Chinese higher education institutions to construct a dataset that encompasses 112 distinct subjects spanning 14 disciplinary categories. Additionally, DomMa employs as many as 217 more refined subject labels to annotate each sample, while also modeling the relationships between subjects, enabling the extraction of correlations between subjects and providing more information for each sample.

To effectively evaluate generative models, we have structured the evaluation data in DomMa as multiple-choice questions with four and fifty options. Furthermore, to assess different capabilities and openness levels of Language Models (LLMs), we have established three distinct evaluation schemes for a fairer and more effective assessment.

Periodically, the dataset can be automatically updated by crawling questions from the Chinese postgraduate entrance examination. Simultaneously, we have manually annotated a question bank containing 5 million questions, allowing the classifier to learn the annotation content of this question bank and subsequently perform automatic annotation.


% DomMa借鉴了中国高校教育的学科分类系统来构建数据集，涵盖了112个不同的subjects，跨越了14个学科门类。
% DomMa还使用了多达217个更细化的学科标签对每个样本进行标注，同时建模了subjects之间的关系，从而可以获得subjects之间的关联性，也可以为每个样本得到更多的信息。
% 为了能够有效地评估生成式模型，我们将DomMa中的评估数据构建成了四选一以及五十选一的选择题。
% 更进一步，为了能够评估不同能力，以及不同开源程度的LLMs，我们设置了三种不同的评估方案，来更公正更有效地进行评估。
% 每隔一段时间可以通过爬取中国研究生入学考试的题目来进行自动更新，同时，我们人工标注了一份拥有500w题目的题库，让分类器在学习这份题库的标注内容，之后可以进行自动标注。


我们发现\red{一些结论，一些结论，一些结论，一些结论，一些结论，一些结论，一些结论，一些结论，一些结论，一些结论，一些结论，}

% To cover as many domains as possible, we refer to the classification of 112 first-level subjects in Chinese University Education System to construct our benchmark. 
% These subjects span 14 categories: philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields.
% And we used as many second-level subjects as possible to label each question. 
% These second-level subject labels provide greater detail compared to first-level, which give the benchmark a detail design of domain depth.

% {To ensure the data quality and volume,}
% we collected a significant number of graduate entrance examination questions and undergraduate midterm and final exam questions from Chinese universities. 
% We categorized the questions from graduate entrance examination into seed benchmarks using the first-level subject labels, and keep collecting final exams from undergraduate exams and do auto-annotation based on the seed benchmarks and subject information of the exams.

% To effectively verify the model's output, we selected questions with definite ground truth, primarily comprising fill-in-the-blank, multiple-choice, and true-or-false questions.
% During model prediction, we use five different instructions to test every samples since models are sensitive to prompts~\cite{jiang2020can} .
% And we design instruction to encourage the model to provide responses that are completely the same to one of the given options, thereby reducing the difficulty of evaluation.
% Considering that we have no access to all models' parameters, and not all models have the ability to give the response exactly as we want.
% Three distinct evaluation methods have been developed to address these scenarios, with the goal of accurately assessing a model's capabilities in the most precise manner possible.


In summary, our contributions can be summarized as follows:

1. We construct DomMa Benchmark, which aims at providing a metric to evaluate the extent to which models can manage domain-specific knowledge.
2. The DomMa Benchmark caters particularly to LLMs, and we propose three distinct evaluation methods tailored to assess the outputs generated by the models.
3. We have conducted extremely detailed evaluation and analysis of models that are currently open source parameters or APIs.
We present all of our analysis and several of the most interesting experimental results in the main text, as for all the experimental results, we put them in the appendix


==> old_version/01Introduction.4.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, Gopher~\cite{rae2021gopher}, UL2~\cite{tay2022ul2}, Bard~\cite{pichai2023important}, and GPT4~\cite{openai2023gpt4, bubeck2023sparks} have shown remarkable capabilities in domain understanding~\cite{wei2022emergent}.
We cannot help but raise the following questions, and hope to quantify these doubts through experiments:

\begin{center}
    
\textit{In which domains do LLMs perform well?
To what degree can LLMs perform?
How do LLMs compare to human experts?}
\end{center}

% Benchmark is critical for automatic domain mastery evaluation since it enables efficient, systematic, and scalable comparisons between models in general.
% However, due to the rapid develop of Language Models~(LMs) these months, existing benchmarks are inadequate for effective domain mastery evaluation.
% Samples in many classic benchmarks, such as GLUE~\cite{wang2018glue} or SuperGLUE~\cite{wang2019superglue}, can be easily achieve high performance by LMs a few years ago, so these benchmarks are no longer suitable for assessing the ability of LMs any more.
% Recently introduced benchmarks, such as MMLU~\cite{hendrycks2021measuring}, BIG-Bench~\cite{srivastava2022bigbench} or HELM~\cite{liang2022holistic}, have brought challenges to LMs at the time.
% But since some of them targets at functional evaluation, like BIG-Bench or HELM, thus only covered limited domain related tasks, while others, like MMLU, have also for short in assessing the cutting-edge LMs because LMs capabilities have grown rapidly in recent months, the prevailing LMs have already made a good performance on these benchmarks~(GPT4 reaches 86\% average accuracy in MMLU with only k=5 few shot setting).
% There also emerge a trend of domain knowledge evaluation proposed by GPT-4~\cite{openai2023gpt4, bubeck2023sparks} like using JavaScript to draw a unicorn or proving mathematical formulas in the style of Shakespearean language. 
% But these kind of tasks are all open response, which need extra manual efforts to do the evaluation.


% In addition to the benchmarks, how to do effective and fair evaluation become more problematic than before.
% Recently emerging LLMs are predominantly text-to-text models, which take text input and generate text probabilistically, making it difficult to determine whether the output of models have the same semantic with ground-truth.
% Furthermore, the corpora used by large models are becoming increasingly extensive, and cutting-edge LLMs, like GPT-4, use data covering almost all open-source information found on the internet. 
% Ensuring that evaluation samples are not part of the model's training data, therefore, poses another challenge.

Benchmarking is crucial for automatic domain mastery evaluation as it facilitates efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they become better at solving a wide range of tasks. 
This makes it increasingly difficult for benchmarks like GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue} or MMLU~\cite{hendrycks2021measuring}, to provide a comprehensive evaluation of their capabilities, for they covered only limited spectrum of domain tasks that LLMs can handle.

Moreover, conducting effective and fair evaluations has become increasingly challenging. 
One reason is that the emerging Large Language Models (LLMs) are predominantly text-to-text models, which generate text probabilistically, complicating the determination of semantic equivalence between model outputs and ground-truth. 
Another reason is that the extensive corpora used by large models, such as GPT-4, encompass nearly all open-source information available on the internet, posing challenges in ensuring evaluation samples are not part of the model's training data.


Based on the aforementioned points, we summarize the limitations of previous works as follows:
(1) \textit{Limited subjects or tasks coverage}: The previous benchmarks have limited coverage towards domain aspects, which prevent these benchmarks serving as a comprehensive criterion for domain mastery. 
(2) \textit{Lack of detailed and in-depth designs}: Previous works did not annotate the samples in each domain with difficulty, released time or other labels, nor did they analyze the connections among each samples, making it hard to draw a thorough evaluation results to the models
(3) \textit{Have open-ended questions}: Many evaluations are open-ended, necessitating substantial human efforts to verify the model's output results, which introduces uncertainty and potential unfairness in the assessment of models.
(4) \textit{Difficult to identify generative models' outputs}: Current benchmarks are unsuitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
This will make models to fit the benchmarks in order to achieve the best performance, potentially compromising their generalizability.
(5) \textit{Evaluation dataset contamination}: As LLMs absorbing increasingly extensive corpora, newly released evaluation data may become part of the LLMs' training data sooner than before, thereby jeopardizing the truthfulness of the evaluation.


In this work, we present \textbf{DomMa}, a \textbf{Dom}ain \textbf{Ma}stery Benchmark designed to assess the proficiency of LLMs in comprehending domain knowledge.
The benchmark is characterized by its extensive coverage of domain-specific knowledge, substantial data volume, and continuously auto updating.
We also propose three evaluation scheme for generative models with different instruction learning abilities and different degree of open source to better suit the prevailing trend of LLMs.

Inspired by the Discipline Classification System of Chinese Higher Education, DomMa constructed a dataset containing 112 different disciplines in 14 disciplinary categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields.
In addition, DomMa uses up to 393 more detailed subject labels and annotates each sample with the date of release, the highest and average student scores.
In order to effectively assess generative LMs, we have structured the assessment data in DomMa as multiple choice questions with four, ten and fifty options.
In addition, to better assess LMs with different abilities and open-resource, we created three different assessment schemes to achieve fairer, safer and more valid assessments.
DomMa can be automatically updated periodically by capturing questions from the Chinese Graduate Entrance Examination.
Since we manually annotated the first version of DomMa, which contains 5 million questions, we use this data to train a classifier to learn how to annotate each question with a topic label, and then to automatically annotate them for future versions.

% DomMa draws inspiration from the subject classification system of Chinese Higher Education to construct a dataset that encompasses 112 distinct subjects spanning 14 disciplinary categories, these categories are: philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields. 
% Additionally, DomMa employs as many as 217 more detailed subject labels with released time, top or average students' scores to annotate each sample.
% To effectively evaluate generative LMs, we have structured the evaluation data in DomMa as multiple-choice questions with four, ten and fifty options. 
% Furthermore, to better assess LMs with different capabilities and openness, we have established three distinct evaluation schemes for a fairer, safer and more effective assessment.
% Periodically, the DomMa can be automatically updated by crawling questions from the Chinese postgraduate entrance examination. 
% Since we have manually annotated the first version of DomMa which contains 5 million questions, we use such data to train a classifier to learn how to annotate each questions with subject labels and subsequently perform automatic annotation for future version.


In summary, our contributions can be summarized as follows:
(1) We construct DomMa Benchmark, which aims at providing a metric to evaluate the extent to which models can manage domain knowledge.
(2) The DomMa Benchmark caters particularly to generative LMs, and we propose three evaluation methods tailored to assess the outputs generated by the different capabilities and different degree of open source LMs.
(3) We have conducted extremely detailed evaluation and analysis of 50 models that are currently open source parameters or APIs.
We present all of our analysis and several of the most interesting experimental results in the main text, as for all the experimental results, we put them in the appendix


==> old_version/01Introduction.5.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, have shown remarkable capabilities in domain understanding~\cite{wei2022emergent}.
We cannot help but raise the following questions, and hope to quantify these doubts through experiments:

\begin{center}
    
\textit{In which domains do LLMs perform well?
To what degree can LLMs perform?
How do LLMs compare to human experts?}
\end{center}

Benchmarking is crucial for automatic domain mastery evaluation as it facilitates efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they become better at solving a wide range of tasks. 
This makes it increasingly difficult for benchmarks like GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue} or MMLU~\cite{hendrycks2021measuring} to provide a comprehensive evaluation of LLMs' capabilities, for they covered only limited spectrum of domain tasks and out of date questions.

Moreover, conducting effective and fair evaluations has become increasingly challenging~\cite{hendrycks2021measuring, liang2022holistic}. 
One reason is that the emerging LLMs are predominantly text-to-text models, which generate text probabilistically, complicating the determination of semantic equivalence between model outputs and ground-truth~\cite{sai2022survey,zellers2020evaluating}. 
Another reason is that the extensive corpora used by large models, such as GPT-4, encompass nearly all open-source information available on the internet, posing challenges in ensuring evaluation samples are not part of the model's training data~\cite{yang2023harnessing,openai2023gpt4}.


Based on the aforementioned points, we summarize the limitations of previous works as follows:
(1) \textit{Limited subjects or tasks coverage}: The previous benchmarks have limited coverage towards domain aspects, even the most comprehensive domain benchmark cover no more than 70 domain-specific knowledge areas, which prevent these benchmarks serving as a comprehensive criterion for domain mastery.
(2) \textit{Lack of detailed and in-depth designs}: 
Previous works have not sufficiently labeled each questions within their benchmarks.
Numerous studies allocate only one label to each question, potentially conflicting with the diverse domain the question encompasses.
As a result, evaluation based on these benchmarks tend to lack depth and comprehensiveness, given the absence of substantial information pertaining to a particular question.
(3) \textit{Open-ended questions}: Many evaluations are open-ended, necessitating substantial human efforts to verify the model's output results, which introduces uncertainty and potential unfairness in the assessment of models.
(4) \textit{Difficulty in evaluating generative models' outputs}: Current benchmarks are unsuitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
This will make models to fit the benchmarks in order to achieve the best performance, potentially compromising their generalizability.
(5) \textit{Quickly out-of-date}: As LLMs absorbing increasingly extensive corpora, newly released evaluation data may become part of the LLMs' training data sooner than before, thereby jeopardizing the truthfulness of the evaluation.


In this work, we present \textbf{DomMa}, a \textbf{Dom}ain \textbf{Ma}stery Benchmark, to better alleviate the above limitations in Domain text understanding evaluation.
The benchmark is characterized by its extensive coverage of domain-specific knowledge, substantial data volume, and continuous automatic updates.


Inspired by the Discipline Classification System of Chinese Higher Education, DomMa containing all of 112 top disciplines in this system among 14 disciplinary categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields.
In addition, DomMa also employed an additional 393 subject labels to annotate the questions, as well as providing the appearance date, average student score, and highest student score for each question.
In order to effectively evaluate the generative models, we constructed dataset in the format of multiple-choice questions. 
And to increase the performance disparity between models, we set 50 options for each multiple-choice question.


We mainly collect questions from the Chinese Graduate Entrance Examination and from mid or final term exams in chinese universities.
In the original version, we manually annotated 400k questions and used our automatic update system to annotate an additional 100k questions in Chinese language.
Then we utilized ChatGPT~\cite{openaichatgpt} to translate all these 500k questions into English.
In order to evaluate more effectively and address the issue of China-centric bias, we constructed two additional benchmarks, DomMa-Medium and DomMa-Hard, each containing 30k questions, both of which removed some China-centric and other sensitive questions. 
In DomMa-Medium, each question involves only two to four domain-specific knowledge areas, making it relatively hard for models to answer correctly. 
In contrast, DomMa-Hard contains questions that involve five or more completely different domain-specific knowledge areas, making it extremely difficult even for the most cutting-edge models to achieve satisfactory performance on these questions.

\red{要不跟MMLU一样，就不写Contribution了，直接写发现的结论}
In summary, our contributions can be summarized as follows:
(1) We construct DomMa Benchmark, which aims at providing a metric to evaluate the extent to which models can manage domain knowledge.
(2) The DomMa Benchmark caters particularly to generative LMs, and we propose three evaluation methods tailored to assess the outputs generated by the different capabilities and different degree of open source LMs.
(3) We have conducted extremely detailed evaluation and analysis of 50 models that are currently open source parameters or APIs.
We present all of our analysis and several of the most interesting experimental results in the main text, as for all the experimental results, we put them in the appendix


==> old_version/01Introduction.6.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
The reasons may stem from the 模型参数量太少，训练语料不足，算力不够~\cite{}.
模型拥有大的参数量，可以拥有更强的知识编码能力；训练语料越大，则更多的知识可以被注入模型；而算力是让模型能够有效进行训练的基础。
最近，随着这三个

Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, 拥有了极其强大的能力，以至于大家都推断LLMs have remarkable capabilities in domain understanding~\cite{wei2022emergent, openai2023gpt4}.
但事实真的如此吗？

作为人造工具，机器学习模型所拥有的具体功能更受人们关注，但是机器学习模型所学会的知识却很容易被人忽视。
近来有很多功能针对于模型的功能进行了非常细致的评估，却没有多少工作认真地评估过机器学习模型到底学到了哪些领域知识。
不考虑模型学到了哪些知识，只考虑模型让模型拟合到具体的功能，将会极大地增加模型的不可控性，同时也会降低大语言模型在泛化任务上的安全性。


(1) \textit{Limited subjects or tasks coverage}: The previous benchmarks have limited coverage towards domain aspects, even the most comprehensive domain benchmark cover no more than 70 domain-specific knowledge areas, which prevent these benchmarks serving as a comprehensive criterion for domain mastery.
(2) \textit{Lack of detailed and in-depth designs}: 
Previous works have not sufficiently labeled each questions within their benchmarks.
Numerous studies allocate only one label to each question, potentially conflicting with the diverse domain the question encompasses.
As a result, evaluation based on these benchmarks tend to lack depth and comprehensiveness, given the absence of substantial information pertaining to a particular question.
(3) \textit{Open-ended questions}: Many evaluations are open-ended, necessitating substantial human efforts to verify the model's output results, which introduces uncertainty and potential unfairness in the assessment of models.
(4) \textit{Difficulty in evaluating generative models' outputs}: Current benchmarks are unsuitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
This will make models to fit the benchmarks in order to achieve the best performance, potentially compromising their generalizability.
(5) \textit{Quickly out-of-date}: As LLMs absorbing increasingly extensive corpora, newly released evaluation data may become part of the LLMs' training data sooner than before, thereby jeopardizing the truthfulness of the evaluation.


In this work, we present \textbf{DomMa}, a \textbf{Dom}ain \textbf{Ma}stery Benchmark, to better alleviate the above limitations in Domain text understanding evaluation.
The benchmark is characterized by its extensive coverage of domain-specific knowledge, substantial data volume, and continuous automatic updates.


Inspired by the Discipline Classification System of Chinese Higher Education, DomMa containing all of 112 top disciplines in this system among 14 disciplinary categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields.
In addition, DomMa also employed an additional 393 subject labels to annotate the questions, as well as providing the appearance date, average student score, and highest student score for each question.
In order to effectively evaluate the generative models, we constructed dataset in the format of multiple-choice questions. 
And to increase the performance disparity between models, we set 50 options for each multiple-choice question.


We mainly collect questions from the Chinese Graduate Entrance Examination and from mid or final term exams in chinese universities.
In the original version, we manually annotated 400k questions and used our automatic update system to annotate an additional 100k questions in Chinese language.
Then we utilized ChatGPT~\cite{openaichatgpt} to translate all these 500k questions into English.
In order to evaluate more effectively and address the issue of China-centric bias, we constructed two additional benchmarks, DomMa-Medium and DomMa-Hard, each containing 30k questions, both of which removed some China-centric and other sensitive questions. 
In DomMa-Medium, each question involves only two to four domain-specific knowledge areas, making it relatively hard for models to answer correctly. 
In contrast, DomMa-Hard contains questions that involve five or more completely different domain-specific knowledge areas, making it extremely difficult even for the most cutting-edge models to achieve satisfactory performance on these questions.

\red{要不跟MMLU一样，就不写Contribution了，直接写发现的结论}
In summary, our contributions can be summarized as follows:
(1) We construct DomMa Benchmark, which aims at providing a metric to evaluate the extent to which models can manage domain knowledge.
(2) The DomMa Benchmark caters particularly to generative LMs, and we propose three evaluation methods tailored to assess the outputs generated by the different capabilities and different degree of open source LMs.
(3) We have conducted extremely detailed evaluation and analysis of 50 models that are currently open source parameters or APIs.
We present all of our analysis and several of the most interesting experimental results in the main text, as for all the experimental results, we put them in the appendix

==> old_version/01Introduction.7.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, have shown remarkable capabilities in various downstream tasks~\cite{wei2022emergent}.
With regard to the increasing capabilities of models, a question has been raised~\cite{srivastava2022bigbench}:

\begin{center}
\textit{Is the remarkable performance of LLMs attribute the acquisition of extensive knowledge and the development of reasoning abilities, or is it merely a reflection of their enhanced ability for imitation?}
\end{center}

Constructing benchmarks is crucial for automatic domain mastery evaluation as benchmarks facilitate efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they exhibit outstanding performance across a wide range of domain-specific tasks.
This makes it increasingly difficult for benchmarks like GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue} or MMLU~\cite{hendrycks2021measuring} to provide a comprehensive evaluation of LLMs' capabilities, for they covered only limited spectrum of domain tasks and out of date questions.

Moreover, conducting effective and fair evaluations has become increasingly challenging~\cite{hendrycks2021measuring, liang2022holistic}. 
One reason is that the emerging LLMs are predominantly text-to-text models, which generate text probabilistically, complicating the determination of semantic equivalence between model outputs and ground-truth~\cite{sai2022survey,zellers2020evaluating}. 
Second reason is that the extensive corpora used by large models, such as GPT-4, encompass nearly all open-source information available on the internet, posing challenges in ensuring evaluation samples are not part of the model's training data~\cite{yang2023harnessing,openai2023gpt4}.

Based on the aforementioned points, we summarize the limitations of previous benchmarks as follows:
(1) \textit{Cover limited subjects or tasks}: The previous benchmarks have limited coverage towards domain aspects, even the most comprehensive domain benchmark cover no more than 70 domain-specific knowledge areas, which prevent these benchmarks serving as a comprehensive criterion for domain mastery.
(2) \textit{Lack of detailed and in-depth designs}: 
Previous works have not sufficiently labeled each questions within their benchmarks.
Numerous studies allocate only one label to each question, potentially conflicting with the diverse domain the question encompasses.
As a result, evaluation based on these benchmarks tend to lack depth and comprehensiveness, given the absence of substantial information pertaining to a particular question.
(3) \textit{Have Open-ended questions}: Many evaluations are open-ended, necessitating substantial human efforts to verify the model's output results, which introduces uncertainty and potential unfairness in the assessment of models.
(4) \textit{Struggle in evaluating generative models' outputs}: Current benchmarks are unsuitable for evaluating text-to-text models, as they struggle to generate answers identical to the ground truth.
This will make models to fit the benchmarks in order to achieve the best performance, potentially compromising their generalizability.
(5) \textit{Prone to Quickly out-of-date}: As LLMs absorbing increasingly extensive corpora, newly released evaluation data may become part of the LLMs' training data sooner than before, thereby jeopardizing the truthfulness of the evaluation.


In this work, we present \textbf{DomMa}, a \textbf{Dom}ain \textbf{Ma}stery Benchmark, to better alleviate the above limitations in Domain text understanding evaluation.
The benchmark is characterized by its extensive coverage of domain-specific knowledge, substantial data volume, and continuous automatic updates.


Inspired by the Discipline Classification System of Chinese Higher Education, DomMa containing all of 112 top disciplines in this system among 14 disciplinary categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management, arts, and interdisciplinary fields.
In addition, DomMa also employed an additional 393 subject labels to annotate the questions, as well as providing the appearance date, average student score, and highest student score for each question.
In order to effectively evaluate the generative models, we constructed dataset in the format of multiple-choice questions. 
And to increase the performance disparity between models, we set 50 options for each multiple-choice question.


We mainly collect questions from the Chinese Graduate Entrance Examination and from mid or final term exams in chinese universities.
In the original version, we manually annotated 400k questions and used our automatic update system to annotate an additional 100k questions in Chinese language.
Then we utilized ChatGPT~\cite{openaichatgpt} to translate all these 500k questions into English.
In order to evaluate more effectively and address the issue of China-centric bias, we constructed two additional benchmarks, DomMa-Medium and DomMa-Hard, each containing 30k questions, both of which removed some China-centric and other sensitive questions. 
In DomMa-Medium, each question involves only two to four domain-specific knowledge areas, making it relatively hard for models to answer correctly. 
In contrast, DomMa-Hard contains questions that involve five or more completely different domain-specific knowledge areas, making it extremely difficult even for the most cutting-edge models to achieve satisfactory performance on these questions.

\red{要不跟MMLU一样，就不写Contribution了，直接写发现的结论}
We have conducted extremely detailed evaluation and analysis of 50 chat bot LMs that are currently open source parameters or APIs.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
% In summary, our contributions can be summarized as follows:
% (1) We construct DomMa Benchmark, which aims at providing a metric to evaluate the extent to which models can manage domain knowledge.
% (2) The DomMa Benchmark caters particularly to generative LMs, and we propose three evaluation methods tailored to assess the outputs generated by the different capabilities and different degree of open source LMs.
% (3) We have conducted extremely detailed evaluation and analysis of 50 models that are currently open source parameters or APIs.
% We present all of our analysis and several of the most interesting experimental results in the main text, as for all the experimental results, we put them in the appendix


==> old_version/01Introduction.8.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as abstraction, reasoning, and imagination. 
Humans have exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, have shown remarkable capabilities in domain text understanding~\cite{wei2022emergent}.
We cannot help but raise the following questions, and hope to quantify these doubts through experiments:

\begin{center}
    
\textit{In which domains do LLMs perform well?
To what degree can LLMs perform?
How do LLMs compare to human experts?}
\end{center}
Constructing benchmarks is crucial for automatic domain mastery evaluation as benchmarks facilitate efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they exhibit outstanding performance across a wide range of domain-specific tasks.
This makes it increasingly difficult for benchmarks like MMLU~\cite{hendrycks2021measuring}, BIG-bench~\cite{srivastava2022bigbench} or HELM~\cite{liang2022holistic} to provide a comprehensive evaluation of LLMs' capabilities, for they covered only limited spectrum of domain tasks and mostly too simple questions~\cite{suzgun2022big-bench-hard}.

Moreover, conducting effective and fair evaluations has become increasingly challenging~\cite{hendrycks2021measuring, liang2022holistic}. 
One reason is that the emerging LLMs are predominantly generative models, which is hard to assess their outputs~\cite{sai2022survey,zellers2020evaluating}. 
Second reason is that the extensive corpora used by large models, such as GPT-4, encompass nearly all open-source information available on the internet, posing challenges in ensuring evaluation samples are not part of the model's training data~\cite{yang2023harnessing,openai2023gpt4}.

Based on the aforementioned points, we contend that a domain evaluation benchmark and evaluation methods tailored for LLMs should embody the following attributes:
(1) \textit{Cover wide range of subjects}: The previous benchmarks have limited coverage towards domain aspects, even the most comprehensive domain benchmark cover no more than 70 domain-specific knowledge areas, which prevent these benchmarks serving as a comprehensive criterion for domain mastery evaluation.
(2) \textit{Split domain into more detailed labels}: 
Considering the emergent capacity of the models~\cite{wei2022emergent}, it is likely that the SoTA LLMs now have a certain level of performance in all domains. 
Benchmark therefore needs to split the evaluation dimensions more detailed so that it can assess exactly how well the model performs.
(3) \textit{Exclude Open-ended questions}: Some evaluation works contain open-ended questions~\footnote{http://www.llmeval.com/}, which necessitates substantial human efforts to verify the model's output results and introduces uncertainty and potential unfairness in the assessment of models.
(4) \textit{Effectively evaluating the output of generative models}: \blue{Most of existing benchmarks are unsuitable for evaluating generative models, as they struggle to verify the output of the model to the ground truth.}
(5) \textit{Frequently update}: As LLMs trained on increasingly extensive corpora, newly released benchmark may become part of the LLMs' training data much sooner than before.
Frequently updated benchmarks are needed to keep the evaluation samples fresher than the training data used by LLMs.


In this work, we present Domain Mastery Benchmark, to better alleviate the above limitations in Domain text understanding evaluation.
We use \textbf{Xiezhi} to name this benchmark, since Xiezhi is a mythical animal in charge of justice, we do expect this benchmark perform fairly and effectively evaluation towards each language models.
Xiezhi is characterized by its extensive coverage of domain knowledge, substantial data volume, and continuous automatic updates.


Inspired by the Discipline Classification System of Chinese Higher Education, Xiezhi containing all of 118 top-level disciplines in this system among 13 categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management and arts.
In addition, Xiezhi also employed an additional 393 subject labels to annotate the questions, as well as providing the appearance date, average student score, and highest student score for each question.
In order to effectively evaluate the generative models, we constructed dataset in the format of multiple-choice questions. 
And to increase the performance disparity between models, we set 50 options for each multiple-choice question.


We mainly collect questions from the Chinese Graduate Entrance Examination and from mid or final term exams in chinese universities.
In the original version, we manually annotated 400k questions and used our automatic update system to annotate an additional 100k questions in Chinese language.
Then we utilized ChatGPT~\cite{openaichatgpt} to translate all these 500k questions into English.
In order to evaluate more effectively and address the issue of China-centric bias, we constructed two additional benchmarks, Xiezhi-Easy and Xiezhi-Hard, each containing 30k questions, both of which removed some China-centric and other sensitive questions. 
In Xiezhi-Easy, each question involves only two to four domain-specific knowledge areas, making it relatively hard for models to answer correctly. 
In contrast, Xiezhi-Hard contains questions that involve five or more completely different domain-specific knowledge areas, making it extremely difficult even for the most cutting-edge models to achieve satisfactory performance on these questions.

\red{要不跟MMLU一样，就不写Contribution了，直接写发现的结论}
\blue{
We have conducted extremely detailed evaluation and analysis of 50 chat bot LMs that are currently open source parameters or APIs.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
We find out that they are very good.
}


==> old_version/01Introduction.9.tex <==
Domain knowledge encompasses an in-depth comprehension of the world, necessitating the cultivation of various cognitive skills, such as memorization, abstraction, logical thinking, reasoning and imagination. 
Human has exhibited unparalleled proficiency in domain knowledge, far exceeding any machine learning models in a long time.
Nevertheless, recent advancements in Large Language Models (LLMs), including Bloom~\cite{scao2022bloom}, Llama~\cite{touvron2023llama}, ChatGLM~\cite{du2022glm}, GPT4~\cite{openai2023gpt4, bubeck2023sparks} and so many other models, have shown remarkable capabilities in domain text understanding~\cite{wei2022emergent}.
It is time to propose more comprehensive and more prospective evaluations than before to explore whehter language models~(LMs) have actually acquired knowledge, or just acquired enhancement in their imitation ability~\cite{srivastava2022bigbench}.

Constructing benchmarks is crucial for automatic evaluation as benchmarks facilitate efficient, systematic, and scalable comparisons among models. 
However, as LLMs continue to grow in size and complexity, they exhibit outstanding performance across a wide range of domain-specific tasks.
This makes even the newly released benchmarks like MMLU~\cite{hendrycks2021measuring}, BIG-bench~\cite{srivastava2022bigbench} or HELM~\cite{liang2022holistic} all lag behind the capabilities of the language models quickily~\cite{suzgun2022big-bench-hard}.

Today's LMs have emergent task solving abilities and iterate much faster than before. 
Therefore, we conclude that a benchmark in the era of LLMs should meet the following needs:
(1) \textit{Needs to cover more tasks}: 
The previous benchmarks have limited coverage towards domain aspects, even the most comprehensive domain benchmark cover no more than 70 domain-specific knowledge areas, which prevent these benchmarks serving as a comprehensive criterion for domain mastery evaluation.
(2) \textit{Needs to cover more difficulties}: 
Considering the emergent capacity of the models~\cite{wei2022emergent}, it is likely that the SoTA LLMs now have a certain level of performance in all domains. 
Benchmark therefore needs to split the evaluation dimensions more detailed so that it can assess exactly how well the model performs.
(3) \textit{Needs frequent updates}: 
As LLMs trained on increasingly extensive corpora, newly released benchmark may become part of the LLMs' training data much sooner than before.
Frequently updated benchmarks are needed to keep the evaluation samples fresher than the training data used by LLMs.

In the light of the aforementioned needs, we propose Xiezhi-Benchmark, a comprehensive, multi-disciplinary, self-updating benchmark for the assessment of domain knowledge.
Xiezhi consists of 118 different disciplinary questions，ranging from 13 different categories: philosophy, economics, law, education, literature, history, natural sciences, engineering, agriculture, medicine, military science, management and arts.
针对这118个学科，xiezhi对样本还打上了更加细分的396个学科标签。
这总共500多个学科所构成的分类体系来源于中国学科分类系统，这个分类系统被所有中国高校使用，具有广泛的认可度。
Xiezhi从中国考研题目中收集了50k道带有标注的题目进行了人工二次标注，以此为基础训练了自动标注系统，并自动标注了额外的150k道来源不同的考试题目，比如大中小学考试题，职业考试题等。
基于上述方法获得的总共200k道题目，我们进一步地提出Xiezhi-Easy和Xiezhi-Hard，这两个数据集的样本更加平衡，并过滤了敏感知识（如military science）以及中文倾向知识，每个数据集都包含了15,000条数据。
Xiezhi-Easy专门为中小模型设计的，Xiezhi-Easy的题目只包含了每个领域最基础的知识，中小模型在Xiezhi-Easy上表现的差异非常大。
Xiezhi-Hard专门为大模型设计的，即便是GPT-4也只能在3-shot的设定下拿40\%的准确率。

相较于其他为生成模型以及为大模型做评估的工作，我们在评估的方式上进行了一些改进。
我们为每道选择题设置了50个选项，这极大地减少了随机猜测的准确率，从而更能测试出模型的真实能力。
我们使用了生成概率去计算每个模型选择所有选项的概率，从而可以避免模型因为在回答选择题能力上的缺失以及结果抽取上的误差而导致不准确的评估。
因为我们的方法能够计算模型选择每个选项的概率，所以我们可以使用hit@k指标来细致地观察模型的表现。


最后，我们在48个模型上进行了实验。
所有模型都在中文Xiezhi和英文Xiezhi上进行了测试，并取最好的结果来进行分析。
我们发现，GPT-4虽然能在各个领域都取得最好的成绩，但在任何一个领域上都没有达到领域从业者的平均水平。
另外，尽管大模型被认为在没见过的任务上具有涌现能力，但是在一些语料不多的领域，模型的表现甚至比需要复杂推理的任务还要差。
同时，我们发现模型对于领域知识的理解能力和ift数据量无关，甚至很多模型会因为注入ift数据之后，对于领域知识的掌握能力会剧烈下降。
除此之外我们还将最近提出的领域benchmark用我们的评估设定进行了测试。
在hit@3指标下，不同模型在Xiezhi-Easy上表现的bias是最大的。
这说明了Xiezhi不仅覆盖了最全面的领域，包含了最多的题目，还最能够区分不同LLMs的能力差异，是最适合所有能力段的LLMs评估的benchmark。


==> old_version/02RelatedWorks.0.tex <==


Benchmarks orient AI~\cite{liang2022holistic}.
They encode values and priorities~\cite{ethayarajh2020utility,birhane2022values} that specify directions for the AI community to improve upon~\cite{kiela2021dynabench,bowman2021will,raji2021ai}.
When implemented and interpreted appropriately, they enable the broader community to better understand AI technology and influence its trajectory.

% \subsection{传统评估}


% \subsection{基于LLM的评估}
Several other benchmarks have been organized through similar community efforts, and this approach has increasingly been adopted to source diverse ideas and contributions.
XTREME~\cite{hu2020xtreme} is a benchmark proposed by Google for evaluating the cross-lingual generalization ability of pre-trained multilingual models. It covers 40 typologically diverse languages spanning 12 language families and includes nine tasks that require reasoning at different levels of syntax and semantics.
To address the lack of geographic diversity in NLP, ~\cite{mulligan-etal-2021-structure} used participatory researhc to construct a machine-translation benchmark for over 30 low-resource languages.
EleutherAI's Language Model Evaluation Harness~\cite{eval-harness} is another open-sourece collaborative benchmarking codebase.
The GEM benchmark is a living benchmark for natural language generation, evaluation, and metrics~\cite{gehrmann2021gem}, constructed by a broad collaboration of more than 50 contributors.
GEM provides an environment in which models can be tested on a wide set of tasks and with different evaluation strategies that can evolve alongside the models.
A related project that grew out of GEM is NL-Augmenter~\cite{dhole2021nl}, which crowd-sources transformations and augmentation of textual datasets.
The Natural Instructions Expansion project has been initiated in an effort to source a large collection of natual-language tasks and their natural-language definitions/instructions.
This project is an expansion of NATURAL INSTRUCTIONS~\cite{mishra2021cross}, which contained dataset creation and model benchmarking that uses human-and-model-in-the-loop to identify and collect examples where models will fail but humans would not.
SyntaxGym~\cite{gauthier2020syntaxgym} is an online platform designed to make targeted evaluations following the norms of psycholinguistic experimental design.
New evaluations can be contributed as test suits on their project website.
The Massive Multitask Language Understanding (MMLU) benchmark~\cite{hendricks2018women} is a collection of 57 diverse tasks, collated by 7 authors.

As language models increase in scale, their quantitative improvement and new qualitative capabilities may have potentially transformative impacts~\cite{wei2022emergent}.
In order to facilitate future research, prepare for disruptive new model capabilities and mitigate socially harmful effects, it is essential to understand the current and near-future capabilities and limitations of language models. 
BIG-bench~\cite{srivastava2022bigbench} was created to probe large language models and extrapolate their future capabilities.
It includes more than 200 tasks that are diverse and focus on areas believed to be beyond the capabilities of current language models.




Center for Research on Foundation Models (CRFM) Benchmark~\cite{liang2022holistic} has benchmark 30 prominent language models across a wide range of scenarios and for a broad range of metrics to elucidate their capabilities and risks.

% \subsection{传统评估}
% Similar to the language models, benchmarking has a long history in NLP.
% With the rise of deep learning, large benchmarks such as SNLI, QNLI, SQuAD were developed to provide both adequate data from training systems in addition to evaluating systems.
% These benchmarks assign each model a single score to measure the accuracy for a single tasks.

% With the language models become bigger and more general~\cite{wei2022emergent}, many task-specific approaches has been taken placed, new benchmakrs such as SentEval, DecaNLP, GLUE, and SuperGLUE co-evolved to evaluate their capabilities.
% In contrast to the previous class of benchmarks, these benchmarks assign each model a vector of scores to measure the accuracy for a suite of scenarios.
% In some cases, these benchmarks also provide an aggregate score.

% \subsection{近年来的评估}
% More recently, this theme of meta-benchmakrs that assess model accuracy accross a range of tasks has continued.
% % Several other benchmarks have been organized through similar community efforts, and this approach has increasingly been adopted to source diverse ideas and contributions.
% XTREME~\cite{hu2020xtreme} is a benchmark proposed by Google for evaluating the cross-lingual generalization ability of pre-trained multilingual models. It covers 40 typologically diverse languages spanning 12 language families and includes nine tasks that require reasoning at different levels of syntax and semantics.
% To address the lack of geographic diversity in NLP, ~\cite{mulligan-etal-2021-structure} used participatory researhc to construct a machine-translation benchmark for over 30 low-resource languages.
% EleutherAI's Language Model Evaluation Harness~\cite{eval-harness} is another open-sourece collaborative benchmarking codebase.
% The GEM benchmark is a living benchmark for natural language generation, evaluation, and metrics~\cite{gehrmann2021gem}, constructed by a broad collaboration of more than 50 contributors.
% GEM provides an environment in which models can be tested on a wide set of tasks and with different evaluation strategies that can evolve alongside the models.
% A related project that grew out of GEM is NL-Augmenter~\cite{dhole2021nl}, which crowd-sources transformations and augmentation of textual datasets.
% The Natural Instructions Expansion project has been initiated in an effort to source a large collection of natual-language tasks and their natural-language definitions/instructions.
% This project is an expansion of NATURAL INSTRUCTIONS~\cite{mishra2021cross}, which contained dataset creation and model benchmarking that uses human-and-model-in-the-loop to identify and collect examples where models will fail but humans would not.
% SyntaxGym~\cite{gauthier2020syntaxgym} is an online platform designed to make targeted evaluations following the norms of psycholinguistic experimental design.
% New evaluations can be contributed as test suits on their project website.
% The Massive Multitask Language Understanding (MMLU) benchmark~\cite{hendricks2018women} is a collection of 57 diverse tasks, collated by 7 authors.

% As language models increase in scale, their quantitative improvement and new qualitative capabilities may have potentially transformative impacts~\cite{wei2022emergent}.
% In order to facilitate future research, prepare for disruptive new model capabilities and mitigate socially harmful effects, it is essential to understand the current and near-future capabilities and limitations of language models. 
% BIG-bench~\cite{srivastava2022bigbench} was created to probe large language models and extrapolate their future capabilities.
% It includes more than 200 tasks that are diverse and focus on areas believed to be beyond the capabilities of current language models.

==> old_version/02RelatedWorks.1.tex <==
\subsection{Benchmarks before the era of LLMs}
% 过去有很多语言理解数据集被精心整理并开源出来为NLP模型的发展提供了指引和评估。
% 这些数据集一般都会涵盖若干个单独的任务，并且每个样本都有着明确的ground truth和metric，可以精确地展示模型在特定任务上的表现能力。
In the past, numerous language understanding datasets have been meticulously curated and made available as open-source resources, providing guidance and evaluation for the development of NLP models. These datasets generally encompass a variety of individual tasks, with each sample possessing a clear ground truth and metric, allowing for a precise illustration of a model's performance capabilities in specific tasks.
SentEval~\cite{conneau2018senteval}, DecaNLP~\cite{mccann2018decanlp}, GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}, EleutherAI's Language Model Evaluation Harness~\cite{eval-harness} are open-source collaborative benchmarking codabases, they organizes existing tasks and EleutherAI even defines a unified API for evaluating models on them.
GEM provides an environment in which models can be tested on a wide set of tasks and with different evaluation strategies that can evolve alongside the models.
A related project that grew out of GEM is NL-Augmenter~\cite{dhole2021nl}, which crowd-sources transformations and augmentation of textual datasets.
The Natural Instructions Expansion project has been initiated in an effort to source a large collection of natual-language tasks and their natural-language definitions/instructions.
This project is an expansion of NATURAL INSTRUCTIONS~\cite{mishra2021cross}, which contained dataset creation and model benchmarking that uses human-and-model-in-the-loop to identify and collect examples where models will fail but humans would not.
SyntaxGym~\cite{gauthier2020syntaxgym} is an online platform designed to make targeted evaluations following the norms of psycholinguistic experimental design.
New evaluations can be contributed as test suits on their project website.
The Massive Multitask Language Understanding (MMLU) benchmark~\cite{hendricks2018women} is a collection of 57 diverse tasks, collated by 7 authors.

\subsection{Benchmarks in the era of LLMs}
% BIG-Bench正式掀开了大模型评估的序章，这是个由Google发起的合作项目所创造出来的大规模语言模型基准测试，目标是评估各种语言模型的多个方面的能力。
% 相较于之前的Benchmarks，针对于LLM的评估更加注重检验模型解决推理、记忆、理解上下文以及一些高级认知问题的能力。
% HELM~\cite{liang2022holistic}为42个语言场景设计了benchmark，他们使用了总共57个metrics来提供更加精细的评估。
% LILA~\cite{mishra2022lila}目标是评估语言模型的数学能力，他们的benchmark涵盖了23个不同的数学推理任务，他们给每个问题标有insturction annotations，并且还以python程序的形式给出了每个问题的解决方案。
The BIG-Bench has officially initiated the evaluation of large-scale models, a collaborative project launched by Google to establish a comprehensive benchmark for assessing various aspects of language models' capabilities. In contrast to prior benchmarks, the evaluation of large language models (LLMs) emphasizes examining their ability to solve problems involving reasoning, memory, context understanding, and advanced cognitive abilities.
HELM~\cite{liang2022holistic} devised a benchmark for 42 language domains, employing a total of 57 metrics to provide a more nuanced evaluation. Meanwhile, LILA~\cite{mishra2022lila} aims to assess language models' mathematical abilities, with their benchmark encompassing 23 different mathematical reasoning tasks. Each problem in their benchmark is labeled with instruction annotations, and solutions are provided in the form of Python programs.
GPT-Plan~\cite{valmeekam2022large} is about to test how model do testing about actions and change involving common-sense planning tasks，which are core aspects of human intelligence and required for many of the tasks considered as potential applications of LLMs.
ALERT~\cite{yu2022alert} provides a test bed to assess any language model on fine-grained reasoning skills, which spans over 20 datasets and covers 10 different reasoning skills.
MEGA~\cite{ahuja2023mega} is the first comprehensive benchmark with various languages of generative LLMs, which evaluates models on standard NLP benchmarks covering 8 diverse tasks and 33 typologically diverse langauges.
GLUE-X~\cite{yang2022glue} targets at creating a unified benchmark for evaluating out-of-distribution robustness in NLP models, highlighting the importance of out-of-distribution robustness and probiding insights on how to measure the robustness of a model and how to improve it.


==> old_version/02RelatedWorks.2.tex <==
\subsection{Benchmarks Before the Era of LLMs}
In the past, a plethora of language comprehension datasets have been painstakingly curated and provided as open-source assets, offering guidance and assessment for natural language processing (NLP) model development. These datasets generally encompass a myriad of distinct tasks, with each instance possessing a definitive ground truth and metric, facilitating an accurate depiction of a model's performance capacities in specific assignments.
Open-source collaborative benchmarking databases, such as SentEval~\cite{conneau2018senteval}, DecaNLP~\cite{mccann2018decanlp}, GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}, and EleutherAI's Language Model Evaluation Harness~\cite{eval-harness}, organize existing tasks and Even offer a unified API for model evaluation. GEM provides an environment wherein models can be assessed across a diverse array of tasks and varying evaluation strategies, evolving in tandem with the models.
A related endeavor that emerged from GEM is NL-Augmenter~\cite{dhole2021nl}, which crowd-sources transformations and augmentations of textual datasets. The Natural Instructions Expansion project was initiated with the aim of curating a substantial compendium of natural language tasks and their corresponding natural language definitions/instructions. This project expands upon NATURAL INSTRUCTIONS~\cite{mishra2021cross}, which comprised dataset creation and model benchmarking utilizing a human-and-model-in-the-loop approach to identify and gather examples where models fail yet humans succeed.
SyntaxGym~\cite{gauthier2020syntaxgym} is an online platform designed to enable targeted evaluations adhering to the standards of psycholinguistic experimental design. New evaluations can be contributed as test suites via the project website. The Massive Multitask Language Understanding (MMLU) benchmark~\cite{hendricks2018women} is an assemblage of 57 diverse tasks, compiled by 7 authors.

\subsection{Benchmarks in the Era of LLMs}
The BIG-Bench project, officially initiated by Google, marks a collaborative effort to establish a comprehensive benchmark for evaluating various aspects of language models' capabilities. Unlike earlier benchmarks that assessed large language models (LLMs), this evaluation focuses on examining their abilities to solve problems involving reasoning, memory, context understanding, and advanced cognitive abilities.
HELM~\cite{liang2022holistic} has developed a benchmark comprising 42 language domains, using a total of 57 metrics to provide a more nuanced evaluation. Concurrently, LILA~\cite{mishra2022lila} seeks to assess language models' mathematical abilities through their benchmark, which includes 23 distinct mathematical reasoning tasks. Within this benchmark, each problem bears instruction annotations, and solutions are supplied in the form of Python programs.
GPT-Plan~\cite{valmeekam2022large} aims to analyze how models perform tests involving actions and changes in common-sense planning tasks—core aspects of human intelligence that are requisite for numerous tasks considered as potential applications of LLMs. ALERT~\cite{yu2022alert} offers a test bed to evaluate various language models on fine-grained reasoning skills, encompassing over 20 datasets and covering 10 distinct reasoning skills.
MEGA~\cite{ahuja2023mega}, the first comprehensive benchmark for generative LLMs in multiple languages, evaluates models based on standard NLP benchmarks that include 8 diverse tasks and 33 typologically different languages. Meanwhile, GLUE-X~\cite{yang2022glue} focuses on creating a unified benchmark to assess out-of-distribution robustness in NLP models, highlighting the importance of such robustness and providing insights on how to measure and improve model robustness.

==> old_version/02RelatedWorks.3.tex <==
\subsection{Benchmarks before the Era of LLMs}
In the past, numerous language comprehension benchmarks have been diligently curated and made openly available to guide and assess the development of natural language processing (NLP) models. 
These benchmarks typically cover a wide range of distinct tasks, each with a definitive ground truth and metric, enabling an accurate portrayal of a model's performance capabilities in specific assignments.
Open-source collaborative benchmarking databases, such as SentEval~\cite{conneau2018senteval}, DecaNLP~\cite{mccann2018decanlp}, GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}, and EleutherAI's Language Model Evaluation Harness~\cite{eval-harness}, aggregate existing tasks and provide a unified API for model evaluation. GEM offers an environment where models can be assessed across diverse tasks with varying evaluation strategies, evolving in line with the models themselves.
NL-Augmenter~\cite{dhole2021nl} is crowdsourced by transformations and augmentations of textual datasets. 
The Natural Instructions Expansion project aims to curate a substantial collection of natural language tasks and their corresponding natural language definitions/instructions, building on NATURAL INSTRUCTIONS~\cite{mishra2021cross}, which involved dataset creation and model benchmarking using a human-and-model-in-the-loop approach to identify and gather examples where models fail, and humans succeed.
SyntaxGym~\cite{gauthier2020syntaxgym} is an online platform designed to facilitate targeted evaluations adhering to psycholinguistic experimental design standards, with new evaluations contributed as test suites through the project website. The Massive Multitask Language Understanding (MMLU) benchmark~\cite{hendricks2018women} is a compilation of 57 diverse tasks, assembled by seven authors.


\subsection{Benchmarks in the Era of LLMs}
The BIG-Bench project, endorsed by Google, represents a collaborative initiative aimed at developing an all-encompassing benchmark for assessing the multifaceted capabilities of language models. In contrast to previous benchmarks concerning large language models (LLMs), this evaluation emphasizes scrutinizing their potential to address challenges involving reasoning, memory, context comprehension, and sophisticated cognitive skills.
HELM~\cite{liang2022holistic} establishes a benchmark encompassing 42 linguistic domains and employs 57 distinct metrics to deliver a comprehensive assessment. Simultaneously, LILA~\cite{mishra2022lila} evaluates language models' mathematical proficiency via a benchmark containing 23 unique mathematical reasoning tasks, with annotated problem instructions and Python-based solutions.
GPT-Plan~\cite{valmeekam2022large} investigates model performance in tasks involving actions and shifts in common-sense planning tasks — fundamental components of human intelligence required for numerous LLM applications. ALERT~\cite{yu2022alert} serves as a testing platform to gauge language models' fine-grained reasoning abilities, incorporating over 20 datasets and addressing 10 specific reasoning competencies.
MEGA~\cite{ahuja2023mega}, a pioneering comprehensive multi-lingual benchmark for generative LLMs, evaluates models using a variety of standard NLP benchmarks, featuring eight diverse tasks in 33 typologically distinct languages. Concurrently, GLUE-X~\cite{yang2022glue} concentrates on devising a unified benchmark for examining out-of-distribution robustness in NLP models, underscoring the significance of robustness and offering insights for enhancing model sturdiness.

==> old_version/02RelatedWorks.4.tex <==
% \subsection{Benchmarks for Single Domain}
% In the past, numerous language comprehension benchmarks have been diligently curated and made openly available to guide and assess the development of natural language processing (NLP) models. 
% These benchmarks typically cover a wide range of distinct tasks, each with a definitive ground truth and metric, enabling an accurate portrayal of a model's performance capabilities in specific assignments.
% Open-source collaborative benchmarking databases, such as SentEval~\cite{conneau2018senteval}, DecaNLP~\cite{mccann2018decanlp}, GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}, and EleutherAI's Language Model Evaluation Harness~\cite{eval-harness}, aggregate existing tasks and provide a unified API for model evaluation. GEM offers an environment where models can be assessed across diverse tasks with varying evaluation strategies, evolving in line with the models themselves.
% NL-Augmenter~\cite{dhole2021nl} is crowdsourced by transformations and augmentations of textual datasets. 
% The Natural Instructions Expansion project aims to curate a substantial collection of natural language tasks and their corresponding natural language definitions/instructions, building on NATURAL INSTRUCTIONS~\cite{mishra2021cross}, which involved dataset creation and model benchmarking using a human-and-model-in-the-loop approach to identify and gather examples where models fail, and humans succeed.
% SyntaxGym~\cite{gauthier2020syntaxgym} is an online platform designed to facilitate targeted evaluations adhering to psycholinguistic experimental design standards, with new evaluations contributed as test suites through the project website. The Massive Multitask Language Understanding (MMLU) benchmark~\cite{hendricks2018women} is a compilation of 57 diverse tasks, assembled by seven authors.
\subsection{Large Language Models}
Recently, various companies released their LLMs, such as BARD~\footnote{https://bard.google.com/?hl=en}, ERNIE Bot~\footnote{https://yiyan.baidu.com/}, Bloom~\cite{scao2022bloom}, pythia~\cite{biderman2023pythia}, Llama~\cite{touvron2023llama}, Claude~\footnote{https://www.anthropic.com/product}, ChatGPT~\cite{openaichatgpt}, GPT-4~\cite{openai2023gpt4}, and ChatGLM~\cite{du2022glm}.
These language models typically possess a vast number of parameters and utilize an extensive amount of training data~\cite{zhou2023comprehensive}. 
Their performance on numerous tasks significantly surpasses that of previous models, which can be attributed to the activation of the models' problem-solving abilities through instruction fine-tuning and the acquisition of extensive knowledge from large-scale corpora~\cite{scao2022bloom,bubeck2023sparks}.
Researches have also indicated that LLMs have exhibited emergent phenomena, enabling them to perform well on unseen tasks~\cite{chung2022scaling}. 
Furthermore, their ability to learn from examples or context is considerably superior to that of earlier models, endowing them with remarkable adaptability~\cite{li2023context, min2022rethinking}. 
Consequently, the evaluation of LLMs' capabilities should focus more on a wide range of tasks, numerous diverse domains and more difficult samples.

The development of LLMs has spurred the growth of a series of small-scale conversational LMs, such as Alpaca~\cite{alpaca}, Vicuna~\cite{vicuna2023}, H2OGPT~\cite{2023h2ogpt}, and Moss~\cite{sun2023moss}.
Most of these conversational LMs, such as Alpaca~\cite{alpaca}, Vicuna~\cite{vicuna2023}, BELLE~\cite{ji2023belle}, Huatuo~\cite{wang2023huatuo}, Baize~\cite{xu2023baize}, are trained based on existing pre-trained LMs.
Many of these works, such as BELLE~\cite{ji2023belle}, Baize~\cite{xu2023baize}, used high-quality data generated from LLMs.
Some of these works trained in an parameter-efficient tuning methods~\cite{hu2023llm, hu2021lora}.
During their development, these conversational models also require performance evaluation to obtain effective feedback that guides their direction of growth.
However, small-scale conversational models iterate new versions every few days, and as the training data continuously expands, any new benchmark will quickly become outdated as it is incorporated into the model's training data. 
Previous models did not iterate as rapidly as they do today, so no work has considered a self-updating benchmark. 
DomMa's self-updating mechanism ensures that it consistently stays ahead of the model's training data, providing an effective measure of the model's performance.

% 最近一段时间，各大公司陆续推出了自己具有超强能力的语言模型，如bard~\cite{2019bart}，ERNIE Bot~\footnote{https://yiyan.baidu.com/}，bloom，llama，chatgpt，gpt-4，chatGLM。
% 这些语言模型通常参数量十分庞大，使用了非常大量的训练语料。
% 这些模型在许多任务上有着远超以往模型的表现，这是由于指令微调激活了模型解决任务的能力，也因为模型从大规模语料中学习到了非常多的知识。
% 有研究指出，大模型已经产生了涌现现象，这能够使大模型在没见过的任务上同样具有很好的表现。
% 同时，大模型对于样例的学习能力也远强于以往的模型，使得大模型能具有很强的适应能力。
% 因此，对于大模型能力的评估应当更加聚焦于广泛的任务和大量不同的领域。

% 大模型的发展，催生了一批小规模的对话模型的发展，比如alpaca, vicuna，h2ogpt, moss等。
% 这些对话模型大多使用了已有的预训练参数，从语言模型中诱导出了高质量数据，有些还使用了高效的微调训练方法。
% 这些对话模型在发展的过程中也需要评估效果，从而得到有效的反馈以指引他们发展的方向。
% 但小规模的对话模型每隔几天就会迭代出新的版本，随着训练语料不断地扩大，任何一个新的benchmark将很快被作为模型的训练数据从而过时。
% 以前的模型不会像今天这样迅速迭代，所以没有工作考虑过一个能自更新的benchmark，而DomMa的自更新机制能保证DomMa不断地领先模型的训练语料，为模型的效果提出有效的度量。

\subsection{Benchmarks}
Since the inception of BIG-Bench, the goal of benchmark design has been to surpass the capabilities of existing models and pre-design comprehensive and meaningful tasks for model development. However, language models quickly achieved superhuman performance on most tasks in Big-bench. Following Big-bench, numerous studies have focused on proposing more comprehensive benchmarks that are ahead of language model capabilities, providing insights and evaluation criteria for language model development. Such works include Big-Bench-Hard, Hard-Bench, and HELM. Although these works aim for comprehensive evaluation, they only propose a large number of dimensions with coarse granularity. In contrast, DomMa's objective is to provide both comprehensive and in-depth evaluation for the entire domain knowledge.

Some research also focuses on evaluating the knowledge acquired by language models. Some works, such as HellaSwag, Physical IQA, and CosmosQA, concentrate on assessing language models' grasp of common-sense knowledge. Other studies, like MMLU, LILA, and LexTreme, are dedicated to evaluating models' mastery of domain-specific knowledge. However, language models have already achieved performance surpassing human experts in these works, making it difficult to effectively distinguish the differences in capabilities between different models.

In addition, conducting few-shot evaluation for generative language models can be challenging. Starting from MMLU, many works have proposed using generative models to solve classification problems. Recently, several evaluation studies, such as SuperClue, have suggested using a unified instruction to question models and employing a unified extraction rule to extract model answers. This approach demands a high level of capability from the models, as many models cannot effectively understand the instructions, resulting in unfair evaluations. Therefore, we use the probability of models generating correct answers as a substitute for question-answering, which provides a more equitable evaluation for models with varying capabilities.

% 从BIG-Bench开始，benchmark设计的目标在于超越现有模型的能力，为模型的发展预设计出全面有意义的任务。
% 但是，语言模型很快在Big-bench上的大多数任务中达到了超越人类的效果。
% 从Big-bench之后，有很多工作也专注于提出更加全面且超前于语言模型能力的benchmark来为语言模型的发展提供思路与评估准则。
% 这类的工作有Big-Bench-Hard，Hard-Bench，HELM。
% 然而这类工作的目标虽然是全面评估，但他也只是提出了数量很多粒度却很粗的维度。
% In contrast，DomMa的目标在于为整个领域知识提供既全面又有深度的评估。

% 有些研究也侧重于评估语言模型所掌握的知识。
% 有些工作，比如HellaSwag，Physical IQA，CosmosQA，专注于评估语言模型对于常识知识的掌握。
% 还有些工作，比如MMLU，LILA，LexTreme，专注于评估模型对于领域知识的掌握。
% 但是语言模型在这些工作上已经取得了超越人类专家的表现，这些工作已经很难有效的区分出不同模型之间能力的差异了。

% 除此之外，生成式语言模型去做few-shot评估比较困难。
% 从MMLU开始，许多工作都提出让生成式模型去做分类题。
% 而最近，有很多评估工作，比如SuperClue，提出用统一的指令去提问模型，并使用了统一的抽取规则去抽取模型的答案。
% 这种方法对于模型的能力有着较大的要求，很多模型并不能有效地理解指令，从而得到了不公平的评估。
% 因此我们使用计算模型生成正确答案的概率来替代问答，这个方式可以给与能力不同的模型更加公平的评估。


% The BIG-Bench project, endorsed by Google, represents a collaborative initiative aimed at developing an all-encompassing benchmark for assessing the multifaceted capabilities of language models. In contrast to previous benchmarks concerning large language models (LLMs), this evaluation emphasizes scrutinizing their potential to address challenges involving reasoning, memory, context comprehension, and sophisticated cognitive skills.
% HELM~\cite{liang2022holistic} establishes a benchmark encompassing 42 linguistic domains and employs 57 distinct metrics to deliver a comprehensive assessment. Simultaneously, LILA~\cite{mishra2022lila} evaluates language models' mathematical proficiency via a benchmark containing 23 unique mathematical reasoning tasks, with annotated problem instructions and Python-based solutions.
% GPT-Plan~\cite{valmeekam2022large} investigates model performance in tasks involving actions and shifts in common-sense planning tasks — fundamental components of human intelligence required for numerous LLM applications. ALERT~\cite{yu2022alert} serves as a testing platform to gauge language models' fine-grained reasoning abilities, incorporating over 20 datasets and addressing 10 specific reasoning competencies.
% MEGA~\cite{ahuja2023mega}, a pioneering comprehensive multi-lingual benchmark for generative LLMs, evaluates models using a variety of standard NLP benchmarks, featuring eight diverse tasks in 33 typologically distinct languages. Concurrently, GLUE-X~\cite{yang2022glue} concentrates on devising a unified benchmark for examining out-of-distribution robustness in NLP models, underscoring the significance of robustness and offering insights for enhancing model sturdiness.

==> old_version/02RelatedWorks.5.tex <==

\subsection{Large Language Models}
Recently, various companies released their LLMs, such as BARD~\footnote{https://bard.google.com/?hl=en}, ERNIE Bot~\footnote{https://yiyan.baidu.com/}, Bloom~\cite{scao2022bloom}, pythia~\cite{biderman2023pythia}, Llama~\cite{touvron2023llama}, Claude~\footnote{https://www.anthropic.com/product}, ChatGPT~\cite{openaichatgpt}, GPT-4~\cite{openai2023gpt4}, and ChatGLM~\cite{du2022glm}.
Apart from their outstanding performance on trained tasks, researches has also discovered that they emerge to have strong performance on many unseen tasks~\cite{zhou2023comprehensive, chung2022scaling}.
Consequently, the evaluation of LLMs' capabilities today should focus more on a wide range of tasks, consist of numerous diverse domains and contain samples with different difficult-level.

The development of LLMs has spurred the growth of a series of small-scale conversational LMs, such as Alpaca~\cite{alpaca}, Vicuna~\cite{vicuna2023}, H2Ogpt~\cite{2023h2ogpt}, and Moss~\cite{sun2023moss}.
Most of these small conversational LMs are fine-tuned based on existing pre-trained LMs through high-quality dialog data generated from LLMs~\cite{ji2023belle, xu2023baize} by parameter-efficient tuning methods~\cite{hu2021lora, hu2023llm}.
In order to achieve excellent performance, these models continuously acquire the latest data from the internet, and their iteration speed is much faster than LLMs~\footnote{https://www.semianalysis.com/p/google-we-have-no-moat-and-neither}.
Any new benchmark will quickly become outdated as it is incorporated into the model's training data.

% Xiezhi's self-updating mechanism ensures that it consistently stays ahead of the model's training data, providing an effective measurement of the model's performance.



\subsection{Benchmarks}
% Start from BIG-Bench, the primary objective of benchmark design has been to go beyond the abilities of current LMs and develop detailed, meaningful tasks for models' advancement~\cite{srivastava2022bigbench}. 
% However, examples of such works, like Big-Bench-Hard~\cite{suzgun2022big-bench-hard}, Hard-Bench~\cite{wang2023hard-bench}, and HELM~\cite{liang2022holistic} were designed to assess various abilities ahead of the LMs. 
% However, with the development of LLMs today, both the evaluation dimensions and difficulty level of these benchmarks have fallen considerably behind.


A number of studies concentrate on assessing a model's knowledge and reasoning ability. 
Certain works, including HellaSwag~\cite{zellers2019hellaswag}, Physical IQA~\cite{bisk2020piqa}, and CosmosQA~\cite{huang2019cosmos}, focus on evaluating the understanding of LMs' commonsense knowledge. 
Meanwhile, other researches, such as MMLU~\cite{hendrycks2021measuring}, Lila~\cite{mishra2022lila}, AGI-Eval~\cite{zhong2023agieval}, MMCU~\cite{zeng2023measuring}, C-Eval~\cite{huang2023ceval}, M3KE~\cite{liu2023m3ke} and LexTreme~\cite{niklaus2023lextreme}, targets at evaluating the models' proficiency in domain knowledge.
However, whether these benchmarks can provide effective evaluations for all language models remains debatable. 
This is because only LLMs with super abilities \red{perform defferentially} on their datasets, while small LMs only perform at a level close to random guessing, leading to different evaluation reasearches have different or even contradictory results on small LMs.
Furthermore, as the training corpora for models become increasingly larger, these benchmarks might lose their evaluative significance shortly after they are proposed, due to their incorporation into the training sets of LMs.

Moreover, the raise of the generative LMs presents its own difficulties in evaluation~\cite{sai2022nlg-metric}. 
Beginning with MMLU~\cite{hendrycks2021measuring}, numerous works have proposed to use multiple-choice questions to assess generative models. 
Recently, a variety of evaluation studies, such as SuperClue~\footnote{https://github.com/CLUEbenchmark/SuperCLUE}, \blue{have recommended utilizing a single, unified instruction to query all models, and use doing answer extraction to get models' choices.}
This approach require models to have strong abilities in instruction understanding especially in multiple-choice answering, as many LMs are unable to meet that needs, leading to unfair evaluation results. 

% In contrast, Xiezhi is capable of providing \blue{sufficiently differentiated evaluations for models of all capabilities across a wide range of domains}. 
% This advantage is attributed to the integration of a domain taxonomy, extensive question collection, and the development of an auto-updating system, allowing for the accumulation of diverse and up-to-date data with varying difficulty levels.
% Furthermore, the adoption of a 50-option selection setting and the methodology for calculating generative probabilities introduced in this study contribute to a significantly more stable assessment outcome compared to previous works.


% In contrast, Xiezhi可以为全能力段的模型在全领域提出有足够区分度的评估。
% 这得益于Xiezhi对领域分类体系的整理，大量的题目收集，以及自更新系统的开发，使得Xiezhi有了足够多样且难度不同的最新数据。
% 也得益于本文提出的50选1的设定，以及计算生成概率的方法，使得评估结果比前人的工作稳定许多。


% In addition, conducting few-shot evaluation for generative LMs can be challenging. Starting from MMLU, many works have proposed using generative models to solve classification problems. Recently, several evaluation studies, such as SuperClue, have suggested using a unified instruction to question models and employing a unified extraction rule to extract model answers. This approach demands a high level of capability from the models, as many models cannot effectively understand the instructions, resulting in unfair evaluations. Therefore, we use the probability of models generating correct answers as a substitute for question-answering, which provides a more equitable evaluation for models with varying capabilities.


==> old_version/03BenchmarkDescription.0.tex <==
我们将在本章节中详细介绍我们的工作。
我们的目标是针对领域知识进行评估，并使用了中国的学科分类系统来构建我们的Benchmark，我们将在第~\ref{031}章节对领域一词进行定义，并详细描述中国的学科系统与领域知识的相关性。
我们将在~\ref{032}章节详细讲述我们数据集的收集过程，以及我们人工过滤的方法，以及我们是如何保证数据集永远能够领先于LLM的训练。
最后，我们在~\ref{033}章节讲述了我们为LLM的输出而设计的评估方法。


\subsection{Domain Knowledge}
\label{031}

\subsubsection{Definition}
领域知识（Domain Knowledge）指的是关于特定学科、行业或业务领域的专业知识和理解。这类知识通常由专家或从业者掌握，并逐步在相关领域的研究和工作中积累和完善。领域知识的掌握程度直接影响到工作、研究的效率和质量。

\red{领域知识的定义还要继续搜集}
在自然语言处理（Natural Language Processing, NLP）领域，领域知识可以用来提高模型在特定领域的任务中的表现。例如，在金融领域的文本分类任务中，也许根据基本的NLP技术就能取得相对不错的结果，但如果在此基础上加入金融领域的专业知识（如金融术语、法规、行业动态等），则可以进一步提高模型的精确度和实用性。

\subsubsection{Chinese Subject Classification System}
中国的学科分类体系是指由中国教育部制定的对高等教育领域中各个学科进行分类和编码的体系。该体系将学科划分为学科门类、一级学科、二级学科等多个层次。这几个层次的意义介绍如下：

学科门类：这是学科分类的最高层次，按照学科的性质、特点和相互关系进行大致划分。共有十四个学科门类，分别为哲学、经济学、法学、教育学、文学、历史学、理学、工学、农学、医学、军事学、管理学、艺术学、交叉学科。

一级学科：在学科门类的基础上，将具有相似性和相关性的研究领域归纳为一级学科。例如，经济学门类下可以设有“政治经济学”、“财政学”、“金融学”等一级学科。一级学科为学科分支分类的基本单位，其下又可以设置二级学科。

二级学科：它位于一级学科之下，是对一级学科进行更细分的研究领域。例如，在金融学这个一级学科下，可以进一步划分为金融市场、银行学、保险学、国际金融等二级学科。二级学科可以进一步细化为具体的研究方向或主题。

中国学科分类体系是一个层次结构体系，学科门类是顶层，代表了一个学科的更广泛的范围和内涵; 一级学科和二级学科则分别代表了在学科门类中的具体领域和更细分的研究领域。在实际运作中，这一分级体系有助于更好地管理、规划和指导高等教育的教学和科研工作。同时，它也为教师、学者、学生等提供了一个清晰、有序的学科发展和研究的框架。

\subsection{数据集收集}
\label{032}
这一章节，我们主要阐述了我们数据集收集的过程，并详细介绍了人工筛选的标准，以及数据集自动化更新的方案。
我们在论文投稿放出时收集到的数据量以及数据的分布如图~\ref{fig:benchstatistic}所示。

\subsubsection{Collection}
我们主要从两个数据源获取数据。
第一个数据源是升学考试题目，我们收集了中国研究生升学考试题共计\red{100,000}条数据。
另一个数据源是开源网站上收集的各大高校的期中期末考试题，我们总共收集了\red{1,000,000}条数据。
为了能够进行自动化评估，所以我们只收集了具有明确ground truth的题目，这类题目的题型主要有：选择题、填空题、判断题、解答题。
我们还在数据收集过程使用了GPT-4把所有的中文题目都翻译为了英文。


\subsubsection{Annotation}
我们认为升学考试题目的质量是最为优质的，所以我们主要针对升学考试的题目进行了大量的人工标注和清洗工作，这些数据集也将单独开源出来。
我们付费请了高校研究生来给我们标注和清洗数据。
我们对所有的应聘的标注者进行了培训，并对培训的内容进行了测试，以充分了解我们的注释者。
最后，我们选择了其中的8位来自不同学科门类的研究生作为我们的标注者，他们的工资都要高于当地最低的工资。

\begin{figure}[h]


\begin{center}

\includegraphics[width=0.6\textwidth]{BenchmarkStatistic.jpg}

\end{center}
\label{fig:benchstatistic}
\caption{A gull}


\end{figure}

注释的内容主要包括对题目进行以下标注：1.标注仅靠文本信息无法回答的题目，这类题目包括需要读取图片的题目，以及需要读取音频信息的听力题目，我们将这些需要非文本信息的题目暂时剔除出benchmark。2.标注题目所涉及的一级学科标签，我们可以很容易地根据考试科目获得题目的一级学科标签，但很多题目不只属于单一学科，比如一道题可以既涉及历史学科，又涉及文学学科，而这样的信息无法从数据源直接获取。


\subsubsection{Expansion}
为了保证我们的数据集能够时刻领先于大模型所用到的训练语料，我们需要不断获取最新的领域数据。
不断获取最新的数据是个数据量非常大，且会不断进行更新，使用人工评估会存在巨大的经济开销和时间开销。

我们使用一些后处理，来筛选那些语言模型无法回答的问题。
我们利用之前的标注数据来训练小规模语言模型作为分类器，并为每个数据打上一级学科的标签。

这些数据的质量会低于人工标注的题目，但这类题目的更新速度将会很快，因此这部分数据集是评估前沿语言模型的重要指标。



\subsection{LLM输出的评估}
\label{033}
受instruction-tuning~\cite{chung2022scaling}这篇工作的启发，现在的LLMs几乎都是用自回归生成的方式来对输入模型的文本内容做出反馈。
而这种方式难以生成和ground truth一模一样的结果，因此如何有效地评估LLMs输出的难点在于如何确定模型的输出和ground truth具有相同的语义。

\subsubsection{针对能力较强的LLMs去缩小值域}
有许多工作使用的思路是将原来的问题构建成选择题的答题形式，将所有题目的ground truth一同构建成选项，让LLM去做选择题~\cite{}。
但我们认为这样会存在一些问题，而导致评估不公平，因此我们参考Zhu et al.~\cite{}和Zhang et al.~\cite{}的工作，设计了一些改进方法。

1.模型存在猜中答案的可能性是未知的，所以无法根据准确率判断模型的表现：我们提出通过固定每道题的选项数量来确定模型猜中的概率，同时我也可以通过增大选项的数量来降低模型猜中答案的概率，甚至可以使模型猜中答案的概率被忽略不计。
2.答案之间的字符差异性以及答案和题目之间的字符相关性也可能导致模型猜中某个答案：我们不使用所有可能的ground truth去构建题目的选项，而是通过学科的词库去获取与ground truth具有较高的字符相似性的内容作为选项。
3.现在的模型对于指令都非常敏感，模型可能会因为理解错误了指令而导致预测错误：这也会妨碍我们评估模型是否理解了某类领域知识，因此我们为每种题型设计了至少五种不同的instruction来诱导模型给出结果。

\subsubsection{模型输出和结果的链接}
尽管我们尝试缩小LLMs的值域，但是LLMs依然可能会输出一些我们意想不到的冗余内容。
我们认为大多数的冗余内容都是帮助模型表达语义的，所以我们提出使用一些后处理来拜托这些冗余内容的干扰。
我们借鉴了BLEU工作的思想，通过计算模型输出和选项文本的相匹配的词元数量来确定模型输出和各个选项的相似度，并取相似度最高的结果为模型选择的选项。



==> old_version/03BenchmarkDescription.1.tex <==
In this section, we will provide a detailed explanation of our work. Our goal is to evaluate domain knowledge, and we use China's subject classification system to construct our Benchmark. In Section \ref{031}, we will define the term "domain" and elaborate on the relationship between China's subject system and domain knowledge. We will then describe our dataset collection process, the manual filtering method, and how we ensure that our dataset always remains ahead of LLM training in Section \ref{032}. Lastly, in Section \ref{033}, we will discuss the evaluation methods we designed for LLM outputs.


\subsection{Domain Knowledge}
\label{031}

\subsubsection{Definition}
领域知识（Domain Knowledge）指的是关于特定学科、行业或业务领域的专业知识和理解。这类知识通常由专家或从业者掌握，并逐步在相关领域的研究和工作中积累和完善。领域知识的掌握程度直接影响到工作、研究的效率和质量。

\red{领域知识的定义还要继续搜集}
在自然语言处理（Natural Language Processing, NLP）领域，领域知识可以用来提高模型在特定领域的任务中的表现。例如，在金融领域的文本分类任务中，也许根据基本的NLP技术就能取得相对不错的结果，但如果在此基础上加入金融领域的专业知识（如金融术语、法规、行业动态等），则可以进一步提高模型的精确度和实用性。

\subsubsection{Chinese Subject Classification System}
The discipline classification system in China, developed by the Ministry of Education of China, classifies and codes various disciplines in higher education. The system divides disciplines into multiple levels, such as academic categories, first-level disciplines, and second-level disciplines. The meanings of these levels are explained below:

Academic categories: This is the highest level of discipline classification, roughly divided according to the nature, characteristics, and relationships of disciplines. There are fourteen academic categories, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, art, and interdisciplinary studies.

First-level disciplines: Based on academic categories, research fields with similarities and relationships are categorized as first-level disciplines. For example, under the economics category, there may be first-level disciplines such as "Political Economy," "Public Finance," and "Finance." There are a total of 112 different first-level disciplines, which are the basic units for branch classifications, with second-level disciplines established under them.

Second-level disciplines: Located under first-level disciplines, these represent more refined research areas within first-level disciplines. For example, within the "Finance" first-level discipline, further divisions may include financial markets, banking, insurance, and international finance as second-level disciplines. Second-level disciplines can be further refined into specific research directions or themes.

China's discipline classification system is a hierarchical structure where academic categories are at the top, representing a broader range and connotation of a discipline. First-level and second-level disciplines, in turn, represent more specific areas and more finely divided research areas within academic categories. In practice, this classification system aids in better managing, planning, and guiding teaching and scientific research in higher education. Simultaneously, it provides a clear and orderly framework for the development and research of disciplines for teachers, scholars, and students.

\subsection{数据集收集}
\label{032}

In this section, we primarily describe the process of collecting our dataset, the criteria for manual selection, and the automated dataset updating scheme. 
The volume and distribution of the data we collected at the time of the paper submission are shown in Figure~\ref{fig:benchstatistic}.

\subsubsection{Collection}
We primarily obtained data from two sources. The first source is the college entrance exam questions, from which we collected \red{100,000} questions related to China's graduate school entrance examinations. The second source is the mid-term and final exam questions of major universities collected from open-source websites, totaling \red{1,000,000} questions.
To facilitate automated evaluation, we only collected questions with clear ground truths. The primary question types include multiple-choice, fill-in-the-blank, true/false, and short-answer questions.
During the data collection process, we also utilized GPT-4 to translate all the Chinese questions into English.


\subsubsection{Annotation}
The quality of questions in entrance examinations is higher than those in websites, therefore, we focused on annotating and cleaning a significant amount of entrance exam questions.
We will also share these datasets separately as open-source resources.
We hired and paid graduate students with various majors to annotate and clean the data. 
We provided training for all potential annotators and tested their understanding of the training content to ensure that they fully grasped our requirements.
Finally, we selected eight graduate students from different academic categories as our annotators. 
Their wages are higher than the local minimum wage rates.

\begin{figure}[h]


\begin{center}

\includegraphics[width=0.6\textwidth]{BenchmarkStatistic.jpg}

\end{center}
\label{fig:benchstatistic}
\caption{A gull}


\end{figure}

The annotations mainly include the following markings for the questions:
1. Marking questions that cannot be answered with text information alone. These questions include those that require reading images, and listening questions that require audio information. We temporarily exclude questions that require non-text information from the benchmark.
2. Marking the first-level discipline labels involved in the questions. We can easily obtain the first-level discipline labels of the questions based on the examination subjects, but many questions do not belong solely to a single discipline. For example, a question may involve both history and literature disciplines, and such information cannot be obtained directly from the data source.


\subsubsection{Expansion}
为了保证我们的数据集能够时刻领先于大模型所用到的语料，不断使用爬取的数据是非常重要的方法。
但是爬取的数据量非常大，且会不断进行更新，使用人工评估会存在巨大的经济开销和时间开销。

我们使用一些后处理，来筛选那些语言模型无法回答的问题。
我们利用之前的标注数据来训练小规模语言模型作为分类器，并为每个数据打上一级学科的标签。

这些数据的质量会低于人工标注的题目，但这类题目的更新速度将会很快，因此这部分数据集是评估前沿语言模型的重要指标。


\subsection{LLM输出的评估}
\label{033}
对于Text-to-Text类型的模型输出的评估最大的问题在于，模型很难生成和ground truth一模一样的结果。
Text-to-Text模型评估的难点在于如何比较两个不同文本内容的语义。
因此，我们在本文中提出三个评测思路，分别是使用LLM去进行评估、设置prompt去进行评估、最后是使用加权的字符相似度进行评估。

\subsubsection{LLM Based Evaluation}
最直接的思路就是让LLM自己去判断LLM输出的内容和ground truth是否一致。
可以使用被评估的LLM，或者其他具有公认较强能力的LLM，如ChatGPT或GPT4，进行评估。

However,这两个方法具有一定的可行性，但也存在一些问题。
直接使用被评估的LLM去评估自己输出的内容是否与ground truth一致，受限于LLM对于领域知识的理解能力，如果LLM不理解一个领域，那他便无法看懂领域术语，很可能会给出一系列不正确的评估结果。
使用公认能力较强的LLM很大程度上能避免上述的问题，但即便是目前公认的能力最强的GPT-4，在构建的领域benchmark面前也无法得到很好的效果，所以这又会导致无法公正有效地给出评估结果。

\subsubsection{Prompt Based Evaluation}
另外一个思路是，通过设计prompt，来使模型输出能够和ground truth完全相同的内容。
我们提出将一道题所有可能的候选答案作为LLM的输入，让LLM从所有的候选答案中选择一个选项作为问题的结果。
同时，为了保证候选答案之间具有一定的混淆性，我们还通过同义词库选择了很多ground truth的同义词作为候选选项一同作为输入。

这样做的好处是如果模型能够理解某个领域知识，则一定会生成和ground truth一模一样的内容。
当候选选项足够多时，模型蒙对某道题目的概率也不会很高。

但缺点是会很大程度上加长输入的长度，很有可能会超过LLM最大的输出长度而被截断。
将所有的候选选项都作为输入时，这些选项本身也会为模型提供丰富的信息，从而可以使LLM获得一些题目之外的信息来帮助答题。




==> old_version/03BenchmarkDescription.2.tex <==
In this section, we will provide a comprehensive description of DomMa Benchmark. 
We begin by defining the term "domain" in the context of our study and elaborating the relation between Chinese subject system and domain knowledge in subsection~\ref{031}.
We will describe the process of data collection in subsection~\ref{032}.
Finally, we will discuss the evaluation methods we designed for assessing LLM outputs in subsection~\ref{033}.
% We focusing mainly on how do we construct the benchmark.

% focusing on the process of constructing our FS-Benchmark, which is used to evaluate LLMs' domain knowledge based on China's subject classification system. The section will be organized as follows:

% \subsection{Domain Definition}\label{031}

% We begin by defining the term "domain" in the context of our study and elaborating the relation between Chinese subject system and domain knowledge. 
% By anchoring our definition of domain knowledge within the context of this classification system, we will create a solid foundation for constructing the FS-Benchmark, ensuring that it offers comprehensive coverage of diverse and relevant subjects.

% \subsection{Data Collection and Continuous Update}\label{032}

% Next, we will describe the process of data collection, focusing on the sources from which we obtain questions for our dataset. 
% These sources include graduate entrance examinations, undergraduate midterm exams, and final exams from Chinese universities. We will also detail the manual filtering method we employ to ensure the quality and relevance of the selected questions. Additionally, we will discuss how we update our dataset periodically to maintain a competitive edge over LLM training and avoid evaluation dataset contamination.

% \subsection{Evaluation Methodology}\label{033}

% Finally, we will discuss the evaluation methods we designed for assessing LLM outputs. This will involve an explanation of the pipeline-style evaluation method, which features multiple-choice questions to maintain consistency between models' outputs and ground truth. We will also describe the weighted character similarity-based method we employ for calculating the similarity between model outputs and ground truth, as well as the similarity score used to judge the correctness of a model's answer.

% By providing a detailed account of our work, this section aims to offer a transparent and thorough explanation of the FS-Benchmark construction process. This will enable both a better understanding of our methodology and a more accurate evaluation of LLMs' domain knowledge.


\subsection{Domain Knowledge}
\label{031}

\subsubsection{Definition}
Domain knowledge refers to the in-depth understanding, expertise, and familiarity with a specific subject, industry, field, or area of special interest. 
This knowledge is often held by experts or practitioners and is gradually accumulated and refined through research and work in the relevant field.
The mastery of domain knowledge directly affects the efficiency and quality of work and research.

% 在我们的基准中，我们
% {Domain knowledge refers to the expertise and understanding of a specific subject, industry, or business area. 
% This knowledge is often held by experts or practitioners and is gradually accumulated and refined through research and work in the relevant field. 
% The mastery of domain knowledge directly affects the efficiency and quality of work and research.

% In the field of NLP, domain knowledge can be used to improve the performance of models in domain-specific tasks. 
% For example, in a financial text classification task, a satisfactory result might be attained using basic NLP techniques. However, by incorporating domain knowledge from the financial sector (such as financial terminology, regulations, industry trends, etc.), the model's accuracy and practicality can be further enhanced.

% Incorporating domain knowledge into NLP models often involves fine-tuning and adapting pre-trained models, enriching the training data with domain-specific examples, and applying feature engineering techniques that capture domain-specific characteristics. 
% By integrating domain knowledge into NLP systems, we can develop more accurate and effective solutions for specific industries and subjects, meeting the unique needs and challenges that arise within those domains.}

\subsubsection{Chinese Subject Classification System}
The subject classification system in China, developed by the Ministry of Education of China, organizes and codes various subjects in college education. 
The system divides all domains into multiple subjects categories, first-level subjects, and second-level subjects. 
The meanings of these levels are as follows:

\textbf{Subject categories}: This is the highest level of subject classification, roughly divided according to the nature, characteristics, and relationships of subjects. 
There are fourteen subject categories in Chinese subject classification, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, art, and interdisciplinary studies.

\textbf{First-level subjects}: Based on \textit{subject categories}, related research fields sharing similarities are categorized as first-level subjects. 
For example, under the economics category, there are first-level subjects such as "Political Economy", "Econometrics", "Finance" and so on. 
There are a total of 112 different first-level subjects, which are the basic units for classifications of domain knowldege, with second-level subjects established under them.

\textbf{Second-level subjects}: Located under first-level subjects, these represent more refined research areas within first-level subjects. 
For example, within the "Finance" first-level subject, further divisions may include ``financial markets'', ``banking'', ``insurance'', and ``international finance'' as second-level subjects. 
{Second-level subjects can be further refined into specific research directions or themes.}

Chinese subjects classification system is a hierarchical structure, where academic categories are at the top, representing a broader range and connotation of a subject. 
First-level and second-level subjects, in turn, represent more specific areas and more finely divided research areas within academic categories. 
In practice, this classification system aids in better managing, planning, and guiding teaching and scientific research in college education. 
Simultaneously, it provides a clear and orderly framework for the development and research of subjects for teachers, scholars, and students.

\subsection{Dataset Construction} \label{032}

In this section, we primarily outline the process of collecting our dataset, the criteria for manual selection, and the automated dataset updating scheme. 
The data volume and distribution at the time of the paper submission are shown in Figure~\ref{fig:benchstatistic}.

\subsubsection{Data Collection} We mainly obtained data from two sources. The first source is the graduate entrance exam questions.
The Chinese graduate entrance examination allows admission units to set their own tests on different first and second level subjects, from which we collected more than 0.1M questions. 
The second source is the mid-term and final exam questions of major universities collected from open-source websites, totaling 1M questions. 
To facilitate automated evaluation, we only collected questions with clear ground truths. 
The primary question types include multiple-choice, fill-in-the-blank, true/false questions. During the data collection process, we also utilized Baidu Translation System~\footnote{https://fanyi.baidu.com/} to translate all the Chinese questions into English.

\subsubsection{Manual Annotation} The quality of questions from entrance examinations is higher than those from websites; therefore, we focused on annotating and cleaning a substantial volume of entrance exam questions. 
We hired and paid graduate students from various majors to annotate and clean the data. 
We provided training for all potential annotators and tested their understanding of the training content to ensure they fully met our requirements. 
And we selected 20 graduate students from different subject categories as our annotators. 
All of them are paid above the local minimum wage.

The annotations include the following markings for the questions:

(1). Marking questions that cannot be answered with text information alone. 
These questions include those requiring image interpretation and listening questions requiring audio information. 
We exclude the questions requiring non-text information from the benchmark.
(2). Marking the first-level subject labels involved in the questions. 
We can easily obtain the first-level subject labels of the questions based on the examination information, but many questions do not belong solely to a single subject. 
For example, a question may involve both history and literature subjects, and such information cannot be obtained directly from the data source.

\subsubsection{Auto Updating} 
To ensure that our benchmark stays ahead of the corpus used by large models, continuously updating by using the latest questions is important.
However, continuously annotate all questions by manual works incurs significant economic and time costs, which is not an ideal way for benchmark updating in a extremly long time.

We employ manually annotated questions as seed data, supplemented with additional information, such as the source of the exam questions, to train an annotation model. 
This annotation model will then be used to continuously label new data, and the labeled new data will be updated to the benchmarks. 
To ensure that the annotation model maintains its proficiency in capturing the characteristics of recent questions, we periodically provide the model with a small quantity of manually annotated data. 
Simultaneously, we adopt the idea of curriculum learning, finetune the latest manually updated data in the latter epochs, to enable the model to focus on the features of the most recent questions.
Notably, the annotation process, in comparison to the evaluation process, utilizes a more significant amount of information, which may result in an enhanced performance of the annotation model.

% We utilize the manually annotated questions as seed data, supplemented with additional information such as the source of the exam questions, to train an annotation model. 
% This model will subsequently be employed to continuously label new data.
% To ensure that the annotation model remains adept at capturing the characteristics of recent questions, we periodically provide the model with a few manually data. 
% Concurrently, we incorporate the design from curriculum learning, establishing distinct fine-tuning sequences in relation to the questions' posting time, to enable the model to concentrate on the features of the most up-to-date queries.
% It is noteworthy that, in comparison to the evaluation process, the auto annotating procedure employs a more substantial amount of information which improve the performance of the annotation model and make it expected to surpass that of the evaluation model.

% We use labeled questions as seed data, and combine it with other information, like from which kind of exam we get this question, to train an annotation model. 
% This annotation model will continuously label new data. 
% Moreover, to ensure that the annotation model can capture the characteristics of the latest questions, provide a small amount of labeled data to the model at regular intervals is a good approach. At the same time, in order for the model to focus on the features of the latest questions, we draw on the idea of curriculum learning and set different finetune sequences based on the questions' posting time. 
% Compared to evaluation, the labeling process uses more information, so the annotation model's performance should be better than the evaluation model.

% 我们使用标注的题目作为种子数据，结合题目的其他信息来训练一个标注模型。
% 这个标注模型将会持续不断地为新数据打上标签。
% 而且为了保证这个标注模型能够捕捉到最新的题目的特点，我们认为每隔一段时间为模型提供少量的标注数据是一个比较好的方式。
% 同时为了模型能够专注与最新的题目的特点，我们借鉴了课程学习的思想，安装题目的提出时间，设置不同的finetune顺序。
% 相较于评估而言，打标签的过程我们用上了更多的信息，所以标注模型的表现应该是要比评估模型要好的。


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.5\textwidth]{benchmark_statistic.png}
\end{center}
\label{fig:benchstatistic}
\caption{The distribution diagram that depicts our annotated data.
The inner circle illustrates the subject categories, while the outer circle signifies the first-level subjects. 
This visual representation allows for a clear understanding of the hierarchical structure and distribution of the data within various domains.}


\end{figure}

\subsection{Ouputs Assessment}
\label{033}

Building upon the notion of instruction-tuning put forth by Chung et al.~\cite{chung2022scaling}, contemporary LLMs predominantly employ auto-regressive generation methodologies to yield responses to textual input. 
Notwithstanding, the intrinsic limitations of this approach render it challenging to generate outcomes that are entirely congruent with the options of the questions. 
Consequently, the effective assessment of LLMs' outputs is contingent upon the verification of semantic equivalence between the generated outputs and ground truth.

Assessment to the output of LLMs effectively poses a challenge. 
Many researchers have attempted to overcome this obstacle by asking LLMs to respond to multiple-choice questions~\cite{liang2022holistic, santurkar2023whose}. 
We inherits this methodology while incorporating novel designs.

In order to minimize the model's chances of happening to answer correctly, we suggests that the model should select the right answer from lots of options, from 100 options for example. 
To prevent the model from deducing the correct answer based on unique character features of the options, we use open-source synonym databases or morphological techniques to construct the options.
Accounting for the sensitivity of LLMs to prompts~\cite{jiang2020can}, each sample is queried by different instruction at least five times. 
Additionally, not all models may possess the ability to comprehend instructions, resulting model's outputs could still deviate from our desired. 
Thus we propose another three evaluation methods:

\textbf{White-box evaluation}: If the model's parameters are abailable, the chosen option can be determined by acquiring the probabilities generated by the model.

\textbf{Grey-box evaluation}: In cases where the model's parameters are unavailable, instructions can still be employed to guide the model to generate probabilities for specific options, thereby inferring model's selection.

\textbf{Black-box evaluation}: If a model's capability is restricted, rendering it unable to generate probabilities based on instructions, the model is asked to directly repeat the options. Subsequently, the preferred choice of the model is identified by assessing the semantic similarity between the produced content and each available option.


% 有效评估LLM的输出，之前有许多人通过让LLMs做选择题的方式来降低评估LLMs输出的难度。
% 这是一个有效的思路，我们继承了他们的思路，并在此之上做出了一些新的设计。
% 为了降低模型猜对答案的可能，我们提出让模型从将近一百个选项中选择正确的答案。
% 考虑到模型有可能会因为答案独特的字符特征而猜对答案，我们使用了开源的同义词库或者构词法来构建了我们的选项。
% 考虑到LLMs对prompt非常敏感，所以我们针对每个sample都进行至少五次提问。
% 也考虑到并不是所有模型都具有理解instruction的能力，尽管我们有之前的那么多新设计，模型的输出可能还是和我们设想的略有差别，因此我们提出了三种评估方法。

% 白盒评估：如果我们能拿到模型的参数，可以通过获取模型生成每个选项的概率来判断模型选择了哪个选项
% 灰盒评估：如果我们不能拿到模型的参数，我们依然可以通过instruction去诱导出模型生成某个选项的概率，来判断模型会选择哪个选项。
% 黑盒评估：如果模型能力比较差，无法根据instruction生成概率，那便让模型直接重复选项，然后根据生成的内容与每个选项的语义相似度来判断模型会选择哪个选项

% \subsubsection{Narrowing Output Range for Advanced LLMs}

% A myriad of studies have formulated problems as multiple-choice questions, wherein the ground truths are incorporated as alternatives for LLMs~\cite{}. This strategy, however, could potentially facilitate evaluation biases. Thus, modifications inspired by the works of Zhu et al.~\cite{} and Zhang et al.~\cite{} have been devised to address such limitations.

% It is rather arduous to ascertain LLM performance based on accuracy due to the indeterminate nature of the model's capacity to deduce the correct response. As a remedy, we introduce the principle of fixing the quantity of alternatives for each query in order to ascertain the model's probability of accurate guessing. Furthermore, by augmenting the range of alternatives, the probability of successful guessing can be diminished or even rendered inconsequential.

% Character variations between responses, as well as the interrelation between queries and responses, may inadvertently contribute to the model's accurate guessing. As such, instead of constructing questions using all feasible ground truths as options, we derive alternatives with high character similarity to the ground truth from subject-specific lexicons.

% Owing to the heightened sensitivity of LLMs to instructions~\cite{jiang2020can}, erroneous interpretations may impede accurate prediction capabilities and the evaluation of domain-specific knowledge comprehension. To counter this effect, a minimum of five distinct instructions is designed for each question type, thereby inducing LLMs to produce results.

% \subsubsection{Correlation between Model Outputs and Ground Truth}

% Despite endeavors to attenuate the output range of LLMs, the possibility of generating unanticipated and superfluous content remains. Presumably, the majority of this extraneous material serves to facilitate the conveyance of semantic meaning. As a countermeasure, we propose the utilization of post-processing techniques to mitigate the repercussions of such redundancy. Drawing upon insights from the BLEU metric, the semblance between model-generated output and option text is ascertained by quantifying matched lexemes, with the alternative demonstrating the highest similarity being deemed the model's selection.


==> old_version/03BenchmarkDescription.3.tex <==
In this section, we will provide a detailed description of DomMa Benchmark. 
We begin by defining the term "domain" in our study and elaborating the relation between Chinese subject system and domain knowledge in subsection~\ref{031}.
The process of data collection, annotation and auto updating are given in subsection~\ref{032}.
Finally, we will discuss the evaluation methods we designed for assessing open-source and non-open-source generative LMs' outputs in subsection~\ref{033}.


\subsection{Domain Knowledge}
\label{031}

\subsubsection{Definition}
\red{
Domain knowledge refers to the in-depth understanding, expertise, and familiarity with a specific subject, industry, field, or area of special interest. 
This knowledge is often held by experts or practitioners and is gradually accumulated and refined through research and work in the relevant field.
The mastery of domain knowledge directly affects the efficiency and quality of work and research.
}

\subsubsection{Chinese Discipline Classification System}
The discipline classification system in China, developed by the Ministry of Education of China, organizes and codes various subjects in college education. 
The system divides all domains into multiple subjects categories, first-level subjects, and second-level subjects. 
The meanings of these levels are as follows:

\textbf{Discipline Categories}: This is the highest level of discipline classification, divided according to the nature, characteristics of subjects. 
There are fourteen subject categories in Chinese discipline classification, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, art, and interdisciplinary studies.

\textbf{First-level disciplines}: Related research fields sharing similarities are categorized as first-level disciplines. 
For example, under the economics category, there are first-level disciplines such as "Political Economy", "Econometrics", "Finance" and so on. 
% There are a total of 112 different first-level disciplines, we take these disciplines as the basic classifications of domain knowldege, with second-level subjects established under them.

\textbf{Second-level disciplines}: These disciplines represent more subdivided areas of study or topics within the primary discipline.
For example, within the first level of 'finance', further divisions may include 'financial markets', 'banking', 'insurance "and "international finance" as secondary disciplines.

As shown in Fig.~\ref{fig:benchstatistic}, Chinese Discipline Classification is a hierarchical structure, where academic categories are at the top, representing a broader range and connotation of a subject. 
First-level, second-level and even third-level disciplines represent more specific areas and more finely divided research areas within academic categories.
There are a total of 112 first-level disciplines, we take these disciplines as the basic classifications of domain knowledge.
And there are about 300+ second-level and 1000+ third-level disciplines, we take 217 of second-level to further annotate the questions in our benchmark.
We give a more detailed table of Chinese Discipline Classification, which include all of three level disciplines with discipline categories, in appendix.

\subsection{Dataset Construction} \label{032}


\subsubsection{Data Collection} 
The questions in dataset were manually collected from two freely available sources online.
One is from the Chinese graduate entrance exam questions.
Chinese universities are allowed to set their own questions for the enrollment of their first and second level disciplines, so an extremely large amount of questions are generated each year.
The quality of the questions from this source is high as they are reviewed by the Chinese Education Department.
To further improve the quality through manual annotation, we have collected around 400,000 questions from this source.
Another source is the questions from mid-term and final exams in each universities.
The quality of the questions from this source varies a lot, since teachers in each school have a different attitude towards the exam.
However, the questions from this source is updated more frequently than previous one, and also much more questions are generated in this source.
So as long as we do a good job in automaticly filtering and annotating, the data from this source will be available to continuously update to DomMa.
We have finally collected 100,000 questions from this source through automatic filtering and annotation.


\subsubsection{Manual Annotation}
We build our first version of DomMa Benchmark by manually annotating questions from the Graduate Entrance Examination.
The aim of annotation is to remove unanswerable questions and to tag each question with as many first and second level disciplines as possible.

We first used ChatGPT to tag each question with first or second level disciplines. 
In the process of tagging, we build prompt by concatenate the content of a question with its options, answers and exam information with the description of each disciplines to increase chatGPT's understanding to the question so that the question could be better tagged.
We again used chatGPT's perplexity to differentiate the quality of the questions.
The detailed template of the prompt and how we use the perplexity is listed in appendix.
We find that the questions annotated by chatGPT can be used to test chatGPT or even more powerful LMs, because chatGPT use a lot of additional information in the annotation process.
As for DomMa, we have subsequent manual annotation to further ensure the quality of the questions.

The manually annotations include the following requirement for each questions:
(1). Mark questions that cannot be answered with text information alone. 
These questions include those requiring image interpretation or audio information. 
We exclude the questions that requires non-text information from the benchmark.
The annotators are extra paid if they find any unanswerable questions.
(2). Check the output of ChatGPT or remark the first-level and second-level discipline labels involved in the questions.
The annotators are also extra paid if they find the error made by chatGPT or tagged more labels than chatGPT to the questions.

We hired and paid graduate students from various majors to annotate and clean the questions we collected. 
We provided training for all potential annotators and tested their understanding of the training content to ensure they fully met our requirements. 
20 graduate students are selected from different subject categories as our annotators. 
All of them are paid above the local minimum wage.
And to ensure the quality of the annotations, each sample is annotated by at least three annotators.



\subsubsection{Auto Updating} 
To ensure that DomMa is fresher than the LM training set, we need to be able to automate updates to DomMa
To ensure that our benchmark stays ahead of the corpus used by large models, continuously updating by using the latest questions is important.
However, continuously annotate all questions by manual works incurs significant economic and time costs, which is not an ideal way for benchmark updating in a extremly long time.

We employ manually annotated questions as seed data, supplemented with additional information, such as the source of the exam questions, to train an annotation model. 
This annotation model will then be used to continuously label new data, and the labeled new data will be updated to the benchmarks. 
To ensure that the annotation model maintains its proficiency in capturing the characteristics of recent questions, we periodically provide the model with a small quantity of manually annotated data. 
Simultaneously, we adopt the idea of curriculum learning, finetune the latest manually updated data in the latter epochs, to enable the model to focus on the features of the most recent questions.
Notably, the annotation process, in comparison to the evaluation process, utilizes a more significant amount of information, which may result in an enhanced performance of the annotation model.

% We utilize the manually annotated questions as seed data, supplemented with additional information such as the source of the exam questions, to train an annotation model. 
% This model will subsequently be employed to continuously label new data.
% To ensure that the annotation model remains adept at capturing the characteristics of recent questions, we periodically provide the model with a few manually data. 
% Concurrently, we incorporate the design from curriculum learning, establishing distinct fine-tuning sequences in relation to the questions' posting time, to enable the model to concentrate on the features of the most up-to-date queries.
% It is noteworthy that, in comparison to the evaluation process, the auto annotating procedure employs a more substantial amount of information which improve the performance of the annotation model and make it expected to surpass that of the evaluation model.

% We use labeled questions as seed data, and combine it with other information, like from which kind of exam we get this question, to train an annotation model. 
% This annotation model will continuously label new data. 
% Moreover, to ensure that the annotation model can capture the characteristics of the latest questions, provide a small amount of labeled data to the model at regular intervals is a good approach. At the same time, in order for the model to focus on the features of the latest questions, we draw on the idea of curriculum learning and set different finetune sequences based on the questions' posting time. 
% Compared to evaluation, the labeling process uses more information, so the annotation model's performance should be better than the evaluation model.

% 我们使用标注的题目作为种子数据，结合题目的其他信息来训练一个标注模型。
% 这个标注模型将会持续不断地为新数据打上标签。
% 而且为了保证这个标注模型能够捕捉到最新的题目的特点，我们认为每隔一段时间为模型提供少量的标注数据是一个比较好的方式。
% 同时为了模型能够专注与最新的题目的特点，我们借鉴了课程学习的思想，安装题目的提出时间，设置不同的finetune顺序。
% 相较于评估而言，打标签的过程我们用上了更多的信息，所以标注模型的表现应该是要比评估模型要好的。


% 我们设计了一种自动更新的方法来不断地为DomMa加入最新的数据。
% 自动标注和人工标注不同，除了识别不可回答的题目，以及为每道题目打上尽量多的一二级学科标签之外，因为题目的来源于未经过审查，我们还需要考虑题目本身是否会有错误。

% 针对于不可回答的题目，我们提取了人工标注结果中的关键词，如“如下图所示”、“如表中所示”等，并用这些关键词来题目删除出我们的benchmark。
% 针对于打标签这个目的，我们发现chatGPT具有良好的标注能力，并且价格合适，预期每标注10000道题目大概只需要花费50\$不到。
% 所以跟上个subsection一样，我们将一道题目的详细信息和类别的描述信息输入给chatGPT，让chatGPT帮助我们进行题目标注。
% 同时我们还利用了人工标注过的题目训练了一个GPT-Classifier。
% 这个GPT-Classifier可以根据类别的描述，以及文本的内容，确定文本和该类别的相关程度。
% 我们使用我们训练的GPT-Classifier和chatGPT进行联合标注。
% 我们将其中一方的标注结果构建prompt去询问另一个标注器。
% 最后根据我们的实验结果，我们选择将两个标注器的结果取并集作为一道题目最终的标签。
% 而针对于题目本身的质量，我们选择那些带有答案解析的题目，我们认为构建者对于这样的题目花费了更多的精力，所以题目的质量应该会更好。

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.5\textwidth]{benchmark_statistic.png}
\end{center}
\caption{The distribution diagram that depicts our annotated data.
The inner circle illustrates the subject categories, while the outer circle signifies the first-level subjects. 
This visual representation allows for a clear understanding of the hierarchical structure and distribution of the data within various domains.}
\label{fig:benchstatistic}
\end{figure}

\subsection{Ouputs Assessment}
\label{033}

Building upon the notion of instruction-tuning put forth by Chung et al.~\cite{chung2022scaling}, contemporary LLMs predominantly employ auto-regressive generation methodologies to yield responses to textual input. 
Notwithstanding, the intrinsic limitations of this approach render it challenging to generate outcomes that are entirely congruent with the options of the questions. 
Consequently, the effective assessment of LLMs' outputs is contingent upon the verification of semantic equivalence between the generated outputs and ground truth.

Assessment to the output of LLMs effectively poses a challenge. 
Many researchers have attempted to overcome this obstacle by asking LLMs to respond to multiple-choice questions~\cite{liang2022holistic, santurkar2023whose}. 
We inherits this methodology while incorporating novel designs.

In order to minimize the model's chances of happening to answer correctly, we suggests that the model should select the right answer from lots of options, from 100 options for example. 
To prevent the model from deducing the correct answer based on unique character features of the options, we use open-source synonym databases or morphological techniques to construct the options.
Accounting for the sensitivity of LLMs to prompts~\cite{jiang2020can}, each sample is queried by different instruction at least five times. 
Additionally, not all models may possess the ability to comprehend instructions, resulting model's outputs could still deviate from our desired. 
Thus we propose another three evaluation methods:

\textbf{White-box evaluation}: If the model's parameters are abailable, the chosen option can be determined by acquiring the probabilities generated by the model.

\textbf{Grey-box evaluation}: In cases where the model's parameters are unavailable, instructions can still be employed to guide the model to generate probabilities for specific options, thereby inferring model's selection.

\textbf{Black-box evaluation}: If a model's capability is restricted, rendering it unable to generate probabilities based on instructions, the model is asked to directly repeat the options. Subsequently, the preferred choice of the model is identified by assessing the semantic similarity between the produced content and each available option.


% 有效评估LLM的输出，之前有许多人通过让LLMs做选择题的方式来降低评估LLMs输出的难度。
% 这是一个有效的思路，我们继承了他们的思路，并在此之上做出了一些新的设计。
% 为了降低模型猜对答案的可能，我们提出让模型从将近一百个选项中选择正确的答案。
% 考虑到模型有可能会因为答案独特的字符特征而猜对答案，我们使用了开源的同义词库或者构词法来构建了我们的选项。
% 考虑到LLMs对prompt非常敏感，所以我们针对每个sample都进行至少五次提问。
% 也考虑到并不是所有模型都具有理解instruction的能力，尽管我们有之前的那么多新设计，模型的输出可能还是和我们设想的略有差别，因此我们提出了三种评估方法。

% 白盒评估：如果我们能拿到模型的参数，可以通过获取模型生成每个选项的概率来判断模型选择了哪个选项
% 灰盒评估：如果我们不能拿到模型的参数，我们依然可以通过instruction去诱导出模型生成某个选项的概率，来判断模型会选择哪个选项。
% 黑盒评估：如果模型能力比较差，无法根据instruction生成概率，那便让模型直接重复选项，然后根据生成的内容与每个选项的语义相似度来判断模型会选择哪个选项

% \subsubsection{Narrowing Output Range for Advanced LLMs}

% A myriad of studies have formulated problems as multiple-choice questions, wherein the ground truths are incorporated as alternatives for LLMs~\cite{}. This strategy, however, could potentially facilitate evaluation biases. Thus, modifications inspired by the works of Zhu et al.~\cite{} and Zhang et al.~\cite{} have been devised to address such limitations.

% It is rather arduous to ascertain LLM performance based on accuracy due to the indeterminate nature of the model's capacity to deduce the correct response. As a remedy, we introduce the principle of fixing the quantity of alternatives for each query in order to ascertain the model's probability of accurate guessing. Furthermore, by augmenting the range of alternatives, the probability of successful guessing can be diminished or even rendered inconsequential.

% Character variations between responses, as well as the interrelation between queries and responses, may inadvertently contribute to the model's accurate guessing. As such, instead of constructing questions using all feasible ground truths as options, we derive alternatives with high character similarity to the ground truth from subject-specific lexicons.

% Owing to the heightened sensitivity of LLMs to instructions~\cite{jiang2020can}, erroneous interpretations may impede accurate prediction capabilities and the evaluation of domain-specific knowledge comprehension. To counter this effect, a minimum of five distinct instructions is designed for each question type, thereby inducing LLMs to produce results.

% \subsubsection{Correlation between Model Outputs and Ground Truth}

% Despite endeavors to attenuate the output range of LLMs, the possibility of generating unanticipated and superfluous content remains. Presumably, the majority of this extraneous material serves to facilitate the conveyance of semantic meaning. As a countermeasure, we propose the utilization of post-processing techniques to mitigate the repercussions of such redundancy. Drawing upon insights from the BLEU metric, the semblance between model-generated output and option text is ascertained by quantifying matched lexemes, with the alternative demonstrating the highest similarity being deemed the model's selection.


==> old_version/03BenchmarkDescription.4.tex <==
% In this section, we will provide a detailed description of DomMa Benchmark. 
% We begin by defining the term "domain" in our study and elaborating the relation between Chinese subject system and domain knowledge in subsection~\ref{031}.
% The process of data collection, annotation and auto updating are given in subsection~\ref{032}.
% Finally, we will discuss the evaluation methods we designed for assessing open-source and non-open-source generative LMs' outputs in subsection~\ref{033}.


\subsection{Chinese Discipline Classification System}
\label{031}

% \subsubsection{Definition}
% \red{
% 还没开始写。

% Domain knowledge refers to the in-depth understanding, expertise, and familiarity with a specific subject, industry, field, or area of special interest. 
% This knowledge is often held by experts or practitioners and is gradually accumulated and refined through research and work in the relevant field.
% The mastery of domain knowledge directly affects the efficiency and quality of work and research.
% }

% \subsubsection{Chinese Discipline Classification System}
The discipline classification system in China, developed by the Ministry of Education of China, organizes subjects of different domain education in college education. 
The system divides all domains into 14 subjects categories, and various levels of subjects. 
The meanings of these levels are as follows:

\textbf{Discipline Categories}: This is the highest level of discipline classification, divided according to the nature, characteristics of subjects. 
There are 14 subject categories in Chinese discipline classification, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management, art, and interdisciplinary studies.

\textbf{First-level disciplines}: Related research fields sharing similarities are categorized as first-level disciplines. 
For example, under the economics category, there are first-level disciplines such as "Political Economy", "Econometrics", "Finance" and so on. 
% There are a total of 112 different first-level disciplines, we take these disciplines as the basic classifications of domain knowldege, with second-level subjects established under them.

\textbf{Second-level disciplines}: These disciplines represent more subdivided areas of study or topics within the primary discipline.
For example, within the first level of 'finance', further divisions may include 'financial markets', 'banking', 'insurance "and "international finance" as secondary disciplines.

As shown in Fig.~\ref{fig:benchstatistic}, Chinese Discipline Classification is a hierarchical structure, where academic categories are at the top, representing a broader range and connotation of a subject. 
First-level, second-level and even third-level disciplines represent more specific areas and more finely divided research areas within academic categories.
There are a total of 112 first-level disciplines, we take all of these disciplines as the basic classifications of domain knowledge.
And there are about 400+ second-level and 1000+ third-level disciplines, we take 393 of second-level to further annotate the questions in our benchmark.
We give a more detailed table of Chinese Discipline Classification, which include all of three level disciplines with discipline categories, in appendix.

\subsection{Dataset Construction} \label{032}


\subsubsection{Data Collection} 
The questions in dataset were manually collected from two freely available sources online.
One is from the Chinese graduate entrance exam questions.
Chinese universities are allowed to set their own questions for the enrollment of their first and second level disciplines, so an extremely large amount of questions are generated each year.
The quality of the questions from this source is high as they are reviewed by the Chinese Education Department.
To further improve the quality through manual annotation, we have collected around 400k questions from this source.
Another source is the questions from mid-term and final exams in each universities.
The quality of the questions from this source varies a lot, while the update frequency of the questions from this source is much higher than the previous one.
So as long as we do a good job in automaticly filtering and annotating, the data from this source will be available to continuously update to DomMa.
We have finally collected 100k questions from this source through automatic filtering and annotation.


\subsubsection{Manual Annotation}
We manually annotated the questions collected from the Graduate Entrance Examination to form the meta version of DomMa.
The aim of annotation is to remove unanswerable questions and to tag each question with as many first and second level disciplines as possible.

We first used ChatGPT to tag each question with first or second level disciplines. 
In the process of tagging, we build prompt by concatenate the content of a question with its options, answers and exam information with the description of each disciplines to increase chatGPT's understanding to the question so that the question could be better tagged.
We again used chatGPT's perplexity to differentiate the quality of the questions.
The detailed template of the prompt and how we use the perplexity is listed in appendix~\ref{}.
\blue{We find that the questions annotated by chatGPT can be used to test chatGPT or even more powerful LLMs, since chatGPT use a lot of additional information in the annotation process and use only the question description in the inference process.}
As for DomMa, we have subsequent manual annotation to further ensure the quality of the questions.

The manually annotations include the following requirement for each questions:
(1). Mark questions that cannot be answered with text information alone. 
These questions include those requiring image interpretation or audio information. 
We exclude the questions that requires non-text information from the benchmark.
The annotators are extra paid if they find any unanswerable questions.
(2). Check the output of ChatGPT or remark the first-level and second-level discipline labels involved in the questions.
The annotators are also extra paid if they find the error made by chatGPT or tagged more labels than chatGPT to the questions.

We hired and paid graduate students from various majors to annotate and clean the questions we collected. 
We provided training for all potential annotators and tested their understanding of the training content to ensure they fully met our requirements. 
20 graduate students are selected from different subject categories as our annotators. 
All of them are paid above the local minimum wage.
And to ensure the quality of the annotations, each sample is annotated by at least three annotators.



\subsubsection{Auto Updating} 
Except for the meta version build by manually works, we plan to automatically update the future version of DomMa.
Automatic update has the same requirement as manual annotation, that is, to exclude unanswerable questions and tag the disciplines labels involved in each question.

For unanswerable questions, we first only selected questions with answer explanations, as we believe that creators exert more effort on these questions, may result in higher quality.
Then we extracted keywords from the manual annotation results, such as "as shown in the figure below" or "as listed in the table" and so on, and used these keywords to remove questions from our benchmark. 

And to achieve the purpose of first and second disciplines labeling, we, similar to the previous subsection, input the detailed information of a question and disciplines with their descriptions to ChatGPT to help us with question annotation.
In addition, we trained a GPT-Classifier using human-annotated questions. 
This GPT-Classifier can determine the relevance between text content and a specific category based on the category description. 
Finally, we use trained GPT-Classifier and ChatGPT to do joint annotation.






\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics[0.4\textwidth]{DomMa.png}
\includegraphics[0.3\textwidth]{DomMaMedium.png}
\includegraphics[0.3\textwidth]{DomMaHard.png}
}
\end{center}
\caption{
\red{数据标完之后，图还要继续变动}
The figure on the right is the statistics of all questions collected by DomMa.
The middle figure shows statistics for DomMa-Medium and the left shows DomMa-Hard.}
\label{fig:benchstatistic}
\end{figure}

\subsection{Ouputs Assessment}
\label{033}
生成式模型评估的难点主要在于：
如何有效地从模型的输出中抽取模型选择的选项。
一种思路是，做few-shot或zero-shot评估时，利用指令去控制模型的输出，使模型做出的选择容易被抽取。
但模型对于指令非常敏感，我们难以用统一的指令控制所有模型的输出。
而且不是所有模型都适合做选择题，这会给做选择题能力较差的模型带来不公平的评估。

对于开源模型，我们提出通过获取模型生成每个选项的概率，来判断模型选择的选项。
至于非开源模型，我们发现这些模型的能力都极强，所以我们要求模型输出他们选择每个选项的概率，并以此作为判断。

% Evaluating the outputs of current language models have two main challenges:
% (1) Most models are generative models.
% Controlling the content of the output becomes difficult.
% Although some models have a good ability in following instructions, so the output of these models can be effectively restricted by instructions.
% But we expect to enable models of all abilities to be evaluated by DomMa.
% (2) Many models are not open-source and can only be accessed through APIs.
% Therefore, we propose the following three evaluation approaches:

% If the model's parameters are available, the chosen option can be determined by acquiring the probabilities generated by the model. 
% This method can effectively avoid differences in the final results due to variations in the models' ability to understand instructions.

% If the model's parameters are not open-source, which are some powerful and really large-scale language models, we still expect to obtain the probabilities to each option but not directly ask the model to give textual response. 
% Some APIs support to response user with the perplexity or confidence to the input, or we can instruct models to reveal the probabilities or confidence for each option since the non-open-source models are mostly powerful enough.

% \textbf{Black-box evaluation}: If the model's parameters are not open-source, the API does not support providing perplexity, and the model do not have the ability to reveal probabilities or confidence levels, we have no choice but to ask the model to reply with its selected option directly. 
% In this case, we request the models not to provide any additional content and only repeat the option it believes is correct. 
% We then calculate the character similarity between the model's response and each option to determine the model's choice or ascertain if the model is simply producing nonsense.


% 评估现在语言模型的输出存在以下两个难点：
% 一个是现在的模型大多都是生成模型，如果指令微调的效果不好，则难以控制其输出的内容。
% 二个时现在的模型有很多是不开源的，只能通过API的形式去访问。
% 所以我们提出了以下的三种评估思路：

% \textbf{White-box evaluation}: If the model's parameters are abailable, the chosen option can be determined by acquiring the probabilities generated by the model.
% 获取生成概率的方式可以有效避免因为模型对于指令理解能力差异而导致的最终结果的差异。

% \textbf{Grey-box evaluation}: 
% 如果模型的参数是不开源的，我们依然期望获得模型选择每个选项的概率。
% 有些API是可以计算一句话的困惑度或者置信度，而有些模型可以通过指令诱导出他选择每个选项的概率，或者是置信度。


% \textbf{Black-box evaluation}: 
% 如果模型参数不开源，API不支持回复困惑度，模型也没有回复概率和置信度的能力。
% 我们只能要求模型直接回复给我们的它的选项。
% 其中，我们会要求模型不要回复多余内容，只重复它认为是正确的选项。
% 我们会计算模型的回复和每个选项的字符相似度，来确定模型选择的内容，亦或是模型根本是在胡说。


% If a model's capability is restricted, rendering it unable to generate probabilities based on instructions, the model is asked to directly repeat the options. Subsequently, the preferred choice of the model is identified by assessing the semantic similarity between the produced content and each available option.


% Building upon the notion of instruction-tuning put forth by Chung et al.~\cite{chung2022scaling}, contemporary LLMs predominantly employ auto-regressive generation methodologies to yield responses to textual input. 
% Notwithstanding, the intrinsic limitations of this approach render it challenging to generate outcomes that are entirely congruent with the options of the questions. 
% Consequently, the effective assessment of LLMs' outputs is contingent upon the verification of semantic equivalence between the generated outputs and ground truth.

% Assessment to the output of LLMs effectively poses a challenge. 
% Many researchers have attempted to overcome this obstacle by asking LLMs to respond to multiple-choice questions~\cite{liang2022holistic, santurkar2023whose}. 
% We inherits this methodology while incorporating novel designs.

% In order to minimize the model's chances of happening to answer correctly, we suggests that the model should select the right answer from lots of options, from 100 options for example. 
% To prevent the model from deducing the correct answer based on unique character features of the options, we use open-source synonym databases or morphological techniques to construct the options.
% Accounting for the sensitivity of LLMs to prompts~\cite{jiang2020can}, each sample is queried by different instruction at least five times. 
% Additionally, not all models may possess the ability to comprehend instructions, resulting model's outputs could still deviate from our desired. 
% Thus we propose another three evaluation methods:

% \textbf{White-box evaluation}: If the model's parameters are abailable, the chosen option can be determined by acquiring the probabilities generated by the model.

% \textbf{Grey-box evaluation}: In cases where the model's parameters are unavailable, instructions can still be employed to guide the model to generate probabilities for specific options, thereby inferring model's selection.

% \textbf{Black-box evaluation}: If a model's capability is restricted, rendering it unable to generate probabilities based on instructions, the model is asked to directly repeat the options. Subsequently, the preferred choice of the model is identified by assessing the semantic similarity between the produced content and each available option.



==> old_version/03BenchmarkDescription.5.tex <==
% In this section, we will provide a detailed description of Xiezhi Benchmark. 
% We begin by defining the term "domain" in our study and elaborating the relation between Chinese subject system and domain knowledge in subsection~\ref{031}.
% The process of data collection, annotation and auto updating are given in subsection~\ref{032}.
% Finally, we will discuss the evaluation methods we designed for assessing open-source and non-open-source generative LMs' outputs in subsection~\ref{033}.


\subsection{Chinese Discipline Classification System}
\label{031}

% \subsubsection{Definition}
% \red{
% 还没开始写。

% Domain knowledge refers to the in-depth understanding, expertise, and familiarity with a specific subject, industry, field, or area of special interest. 
% This knowledge is often held by experts or practitioners and is gradually accumulated and refined through research and work in the relevant field.
% The mastery of domain knowledge directly affects the efficiency and quality of work and research.
% }

% \subsubsection{Chinese Discipline Classification System}
The discipline classification system in China, developed by the Ministry of Education of China, organizes subjects of different domain education in college education. 
The system divides all domains into 14 subjects categories, and various levels of subjects. 
The meanings of these levels are as follows:

\textbf{Discipline Categories}: This is the highest level of discipline classification, divided according to the nature, characteristics of subjects. 
There are 13 subject categories in Chinese discipline classification, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management and art.

\textbf{First-level disciplines}: Related research fields sharing similarities are categorized as first-level disciplines. 
For example, under the economics category, there are first-level disciplines such as "Political Economy", "Econometrics", "Finance" and so on. 

\textbf{Second-level disciplines}: These disciplines represent more subdivided areas of study or topics within the primary discipline.
For example, within the first level of 'finance', further divisions may include 'financial markets', 'banking', 'insurance "and "international finance" as secondary disciplines.

As shown in Fig.~\ref{fig:subjectclassification}, Chinese Discipline Classification is a hierarchical structure, where academic categories are at the top, representing a broader range and connotation of a subject. 
First-level, second-level and even third-level disciplines represent more specific areas and more finely divided research areas within academic categories.
There are a total of 118 first-level disciplines, we take all of these disciplines as the basic classifications of domain knowledge.
And there are about 400+ second-level and 1000+ third-level disciplines, we take 393 of second-level to further annotate the questions in our benchmark.

\subsection{Dataset Construction} \label{032}


\subsubsection{Data Collection} 
獬豸包含了主要两种题目，一种是现实世界中有真实来源的题目，另一种是根据已有新闻或学术报告生成的题目。
针对第一种题目，獬豸主要收集了六种不同来源的题目：小学题、中考题、高考题、本科题、研究生入学考试题、成人教育题。
其中，我们主要针对研究生入学考试题进行了人工标注，并使用了标注结果中的50,000道题目作为元数据集训练了自动标注器来标注其他的题目。
我们使用了自动标注器标注了第一种来源的剩余题目，并选出了100,000道题进行开源。
同时，我们也使用了自动标注器标注了第二个来源的题目，并选出了50,000道题进行开源。




The questions in dataset were manually collected from two freely available sources online.
One is from the Chinese graduate entrance exam questions.
Chinese universities are allowed to set their own questions for the enrollment of their first and second level disciplines, so an extremely large amount of questions are generated each year.
The quality of the questions from this source is high as they are reviewed by the Chinese Education Department.
To further improve the quality through manual annotation, we have collected around 400k questions from this source.
Another source is the questions from mid-term and final exams in each universities.
The quality of the questions from this source varies a lot, while the update frequency of the questions from this source is much higher than the previous one.
So as long as we do a good job in automaticly filtering and annotating, the data from this source will be available to continuously update to Xiezhi.
We have finally collected 100k questions from this source through automatic filtering and annotation.


\subsubsection{Manual Annotation}
We manually annotated the questions collected from the Graduate Entrance Examination to form the meta version of Xiezhi.
The aim of annotation is to remove unanswerable questions and to tag each question with as many first and second level disciplines as possible.

We first used ChatGPT to tag each question with first or second level disciplines. 
In the process of tagging, we build prompt by concatenate the content of a question with its options, answers and exam information with the description of each disciplines to increase chatGPT's understanding to the question so that the question could be better tagged.
We again used chatGPT's perplexity to differentiate the quality of the questions.
The detailed template of the prompt and how we use the perplexity is listed in appendix~\ref{}.
\blue{We find that the questions annotated by chatGPT can be used to test chatGPT or even more powerful LLMs, since chatGPT use a lot of additional information in the annotation process and use only the question description in the inference process.}
As for Xiezhi, we have subsequent manual annotation to further ensure the quality of the questions.

The manually annotations include the following requirement for each questions:
(1). Mark questions that cannot be answered with text information alone. 
These questions include those requiring image interpretation or audio information. 
We exclude the questions that requires non-text information from the benchmark.
The annotators are extra paid if they find any unanswerable questions.
(2). Check the output of ChatGPT or remark the first-level and second-level discipline labels involved in the questions.
The annotators are also extra paid if they find the error made by chatGPT or tagged more labels than chatGPT to the questions.

We hired and paid graduate students from various majors to annotate and clean the questions we collected. 
We provided training for all potential annotators and tested their understanding of the training content to ensure they fully met our requirements. 
20 graduate students are selected from different subject categories as our annotators. 
All of them are paid above the local minimum wage.
And to ensure the quality of the annotations, each sample is annotated by at least three annotators.



\subsubsection{Auto Updating} 
Except for the meta version build by manually works, we plan to automatically update the future version of Xiezhi.
Automatic update has the same requirement as manual annotation, that is, to exclude unanswerable questions and tag the disciplines labels involved in each question.

For unanswerable questions, we first only selected questions with answer explanations, as we believe that creators exert more effort on these questions, may result in higher quality.
Then we extracted keywords from the manual annotation results, such as "as shown in the figure below" or "as listed in the table" and so on, and used these keywords to remove questions from our benchmark. 

And to achieve the purpose of first and second disciplines labeling, we, similar to the previous subsection, input the detailed information of a question and disciplines with their descriptions to ChatGPT to help us with question annotation.
In addition, we trained a GPT-Classifier using human-annotated questions. 
This GPT-Classifier can determine the relevance between text content and a specific category based on the category description. 
Finally, we use trained GPT-Classifier and ChatGPT to do joint annotation.






\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics[0.4\textwidth]{DomMa.png}
\includegraphics[0.3\textwidth]{DomMaMedium.png}
\includegraphics[0.3\textwidth]{DomMaHard.png}
}
\end{center}
\caption{
The figure on the right is the statistics of all questions collected by Xiezhi.
The middle figure shows statistics for Xiezhi-Easy and the left shows Xiezhi-Hard.}
\label{fig:benchstatistic}
\end{figure}

\subsection{Ouputs Assessment}
\label{033}
The difficulties of generative model evaluation mainly lie in:
How to efficiently extract the options chosen by the model from the output of the model.
One way of thinking is to use instructions to control the output of the model when doing few-shot or zero-shot evaluation, so that the choices made by the model can be easily extracted.
However, the model is very sensitive to instructions, and it is difficult for us to control the output of all models with a unified instruction.
Moreover, not all models are suitable for multiple-choice questions, which will bring unfair evaluation to models with poor ability to do multiple-choice questions.

For the open source model, we propose to judge the options selected by the model by obtaining the probability of each option generated by the model.
As for the non-open source models, we found that these models are extremely capable, so we asked the models to output the probability that they chose each option, and used this as a judgment.


% 生成式模型评估的难点主要在于：
% 如何有效地从模型的输出中抽取模型选择的选项。
% 一种思路是，做few-shot或zero-shot评估时，利用指令去控制模型的输出，使模型做出的选择容易被抽取。
% 但模型对于指令非常敏感，我们难以用统一的指令控制所有模型的输出。
% 而且不是所有模型都适合做选择题，这会给做选择题能力较差的模型带来不公平的评估。

% 对于开源模型，我们提出通过获取模型生成每个选项的概率，来判断模型选择的选项。
% 至于非开源模型，我们发现这些模型的能力都极强，所以我们要求模型输出他们选择每个选项的概率，并以此作为判断。


==> old_version/03BenchmarkDescription.6.tex <==
% In this section, we will provide a detailed description of Xiezhi Benchmark. 
% We begin by defining the term "domain" in our study and elaborating the relation between Chinese subject system and domain knowledge in subsection~\ref{031}.
% The process of data collection, annotation and auto updating are given in subsection~\ref{032}.
% Finally, we will discuss the evaluation methods we designed for assessing open-source and non-open-source generative LMs' outputs in subsection~\ref{033}.


\subsection{Chinese Discipline Classification System}
\label{031}

% \subsubsection{Definition}
% \red{
% 还没开始写。

% Domain knowledge refers to the in-depth understanding, expertise, and familiarity with a specific subject, industry, field, or area of special interest. 
% This knowledge is often held by experts or practitioners and is gradually accumulated and refined through research and work in the relevant field.
% The mastery of domain knowledge directly affects the efficiency and quality of work and research.
% }

% \subsubsection{Chinese Discipline Classification System}
The discipline classification system in China, developed by the Ministry of Education of China, organizes subjects of different domain education in college education. 
The system divides all domains into 14 subjects categories, and various levels of subjects. 
The meanings of these levels are as follows:

\textbf{Discipline Categories}: This is the highest level of discipline classification, divided according to the nature, characteristics of subjects. 
There are 13 subject categories in Chinese discipline classification, including philosophy, economics, law, education, literature, history, science, engineering, agriculture, medicine, military science, management and art.

\textbf{First-level disciplines}: Related research fields sharing similarities are categorized as first-level disciplines. 
For example, under the economics category, there are first-level disciplines such as "Political Economy", "Econometrics", "Finance" and so on. 

\textbf{Second-level disciplines}: These disciplines represent more subdivided areas of study or topics within the primary discipline.
For example, within the first level of 'finance', further divisions may include 'financial markets', 'banking', 'insurance "and "international finance" as secondary disciplines.

As shown in Fig.~\ref{fig:subjectclassification}, Chinese Discipline Classification is a hierarchical structure, where academic categories are at the top, representing a broader range and connotation of a subject. 
First-level, second-level and even third-level disciplines represent more specific areas and more finely divided research areas within academic categories.
There are a total of 118 first-level disciplines, we take all of these disciplines as the basic classifications of domain knowledge.
And there are about 400+ second-level and 1000+ third-level disciplines, we take 393 of second-level to further annotate the questions in our benchmark.

\subsection{Dataset Construction} \label{032}

\subsubsection{Data collection}
Xiezhi comprises two main categories of questions, one is questions from exams and the other is generated questions. 
Xiezhi has primarily collected 150,000 questions from six distinct exam types, which include elementary school exams, middle school entrance exams, college entrance exams, undergraduate exams, graduate entrance exams, and adult education exams. 
Additionally, Xiezhi encompasses 50,000 generated questions, primarily created by words masking and options generating in academic surveys across various domains and crafting multiple-choice questions.

\subsubsection{Annotation Process}
We annotated 50,000 questions collected from the Graduate Entrance Examination to form the meta version of Xiezhi through both manual efforts and chatGPT.
The aim of annotation is to remove unanswerable questions and to tag each question with as many first and second level disciplines as possible.

We first used ChatGPT to tag each question with first or second level disciplines. 
In the process of tagging, we build prompt by concatenate the content of a question with its options, answers and exam information with the description of each disciplines to increase chatGPT's understanding to the question so that the question could be better tagged.
The questions annotated by chatGPT can be used to test chatGPT or even more powerful LLMs, since lot of additional information is used during the annotation process and only the question description is used in the inference process.

Based on the annotated results, we do the manual annotation to further ensure the quality of the dataset.
The manually annotations include the following requirement for each questions:
(1). Mark questions that cannot be answered with text information alone. 
These questions include those requiring image interpretation or audio information. 
We exclude the questions that requires non-text information from the benchmark.
The annotators are extra paid if they find any unanswerable questions.
(2). Check the output of ChatGPT or remark the first-level and second-level discipline labels involved in the questions.
The annotators are also extra paid if they find the error made by chatGPT or tagged more labels than chatGPT to the questions.

We hired and paid graduate students from various majors to annotate and clean the questions we collected. 
We provided training for all potential annotators and tested their understanding of the training content to ensure they fully met our requirements. 
11 graduate students are selected as our annotators, and all of them are paid above the local minimum wage.
And to ensure the quality of the annotations, each question is annotated by at least three annotators.


\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{DomMa.png}
\includegraphics{DomMaMedium.png}
\includegraphics{DomMaHard.png}
}
\end{center}
\caption{
The figure on the right is the statistics of all questions collected by Xiezhi.
The middle figure shows statistics for Xiezhi-Easy and the left shows Xiezhi-Hard.}
\label{fig:benchstatistic}
\end{figure}


\subsubsection{Question Generation}
We generated 50,000 multiple-choice questions utilizing texts from various academic surveys as they contain well-established domain knowledge. 
We selected longest sentences from these surveys and masked keywords within them to construct questions that target the most critical parts of the sentences. 
We collected all of the options available in Xiezhi and randomly selected several items to fill up the required number of options.

\subsubsection{Auto Annotation}

Except for the meta version build by manually works, we wish to automatically update the future version of Xiezhi.
Automatic update has the same requirement as manual annotation, that is, to exclude unanswerable questions and tag the disciplines labels involved in each question.

For unanswerable questions, we extracted keywords from the Xiezhi-meta, such as "as shown in the figure below" or "as listed in the table" and so on, and exclude questions which contain any of these keywords from collected data.

And to achieve the purpose of first and second disciplines labeling, we, similar to the previous subsection, input the detailed information of a question and disciplines with their descriptions to ChatGPT to help us with question annotation.
In addition, we trained a GPT-Classifier using human-annotated questions. 
This GPT-Classifier can determine the relevance between text content and a specific category based on the category description. 
Finally, we use trained GPT-Classifier and ChatGPT to do joint annotation.

\subsubsection{Xiezhi-Easy \& Xiezhi-Hard}
To ensure the validity of the evaluation results, we further propose two additional datasets, Xiezhi-Easy and Xiezhi-Hard. These datasets are derived from the original Xiezhi Benchmark with the exclusion of certain sensitive questions (e.g., military science) and items containing Chinese-bias in the text. We utilized two models, bloomz-7b1 and chatglm-6b, to predict responses for all questions within the Xiezhi Benchmark under a four-option setting. Ensuring a balanced sample, Xiezhi-Easy was constructed by selecting as many questions as possible that both models could answer correctly, while Xiezhi-Hard included as many questions as possible that both models answered incorrectly.



% The questions in dataset were manually collected from two freely available sources online.
% One is from the Chinese graduate entrance exam questions.
% Chinese universities are allowed to set their own questions for the enrollment of their first and second level disciplines, so an extremely large amount of questions are generated each year.
% The quality of the questions from this source is high as they are reviewed by the Chinese Education Department.
% To further improve the quality through manual annotation, we have collected around 400k questions from this source.
% Another source is the questions from mid-term and final exams in each universities.
% The quality of the questions from this source varies a lot, while the update frequency of the questions from this source is much higher than the previous one.
% So as long as we do a good job in automaticly filtering and annotating, the data from this source will be available to continuously update to Xiezhi.
% We have finally collected 100k questions from this source through automatic filtering and annotation.


% \subsubsection{Manual Annotation}
% We manually annotated the questions collected from the Graduate Entrance Examination to form the meta version of Xiezhi.
% The aim of annotation is to remove unanswerable questions and to tag each question with as many first and second level disciplines as possible.

% We first used ChatGPT to tag each question with first or second level disciplines. 
% In the process of tagging, we build prompt by concatenate the content of a question with its options, answers and exam information with the description of each disciplines to increase chatGPT's understanding to the question so that the question could be better tagged.
% We again used chatGPT's perplexity to differentiate the quality of the questions.
% The detailed template of the prompt and how we use the perplexity is listed in appendix~\ref{}.
% \blue{We find that the questions annotated by chatGPT can be used to test chatGPT or even more powerful LLMs, since chatGPT use a lot of additional information in the annotation process and use only the question description in the inference process.}
% As for Xiezhi, we have subsequent manual annotation to further ensure the quality of the questions.

% The manually annotations include the following requirement for each questions:
% (1). Mark questions that cannot be answered with text information alone. 
% These questions include those requiring image interpretation or audio information. 
% We exclude the questions that requires non-text information from the benchmark.
% The annotators are extra paid if they find any unanswerable questions.
% (2). Check the output of ChatGPT or remark the first-level and second-level discipline labels involved in the questions.
% The annotators are also extra paid if they find the error made by chatGPT or tagged more labels than chatGPT to the questions.

% We hired and paid graduate students from various majors to annotate and clean the questions we collected. 
% We provided training for all potential annotators and tested their understanding of the training content to ensure they fully met our requirements. 
% 20 graduate students are selected from different subject categories as our annotators. 
% All of them are paid above the local minimum wage.
% And to ensure the quality of the annotations, each sample is annotated by at least three annotators.



% \subsubsection{Auto Updating} 







% \subsection{Ouputs Assessment}
% \label{033}
% The difficulties of generative model evaluation mainly lie in:
% How to efficiently extract the options chosen by the model from the output of the model.
% One way of thinking is to use instructions to control the output of the model when doing few-shot or zero-shot evaluation, so that the choices made by the model can be easily extracted.
% However, the model is very sensitive to instructions, and it is difficult for us to control the output of all models with a unified instruction.
% Moreover, not all models are suitable for multiple-choice questions, which will bring unfair evaluation to models with poor ability to do multiple-choice questions.

% For the open source model, we propose to judge the options selected by the model by obtaining the probability of each option generated by the model.
% As for the non-open source models, we found that these models are extremely capable, so we asked the models to output the probability that they chose each option, and used this as a judgment.


% 生成式模型评估的难点主要在于：
% 如何有效地从模型的输出中抽取模型选择的选项。
% 一种思路是，做few-shot或zero-shot评估时，利用指令去控制模型的输出，使模型做出的选择容易被抽取。
% 但模型对于指令非常敏感，我们难以用统一的指令控制所有模型的输出。
% 而且不是所有模型都适合做选择题，这会给做选择题能力较差的模型带来不公平的评估。

% 对于开源模型，我们提出通过获取模型生成每个选项的概率，来判断模型选择的选项。
% 至于非开源模型，我们发现这些模型的能力都极强，所以我们要求模型输出他们选择每个选项的概率，并以此作为判断。


==> old_version/04Experiments.1.tex <==

% In the experiments, we wish to answer two question: \textit{Q1)} DomMa是否可以评估出不同LLMs对于领域知识的回答能力？\textit{Q2)} DomMa针对于一些LLMs所特有的设计是否合理？
% 因此，我们在第~\ref{041}章节详细介绍了我们的实验设定；在第~\ref{042}章节展示了目前主流的LLM和一些经典的LM在我们的Domain Benchmark上的结果；在第~\ref{043}设计实验来验证DomMa的一些针对于LLMs设计的合理性。

In the experiments, we aim to answer two questions: 
\textit{Q1)} Can DomMa evaluate the domain knowledge answering capabilities of different LLMs? 
\textit{Q2)} Is the design of DomMa specifically for some LLMs reasonable?

Therefore, we provide a detailed description of our experimental setup in subsection~\ref{041}. 
In subsection~\ref{042}, we present the results of the current mainstream LLMs and some classic LMs on our Domain Benchmark.
In subsection~\ref{043}, we design experiments to verify the rationality of some of the DomMa designs for LLMs.

\subsection{Experiment Setup}
\label{041}

% 我们将所有的模型分为两组：
% \textbf{15B以下的开源LLM：}同时为了方便比较，我们使用了主要以Bloomz和LlaMa作为base模型进行指令微调得到的LLM。Bloomz、BELLE-2M、LlaMa、Alpaca、。
% \textbf{超大规模的未开源LLM：}因为很多模型都处于内测阶段，同时不是所有模型都开放了API，所以我们的评估仅针对目前已经完全开放使用的模型。130BchatGLM、ChatGPT(3.5-turbo)、GPT-4、Claude、。

% 我们在不同的实验设定中使用了不同的指标：在Overall Experiments中，选项的数量从设置为4一直增大到设置为50，在这个实验中我们使用了Hit@k和MRR这两个指标、在Feasibility Verification中，我们设置了选项数量为4，并使用了Accuracy和MSE这两个指标。
% 同时我们期望测试模型对于demonstration的理解能力，同时考虑到模型输入的长度有限，所以我们测试了模型在0-shot、1-shot、3-shot设定下的能力。

\subsubsection{Models}

\textbf{Open-source LLMs with less than 15B parameters:} For the sake of comparison, we use LLMs obtained by fine-tuning the base models, mainly Bloomz and LlaMa, with instructions. These include Bloomz, BELLE-2M, LlaMa, Alpaca, etc.

\textbf{Ultra-large-scale non-open-source LLMs:} Since many models are in the beta testing stage and not all models have open APIs, our evaluation is only for the models currently fully available for use. These include 130BchatGLM, ChatGPT(3.5-turbo), GPT-4, Claude, etc.


\subsubsection{Metirc}
We use different metrics in various experimental settings: in Overall Experiments, the number of options is increased from 4 to 50; in this experiment, we use \textit{Hits@k} and \textit{MRR} as the evaluation metrics. 
In Feasibility Verification, we set the number of options to 4 and use \textit{Accuracy~(Hits@1)} and \textit{MSE} as evaluation metrics.

\subsubsection{Few-Shot Demonstration}

Additionally, we aim to test the models' understanding of demonstrations while considering the limited input length. Therefore, we evaluate the models' capabilities under 0-shot, 1-shot, and 3-shot settings.



\subsection{Overall Results}
\label{042}
我们在这节首先展示各个模型在所有学科门类上的表现结果，并在图~\ref{fig:overall_experiments}中进行了展示。
其次，我们展示了chatGPT和GPT-4在所有一级学科上的结果，并在图~\ref{fig:overall_experiments}中进行了展示。
至于所有模型在所有一级学科上的表现结果，我们放在了Appendix中进行展示。

从结果中我们可以看到，小模型在各项能力上的表现都不如大模型。
在0-shot的设定上，小模型普遍比大模型要差10\%的accuracy。
在1-shot和3-shot的设定上，小模型本来应该有较大的提升空间，但他们的的提升也远不如大模型，所以可以认为小模型对于demonstration的理解能力非常有限。

我们还可以注意到，工科、理科这种涉及逻辑推理和符号推理的学科一般表现都会比较差。
而像历史、文学这种比较需要知识积累的学科，模型的表现都比较好。
这也对应了前人的实验结果——模型擅长记忆而不擅长推理。
同时可以看到随着模型的参数量越来越大，模型在工科和理科上的提升要逼历史学科上的提升更大，由此可以认为模型参数将非常有助于模型推理能力的提升。

\red{对于方差的分析}

\red{每个一级学科的结果分析}

\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{Overall_hit1.png}
\includegraphics{Overall_hit3.png}
\includegraphics{Overall_hit5.png}
\includegraphics{Overall_mrr.png}
}
\end{center}
\label{fig:overall_experiments}
\caption{所有模型用灰盒、白盒、黑盒中效果最好的方法做50选1的结果，x轴为各个学科门类，y轴为Hit@1，Hit@3，Hit@5, MRR}
\end{figure}



\subsection{Feasibility Verification}
\label{043}




\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{OverallExperiments.png}
\includegraphics{OverallExperiments.png}
\includegraphics{OverallExperiments.png}
}
\end{center}
\label{fig:feasibility_verification}
\caption{左边是黑盒测试的四选一结果，中间是灰盒测试的四选一结果，右边是白盒测试的四选一结果。}
\end{figure}


我们在这一小节详细展示了DomMa设计的可行性，并将结果展示在图~\ref{fig:feasibility_verification}中。
\subsubsection{Feasible to Answer Multiple-Choice QA}
图~\ref{fig:feasibility_verification}的左侧是黑盒测试的结果，我们可以看到在Overall Experiments的图~\ref{fig:overall_experiments}中展示的baseline都达到了至少25\%的能力，这说明了这些模型能够理解指令，并且能够根据指令做出正确的回应。
但同时，我们也能发现BELLE-2m、BELLE-1m这几个模型的表现都明显低于25\%的能力，根据我们的设计，我们可以认为这些模型没有进行过相关的预训练或者指令微调，所以黑盒测试无法有效地测试这些模型的真实表现水平。

图~\ref{fig:feasibility_verification}的中间是灰盒测试的结果，我们可以看到在黑盒中表现一般的ChatGLM-130B在灰盒中效果明显好多了，但是各种10B以下的小模型在灰盒中的效果明显下降了。
根据我们的设计，我们认为ChatGLM-130B表现好的原因是因为它并没有在选择题的环境中进行过指令微调，所以不适合黑盒的测试方式，而灰盒的测试方式就会明显好很多。
各种10B以下的小模型应该都没有被要求输出过困惑度，所以他们理解不了这一指令，从而带来的效果的降低。

图~\ref{fig:feasibility_verification}的右侧是白盒测试的结果，因为我们无法得到未开源模型的参数，所以白盒的设定存在先天不足。
但针对能获取到开源参数的模型，我们可以看到，所以模型的效果都达到了至少25\%的水平，这可以认为所有的模型在白盒的测试方法下，都具备了回答选择题的能力。
\subsubsection{Show the Difference Among LLMs}
我们可以看到，DomMa是能够体现LLMs的区分度的。
比如ChatGPT和GPT-4这俩公认比较厉害的模型就明显比其他模型要厉害很多
而像Huatuo、Blooger这些领域LLMs，在他们各自的领域上效果也表现得非常好。
而像BELLE这些重点在于闲聊的模型，在他们做了大量的指令微调之后，效果还要比他们的基地模型Bloomz要差。
\subsubsection{Data Contamintaion}
我们可以在图~\ref{fig:openai_experiments}中看到，哪怕是GPT-4在zero-shot的设定下的表现都不是很高，而在3-shot的设定下会明显比0-shot的要好很多。
由此我们可以认为，DomMa里面确实存储了很多不存在与GPT-4预训练语料中的知识（0-shot效果差），但是这些知识是理论上可以被答对的，并且同个学科下的知识之间是具有较强关联性的（3-shot效果好），不过题目之间依然是存在区分度的（因为10-shot相较于3-shot依然能带来很多提升）




\begin{figure}[h]
\begin{center}
\resizebox{0.6\textwidth}{!}{
\includegraphics{OverallExperiments.png}
}
\end{center}
\label{fig:openai_experiments}
\caption{chatGPT和GPT-4用灰盒方法0-shot、3-shot、10-shot设定下做50选1的结果，y轴为Hit@3}
\end{figure}





==> old_version/04Experiments.2.tex <==
\subsection{Setup}
\label{041}

\textbf{Models:}
To measure performance on our multitask test, we compute the classification accuracy across all examples and tasks.
我们使用了68种模型进行了实验，所有模型的介绍和实验结果放在了appendix里。
在接下来的实验中，我们重点在于展示一些我们认为非常有意义和有趣的实验结果以及分析。
因此我们将这些模型按照不同的特点进行分门别类并展示其统计意义上的实验结果。
另外我们还重点对比了几个千亿参数量的模型，这些模型有GPT-3, ChatGPT, GPT-4, ChatGLM, Bloomz。
除了Bloomz之外，我们均调用了这些模型所有者的APIs进行实验。


\textbf{Few-Shot Demonstration:}
Additionally, we aim to test the models' understanding of demonstrations. 
Therefore, we evaluate the models' capabilities under 0-shot, 1-shot, and 3-shot settings.
All the examples used for demonstration are obtained from DomMa's training set, and have at least one first-level discipline label matching with the test questions

% The models we evaluate are listed in~\ref{tab:models}, which covers nearly all of the Causal LMs~(CLMs).
% For GPT-3, ChatGPT, GPT-4, ChatGLM and GLM-130B we use APIs for evaluation.
% Like MMLU~\cite{hendrycks2021measuring}, we also fine-tune RoBERTa, ALBERT and GPT-2 on DomMa and test their ability.
% As for the entire experiments result, please refer to the Appendix.

\input{models_table}

% \textbf{Metric:}
% We use different metrics in various experimental settings:
% 我们用有10以及50个选项的选择题去测试模型的领域文本理解能力，并使用\textit{Hits@k} and \textit{MRR}作为指标来观察模型的能力。
% 我们用4个选项的选择题来观察
% We use multiple-choice question with 10 and 50 options to test the  the number of options is increased 10 and 50, we use \textit{Hits@k} and \textit{MRR} as the evaluation metrics. 
% In Feasibility Verification, we set the number of options to 4 and use \textit{Accuracy~(Hits@1)} and \textit{MSE} as evaluation metrics.




\subsection{Results}
\label{042}
我们在这节首先展示了各个模型在所有学科门类上的表现结果，并将结果可视化在图~\ref{fig:overall_experiments}中，这里我们对于每个模型都取他们在黑白灰盒三种测试方法中所能达到的最好表现。
至于所有模型在所有一级学科上的表现结果，我们放在了Appendix中进行展示。
其次，我们研究了黑白灰盒三种评估方法对于不同模型的影响，并将结果展示在了图~\ref{fig:feasibility_verification}中。
我们还研究了选项数量对于评估结果的影响，并将结果展示在了图~\ref{fig:choice_num}中。
最后，我们针对ChatGPT和GPT-4这两个目前公认的能力最强，且具有继承关系的模型，详细地展示了他们在各一级学科上的结果，并将结果可视化在图~\ref{fig:openai_experiments}中。

\subsubsection{Model Performance:}

\red{小模型的表现差}

\red{小模型理解Demonstration的能力也不强}

\red{领域小模型在对应的领域上能有超过大模型的效果}

\red{参数量在一定范围内的差别不会很大}

\red{Decoder占比越大，模型效果越好}

\red{本来模型对于某个指令具有理解能力，但是指令微调没有相关数据，则模型在指令微调之后也会丧失对于这个指令的理解能力}

\red{GPT-4明显好过其他所有模型，且在一些学科上超过了专家的水平}

% 从结果中我们可以看到，小模型在各项能力上的表现都不如大模型。
% 在0-shot的设定上，小模型普遍比大模型要差10\%的accuracy。
% 在1-shot和3-shot的设定上，小模型本来应该有较大的提升空间，但他们的的提升也远不如大模型，所以可以认为小模型对于demonstration的理解能力非常有限。

% 我们还可以注意到，工科、理科这种涉及逻辑推理和符号推理的学科一般表现都会比较差。
% 而像历史、文学这种比较需要知识积累的学科，模型的表现都比较好。
% 这也对应了前人的实验结果——模型擅长记忆而不擅长推理。
% 同时可以看到随着模型的参数量越来越大，模型在工科和理科上的提升要逼历史学科上的提升更大，由此可以认为模型参数将非常有助于模型推理能力的提升。

% 除此之外，通过展示chatGPT和GPT-4在0-shot、1-shot、3-shot的设定下统计的Hits@5指标，以及直接在数据集上进行fine-tune的Bloom-7B，我们可以得出结论：DomMa里的数据都是可学习的。

% 我们可以在图~\ref{fig:openai_experiments}中看到，哪怕是GPT-4在zero-shot的设定下的表现都不是很高，而在3-shot的设定下会明显比0-shot的要好很多。
% 由此我们可以认为，DomMa里面确实存储了很多不存在与GPT-4预训练语料中的知识（0-shot效果差），但是这些知识是理论上可以被答对的，并且同个学科下的知识之间是具有较强关联性的（3-shot效果好），不过题目之间依然是存在区分度的（因为10-shot相较于3-shot依然能带来很多提升）


\subsubsection{DomMa Feasibility}

\red{DomMa的题目设置具有区分度，不同模型在DomMa上的表现差异很大}

\red{DomMa的学科分类设置合理，同一模型在不同学科分类下的表现差异依然很大，而领域模型在对应的学科分类下效果很好}

\red{DomMa的一级学科分类设置合理，同样的数据规模下，模型在一级学科集合中表现的方差要小于学科分类集合中表现的方差}

\red{DomMa的题目是模型可以答对的，因为fine-tune Bloom的效果极好}

\red{对于无法理解指令的模型而言，预测选项概率能够成功诱导出模型会的知识——黑盒设定低于25\%的准确率，而灰盒白盒设定明显高于25\%的准确率}

\red{增加选项数量是一个有效增加模型之间区分度的方式}

% 图~\ref{fig:feasibility_verification}的左侧是黑盒测试的结果，我们可以看到在Overall Experiments的图~\ref{fig:overall_experiments}中展示的baseline都达到了至少25\%的能力，这说明了这些模型能够理解指令，并且能够根据指令做出正确的回应。
% 但同时，我们也能发现BELLE-2m、BELLE-1m这几个模型的表现都明显低于25\%的能力，根据我们的设计，我们可以认为这些模型没有进行过相关的预训练或者指令微调，所以黑盒测试无法有效地测试这些模型的真实表现水平。

% 图~\ref{fig:feasibility_verification}的中间是灰盒测试的结果，我们可以看到在黑盒中表现一般的ChatGLM-130B在灰盒中效果明显好多了，但是各种10B以下的小模型在灰盒中的效果明显下降了。
% 根据我们的设计，我们认为ChatGLM-130B表现好的原因是因为它并没有在选择题的环境中进行过指令微调，所以不适合黑盒的测试方式，而灰盒的测试方式就会明显好很多。
% 各种10B以下的小模型应该都没有被要求输出过困惑度，所以他们理解不了这一指令，从而带来的效果的降低。

% 图~\ref{fig:feasibility_verification}的右侧是白盒测试的结果，因为我们无法得到未开源模型的参数，所以白盒的设定存在先天不足。
% 但针对能获取到开源参数的模型，我们可以看到，所以模型的效果都达到了至少25\%的水平，这可以认为所有的模型在白盒的测试方法下，都具备了回答选择题的能力。
% \textbf{Show the Difference Among LLMs}
% 我们可以看到，DomMa是能够体现LLMs的区分度的。
% 比如ChatGPT和GPT-4这俩公认比较厉害的模型就明显比其他模型要厉害很多
% 而像Huatuo、Blooger这些领域LLMs，在他们各自的领域上效果也表现得非常好。
% 而像BELLE这些重点在于闲聊的模型，在他们做了大量的指令微调之后，效果还要比他们的基地模型Bloomz要差。








\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{Overall_hit1.png}
\includegraphics{Overall_hit3.png}
\includegraphics{Overall_hit5.png}
\includegraphics{Overall_mrr.png}
}
\end{center}
\label{fig:overall_experiments}
\caption{所有模型用灰盒、白盒、黑盒中效果最好的方法做50选1的结果，x轴为各个学科门类，y轴为Hit@1，Hit@3，Hit@5, MRR}
\end{figure}

\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{OverallExperiments.png}
\includegraphics{OverallExperiments.png}
\includegraphics{OverallExperiments.png}
}
\end{center}
\label{fig:feasibility_verification}
\caption{左边是黑盒测试的四选一结果，中间是灰盒测试的四选一结果，右边是白盒测试的四选一结果。}
\end{figure}



\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{ablationOnChoice.png}
\includegraphics{ablationOnChoice.png}
}
\end{center}
\label{fig:choice_num}
\caption{chatGPT、Bloom-7B、Bert-FT在选项增多时再0-shot、1-shot、3-shot设定下的结果}
\end{figure}

\begin{figure}[h]
\begin{center}
\resizebox{0.6\textwidth}{!}{
\includegraphics{OverallExperiments.png}
}
\end{center}
\label{fig:openai_experiments}
\caption{\red{这张图要调整成MMLU论文里的那种长条状}chatGPT和GPT-4用灰盒方法0-shot、3-shot、10-shot设定下做50选1的结果，y轴为Hit@3}
\end{figure}





==> old_version/04Experiments.3.tex <==
\subsection{Setup}
\label{041}

\textbf{Models:} % 选择哪些模型
We conducted experiments with 68 different models, and the introductions as well as results for all the models are presented in the appendix. 
In the subsequent section, our focus lies in demonstrating some of the results and analysis that we find particularly meaningful and intriguing.
Therefore, we classify these models based on their distinct characteristics and present their statistically significant experimental results.
Furthermore, we place special emphasis on comparing several models with hundreds of billions of parameters, including GPT-3, ChatGPT, GPT-4, ChatGLM, and Bloomz. 
For GPT-3, ChatGPT, GPT-4, and ChatGLM, we used the APIs provided by the respective model owners for experimentation, while we utilized open-source parameters for all the other models.


\textbf{More options:}  % 选项如何设置

\textbf{Results Acquired:}  % 如何获得结果





\textbf{Few-Shot Demonstration:}  % 如何得到few-shot结果
Additionally, we aim to test the models' understanding of demonstrations. 
Therefore, we evaluate the models' capabilities under 0-shot, 1-shot, and 3-shot settings.
All the examples used for demonstration are obtained from Xiezhi's training set, and have at least one first-level discipline label matching with the test questions





\subsection{Results}
\label{042}
我们在正文部分将各个语言模型按照不同的basemodel进行归类，并展示随着参数量的增大，以及各个不同的basemodel随着ift数据量的增强，模型在我们数据集上的整体表现效果，如图~\ref{fig:TheSameBasemodel}所示。
我在图~\ref{fig:LargeBasemodel}中展示了参数量超过100B的几个模型的效果。
最后，我们在表~\ref{tab:detailedModelsPerformance}中分类展示了basemodel相同的不同小模型的效果。

\subsubsection{Model Performance:}

\red{小模型的表现差}

\red{小模型理解Demonstration的能力也不强}

\red{领域小模型在对应的领域上能有超过大模型的效果}

\red{参数量在一定范围内的差别不会很大}

\red{Decoder占比越大，模型效果越好}

\red{本来模型对于某个指令具有理解能力，但是指令微调没有相关数据，则模型在指令微调之后也会丧失对于这个指令的理解能力}

\red{GPT-4明显好过其他所有模型，且在一些学科上超过了专家的水平}

% 从结果中我们可以看到，小模型在各项能力上的表现都不如大模型。
% 在0-shot的设定上，小模型普遍比大模型要差10\%的accuracy。
% 在1-shot和3-shot的设定上，小模型本来应该有较大的提升空间，但他们的的提升也远不如大模型，所以可以认为小模型对于demonstration的理解能力非常有限。

% 我们还可以注意到，工科、理科这种涉及逻辑推理和符号推理的学科一般表现都会比较差。
% 而像历史、文学这种比较需要知识积累的学科，模型的表现都比较好。
% 这也对应了前人的实验结果——模型擅长记忆而不擅长推理。
% 同时可以看到随着模型的参数量越来越大，模型在工科和理科上的提升要逼历史学科上的提升更大，由此可以认为模型参数将非常有助于模型推理能力的提升。

% 除此之外，通过展示chatGPT和GPT-4在0-shot、1-shot、3-shot的设定下统计的Hits@5指标，以及直接在数据集上进行fine-tune的Bloom-7B，我们可以得出结论：Xiezhi里的数据都是可学习的。

% 我们可以在图~\ref{fig:openai_experiments}中看到，哪怕是GPT-4在zero-shot的设定下的表现都不是很高，而在3-shot的设定下会明显比0-shot的要好很多。
% 由此我们可以认为，Xiezhi里面确实存储了很多不存在与GPT-4预训练语料中的知识（0-shot效果差），但是这些知识是理论上可以被答对的，并且同个学科下的知识之间是具有较强关联性的（3-shot效果好），不过题目之间依然是存在区分度的（因为10-shot相较于3-shot依然能带来很多提升）


\subsubsection{Xiezhi Feasibility}

\red{Xiezhi的题目设置具有区分度，不同模型在Xiezhi上的表现差异很大}

\red{Xiezhi的学科分类设置合理，同一模型在不同学科分类下的表现差异依然很大，而领域模型在对应的学科分类下效果很好}

\red{Xiezhi的一级学科分类设置合理，同样的数据规模下，模型在一级学科集合中表现的方差要小于学科分类集合中表现的方差}

\red{Xiezhi的题目是模型可以答对的，因为fine-tune Bloom的效果极好}

\red{对于无法理解指令的模型而言，预测选项概率能够成功诱导出模型会的知识——黑盒设定低于25\%的准确率，而灰盒白盒设定明显高于25\%的准确率}

\red{增加选项数量是一个有效增加模型之间区分度的方式}

% 图~\ref{fig:feasibility_verification}的左侧是黑盒测试的结果，我们可以看到在Overall Experiments的图~\ref{fig:overall_experiments}中展示的baseline都达到了至少25\%的能力，这说明了这些模型能够理解指令，并且能够根据指令做出正确的回应。
% 但同时，我们也能发现BELLE-2m、BELLE-1m这几个模型的表现都明显低于25\%的能力，根据我们的设计，我们可以认为这些模型没有进行过相关的预训练或者指令微调，所以黑盒测试无法有效地测试这些模型的真实表现水平。

% 图~\ref{fig:feasibility_verification}的中间是灰盒测试的结果，我们可以看到在黑盒中表现一般的ChatGLM-130B在灰盒中效果明显好多了，但是各种10B以下的小模型在灰盒中的效果明显下降了。
% 根据我们的设计，我们认为ChatGLM-130B表现好的原因是因为它并没有在选择题的环境中进行过指令微调，所以不适合黑盒的测试方式，而灰盒的测试方式就会明显好很多。
% 各种10B以下的小模型应该都没有被要求输出过困惑度，所以他们理解不了这一指令，从而带来的效果的降低。

% 图~\ref{fig:feasibility_verification}的右侧是白盒测试的结果，因为我们无法得到未开源模型的参数，所以白盒的设定存在先天不足。
% 但针对能获取到开源参数的模型，我们可以看到，所以模型的效果都达到了至少25\%的水平，这可以认为所有的模型在白盒的测试方法下，都具备了回答选择题的能力。
% \textbf{Show the Difference Among LLMs}
% 我们可以看到，Xiezhi是能够体现LLMs的区分度的。
% 比如ChatGPT和GPT-4这俩公认比较厉害的模型就明显比其他模型要厉害很多
% 而像Huatuo、Blooger这些领域LLMs，在他们各自的领域上效果也表现得非常好。
% 而像BELLE这些重点在于闲聊的模型，在他们做了大量的指令微调之后，效果还要比他们的基地模型Bloomz要差。








\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{ModelSizePerformance.png}
\includegraphics{IftSizePerformance.png}
}
\end{center}
\label{fig:TheSameBasemodel}
\caption{
\red{考虑下如何构图，5月18日填上}
主要展示Pythia(1.4b, 7b, 12b, 30b)
Dolly(3b,  6b, 7b, 12b)
Bloomz(1.1b, 1.7b, 3b, 7.1b)
h2oGPT(7b, 12b, 20b)
stableLM(3b, 7b)
llama(7b, 13b, 30b)
vicuna(7b, 13b)
左图为Xiezhi-Easy，右图为Xiezhi-Hard
}
\end{figure}

\begin{figure}[h]
\begin{center}
\resizebox{\textwidth}{!}{
\includegraphics{llm_performance_easy.png}
}
\resizebox{\textwidth}{!}{
\includegraphics{llm_performance_hard.png}
}
\end{center}
\label{fig:LargeBasemodel}
\caption{文心一言、星火大模型（暂无API）、chatGPT、Bloomz、GPT-4用Xiezhi-Easy和Xiezhi-Hard在0-shot、1-shot、3-shot设定下的结果，用Hit@1作为指标\red{两图合并，label放在下面，调色}}
\end{figure}




\input{different_models_performance_table}







==> old_version/04Experiments.4.tex <==
\subsection{Setup}
\label{041}

\textbf{Models:} % 选择哪些模型
We conducted experiments on 52 different models, the detailed introductions as well as results for all the models are presented in the appendix. 
In the subsequent section, our focus lies in demonstrating some of the results and analysis that we find particularly meaningful and intriguing.
Our experiments cover the dominant dialogue LMs obtained from six different base models - bloomz, llama, pythia, gpt-neox, moss, and chatGLM.
These dialogue LMs range from 560M to 30B in terms of number of parameters.
In addition to this, we present the detailed experiments results of some large dialogue LMs contain more than 65B parameters like llama-65B, bloomz-176B, bloomz-mt-176B, bloomz-p3-176B.
Considering the legal issues, we only show the results of two public recognized API-based LMs, ChatGPT and GPT-4.
\red{哪些模型是用生成概率计算结果的}
\red{哪些模型使用指令诱导出结果的}


\textbf{More options:}  % 选项如何设置
We instruct tested model to select the best-fit answer from 50 options for each question.
Each question is set up with 3 confusing options in addition to the correct answer, and another 46 options randomly sampled from all options in all questions in Xiezhi.
It is worth noting that it is possible to use WordNet, open source synonym databases, or other word construction methods to generate more confusing options.
However, the experiments show that the performance of all LMs, even when using so many non-confusing options, had declined dramatically.
This achieves our goal of exacerbating the performance discrimination between models through new experimental settings, and also shows that the traditional 4-choice setting has room for improvement.

\textbf{Few-Shot Demonstration:}  % 如何得到few-shot结果
Additionally, we aim to test the models' understanding of demonstrations. 
Therefore, we evaluate the models' capabilities under 0-shot, 1-shot, and 3-shot settings.
Although most previous works use the 5-shot setting, our experiments are limited by the maximum output length of some LMs, so we don't use 5-shot setting.
All the examples used for demonstration are obtained from Xiezhi's training set, and have at least one first-level discipline label matching with the test questions

\subsection{Results}
The performance of all language models are listed in Tab.~\ref{tab:all-llm}, and the ranking of all models with less than 100B parameters in each domain category are listed in Tab.~\ref{tab:llm-rank}.
The detailed performance of each models in every domain category \red{will} be provided in Appendix.
And here are the evaluation results of the experiments.
% We report the average MRR score, while a detailed breakdown of mrr per sub-discipline \red{will} be provided in Appendix.

\textbf{Pretraining + Finetuning = Best Performance}
在Xiezhi数据集上，baize取得了平均而言最好的表现。
这得益于他们使用的基座模型——llama非常得好，其次也源于他们使用了从ChatGPT诱导出的多轮对话数据。

尽管都从chatGPT获得了数据，BELLE和alpaca对于知识的理解没有baize表现得好。
而且可以看到，随着指令微调数据的增多，BELLE-2M的效果下降得更厉害，这可能是由于alpaca和BELLE都是self-instruct早期的工作，他们是第一批提出了self-instruct这个概念的工作，但并没有对生成数据的质量进行管理，所以导致的效果下降。



\input{tables/table_overall_mrr}

\input{tables/table_llm_rank}

\textbf{Top-tier LLMs have not achieved the level of average practitioners in majority of fields}
我们可以看到，尽管是用指令的方式进行作答，GPT-4在所有任务上都取得了最好的效果。
GPT-4同时展现了0-shot和few-shot learning的能力，并且展现出了极强的多语言能力。
但即便如此，我们在表~\ref{tab:llm-rank}中发现，GPT-4在任何一个领域内依然没有达到领域从业者的平均水平。
这表明语言模型在对于世界的基础知识的学习上依然有着非常巨大的空间。

\textbf{Most LLMs are incapable of performing stably few-shot learning from demonstrations}
我们发现，不是所有的模型都能通过学习更多的样本得到更好的结果。
甚至许多模型会随着学习样例的增多而带来更差的表现。

而GPT-4能较为稳定地从3-shot中提升表现。
我们认为这可能是GPT-4学习到了很多的领域知识，促使他能够有效地理解学习样本中的特征，从而提升表现。
而大多数地语言模型本身便没有对领域知识有很好地理解，强行拟合demonstration反而会带来更差的表现。


\textbf{More LLMs' parameters don't guarantee better performance}
有很多论文只提出了\textit{模型参数量越大，模型效果会越好}这个观点。
这个观点对于比较存在数量级上差距的模型成立，比如146B参数量的bloomz比560m参数量的bloomz要好很多。
但除此之外，我们发现这观点并不成立，比如我们发现Bloomz-3b在大多数任务上的效果都要比Bloomz-7b1要好。
而pythia-1.4b的效果在很多任务上也比其他参数量更大的pythia要好。

我们认为这可能是由于这些模型使用的是相同的数据进行预训练以及指令微调的。
而这些开源的模型所使用的数据量并没有非常庞大，所以小参数量的模型拟合的效果更好。


\textbf{Compare to complicated tasks, lack of corpus has a greater impact on reducing model performance}
大多数研究都认为逻辑推理、数学计算对于语言模型而言是最复杂的任务。
表现为语言模型在这些任务上难以取得很好的表现。

我们的实验表明，相较于工科这种需要公式推理的学科，所有语言模型在诸如管理学、艺术学上的效果可能要更差。
我们认为这可能是由于大多数的模型并没有收集过这些学科上的语料。
所以，尽管有研究指出模型在未见过的任务上具有涌现能力，我们认为在缺少语料的领域，语言模型的表现甚至还不如复杂的任务。

\textbf{LMs enhance domain capabilities at the expense of generic capabilities}

我们测试了两个医学领域的模型，分别是从doctorglm和baize-healthcare。
doctorglm是从chatglm-6b上使用了医学领域数据进行指令微调得到的。
baize-healthcare是从llama-7b上使用了医学领域数据进行指令微调得到的。

我们可以看到，相较于原来的模型而言，领域模型得到了更低的mrr值。
但他们各自在医学领域中都取得了极高的分数。
因此我们可以认为，对于小模型而言，无论是只使用领域数据，还是将领域数据和通用数据混合使用，想要提升小参数量模型对于领域文本的理解能力，势必会牺牲对于通用文本的理解能力。

% \begin{figure}
%     \centering
%     \resizebox{\textwidth}{!}{\includegraphics{llm_performance_easy.png}}
%     \resizebox{\textwidth}{!}{\includegraphics{llm_performance_hard.png}}
%     \caption{Performance of LMs more than 100B parameters}
%     \label{fig:my_label}
% \end{figure}




==> old_version/05Analysis.0.tex <==

\subsection{我们该评估什么}
我们认为语言模型的能力可以分为两种，并且都需要得到有效地评估。
一种是编码世界既有知识的能力，另一种是将已有知识解码并用于服务人类的能力。
针对前者能力地评估更注重在知识性上，针对后者地评估更注重在功能上。

近来有太多的工作都聚焦在大模型的功能性评估上，而我们认为知识性评估和功能性评估同等重要。
后者是AI作为人类工具的天然需求，而前者则是对于模型安全性的重要保障。
一个没有知识只有功能的模型，会是一个为了拟合目标而会进行随意推断的模型。
这样的模型本身就具有不可控性，在OOD任务上泛化之后，将会更加危险。

在大模型时代，知识性评估和功能性评估都需要各行各业的人们进行合力。
任何一个单一的机构都无法全面整合人类的所有知识。
任何一个单一的国家也难以构建适用于所有国际的评估标准。
因此，对于大模型的评估需要针对各种语言、各种领域知识、各种功能进行分门别类的评估。
这也会是我们在未来工作里会考虑的重点。

\subsection{构建Benchmark的目标}
我们认为Benchmark不应该成为各个模型发展的目标，而应该适应各个模型的特性，从而可以真实地反应模型的能力。
最近有些构建benchmark的工作，在评估的过程中为所有的模型提供统一的instruction，并设置统一的答案抽取模板。
我们认为这并不是一个公平的评估方法。
首先，模型对于prompt非常敏感，而这种敏感性可以在部署模型时被开发者用自己设置的prompt模板所掩盖。
而设置统一的instruction，则会导致拟合这些instruction拟合得好的模型表现出更好的效果。
其次，并不是所有的模型都有能力都具有回答选择题的能力。
因为在真实的下游应用中，回答选择题并不是个非常必要的能力，但这又是一个用来自动化评估生成模型非常重要的方式。
导致选择题回答得越好得模型，必然在benchmark上得到越好的结果。

我们在实验中为中英两种语言提供了总共十种不同的instruction模板，从而可以更好地去拟合每个模型所适合的prompt。
我们还使用了生成概率去计算模型选择了哪个选项，从而可以对各种能力不同的模型进行有效地评估。
这些设计极大地增加了我们的实验开销，但也能保证我们的实验结果更能够展示模型的真实能力，从而给出更加有效地分析。


==> old_version/05Analysis.1.tex <==
\subsection{The Classification of Evaluation}
We believe language models have two different capabilities, both of which require \red{effective evaluation}.
One is to encode the existing knowledge of the world, and the other is to decode the knowledge into serving humanity. 
Thus, the evaluations are divided into knowledgeable evaluation and functional evaluation.


Recently, many studies have focused on the functional evaluation of LLMs. 
However, we argue that both knowledgeable and functional evaluations are equally important. 
The latter is a natural requirement for AI as a tool for humanity, while the former is a crucial safeguard for AI security.
A model with functionality but no knowledge would be prone to arbitrary inference in the pursuit of fitting goals.
Such a model would inherently be uncontrollable and could become even more dangerous when generalized to out-of-distribution (OOD) tasks.

In the era of LLM, both knowledgeable and functional evaluations require the collaborative efforts of people from all walks of life. 
Benchmarks need to build a evaluation standard for knowledge in all specific domain, and for knowledge in all language. 
Xiezhi is available in two languages and covers more than 500 different domains of knowledge, but this is not enough for a holistic evaluation towards all human knowledge.
One of our future work priorities is to propose a broader and more detailed knowledge classification system from various industries and countries, and to integrate the knowledge from all walks of life for better evaluation.

\subsection{The Purpose of Benchmark}
We believe that benchmarks should not become the ultimate goal of model development. 
Instead, they should adapt to the characteristics of each model so as to fairly and accurately reflect their capabilities. 
Some recent benchmark construction efforts involve providing uniform instructions for all models during the evaluation process and setting up a uniform answer extraction template. 

We argue these works do not propose a fair evaluation method.
Firstly, models are highly sensitive to prompts, and this sensitivity can be compensated by developers using custom prompt templates when deploying. 
Implementing a uniform instruction may result in models that fit this instruction well, performing better. 
Secondly, not all models possess the ability to answer multiple-choice questions. 
Although answering multiple-choice questions is not a crucial ability in real-world downstream applications, it is an essential method for automating the evaluation of generative models. 
Consequently, models that perform well in multiple-choice tasks will inevitably achieve better results in benchmarks.

In our experiments, we provided a total of ten different instructions for both Chinese and English to better reveal the true ability of each model.
We also utilized generation probabilities to rank each option, allowing for effective evaluation of models with varying capabilities. 
Although these designs substantially increased the cost of our experiments, they also ensured that our results more accurately displayed the true abilities of the models for providing a more effective analysis.




==> old_version/05Analysis.2.tex <==

\textbf{LM有哪些能力需要评估}

我们总结，LM的能力具体体现在三个不同的方面。
第一个能力是LM对于知识的理解，这包括了对于符号语言的记忆、推理、总结。
目前大多数的工作是通过预训练来增强LM对于知识的理解。
第二个能力是LLM对于指令的理解和执行，这是语言模型作为人造工具的重要价值。
大多数的工作是通过对LM进行指令微调使LM得到的这个能力。
目前对于LM功能性的评估主要还是依靠人工校验。
第三个是与人类价值观的对齐，这是语言模型能够成为AGI的重要保证。
虽然许多公司，如OpenAI、Claude为Alignment提出了许多的技术路线。
但因为这个能力不直接提高模型在下游应用上的效果，所以很多工作没有将他们的模型与人类价值观对齐。


在本文写作时，有了许多评估工作提出，但我们认为LLM的发展需要更大量和更多种类的benchmark。
目前在功能性评估和价值观评估这两块并没有很多的benchmark。
而Xiezhi的目标是为全人类的知识建立一个合理的分类体系，并提出评估标准。
但Xiezhi目前只提供中文和英文的benchmark，在不同民族文化以及不同行业的深层知识的收集上也有所欠缺。
獬豸在未来改进的一个重要方向是收集来着不同民族不同行业的深度知识，并提出更多语言的benchmark。
同时，我们也呼吁学术界和工业界对全人类的知识和价值观进行总结，为LLM的发展提出更多有效、全面、超前的benchmark。


\textbf{LLM需要怎样的评估}


现在的语言模型基本上都是生成式的模型。
对于这类模型的评估天然具有挑战。
目前大多数的评估工作都使用选择题去评估生成模型对于知识的理解，使用一些抽取方法来得到模型的选项。

我们认为这并不是一个很好的评估方式。
这种评估方式需要模型具备回答选择题的能力，但回答选择题在真实的应用中并不经常出现。
对于能力有限的小模型，或者是没有经过选择题数据微调的模型，使用这类评估方法并不能有效地为模型提供评估指标。

我们在本文中提出使用生成概率的方式评估模型。
生成概率相较于直接让模型回答问题而言，增大了计算开销，但得到了更加准确有效的评估。
这是我们对于更好的评估方法的一种探索。
未来我们会考虑更加多种多样的评估方法。

==> tables/domain_experiments_table/table_agr.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.130 & 0.137 & 0.132 & 0.123 & 0.110 & 0.117 & 0.143 & 0.146 & 0.146 & 0.116 & 0.114 & 0.164 & 0.120 & 0.112 & 0.141 \\
bigscience/bloomz-1b1 &            0.145 & 0.118 & 0.119 & 0.111 & 0.113 & 0.113 & 0.137 & 0.139 & 0.153 & 0.110 & 0.120 & 0.152 & 0.111 & 0.117 & 0.132 \\
bigscience/bloomz-1b7 &            0.155 & 0.124 & 0.160 & 0.121 & 0.138 & 0.149 & 0.157 & 0.222 & 0.186 & 0.107 & 0.123 & 0.218 & 0.114 & 0.130 & 0.183 \\
bigscience/bloomz-3b &            0.187 & 0.182 & 0.191 & 0.231 & 0.193 & 0.159 & 0.169 & 0.205 & 0.218 & 0.168 & 0.162 & 0.140 & 0.200 & 0.178 & 0.150 \\
bigscience/bloomz-7b1-mt &            0.156 & 0.192 & 0.182 & 0.192 & 0.135 & 0.196 & 0.153 & 0.150 & 0.179 & 0.256 & 0.188 & 0.233 & 0.224 & 0.161 & 0.214 \\
bigscience/bloomz-7b1 &            0.165 & 0.156 & 0.156 & 0.191 & 0.133 & 0.213 & 0.169 & 0.193 & 0.196 & 0.238 & 0.192 & 0.204 & 0.215 & 0.146 & 0.211 \\
bigscience/bloomz-7b1-p3 &            0.174 & 0.213 & 0.161 & 0.117 & 0.116 & 0.179 & 0.188 & 0.178 & 0.186 & 0.176 & 0.152 & 0.187 & 0.138 & 0.124 & 0.180 \\
bigscience/bloomz &            0.129 & 0.160 & 0.190 & 0.036 & 0.037 & 0.029 & 0.114 & 0.153 & 0.256 & 0.104 & 0.157 & 0.051 & 0.066 & 0.090 & 0.039 \\
bigscience/bloomz-mt &            0.205 & 0.147 & 0.194 & 0.300 & 0.203 & 0.283 & 0.202 & 0.115 & 0.142 & 0.439 & 0.308 & 0.252 & 0.366 & 0.253 & 0.269 \\
bigscience/bloomz-p3 &            0.061 & 0.097 & 0.079 & 0.074 & 0.093 & 0.068 & 0.047 & 0.050 & 0.110 & 0.209 & 0.176 & 0.023 & 0.142 & 0.135 & 0.064 \\
\hline
decapoda-research/llama-7b-hf &            0.170 & 0.169 & 0.147 & 0.137 & 0.149 & 0.132 & 0.143 & 0.157 & 0.161 & 0.141 & 0.159 & 0.187 & 0.139 & 0.154 & 0.158 \\
decapoda-research/llama-13b-hf &            0.136 & 0.235 & 0.236 & 0.181 & 0.235 & 0.205 & 0.189 & 0.204 & 0.297 & 0.183 & 0.179 & 0.231 & 0.182 & 0.208 & 0.215 \\
decapoda-research/llama-30b-hf &            0.122 & 0.254 & 0.241 & 0.100 & 0.210 & 0.164 & 0.199 & 0.197 & 0.148 & 0.065 & 0.223 & 0.132 & 0.089 & 0.214 & 0.154 \\
decapoda-research/llama-65b-hf &            0.184 & 0.180 & 0.078 & 0.196 & 0.263 & 0.216 & 0.124 & 0.128 & 0.166 & 0.069 & 0.177 & 0.124 & 0.136 & 0.222 & 0.172 \\
\hline
project-baize/baize-lora-7B &            0.246 & 0.170 & 0.152 & 0.192 & 0.258 & 0.192 & 0.183 & 0.170 & 0.271 & 0.192 & 0.175 & 0.202 & 0.192 & 0.217 & 0.197 \\
project-baize/baize-healthcare-lora-7B &            0.176 & 0.154 & 0.153 & 0.201 & 0.277 & 0.188 & 0.228 & 0.145 & 0.220 & 0.139 & 0.206 & 0.214 & 0.162 & 0.241 & 0.201 \\
project-baize/baize-lora-13B &            0.160 & 0.197 & 0.218 & 0.194 & 0.180 & 0.226 & 0.189 & 0.194 & 0.271 & 0.189 & 0.139 & 0.251 & 0.192 & 0.160 & 0.238 \\
project-baize/baize-lora-30B &            0.149 & 0.318 & 0.162 & 0.195 & 0.200 & 0.053 & 0.065 & 0.265 & 0.183 & 0.039 & 0.100 & 0.108 & 0.125 & 0.155 & 0.105 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.176 & 0.127 & 0.166 & 0.204 & 0.142 & 0.095 & 0.173 & 0.162 & 0.194 & 0.229 & 0.137 & 0.111 & 0.216 & 0.140 & 0.103 \\
BelleGroup/BELLE-7B-0.6M &            0.188 & 0.150 & 0.223 & 0.145 & 0.160 & 0.146 & 0.207 & 0.204 & 0.241 & 0.121 & 0.159 & 0.121 & 0.133 & 0.160 & 0.134 \\
BelleGroup/BELLE-7B-1M &            0.205 & 0.171 & 0.184 & 0.185 & 0.125 & 0.104 & 0.210 & 0.194 & 0.274 & 0.144 & 0.110 & 0.101 & 0.165 & 0.118 & 0.102 \\
BelleGroup/BELLE-7B-2M &            0.149 & 0.186 & 0.138 & 0.136 & 0.086 & 0.151 & 0.180 & 0.166 & 0.169 & 0.075 & 0.067 & 0.091 & 0.122 & 0.077 & 0.138 \\
\hline
THUDM/chatglm-6b &            0.071 & 0.073 & 0.120 & 0.069 & 0.101 & 0.156 & 0.096 & 0.080 & 0.102 & 0.067 & 0.075 & 0.083 & 0.068 & 0.094 & 0.122 \\
THUDM/doctorglm-6b &            0.034 & 0.048 & 0.051 & 0.070 & 0.050 & 0.051 & 0.026 & 0.036 & 0.035 & 0.037 & 0.031 & 0.033 & 0.057 & 0.041 & 0.043 \\
\hline
fnlp/moss-moon-003-base &            0.122 & 0.041 & 0.049 & 0.109 & 0.061 & 0.058 & 0.101 & 0.030 & 0.049 & 0.115 & 0.038 & 0.046 & 0.112 & 0.050 & 0.053 \\
fnlp/moss-moon-003-sft &            0.072 & 0.056 & 0.053 & 0.057 & 0.061 & 0.052 & 0.034 & 0.064 & 0.051 & 0.052 & 0.091 & 0.067 & 0.054 & 0.076 & 0.059 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.171 & 0.204 & 0.184 & 0.191 & 0.225 & 0.192 & 0.137 & 0.188 & 0.219 & 0.172 & 0.186 & 0.192 & 0.182 & 0.206 & 0.192 \\
lmsys/vicuna-13b-delta-v1.1 &            0.175 & 0.186 & 0.200 & 0.050 & 0.107 & 0.142 & 0.155 & 0.175 & 0.135 & 0.172 & 0.177 & 0.219 & 0.112 & 0.142 & 0.178 \\
tloen/alpaca-lora-7b &            0.124 & 0.140 & 0.153 & 0.151 & 0.168 & 0.113 & 0.189 & 0.141 & 0.118 & 0.192 & 0.207 & 0.152 & 0.171 & 0.187 & 0.132 \\
\hline
EleutherAI/pythia-1.4b &            0.130 & 0.130 & 0.157 & 0.164 & 0.126 & 0.147 & 0.070 & 0.098 & 0.094 & 0.225 & 0.134 & 0.150 & 0.193 & 0.130 & 0.148 \\
EleutherAI/pythia-2.8b &            0.138 & 0.151 & 0.169 & 0.063 & 0.101 & 0.139 & 0.100 & 0.143 & 0.142 & 0.089 & 0.089 & 0.076 & 0.076 & 0.096 & 0.108 \\
EleutherAI/pythia-6.9b &            0.091 & 0.101 & 0.102 & 0.056 & 0.077 & 0.105 & 0.105 & 0.064 & 0.057 & 0.050 & 0.107 & 0.105 & 0.053 & 0.091 & 0.105 \\
EleutherAI/pythia-12b &            0.133 & 0.121 & 0.115 & 0.074 & 0.090 & 0.078 & 0.114 & 0.043 & 0.176 & 0.067 & 0.106 & 0.120 & 0.071 & 0.098 & 0.099 \\
\hline
EleutherAI/gpt-neox-20b &            0.147 & 0.114 & 0.095 & 0.067 & 0.079 & 0.109 & 0.156 & 0.098 & 0.097 & 0.042 & 0.069 & 0.122 & 0.060 & 0.074 & 0.116 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.074 & 0.047 & 0.153 & 0.081 & 0.039 & 0.040 & 0.110 & 0.073 & 0.116 & 0.080 & 0.059 & 0.060 & 0.080 & 0.049 & 0.050 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.114 & 0.044 & 0.500 & 0.111 & 0.061 & 0.116 & 0.065 & 0.069 & 0.040 & 0.120 & 0.068 & 0.094 & 0.115 & 0.064 & 0.105 \\
\hline
databricks/dolly-v2-3b &            0.088 & 0.095 & 0.098 & 0.099 & 0.066 & 0.082 & 0.081 & 0.088 & 0.080 & 0.078 & 0.099 & 0.059 & 0.089 & 0.082 & 0.077 \\
databricks/dolly-v2-7b &            0.096 & 0.079 & 0.091 & 0.063 & 0.054 & 0.079 & 0.093 & 0.097 & 0.100 & 0.082 & 0.095 & 0.102 & 0.072 & 0.074 & 0.090 \\
databricks/dolly-v2-12b &            0.109 & 0.121 & 0.088 & 0.083 & 0.086 & 0.093 & 0.079 & 0.132 & 0.116 & 0.121 & 0.109 & 0.117 & 0.102 & 0.097 & 0.105 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.109 & 0.108 & 0.116 & 0.070 & 0.095 & 0.084 & 0.098 & 0.122 & 0.048 & 0.076 & 0.096 & 0.100 & 0.073 & 0.096 & 0.092 \\
stabilityai/stablelm-tuned-alpha-7b &            0.089 & 0.109 & 0.095 & 0.077 & 0.076 & 0.105 & 0.107 & 0.122 & 0.081 & 0.091 & 0.116 & 0.081 & 0.084 & 0.096 & 0.093 \\
\hline
tiiuae/falcon-7b &            0.050 & 0.053 & 0.043 & 0.123 & 0.086 & 0.137 & 0.093 & 0.128 & 0.188 & 0.129 & 0.150 & 0.272 & 0.126 & 0.120 & 0.209 \\
tiiuae/falcon-7b-instruct &            0.058 & 0.092 & 0.095 & 0.133 & 0.206 & 0.290 & 0.119 & 0.163 & 0.206 & 0.165 & 0.168 & 0.265 & 0.151 & 0.185 & 0.276 \\
tiiuae/falcon-40b &            0.082 & 0.066 & 0.048 & 0.035 & 0.053 & 0.082 & 0.033 & 0.032 & 0.036 & 0.136 & 0.179 & 0.125 & 0.083 & 0.107 & 0.101 \\
tiiuae/falcon-40b-instruct &            0.156 & 0.111 & 0.081 & 0.074 & 0.085 & 0.062 & 0.205 & 0.056 & 0.138 & 0.182 & 0.190 & 0.082 & 0.128 & 0.138 & 0.072 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.185 & 0.316 & 0.376 & 0.158 & 0.337 & 0.423 & 0.164 & 0.339 & 0.423 & 0.464 & 0.587 & 0.637 & 0.311 & 0.462 & 0.530 \\
gpt4 &            0.435 & 0.476 & 0.543 & 0.444 & 0.481 & 0.547 & 0.567 & 0.606 & 0.682 & 0.587 & 0.619 & 0.696 & 0.515 & 0.550 & 0.622 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.141 & 0.147 & 0.158 & 0.133 & 0.139 & 0.146 & 0.142 & 0.147 & 0.168 & 0.151 & 0.157 & 0.161 & 0.142 & 0.147 & 0.155\\
Performance-Average & 0.063 & 0.080 & 0.098 & 0.075 & 0.086 & 0.094 & 0.082 & 0.093 & 0.109 & 0.108 & 0.108 & 0.125 & 0.084 & 0.092 & 0.106\\
\bottomrule
\end{tabular}
}
\caption{The performance of Agronomy.}
\end{table}

==> tables/domain_experiments_table/table_art.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.164 & 0.156 & 0.123 & 0.167 & 0.162 & 0.194 & 0.150 & 0.169 & 0.175 & 0.103 & 0.086 & 0.201 & 0.133 & 0.122 & 0.198 \\
bigscience/bloomz-1b1 &            0.175 & 0.113 & 0.155 & 0.181 & 0.181 & 0.182 & 0.119 & 0.149 & 0.162 & 0.103 & 0.098 & 0.169 & 0.140 & 0.137 & 0.175 \\
bigscience/bloomz-1b7 &            0.181 & 0.171 & 0.185 & 0.195 & 0.211 & 0.203 & 0.165 & 0.243 & 0.211 & 0.146 & 0.140 & 0.212 & 0.169 & 0.174 & 0.208 \\
bigscience/bloomz-3b &            0.205 & 0.165 & 0.199 & 0.280 & 0.203 & 0.223 & 0.165 & 0.194 & 0.227 & 0.169 & 0.141 & 0.196 & 0.221 & 0.171 & 0.209 \\
bigscience/bloomz-7b1-mt &            0.188 & 0.183 & 0.143 & 0.182 & 0.243 & 0.287 & 0.150 & 0.174 & 0.193 & 0.156 & 0.192 & 0.216 & 0.168 & 0.216 & 0.250 \\
bigscience/bloomz-7b1 &            0.172 & 0.174 & 0.180 & 0.228 & 0.212 & 0.260 & 0.160 & 0.237 & 0.208 & 0.180 & 0.136 & 0.237 & 0.202 & 0.196 & 0.255 \\
bigscience/bloomz-7b1-p3 &            0.220 & 0.222 & 0.213 & 0.195 & 0.182 & 0.191 & 0.228 & 0.193 & 0.224 & 0.149 & 0.117 & 0.135 & 0.175 & 0.168 & 0.179 \\
bigscience/bloomz &            0.188 & 0.065 & 0.391 & 0.061 & 0.060 & 0.037 & 0.038 & 0.085 & 0.117 & 0.054 & 0.038 & 0.030 & 0.057 & 0.048 & 0.033 \\
bigscience/bloomz-mt &            0.291 & 0.094 & 0.170 & 0.224 & 0.178 & 0.296 & 0.136 & 0.315 & 0.158 & 0.499 & 0.259 & 0.164 & 0.377 & 0.223 & 0.222 \\
bigscience/bloomz-p3 &            0.234 & 0.093 & 0.170 & 0.036 & 0.039 & 0.037 & 0.094 & 0.071 & 0.027 & 0.125 & 0.098 & 0.083 & 0.086 & 0.072 & 0.046 \\
\hline
decapoda-research/llama-7b-hf &            0.144 & 0.129 & 0.102 & 0.133 & 0.105 & 0.075 & 0.113 & 0.170 & 0.063 & 0.183 & 0.141 & 0.151 & 0.154 & 0.120 & 0.108 \\
decapoda-research/llama-13b-hf &            0.160 & 0.347 & 0.236 & 0.180 & 0.159 & 0.192 & 0.340 & 0.324 & 0.376 & 0.207 & 0.160 & 0.258 & 0.193 & 0.160 & 0.217 \\
decapoda-research/llama-30b-hf &            0.124 & 0.166 & 0.082 & 0.055 & 0.235 & 0.175 & 0.071 & 0.099 & 0.120 & 0.128 & 0.241 & 0.267 & 0.085 & 0.238 & 0.213 \\
decapoda-research/llama-65b-hf &            0.108 & 0.166 & 0.029 & 0.074 & 0.117 & 0.096 & 0.065 & 0.044 & 0.029 & 0.047 & 0.070 & 0.044 & 0.061 & 0.093 & 0.067 \\
\hline
project-baize/baize-lora-7B &            0.175 & 0.105 & 0.115 & 0.173 & 0.151 & 0.154 & 0.180 & 0.156 & 0.209 & 0.221 & 0.251 & 0.202 & 0.196 & 0.199 & 0.178 \\
project-baize/baize-healthcare-lora-7B &            0.169 & 0.116 & 0.113 & 0.278 & 0.222 & 0.134 & 0.385 & 0.077 & 0.033 & 0.533 & 0.526 & 0.260 & 0.417 & 0.357 & 0.197 \\
project-baize/baize-lora-13B &            0.178 & 0.316 & 0.292 & 0.203 & 0.153 & 0.248 & 0.185 & 0.255 & 0.309 & 0.257 & 0.200 & 0.241 & 0.229 & 0.176 & 0.245 \\
project-baize/baize-lora-30B &            0.115 & 0.159 & 0.136 & 0.238 & 0.234 & 0.067 & 0.119 & 0.337 & 0.204 & 0.108 & 0.429 & 0.345 & 0.173 & 0.317 & 0.305 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.167 & 0.143 & 0.173 & 0.144 & 0.118 & 0.109 & 0.170 & 0.202 & 0.149 & 0.339 & 0.132 & 0.205 & 0.238 & 0.125 & 0.155 \\
BelleGroup/BELLE-7B-0.6M &            0.227 & 0.195 & 0.246 & 0.236 & 0.153 & 0.140 & 0.198 & 0.207 & 0.205 & 0.128 & 0.129 & 0.132 & 0.184 & 0.141 & 0.136 \\
BelleGroup/BELLE-7B-1M &            0.179 & 0.127 & 0.122 & 0.237 & 0.184 & 0.178 & 0.149 & 0.179 & 0.168 & 0.136 & 0.117 & 0.131 & 0.188 & 0.152 & 0.155 \\
BelleGroup/BELLE-7B-2M &            0.229 & 0.191 & 0.160 & 0.101 & 0.126 & 0.175 & 0.144 & 0.216 & 0.201 & 0.073 & 0.156 & 0.111 & 0.094 & 0.141 & 0.161 \\
\hline
THUDM/chatglm-6b &            0.091 & 0.067 & 0.141 & 0.160 & 0.151 & 0.056 & 0.131 & 0.098 & 0.176 & 0.049 & 0.129 & 0.111 & 0.131 & 0.144 & 0.079 \\
THUDM/doctorglm-6b &            0.026 & 0.190 & 0.039 & 0.034 & 0.032 & 0.022 & 0.032 & 0.028 & 0.034 & 0.070 & 0.038 & 0.042 & 0.054 & 0.035 & 0.033 \\
\hline
fnlp/moss-moon-003-base &            0.110 & 0.054 & 0.086 & 0.257 & 0.070 & 0.089 & 0.117 & 0.056 & 0.087 & 0.188 & 0.043 & 0.058 & 0.224 & 0.057 & 0.076 \\
fnlp/moss-moon-003-sft &            0.062 & 0.077 & 0.125 & 0.098 & 0.042 & 0.034 & 0.028 & 0.115 & 0.067 & 0.063 & 0.177 & 0.117 & 0.081 & 0.107 & 0.074 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.168 & 0.189 & 0.285 & 0.223 & 0.283 & 0.263 & 0.238 & 0.325 & 0.221 & 0.170 & 0.173 & 0.097 & 0.199 & 0.234 & 0.188 \\
lmsys/vicuna-13b-delta-v1.1 &            0.184 & 0.125 & 0.237 & 0.106 & 0.138 & 0.169 & 0.274 & 0.215 & 0.256 & 0.120 & 0.063 & 0.287 & 0.113 & 0.102 & 0.224 \\
tloen/alpaca-lora-7b &            0.159 & 0.120 & 0.113 & 0.308 & 0.230 & 0.218 & 0.195 & 0.049 & 0.054 & 0.135 & 0.095 & 0.093 & 0.227 & 0.167 & 0.160 \\
\hline
EleutherAI/pythia-1.4b &            0.101 & 0.080 & 0.099 & 0.178 & 0.049 & 0.067 & 0.080 & 0.055 & 0.098 & 0.047 & 0.116 & 0.060 & 0.117 & 0.080 & 0.064 \\
EleutherAI/pythia-2.8b &            0.100 & 0.133 & 0.180 & 0.082 & 0.033 & 0.029 & 0.104 & 0.141 & 0.141 & 0.073 & 0.105 & 0.051 & 0.077 & 0.061 & 0.039 \\
EleutherAI/pythia-6.9b &            0.077 & 0.072 & 0.075 & 0.049 & 0.091 & 0.091 & 0.116 & 0.180 & 0.187 & 0.122 & 0.086 & 0.053 & 0.084 & 0.089 & 0.072 \\
EleutherAI/pythia-12b &            0.097 & 0.103 & 0.101 & 0.110 & 0.065 & 0.071 & 0.096 & 0.053 & 0.160 & 0.068 & 0.162 & 0.150 & 0.089 & 0.112 & 0.109 \\
\hline
EleutherAI/gpt-neox-20b &            0.147 & 0.077 & 0.163 & 0.124 & 0.074 & 0.036 & 0.047 & 0.069 & 0.079 & 0.041 & 0.094 & 0.237 & 0.098 & 0.084 & 0.136 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.054 & 0.039 & 0.026 & 0.033 & 0.028 & 0.037 & 0.050 & 0.098 & 0.096 & 0.122 & 0.028 & 0.038 & 0.076 & 0.028 & 0.037 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.110 & 0.033 & -1.000 & 0.285 & 0.034 & 0.082 & 0.115 & 0.052 & 0.161 & 0.154 & 0.062 & 0.074 & 0.221 & 0.047 & 0.078 \\
\hline
databricks/dolly-v2-3b &            0.078 & 0.076 & 0.042 & 0.039 & 0.030 & 0.082 & 0.053 & 0.048 & 0.036 & 0.142 & 0.046 & 0.065 & 0.087 & 0.037 & 0.078 \\
databricks/dolly-v2-7b &            0.122 & 0.105 & 0.138 & 0.120 & 0.062 & 0.106 & 0.092 & 0.093 & 0.114 & 0.139 & 0.130 & 0.125 & 0.129 & 0.094 & 0.115 \\
databricks/dolly-v2-12b &            0.051 & 0.100 & 0.106 & 0.071 & 0.081 & 0.082 & 0.086 & 0.124 & 0.091 & 0.034 & 0.082 & 0.097 & 0.054 & 0.082 & 0.089 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.098 & 0.092 & 0.091 & 0.066 & 0.129 & 0.078 & 0.088 & 0.119 & 0.071 & 0.039 & 0.054 & 0.054 & 0.053 & 0.094 & 0.066 \\
stabilityai/stablelm-tuned-alpha-7b &            0.059 & 0.097 & 0.115 & 0.125 & 0.053 & 0.096 & 0.097 & 0.125 & 0.121 & 0.098 & 0.072 & 0.067 & 0.112 & 0.062 & 0.082 \\
\hline
tiiuae/falcon-7b &            0.080 & 0.053 & 0.046 & 0.089 & 0.125 & 0.237 & 0.200 & 0.055 & 0.109 & 0.161 & 0.138 & 0.092 & 0.128 & 0.132 & 0.158 \\
tiiuae/falcon-7b-instruct &            0.069 & 0.130 & 0.060 & 0.182 & 0.077 & 0.273 & 0.041 & 0.160 & 0.142 & 0.123 & 0.173 & 0.167 & 0.150 & 0.129 & 0.215 \\
tiiuae/falcon-40b &            0.122 & 0.079 & 0.084 & 0.088 & 0.276 & 0.057 & 0.072 & 0.043 & 0.121 & 0.221 & 0.028 & 0.039 & 0.162 & 0.139 & 0.047 \\
tiiuae/falcon-40b-instruct &            0.097 & 0.093 & 0.068 & 0.071 & 0.361 & 0.093 & 0.045 & 0.311 & 0.089 & 0.054 & 0.099 & 0.075 & 0.061 & 0.216 & 0.083 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.302 & 0.430 & 0.487 & 0.015 & 0.170 & 0.248 & 0.456 & 0.665 & 0.758 & 0.664 & 0.708 & 0.712 & 0.339 & 0.439 & 0.480 \\
gpt4 &            0.329 & 0.372 & 0.431 & 0.343 & 0.399 & 0.460 & 0.471 & 0.497 & 0.555 & 0.530 & 0.531 & 0.592 & 0.437 & 0.465 & 0.526 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.147 & 0.140 & 0.129 & 0.150 & 0.143 & 0.143 & 0.146 & 0.167 & 0.166 & 0.163 & 0.155 & 0.160 & 0.158 & 0.149 & 0.154\\
Performance-Average & 0.067 & 0.083 & 0.193 & 0.083 & 0.087 & 0.092 & 0.100 & 0.123 & 0.129 & 0.136 & 0.135 & 0.130 & 0.091 & 0.094 & 0.102\\
\bottomrule
\end{tabular}
}
\caption{The performance of Art Studies.}
\end{table}

==> tables/domain_experiments_table/table_eco.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.098 & 0.110 & 0.108 & 0.110 & 0.098 & 0.113 & 0.108 & 0.107 & 0.108 & 0.098 & 0.082 & 0.165 & 0.105 & 0.090 & 0.137 \\
bigscience/bloomz-1b1 &            0.114 & 0.091 & 0.077 & 0.151 & 0.110 & 0.100 & 0.093 & 0.100 & 0.079 & 0.140 & 0.125 & 0.136 & 0.146 & 0.117 & 0.117 \\
bigscience/bloomz-1b7 &            0.152 & 0.151 & 0.157 & 0.140 & 0.115 & 0.116 & 0.139 & 0.201 & 0.138 & 0.137 & 0.110 & 0.180 & 0.139 & 0.113 & 0.146 \\
bigscience/bloomz-3b &            0.168 & 0.115 & 0.119 & 0.212 & 0.131 & 0.146 & 0.134 & 0.152 & 0.126 & 0.147 & 0.137 & 0.129 & 0.182 & 0.134 & 0.138 \\
bigscience/bloomz-7b1-mt &            0.154 & 0.138 & 0.115 & 0.165 & 0.136 & 0.171 & 0.161 & 0.160 & 0.138 & 0.197 & 0.190 & 0.185 & 0.180 & 0.161 & 0.177 \\
bigscience/bloomz-7b1 &            0.155 & 0.149 & 0.129 & 0.172 & 0.128 & 0.162 & 0.160 & 0.188 & 0.152 & 0.203 & 0.189 & 0.191 & 0.186 & 0.144 & 0.169 \\
bigscience/bloomz-7b1-p3 &            0.164 & 0.180 & 0.140 & 0.142 & 0.125 & 0.153 & 0.182 & 0.149 & 0.144 & 0.132 & 0.180 & 0.151 & 0.138 & 0.139 & 0.152 \\
bigscience/bloomz &            0.200 & 0.076 & 0.303 & 0.051 & 0.061 & 0.049 & 0.177 & 0.046 & 0.286 & 0.060 & 0.062 & 0.053 & 0.055 & 0.061 & 0.051 \\
bigscience/bloomz-mt &            0.175 & 0.258 & 0.119 & 0.054 & 0.067 & 0.040 & 0.124 & 0.156 & 0.051 & 0.617 & 0.327 & 0.356 & 0.310 & 0.185 & 0.184 \\
bigscience/bloomz-p3 &            0.183 & 0.108 & 0.064 & 0.073 & 0.037 & 0.043 & 0.077 & 0.064 & 0.067 & 0.205 & 0.209 & 0.091 & 0.139 & 0.123 & 0.050 \\
\hline
decapoda-research/llama-7b-hf &            0.141 & 0.149 & 0.080 & 0.189 & 0.213 & 0.188 & 0.196 & 0.179 & 0.099 & 0.281 & 0.219 & 0.195 & 0.234 & 0.216 & 0.191 \\
decapoda-research/llama-13b-hf &            0.169 & 0.191 & 0.208 & 0.162 & 0.171 & 0.203 & 0.282 & 0.215 & 0.367 & 0.127 & 0.195 & 0.238 & 0.144 & 0.183 & 0.217 \\
decapoda-research/llama-30b-hf &            0.119 & 0.185 & 0.162 & 0.193 & 0.277 & 0.155 & 0.120 & 0.110 & 0.055 & 0.036 & 0.108 & 0.456 & 0.154 & 0.245 & 0.213 \\
decapoda-research/llama-65b-hf &            0.156 & 0.157 & 0.135 & 0.218 & 0.269 & 0.191 & 0.045 & 0.034 & 0.022 & 0.376 & 0.518 & 0.491 & 0.290 & 0.382 & 0.328 \\
\hline
project-baize/baize-lora-7B &            0.216 & 0.155 & 0.139 & 0.216 & 0.180 & 0.183 & 0.202 & 0.220 & 0.247 & 0.228 & 0.164 & 0.163 & 0.222 & 0.172 & 0.173 \\
project-baize/baize-healthcare-lora-7B &            0.169 & 0.157 & 0.139 & 0.146 & 0.170 & 0.232 & 0.319 & 0.087 & 0.043 & 0.143 & 0.371 & 0.473 & 0.144 & 0.270 & 0.333 \\
project-baize/baize-lora-13B &            0.188 & 0.190 & 0.229 & 0.154 & 0.174 & 0.205 & 0.215 & 0.165 & 0.156 & 0.165 & 0.174 & 0.258 & 0.159 & 0.174 & 0.232 \\
project-baize/baize-lora-30B &            0.093 & 0.163 & 0.146 & 0.097 & 0.180 & 0.200 & 0.050 & 0.233 & 0.145 & 0.051 & 0.177 & 0.172 & 0.079 & 0.179 & 0.174 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.172 & 0.124 & 0.120 & 0.279 & 0.126 & 0.146 & 0.168 & 0.159 & 0.239 & 0.140 & 0.106 & 0.118 & 0.208 & 0.116 & 0.132 \\
BelleGroup/BELLE-7B-0.6M &            0.143 & 0.121 & 0.158 & 0.187 & 0.156 & 0.218 & 0.158 & 0.167 & 0.133 & 0.192 & 0.178 & 0.232 & 0.190 & 0.167 & 0.225 \\
BelleGroup/BELLE-7B-1M &            0.159 & 0.133 & 0.115 & 0.256 & 0.126 & 0.175 & 0.154 & 0.157 & 0.270 & 0.254 & 0.188 & 0.209 & 0.255 & 0.157 & 0.192 \\
BelleGroup/BELLE-7B-2M &            0.120 & 0.127 & 0.103 & 0.202 & 0.115 & 0.207 & 0.146 & 0.167 & 0.135 & 0.181 & 0.184 & 0.176 & 0.196 & 0.149 & 0.199 \\
\hline
THUDM/chatglm-6b &            0.078 & 0.084 & 0.155 & 0.077 & 0.137 & 0.142 & 0.078 & 0.096 & 0.161 & 0.101 & 0.068 & 0.065 & 0.084 & 0.118 & 0.113 \\
THUDM/doctorglm-6b &            0.038 & 0.031 & 0.031 & 0.066 & 0.077 & 0.055 & 0.084 & 0.049 & 0.141 & 0.181 & 0.097 & 0.042 & 0.118 & 0.086 & 0.050 \\
\hline
fnlp/moss-moon-003-base &            0.090 & 0.058 & 0.063 & 0.071 & 0.067 & 0.074 & 0.128 & 0.043 & 0.039 & 0.129 & 0.042 & 0.040 & 0.100 & 0.055 & 0.059 \\
fnlp/moss-moon-003-sft &            0.071 & 0.061 & 0.081 & 0.059 & 0.062 & 0.066 & -1.000 & 0.118 & 0.101 & 0.081 & 0.044 & 0.046 & 0.070 & 0.053 & 0.056 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.173 & 0.137 & 0.124 & 0.229 & 0.252 & 0.247 & 0.238 & 0.159 & 0.157 & 0.198 & 0.166 & 0.149 & 0.214 & 0.209 & 0.197 \\
lmsys/vicuna-13b-delta-v1.1 &            0.162 & 0.128 & 0.123 & 0.144 & 0.169 & 0.128 & 0.224 & 0.224 & 0.292 & 0.185 & 0.174 & 0.155 & 0.164 & 0.171 & 0.141 \\
tloen/alpaca-lora-7b &            0.147 & 0.140 & 0.139 & 0.113 & 0.152 & 0.101 & 0.195 & 0.121 & 0.135 & 0.203 & 0.209 & 0.149 & 0.157 & 0.180 & 0.124 \\
\hline
EleutherAI/pythia-1.4b &            0.148 & 0.153 & 0.177 & 0.153 & 0.144 & 0.127 & 0.103 & 0.282 & 0.122 & 0.066 & 0.147 & 0.093 & 0.114 & 0.145 & 0.112 \\
EleutherAI/pythia-2.8b &            0.112 & 0.146 & 0.152 & 0.104 & 0.103 & 0.067 & 0.122 & 0.078 & 0.082 & 0.090 & 0.124 & 0.182 & 0.097 & 0.112 & 0.119 \\
EleutherAI/pythia-6.9b &            0.084 & 0.123 & 0.084 & 0.092 & 0.114 & 0.094 & 0.115 & 0.141 & 0.128 & 0.114 & 0.093 & 0.113 & 0.103 & 0.104 & 0.103 \\
EleutherAI/pythia-12b &            0.125 & 0.131 & 0.113 & 0.054 & 0.095 & 0.110 & 0.109 & -1.000 & 0.041 & 0.083 & 0.111 & 0.099 & 0.068 & 0.103 & 0.104 \\
\hline
EleutherAI/gpt-neox-20b &            0.180 & 0.140 & 0.147 & 0.076 & 0.106 & 0.142 & 0.239 & 0.108 & 0.082 & 0.071 & 0.087 & 0.193 & 0.075 & 0.098 & 0.164 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.070 & 0.033 & 0.048 & 0.103 & 0.070 & 0.077 & 0.124 & 0.056 & 0.108 & 0.070 & 0.071 & 0.060 & 0.087 & 0.071 & 0.068 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.140 & 0.130 & 0.053 & 0.087 & 0.058 & 0.123 & 0.064 & 0.101 & 0.075 & 0.110 & 0.048 & 0.070 & 0.098 & 0.053 & 0.097 \\
\hline
databricks/dolly-v2-3b &            0.153 & 0.120 & 0.088 & 0.047 & 0.081 & 0.065 & 0.107 & 0.112 & 0.105 & 0.070 & 0.048 & 0.043 & 0.059 & 0.064 & 0.059 \\
databricks/dolly-v2-7b &            0.100 & 0.086 & 0.087 & 0.107 & 0.067 & 0.091 & 0.144 & 0.124 & 0.113 & 0.163 & 0.099 & 0.108 & 0.135 & 0.083 & 0.100 \\
databricks/dolly-v2-12b &            0.083 & 0.088 & 0.097 & 0.079 & 0.092 & 0.060 & 0.095 & 0.111 & 0.082 & 0.080 & 0.128 & 0.132 & 0.080 & 0.110 & 0.097 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.106 & 0.108 & 0.098 & 0.064 & 0.080 & 0.080 & 0.107 & 0.127 & 0.106 & 0.085 & 0.086 & 0.091 & 0.074 & 0.083 & 0.085 \\
stabilityai/stablelm-tuned-alpha-7b &            0.100 & 0.126 & 0.112 & 0.090 & 0.086 & 0.088 & 0.121 & 0.169 & 0.142 & 0.131 & 0.108 & 0.147 & 0.110 & 0.097 & 0.117 \\
\hline
tiiuae/falcon-7b &            0.142 & 0.188 & 0.193 & 0.171 & 0.070 & 0.073 & 0.092 & 0.057 & 0.050 & 0.295 & 0.208 & 0.356 & 0.233 & 0.139 & 0.215 \\
tiiuae/falcon-7b-instruct &            0.123 & 0.121 & 0.137 & 0.244 & 0.285 & 0.163 & 0.128 & 0.082 & 0.027 & 0.178 & 0.176 & 0.124 & 0.214 & 0.236 & 0.146 \\
tiiuae/falcon-40b &            0.054 & 0.029 & 0.039 & 0.028 & 0.023 & 0.050 & 0.087 & 0.206 & 0.218 & 0.125 & 0.061 & 0.055 & 0.072 & 0.040 & 0.052 \\
tiiuae/falcon-40b-instruct &            0.059 & 0.040 & 0.031 & 0.083 & 0.069 & 0.063 & 0.272 & 0.292 & 0.066 & 0.089 & 0.073 & 0.154 & 0.086 & 0.071 & 0.104 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.149 & 0.277 & 0.337 & 0.135 & 0.258 & 0.316 & 0.188 & 0.351 & 0.428 & 0.170 & 0.306 & 0.370 & 0.153 & 0.282 & 0.343 \\
gpt4 &            0.362 & 0.395 & 0.450 & 0.366 & 0.400 & 0.456 & 0.442 & 0.505 & 0.588 & 0.471 & 0.528 & 0.613 & 0.419 & 0.464 & 0.534 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.137 & 0.134 & 0.132 & 0.136 & 0.134 & 0.137 & 0.128 & 0.126 & 0.144 & 0.163 & 0.159 & 0.180 & 0.150 & 0.147 & 0.155\\
Performance-Average & 0.053 & 0.063 & 0.076 & 0.071 & 0.075 & 0.078 & 0.182 & 0.186 & 0.107 & 0.106 & 0.105 & 0.127 & 0.073 & 0.082 & 0.090\\
\bottomrule
\end{tabular}
}
\caption{The performance of Economics.}
\end{table}

==> tables/domain_experiments_table/table_eng.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.135 & 0.122 & 0.146 & 0.127 & 0.140 & 0.142 & 0.136 & 0.141 & 0.144 & 0.162 & 0.153 & 0.176 & 0.145 & 0.147 & 0.159 \\
bigscience/bloomz-1b1 &            0.148 & 0.095 & 0.103 & 0.139 & 0.128 & 0.119 & 0.118 & 0.118 & 0.118 & 0.174 & 0.154 & 0.154 & 0.156 & 0.141 & 0.137 \\
bigscience/bloomz-1b7 &            0.191 & 0.152 & 0.173 & 0.137 & 0.139 & 0.155 & 0.166 & 0.218 & 0.188 & 0.166 & 0.162 & 0.211 & 0.152 & 0.150 & 0.183 \\
bigscience/bloomz-3b &            0.186 & 0.145 & 0.164 & 0.201 & 0.164 & 0.159 & 0.170 & 0.195 & 0.189 & 0.206 & 0.192 & 0.188 & 0.204 & 0.178 & 0.173 \\
bigscience/bloomz-7b1-mt &            0.170 & 0.175 & 0.175 & 0.225 & 0.185 & 0.215 & 0.167 & 0.162 & 0.173 & 0.281 & 0.258 & 0.294 & 0.253 & 0.221 & 0.255 \\
bigscience/bloomz-7b1 &            0.181 & 0.177 & 0.160 & 0.239 & 0.172 & 0.253 & 0.178 & 0.202 & 0.178 & 0.310 & 0.221 & 0.272 & 0.274 & 0.184 & 0.258 \\
bigscience/bloomz-7b1-p3 &            0.192 & 0.199 & 0.167 & 0.150 & 0.153 & 0.179 & 0.196 & 0.190 & 0.190 & 0.188 & 0.169 & 0.156 & 0.164 & 0.157 & 0.174 \\
bigscience/bloomz &            0.142 & 0.143 & 0.209 & 0.087 & 0.121 & 0.080 & 0.113 & 0.112 & 0.177 & 0.046 & 0.052 & 0.041 & 0.067 & 0.087 & 0.061 \\
bigscience/bloomz-mt &            0.259 & 0.241 & 0.255 & 0.375 & 0.283 & 0.314 & 0.206 & 0.159 & 0.123 & 0.398 & 0.202 & 0.190 & 0.387 & 0.243 & 0.253 \\
bigscience/bloomz-p3 &            0.108 & 0.072 & 0.096 & 0.224 & 0.183 & 0.115 & 0.100 & 0.109 & 0.175 & 0.194 & 0.146 & 0.058 & 0.210 & 0.166 & 0.106 \\
\hline
decapoda-research/llama-7b-hf &            0.175 & 0.163 & 0.126 & 0.178 & 0.172 & 0.174 & 0.154 & 0.157 & 0.153 & 0.196 & 0.177 & 0.174 & 0.187 & 0.174 & 0.174 \\
decapoda-research/llama-13b-hf &            0.127 & 0.253 & 0.257 & 0.180 & 0.209 & 0.263 & 0.198 & 0.215 & 0.320 & 0.216 & 0.269 & 0.261 & 0.198 & 0.240 & 0.262 \\
decapoda-research/llama-30b-hf &            0.172 & 0.239 & 0.221 & 0.128 & 0.288 & 0.224 & 0.136 & 0.194 & 0.152 & 0.096 & 0.230 & 0.281 & 0.116 & 0.267 & 0.244 \\
decapoda-research/llama-65b-hf &            0.158 & 0.123 & 0.125 & 0.136 & 0.157 & 0.196 & 0.142 & 0.086 & 0.095 & 0.125 & 0.186 & 0.177 & 0.131 & 0.171 & 0.187 \\
\hline
project-baize/baize-lora-7B &            0.230 & 0.156 & 0.128 & 0.187 & 0.206 & 0.234 & 0.186 & 0.198 & 0.221 & 0.217 & 0.199 & 0.235 & 0.203 & 0.202 & 0.235 \\
project-baize/baize-healthcare-lora-7B &            0.204 & 0.161 & 0.127 & 0.173 & 0.135 & 0.138 & 0.309 & 0.143 & 0.145 & 0.199 & 0.278 & 0.205 & 0.189 & 0.212 & 0.172 \\
project-baize/baize-lora-13B &            0.142 & 0.237 & 0.283 & 0.171 & 0.210 & 0.270 & 0.218 & 0.239 & 0.236 & 0.166 & 0.189 & 0.276 & 0.169 & 0.199 & 0.273 \\
project-baize/baize-lora-30B &            0.117 & 0.267 & 0.212 & 0.151 & 0.307 & 0.119 & 0.126 & 0.268 & 0.227 & 0.087 & 0.236 & 0.210 & 0.121 & 0.273 & 0.205 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.193 & 0.128 & 0.160 & 0.211 & 0.144 & 0.153 & 0.183 & 0.172 & 0.164 & 0.207 & 0.159 & 0.167 & 0.209 & 0.152 & 0.160 \\
BelleGroup/BELLE-7B-0.6M &            0.212 & 0.152 & 0.204 & 0.211 & 0.229 & 0.252 & 0.203 & 0.199 & 0.204 & 0.209 & 0.206 & 0.224 & 0.210 & 0.217 & 0.237 \\
BelleGroup/BELLE-7B-1M &            0.192 & 0.157 & 0.169 & 0.228 & 0.175 & 0.186 & 0.189 & 0.176 & 0.230 & 0.203 & 0.167 & 0.176 & 0.215 & 0.171 & 0.181 \\
BelleGroup/BELLE-7B-2M &            0.182 & 0.161 & 0.136 & 0.175 & 0.122 & 0.179 & 0.182 & 0.178 & 0.180 & 0.159 & 0.135 & 0.128 & 0.171 & 0.129 & 0.166 \\
\hline
THUDM/chatglm-6b &            0.086 & 0.109 & 0.182 & 0.106 & 0.125 & 0.123 & 0.112 & 0.125 & 0.153 & 0.120 & 0.063 & 0.092 & 0.111 & 0.106 & 0.109 \\
THUDM/doctorglm-6b &            0.059 & 0.028 & 0.035 & 0.059 & 0.041 & 0.042 & 0.036 & 0.075 & 0.042 & 0.155 & 0.067 & 0.082 & 0.103 & 0.053 & 0.061 \\
\hline
fnlp/moss-moon-003-base &            0.115 & 0.050 & 0.067 & 0.131 & 0.067 & 0.071 & 0.109 & 0.057 & 0.062 & 0.113 & 0.048 & 0.062 & 0.122 & 0.057 & 0.067 \\
fnlp/moss-moon-003-sft &            0.106 & 0.078 & 0.055 & 0.064 & 0.082 & 0.069 & 0.072 & 0.098 & 0.077 & 0.098 & 0.096 & 0.095 & 0.082 & 0.089 & 0.082 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.200 & 0.185 & 0.183 & 0.198 & 0.197 & 0.207 & 0.155 & 0.180 & 0.217 & 0.230 & 0.210 & 0.205 & 0.215 & 0.204 & 0.206 \\
lmsys/vicuna-13b-delta-v1.1 &            0.204 & 0.191 & 0.198 & 0.145 & 0.141 & 0.145 & 0.158 & 0.145 & 0.184 & 0.192 & 0.196 & 0.220 & 0.169 & 0.169 & 0.184 \\
tloen/alpaca-lora-7b &            0.138 & 0.157 & 0.127 & 0.208 & 0.183 & 0.123 & 0.193 & 0.115 & 0.104 & 0.237 & 0.192 & 0.162 & 0.224 & 0.188 & 0.143 \\
\hline
EleutherAI/pythia-1.4b &            0.130 & 0.150 & 0.165 & 0.162 & 0.155 & 0.121 & 0.096 & 0.141 & 0.134 & 0.159 & 0.141 & 0.129 & 0.160 & 0.147 & 0.125 \\
EleutherAI/pythia-2.8b &            0.131 & 0.136 & 0.144 & 0.125 & 0.142 & 0.169 & 0.095 & 0.122 & 0.115 & 0.122 & 0.163 & 0.133 & 0.123 & 0.153 & 0.149 \\
EleutherAI/pythia-6.9b &            0.103 & 0.095 & 0.101 & 0.088 & 0.111 & 0.111 & 0.122 & 0.116 & 0.087 & 0.104 & 0.100 & 0.104 & 0.096 & 0.105 & 0.107 \\
EleutherAI/pythia-12b &            0.093 & 0.129 & 0.156 & 0.091 & 0.131 & 0.152 & 0.115 & 0.122 & 0.163 & 0.096 & 0.144 & 0.158 & 0.094 & 0.138 & 0.155 \\
\hline
EleutherAI/gpt-neox-20b &            0.126 & 0.089 & 0.110 & 0.096 & 0.111 & 0.101 & 0.117 & 0.106 & 0.086 & 0.097 & 0.097 & 0.138 & 0.096 & 0.103 & 0.120 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.073 & 0.057 & 0.103 & 0.105 & 0.057 & 0.065 & 0.078 & 0.053 & 0.079 & 0.102 & 0.061 & 0.085 & 0.103 & 0.059 & 0.075 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.106 & 0.081 & 0.103 & 0.115 & 0.083 & 0.095 & 0.091 & 0.061 & 0.054 & 0.110 & 0.077 & 0.080 & 0.112 & 0.080 & 0.087 \\
\hline
databricks/dolly-v2-3b &            0.107 & 0.097 & 0.098 & 0.091 & 0.101 & 0.084 & 0.109 & 0.111 & 0.099 & 0.086 & 0.085 & 0.081 & 0.088 & 0.092 & 0.083 \\
databricks/dolly-v2-7b &            0.117 & 0.081 & 0.091 & 0.108 & 0.068 & 0.121 & 0.113 & 0.089 & 0.105 & 0.123 & 0.079 & 0.084 & 0.116 & 0.074 & 0.102 \\
databricks/dolly-v2-12b &            0.094 & 0.094 & 0.093 & 0.085 & 0.097 & 0.098 & 0.069 & 0.091 & 0.096 & 0.117 & 0.113 & 0.104 & 0.102 & 0.106 & 0.101 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.112 & 0.109 & 0.113 & 0.072 & 0.071 & 0.077 & 0.109 & 0.101 & 0.088 & 0.075 & 0.101 & 0.104 & 0.074 & 0.087 & 0.091 \\
stabilityai/stablelm-tuned-alpha-7b &            0.098 & 0.141 & 0.140 & 0.098 & 0.095 & 0.091 & 0.141 & 0.145 & 0.109 & 0.124 & 0.126 & 0.114 & 0.112 & 0.111 & 0.103 \\
\hline
tiiuae/falcon-7b &            0.078 & 0.104 & 0.139 & 0.166 & 0.130 & 0.144 & 0.127 & 0.139 & 0.161 & 0.286 & 0.317 & 0.254 & 0.228 & 0.227 & 0.201 \\
tiiuae/falcon-7b-instruct &            0.077 & 0.085 & 0.090 & 0.166 & 0.278 & 0.186 & 0.092 & 0.117 & 0.117 & 0.219 & 0.209 & 0.163 & 0.194 & 0.242 & 0.174 \\
tiiuae/falcon-40b &            0.093 & 0.072 & 0.047 & 0.090 & 0.094 & 0.099 & 0.093 & 0.061 & 0.073 & 0.063 & 0.044 & 0.051 & 0.077 & 0.070 & 0.075 \\
tiiuae/falcon-40b-instruct &            0.113 & 0.119 & 0.106 & 0.157 & 0.129 & 0.128 & 0.184 & 0.094 & 0.107 & 0.071 & 0.090 & 0.128 & 0.116 & 0.109 & 0.128 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.207 & 0.352 & 0.419 & 0.367 & 0.530 & 0.602 & 0.252 & 0.403 & 0.471 & 0.458 & 0.616 & 0.683 & 0.412 & 0.573 & 0.642 \\
gpt4 &            0.397 & 0.433 & 0.493 & 0.402 & 0.437 & 0.497 & 0.434 & 0.475 & 0.542 & 0.438 & 0.483 & 0.551 & 0.420 & 0.460 & 0.524 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.148 & 0.148 & 0.156 & 0.160 & 0.163 & 0.167 & 0.150 & 0.153 & 0.160 & 0.174 & 0.171 & 0.177 & 0.168 & 0.168 & 0.173\\
Performance-Average & 0.059 & 0.075 & 0.083 & 0.075 & 0.091 & 0.101 & 0.066 & 0.078 & 0.092 & 0.091 & 0.104 & 0.115 & 0.081 & 0.094 & 0.105\\
\bottomrule
\end{tabular}
}
\caption{The performance of Engineer.}
\end{table}

==> tables/domain_experiments_table/table_his.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.124 & 0.131 & 0.118 & 0.099 & 0.108 & 0.115 & 0.128 & 0.139 & 0.132 & 0.103 & 0.096 & 0.149 & 0.101 & 0.102 & 0.131 \\
bigscience/bloomz-1b1 &            0.141 & 0.113 & 0.105 & 0.127 & 0.113 & 0.111 & 0.109 & 0.120 & 0.117 & 0.132 & 0.122 & 0.144 & 0.129 & 0.117 & 0.126 \\
bigscience/bloomz-1b7 &            0.165 & 0.152 & 0.152 & 0.137 & 0.143 & 0.143 & 0.142 & 0.204 & 0.158 & 0.148 & 0.148 & 0.207 & 0.142 & 0.145 & 0.173 \\
bigscience/bloomz-3b &            0.181 & 0.152 & 0.162 & 0.189 & 0.147 & 0.156 & 0.137 & 0.172 & 0.166 & 0.158 & 0.150 & 0.143 & 0.175 & 0.148 & 0.150 \\
bigscience/bloomz-7b1-mt &            0.152 & 0.173 & 0.149 & 0.156 & 0.140 & 0.201 & 0.132 & 0.157 & 0.137 & 0.187 & 0.175 & 0.202 & 0.170 & 0.156 & 0.201 \\
bigscience/bloomz-7b1 &            0.160 & 0.173 & 0.143 & 0.157 & 0.131 & 0.206 & 0.137 & 0.187 & 0.144 & 0.191 & 0.153 & 0.226 & 0.173 & 0.136 & 0.210 \\
bigscience/bloomz-7b1-p3 &            0.172 & 0.194 & 0.146 & 0.120 & 0.119 & 0.159 & 0.170 & 0.158 & 0.151 & 0.141 & 0.122 & 0.128 & 0.127 & 0.119 & 0.152 \\
bigscience/bloomz &            0.193 & 0.121 & 0.292 & 0.068 & 0.077 & 0.051 & 0.188 & 0.087 & 0.252 & 0.077 & 0.053 & 0.064 & 0.073 & 0.064 & 0.058 \\
bigscience/bloomz-mt &            0.246 & 0.200 & 0.183 & 0.237 & 0.165 & 0.127 & 0.222 & 0.195 & 0.186 & 0.301 & 0.154 & 0.150 & 0.272 & 0.159 & 0.139 \\
bigscience/bloomz-p3 &            0.128 & 0.081 & 0.113 & 0.101 & 0.071 & 0.045 & 0.082 & 0.047 & 0.064 & 0.153 & 0.129 & 0.077 & 0.127 & 0.100 & 0.051 \\
\hline
decapoda-research/llama-7b-hf &            0.141 & 0.129 & 0.111 & 0.172 & 0.170 & 0.157 & 0.133 & 0.123 & 0.115 & 0.187 & 0.196 & 0.172 & 0.179 & 0.182 & 0.163 \\
decapoda-research/llama-13b-hf &            0.121 & 0.239 & 0.227 & 0.126 & 0.153 & 0.174 & 0.201 & 0.184 & 0.279 & 0.155 & 0.204 & 0.226 & 0.140 & 0.176 & 0.194 \\
decapoda-research/llama-30b-hf &            0.136 & 0.185 & 0.152 & 0.104 & 0.135 & 0.114 & 0.199 & 0.195 & 0.183 & 0.098 & 0.111 & 0.149 & 0.102 & 0.127 & 0.125 \\
decapoda-research/llama-65b-hf &            0.134 & 0.126 & 0.055 & 0.196 & 0.235 & 0.176 & 0.099 & 0.070 & 0.068 & 0.135 & 0.163 & 0.141 & 0.164 & 0.198 & 0.158 \\
\hline
project-baize/baize-lora-7B &            0.212 & 0.139 & 0.115 & 0.170 & 0.174 & 0.173 & 0.161 & 0.135 & 0.173 & 0.240 & 0.198 & 0.207 & 0.202 & 0.185 & 0.189 \\
project-baize/baize-healthcare-lora-7B &            0.175 & 0.137 & 0.115 & 0.168 & 0.153 & 0.192 & 0.238 & 0.082 & 0.083 & 0.192 & 0.162 & 0.149 & 0.181 & 0.157 & 0.171 \\
project-baize/baize-lora-13B &            0.151 & 0.215 & 0.244 & 0.147 & 0.167 & 0.212 & 0.197 & 0.189 & 0.209 & 0.199 & 0.167 & 0.256 & 0.171 & 0.167 & 0.232 \\
project-baize/baize-lora-30B &            0.110 & 0.186 & 0.194 & 0.166 & 0.211 & 0.199 & 0.161 & 0.240 & 0.211 & 0.068 & 0.171 & 0.191 & 0.125 & 0.194 & 0.191 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.170 & 0.121 & 0.144 & 0.202 & 0.145 & 0.149 & 0.159 & 0.154 & 0.116 & 0.227 & 0.148 & 0.178 & 0.214 & 0.147 & 0.163 \\
BelleGroup/BELLE-7B-0.6M &            0.183 & 0.147 & 0.183 & 0.141 & 0.162 & 0.154 & 0.171 & 0.177 & 0.140 & 0.198 & 0.190 & 0.193 & 0.167 & 0.175 & 0.172 \\
BelleGroup/BELLE-7B-1M &            0.166 & 0.142 & 0.131 & 0.197 & 0.128 & 0.141 & 0.157 & 0.167 & 0.155 & 0.219 & 0.155 & 0.192 & 0.207 & 0.140 & 0.165 \\
BelleGroup/BELLE-7B-2M &            0.158 & 0.164 & 0.126 & 0.150 & 0.101 & 0.156 & 0.149 & 0.176 & 0.151 & 0.153 & 0.155 & 0.137 & 0.151 & 0.126 & 0.152 \\
\hline
THUDM/chatglm-6b &            0.088 & 0.108 & 0.151 & 0.097 & 0.105 & 0.134 & 0.105 & 0.126 & 0.149 & 0.116 & 0.087 & 0.078 & 0.102 & 0.100 & 0.112 \\
THUDM/doctorglm-6b &            0.084 & 0.071 & 0.047 & 0.085 & 0.065 & 0.051 & 0.054 & 0.069 & 0.043 & 0.081 & 0.060 & 0.050 & 0.083 & 0.062 & 0.051 \\
\hline
fnlp/moss-moon-003-base &            0.103 & 0.051 & 0.056 & 0.127 & 0.089 & 0.091 & 0.135 & 0.058 & 0.053 & 0.116 & 0.074 & 0.065 & 0.122 & 0.082 & 0.080 \\
fnlp/moss-moon-003-sft &            0.062 & 0.061 & 0.060 & 0.070 & 0.069 & 0.061 & 0.123 & 0.073 & 0.057 & 0.071 & 0.085 & 0.079 & 0.071 & 0.076 & 0.069 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.157 & 0.165 & 0.135 & 0.166 & 0.191 & 0.171 & 0.111 & 0.204 & 0.212 & 0.192 & 0.225 & 0.165 & 0.178 & 0.206 & 0.168 \\
lmsys/vicuna-13b-delta-v1.1 &            0.163 & 0.159 & 0.149 & 0.111 & 0.136 & 0.111 & 0.123 & 0.137 & 0.165 & 0.140 & 0.167 & 0.176 & 0.124 & 0.150 & 0.141 \\
tloen/alpaca-lora-7b &            0.129 & 0.132 & 0.115 & 0.188 & 0.195 & 0.128 & 0.167 & 0.107 & 0.089 & 0.196 & 0.186 & 0.159 & 0.192 & 0.191 & 0.142 \\
\hline
EleutherAI/pythia-1.4b &            0.123 & 0.123 & 0.124 & 0.143 & 0.100 & 0.101 & 0.113 & 0.134 & 0.114 & 0.183 & 0.123 & 0.116 & 0.162 & 0.111 & 0.108 \\
EleutherAI/pythia-2.8b &            0.110 & 0.109 & 0.126 & 0.155 & 0.110 & 0.099 & 0.082 & 0.095 & 0.095 & 0.117 & 0.134 & 0.086 & 0.137 & 0.121 & 0.093 \\
EleutherAI/pythia-6.9b &            0.077 & 0.083 & 0.086 & 0.089 & 0.082 & 0.074 & 0.080 & 0.075 & 0.065 & 0.100 & 0.084 & 0.085 & 0.094 & 0.083 & 0.079 \\
EleutherAI/pythia-12b &            0.101 & 0.118 & 0.108 & 0.077 & 0.085 & 0.100 & 0.137 & 0.173 & 0.151 & 0.086 & 0.110 & 0.104 & 0.081 & 0.097 & 0.102 \\
\hline
EleutherAI/gpt-neox-20b &            0.129 & 0.109 & 0.106 & 0.084 & 0.095 & 0.124 & 0.107 & 0.090 & 0.083 & 0.095 & 0.098 & 0.135 & 0.087 & 0.097 & 0.129 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.060 & 0.044 & 0.045 & 0.074 & 0.047 & 0.060 & 0.063 & 0.049 & 0.075 & 0.094 & 0.060 & 0.058 & 0.083 & 0.053 & 0.059 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.095 & 0.085 & 0.038 & 0.084 & 0.067 & 0.072 & 0.086 & 0.085 & 0.071 & 0.103 & 0.072 & 0.074 & 0.092 & 0.069 & 0.073 \\
\hline
databricks/dolly-v2-3b &            0.094 & 0.084 & 0.073 & 0.069 & 0.058 & 0.069 & 0.081 & 0.083 & 0.073 & 0.064 & 0.074 & 0.078 & 0.066 & 0.065 & 0.071 \\
databricks/dolly-v2-7b &            0.117 & 0.091 & 0.093 & 0.089 & 0.060 & 0.079 & 0.112 & 0.096 & 0.097 & 0.121 & 0.079 & 0.080 & 0.104 & 0.069 & 0.079 \\
databricks/dolly-v2-12b &            0.105 & 0.109 & 0.113 & 0.083 & 0.078 & 0.096 & 0.095 & 0.119 & 0.109 & 0.077 & 0.084 & 0.102 & 0.080 & 0.080 & 0.099 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.099 & 0.079 & 0.080 & 0.062 & 0.090 & 0.077 & 0.074 & 0.084 & 0.061 & 0.068 & 0.090 & 0.093 & 0.065 & 0.090 & 0.084 \\
stabilityai/stablelm-tuned-alpha-7b &            0.080 & 0.111 & 0.116 & 0.142 & 0.111 & 0.107 & 0.123 & 0.125 & 0.096 & 0.138 & 0.136 & 0.108 & 0.140 & 0.123 & 0.108 \\
\hline
tiiuae/falcon-7b &            0.081 & 0.109 & 0.134 & 0.092 & 0.091 & 0.083 & 0.103 & 0.131 & 0.112 & 0.181 & 0.164 & 0.145 & 0.136 & 0.126 & 0.114 \\
tiiuae/falcon-7b-instruct &            0.074 & 0.082 & 0.091 & 0.161 & 0.195 & 0.147 & 0.039 & 0.123 & 0.105 & 0.103 & 0.147 & 0.120 & 0.132 & 0.171 & 0.134 \\
tiiuae/falcon-40b &            0.067 & 0.052 & 0.052 & 0.040 & 0.064 & 0.056 & 0.054 & 0.065 & 0.046 & 0.062 & 0.094 & 0.079 & 0.052 & 0.080 & 0.068 \\
tiiuae/falcon-40b-instruct &            0.080 & 0.066 & 0.057 & 0.126 & 0.152 & 0.151 & 0.068 & 0.057 & 0.061 & 0.080 & 0.144 & 0.113 & 0.104 & 0.148 & 0.132 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.260 & 0.409 & 0.477 & 0.172 & 0.309 & 0.373 & 0.321 & 0.466 & 0.531 & 0.293 & 0.443 & 0.511 & 0.233 & 0.376 & 0.442 \\
gpt4 &            0.418 & 0.458 & 0.521 & 0.420 & 0.458 & 0.522 & 0.453 & 0.495 & 0.563 & 0.454 & 0.496 & 0.565 & 0.437 & 0.477 & 0.543 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.138 & 0.138 & 0.139 & 0.135 & 0.133 & 0.137 & 0.138 & 0.142 & 0.142 & 0.149 & 0.145 & 0.151 & 0.141 & 0.139 & 0.144\\
Performance-Average & 0.061 & 0.077 & 0.092 & 0.061 & 0.071 & 0.081 & 0.070 & 0.086 & 0.101 & 0.073 & 0.081 & 0.096 & 0.065 & 0.074 & 0.087\\
\bottomrule
\end{tabular}
}
\caption{The performance of History.}
\end{table}

==> tables/domain_experiments_table/table_jur.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.107 & 0.129 & 0.119 & 0.114 & 0.107 & 0.116 & 0.115 & 0.117 & 0.113 & 0.107 & 0.092 & 0.160 & 0.111 & 0.100 & 0.136 \\
bigscience/bloomz-1b1 &            0.110 & 0.118 & 0.106 & 0.140 & 0.133 & 0.104 & 0.112 & 0.116 & 0.090 & 0.140 & 0.115 & 0.143 & 0.140 & 0.125 & 0.122 \\
bigscience/bloomz-1b7 &            0.134 & 0.184 & 0.183 & 0.136 & 0.151 & 0.135 & 0.145 & 0.190 & 0.155 & 0.139 & 0.158 & 0.185 & 0.137 & 0.154 & 0.158 \\
bigscience/bloomz-3b &            0.186 & 0.144 & 0.170 & 0.177 & 0.144 & 0.132 & 0.131 & 0.155 & 0.172 & 0.146 & 0.151 & 0.140 & 0.162 & 0.147 & 0.135 \\
bigscience/bloomz-7b1-mt &            0.135 & 0.162 & 0.156 & 0.142 & 0.141 & 0.183 & 0.139 & 0.154 & 0.147 & 0.182 & 0.142 & 0.173 & 0.160 & 0.141 & 0.178 \\
bigscience/bloomz-7b1 &            0.141 & 0.165 & 0.161 & 0.157 & 0.141 & 0.193 & 0.136 & 0.167 & 0.157 & 0.193 & 0.157 & 0.240 & 0.174 & 0.144 & 0.203 \\
bigscience/bloomz-7b1-p3 &            0.149 & 0.172 & 0.160 & 0.115 & 0.138 & 0.184 & 0.155 & 0.150 & 0.152 & 0.100 & 0.147 & 0.164 & 0.110 & 0.139 & 0.180 \\
bigscience/bloomz &            0.229 & 0.084 & 0.375 & 0.049 & 0.072 & 0.045 & 0.299 & 0.078 & 0.345 & 0.049 & 0.049 & 0.042 & 0.049 & 0.065 & 0.044 \\
bigscience/bloomz-mt &            0.261 & 0.246 & 0.196 & 0.116 & 0.075 & 0.047 & 0.260 & 0.182 & 0.217 & 0.329 & 0.132 & 0.191 & 0.187 & 0.094 & 0.095 \\
bigscience/bloomz-p3 &            0.190 & 0.127 & 0.089 & 0.059 & 0.045 & 0.042 & 0.121 & 0.052 & 0.088 & 0.292 & 0.219 & 0.129 & 0.137 & 0.103 & 0.054 \\
\hline
decapoda-research/llama-7b-hf &            0.165 & 0.146 & 0.116 & 0.171 & 0.144 & 0.177 & 0.174 & 0.135 & 0.093 & 0.261 & 0.202 & 0.197 & 0.210 & 0.170 & 0.186 \\
decapoda-research/llama-13b-hf &            0.148 & 0.227 & 0.230 & 0.165 & 0.223 & 0.218 & 0.274 & 0.162 & 0.271 & 0.213 & 0.255 & 0.304 & 0.187 & 0.238 & 0.252 \\
decapoda-research/llama-30b-hf &            0.136 & 0.180 & 0.052 & 0.079 & 0.145 & 0.089 & 0.171 & 0.152 & 0.133 & 0.111 & 0.101 & 0.240 & 0.087 & 0.135 & 0.123 \\
decapoda-research/llama-65b-hf &            0.130 & 0.118 & 0.086 & 0.346 & 0.327 & 0.196 & 0.130 & 0.115 & 0.078 & 0.275 & 0.441 & 0.265 & 0.323 & 0.365 & 0.220 \\
\hline
project-baize/baize-lora-7B &            0.195 & 0.157 & 0.146 & 0.156 & 0.123 & 0.142 & 0.187 & 0.188 & 0.196 & 0.320 & 0.194 & 0.221 & 0.230 & 0.155 & 0.177 \\
project-baize/baize-healthcare-lora-7B &            0.196 & 0.162 & 0.146 & 0.145 & 0.230 & 0.210 & 0.236 & 0.044 & 0.041 & 0.130 & 0.232 & 0.245 & 0.138 & 0.231 & 0.221 \\
project-baize/baize-lora-13B &            0.168 & 0.224 & 0.242 & 0.156 & 0.183 & 0.175 & 0.238 & 0.152 & 0.199 & 0.204 & 0.171 & 0.286 & 0.177 & 0.177 & 0.225 \\
project-baize/baize-lora-30B &            0.064 & 0.102 & 0.141 & 0.178 & 0.166 & 0.200 & 0.133 & 0.215 & 0.113 & 0.056 & 0.105 & 0.179 & 0.136 & 0.144 & 0.181 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.165 & 0.134 & 0.143 & 0.249 & 0.137 & 0.138 & 0.168 & 0.154 & 0.149 & 0.175 & 0.125 & 0.117 & 0.217 & 0.131 & 0.129 \\
BelleGroup/BELLE-7B-0.6M &            0.159 & 0.151 & 0.181 & 0.163 & 0.151 & 0.151 & 0.168 & 0.169 & 0.128 & 0.161 & 0.161 & 0.137 & 0.163 & 0.156 & 0.145 \\
BelleGroup/BELLE-7B-1M &            0.139 & 0.164 & 0.149 & 0.241 & 0.137 & 0.152 & 0.176 & 0.182 & 0.186 & 0.147 & 0.115 & 0.146 & 0.199 & 0.127 & 0.149 \\
BelleGroup/BELLE-7B-2M &            0.133 & 0.142 & 0.130 & 0.144 & 0.095 & 0.139 & 0.162 & 0.168 & 0.143 & 0.183 & 0.181 & 0.157 & 0.153 & 0.134 & 0.143 \\
\hline
THUDM/chatglm-6b &            0.068 & 0.071 & 0.104 & 0.103 & 0.160 & 0.074 & 0.116 & 0.111 & 0.153 & 0.061 & 0.070 & 0.071 & 0.092 & 0.137 & 0.073 \\
THUDM/doctorglm-6b &            0.031 & 0.035 & 0.043 & 0.124 & 0.080 & 0.045 & 0.045 & 0.043 & 0.051 & 0.036 & 0.038 & 0.041 & 0.095 & 0.066 & 0.043 \\
\hline
fnlp/moss-moon-003-base &            0.089 & 0.047 & 0.058 & 0.105 & 0.085 & 0.096 & 0.119 & 0.044 & 0.059 & 0.131 & 0.070 & 0.065 & 0.116 & 0.078 & 0.083 \\
fnlp/moss-moon-003-sft &            0.076 & 0.059 & 0.065 & 0.079 & 0.079 & 0.061 & 0.099 & 0.084 & 0.065 & 0.084 & 0.090 & 0.045 & 0.081 & 0.084 & 0.053 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.160 & 0.158 & 0.121 & 0.134 & 0.161 & 0.145 & 0.090 & 0.190 & 0.212 & 0.173 & 0.254 & 0.174 & 0.151 & 0.201 & 0.157 \\
lmsys/vicuna-13b-delta-v1.1 &            0.143 & 0.161 & 0.131 & 0.133 & 0.147 & 0.121 & 0.136 & 0.143 & 0.142 & 0.138 & 0.126 & 0.186 & 0.135 & 0.138 & 0.151 \\
tloen/alpaca-lora-7b &            0.156 & 0.158 & 0.146 & 0.184 & 0.203 & 0.088 & 0.187 & 0.096 & 0.106 & 0.203 & 0.187 & 0.177 & 0.192 & 0.196 & 0.128 \\
\hline
EleutherAI/pythia-1.4b &            0.132 & 0.161 & 0.143 & 0.178 & 0.145 & 0.167 & 0.138 & 0.204 & 0.145 & 0.148 & 0.098 & 0.103 & 0.163 & 0.122 & 0.136 \\
EleutherAI/pythia-2.8b &            0.124 & 0.128 & 0.139 & 0.152 & 0.157 & 0.095 & 0.086 & 0.089 & 0.082 & 0.110 & 0.219 & 0.092 & 0.132 & 0.187 & 0.094 \\
EleutherAI/pythia-6.9b &            0.084 & 0.106 & 0.088 & 0.141 & 0.115 & 0.094 & 0.102 & 0.130 & 0.093 & 0.112 & 0.138 & 0.111 & 0.128 & 0.125 & 0.102 \\
EleutherAI/pythia-12b &            0.102 & 0.129 & 0.132 & 0.064 & 0.099 & 0.127 & 0.113 & 0.500 & 0.120 & 0.129 & 0.102 & 0.114 & 0.093 & 0.100 & 0.121 \\
\hline
EleutherAI/gpt-neox-20b &            0.152 & 0.093 & 0.073 & 0.074 & 0.089 & 0.134 & 0.094 & 0.072 & 0.066 & 0.091 & 0.036 & 0.055 & 0.079 & 0.063 & 0.096 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.064 & 0.043 & 0.140 & 0.079 & 0.057 & 0.094 & 0.045 & 0.046 & 0.096 & 0.079 & 0.066 & 0.058 & 0.079 & 0.061 & 0.078 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.124 & 0.143 & 0.032 & 0.104 & 0.058 & 0.078 & 0.088 & 0.133 & 0.079 & 0.110 & 0.082 & 0.074 & 0.107 & 0.069 & 0.076 \\
\hline
databricks/dolly-v2-3b &            0.121 & 0.105 & 0.095 & 0.089 & 0.044 & 0.091 & 0.090 & 0.100 & 0.088 & 0.073 & 0.077 & 0.132 & 0.082 & 0.059 & 0.100 \\
databricks/dolly-v2-7b &            0.079 & 0.094 & 0.084 & 0.116 & 0.072 & 0.101 & 0.113 & 0.079 & 0.105 & 0.184 & 0.149 & 0.106 & 0.147 & 0.107 & 0.103 \\
databricks/dolly-v2-12b &            0.097 & 0.104 & 0.096 & 0.087 & 0.119 & 0.095 & 0.101 & 0.119 & 0.105 & 0.082 & 0.110 & 0.157 & 0.085 & 0.115 & 0.122 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.095 & 0.089 & 0.107 & 0.098 & 0.152 & 0.115 & 0.080 & 0.096 & 0.074 & 0.076 & 0.102 & 0.068 & 0.088 & 0.130 & 0.094 \\
stabilityai/stablelm-tuned-alpha-7b &            0.122 & 0.134 & 0.137 & 0.160 & 0.159 & 0.142 & 0.146 & 0.148 & 0.076 & 0.193 & 0.140 & 0.084 & 0.175 & 0.151 & 0.116 \\
\hline
tiiuae/falcon-7b &            0.140 & 0.230 & 0.222 & 0.072 & 0.104 & 0.126 & 0.173 & 0.210 & 0.161 & 0.073 & 0.081 & 0.097 & 0.072 & 0.094 & 0.114 \\
tiiuae/falcon-7b-instruct &            0.116 & 0.098 & 0.076 & 0.198 & 0.200 & 0.153 & 0.059 & 0.149 & 0.132 & 0.039 & 0.078 & 0.132 & 0.135 & 0.150 & 0.145 \\
tiiuae/falcon-40b &            0.059 & 0.049 & 0.051 & 0.042 & 0.084 & 0.058 & 0.053 & 0.073 & 0.050 & 0.135 & 0.061 & 0.215 & 0.075 & 0.076 & 0.111 \\
tiiuae/falcon-40b-instruct &            0.032 & 0.035 & 0.047 & 0.136 & 0.167 & 0.167 & 0.068 & 0.061 & 0.112 & 0.138 & 0.169 & 0.085 & 0.137 & 0.167 & 0.141 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.126 & 0.250 & 0.308 & 0.297 & 0.432 & 0.492 & 0.118 & 0.264 & 0.333 & 0.129 & 0.263 & 0.327 & 0.213 & 0.347 & 0.409 \\
gpt4 &            0.305 & 0.343 & 0.396 & 0.309 & 0.354 & 0.408 & 0.418 & 0.462 & 0.528 & 0.427 & 0.483 & 0.551 & 0.368 & 0.418 & 0.480 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.133 & 0.137 & 0.139 & 0.142 & 0.143 & 0.139 & 0.143 & 0.146 & 0.140 & 0.150 & 0.148 & 0.157 & 0.145 & 0.145 & 0.144\\
Performance-Average & 0.053 & 0.061 & 0.076 & 0.064 & 0.075 & 0.081 & 0.070 & 0.087 & 0.087 & 0.080 & 0.088 & 0.091 & 0.061 & 0.074 & 0.080\\
\bottomrule
\end{tabular}
}
\caption{The performance of Jurisprudence.}
\end{table}

==> tables/domain_experiments_table/table_lit.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.111 & 0.122 & 0.111 & 0.130 & 0.132 & 0.141 & 0.114 & 0.119 & 0.132 & 0.107 & 0.090 & 0.173 & 0.119 & 0.111 & 0.157 \\
bigscience/bloomz-1b1 &            0.130 & 0.093 & 0.121 & 0.143 & 0.143 & 0.129 & 0.085 & 0.107 & 0.116 & 0.126 & 0.107 & 0.134 & 0.135 & 0.126 & 0.131 \\
bigscience/bloomz-1b7 &            0.164 & 0.152 & 0.171 & 0.162 & 0.168 & 0.163 & 0.134 & 0.212 & 0.165 & 0.153 & 0.144 & 0.223 & 0.158 & 0.157 & 0.192 \\
bigscience/bloomz-3b &            0.185 & 0.128 & 0.169 & 0.216 & 0.166 & 0.173 & 0.121 & 0.173 & 0.180 & 0.157 & 0.146 & 0.165 & 0.187 & 0.156 & 0.169 \\
bigscience/bloomz-7b1-mt &            0.139 & 0.167 & 0.151 & 0.160 & 0.169 & 0.217 & 0.110 & 0.163 & 0.131 & 0.160 & 0.173 & 0.200 & 0.160 & 0.171 & 0.209 \\
bigscience/bloomz-7b1 &            0.134 & 0.161 & 0.156 & 0.165 & 0.155 & 0.197 & 0.114 & 0.185 & 0.136 & 0.184 & 0.136 & 0.178 & 0.174 & 0.150 & 0.193 \\
bigscience/bloomz-7b1-p3 &            0.165 & 0.190 & 0.157 & 0.140 & 0.146 & 0.127 & 0.166 & 0.144 & 0.158 & 0.152 & 0.081 & 0.078 & 0.144 & 0.131 & 0.116 \\
bigscience/bloomz &            0.241 & 0.169 & 0.388 & 0.097 & 0.066 & 0.049 & 0.099 & 0.077 & 0.163 & 0.048 & 0.042 & 0.035 & 0.071 & 0.053 & 0.042 \\
bigscience/bloomz-mt &            0.278 & 0.149 & 0.265 & 0.379 & 0.235 & 0.262 & 0.161 & 0.254 & 0.282 & 0.426 & 0.209 & 0.256 & 0.405 & 0.221 & 0.259 \\
bigscience/bloomz-p3 &            0.175 & 0.081 & 0.131 & 0.050 & 0.038 & 0.035 & 0.069 & 0.046 & 0.045 & 0.151 & 0.107 & 0.064 & 0.103 & 0.074 & 0.043 \\
\hline
decapoda-research/llama-7b-hf &            0.129 & 0.117 & 0.100 & 0.135 & 0.135 & 0.111 & 0.107 & 0.094 & 0.085 & 0.199 & 0.154 & 0.157 & 0.165 & 0.143 & 0.133 \\
decapoda-research/llama-13b-hf &            0.151 & 0.282 & 0.235 & 0.163 & 0.151 & 0.202 & 0.204 & 0.175 & 0.299 & 0.168 & 0.188 & 0.237 & 0.165 & 0.169 & 0.215 \\
decapoda-research/llama-30b-hf &            0.115 & 0.189 & 0.132 & 0.058 & 0.141 & 0.119 & 0.226 & 0.197 & 0.218 & 0.070 & 0.120 & 0.224 & 0.062 & 0.134 & 0.151 \\
decapoda-research/llama-65b-hf &            0.112 & 0.133 & 0.118 & 0.158 & 0.180 & 0.153 & 0.068 & 0.037 & 0.030 & 0.042 & 0.058 & 0.048 & 0.100 & 0.119 & 0.098 \\
\hline
project-baize/baize-lora-7B &            0.179 & 0.116 & 0.106 & 0.213 & 0.150 & 0.203 & 0.146 & 0.077 & 0.176 & 0.213 & 0.175 & 0.196 & 0.213 & 0.162 & 0.200 \\
project-baize/baize-healthcare-lora-7B &            0.157 & 0.126 & 0.106 & 0.219 & 0.133 & 0.143 & 0.245 & 0.059 & 0.041 & 0.349 & 0.291 & 0.164 & 0.284 & 0.194 & 0.152 \\
project-baize/baize-lora-13B &            0.165 & 0.238 & 0.259 & 0.249 & 0.221 & 0.289 & 0.187 & 0.150 & 0.178 & 0.248 & 0.277 & 0.279 & 0.249 & 0.248 & 0.284 \\
project-baize/baize-lora-30B &            0.109 & 0.198 & 0.139 & 0.144 & 0.188 & 0.067 & 0.403 & 0.278 & 0.167 & 0.067 & 0.250 & 0.187 & 0.117 & 0.209 & 0.180 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.144 & 0.106 & 0.182 & 0.169 & 0.124 & 0.128 & 0.150 & 0.151 & 0.111 & 0.221 & 0.124 & 0.171 & 0.194 & 0.124 & 0.149 \\
BelleGroup/BELLE-7B-0.6M &            0.177 & 0.141 & 0.219 & 0.181 & 0.140 & 0.145 & 0.179 & 0.171 & 0.147 & 0.111 & 0.141 & 0.144 & 0.147 & 0.140 & 0.144 \\
BelleGroup/BELLE-7B-1M &            0.151 & 0.165 & 0.145 & 0.220 & 0.116 & 0.129 & 0.137 & 0.153 & 0.132 & 0.148 & 0.083 & 0.132 & 0.186 & 0.100 & 0.130 \\
BelleGroup/BELLE-7B-2M &            0.173 & 0.177 & 0.120 & 0.124 & 0.109 & 0.182 & 0.116 & 0.162 & 0.145 & 0.067 & 0.094 & 0.094 & 0.110 & 0.102 & 0.161 \\
\hline
THUDM/chatglm-6b &            0.082 & 0.088 & 0.124 & 0.124 & 0.136 & 0.128 & 0.122 & 0.089 & 0.145 & 0.057 & 0.068 & 0.064 & 0.109 & 0.120 & 0.107 \\
THUDM/doctorglm-6b &            0.026 & 0.142 & 0.039 & 0.041 & 0.046 & 0.029 & 0.078 & 0.047 & 0.056 & 0.075 & 0.059 & 0.037 & 0.059 & 0.053 & 0.033 \\
\hline
fnlp/moss-moon-003-base &            0.111 & 0.064 & 0.061 & 0.120 & 0.105 & 0.097 & 0.133 & 0.054 & 0.056 & 0.124 & 0.069 & 0.067 & 0.122 & 0.088 & 0.084 \\
fnlp/moss-moon-003-sft &            0.060 & 0.087 & 0.116 & 0.101 & 0.089 & 0.057 & 0.043 & 0.066 & 0.051 & 0.067 & 0.111 & 0.100 & 0.085 & 0.100 & 0.078 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.149 & 0.169 & 0.218 & 0.166 & 0.206 & 0.178 & 0.147 & 0.254 & 0.183 & 0.181 & 0.207 & 0.187 & 0.173 & 0.206 & 0.182 \\
lmsys/vicuna-13b-delta-v1.1 &            0.137 & 0.142 & 0.186 & 0.111 & 0.135 & 0.114 & 0.178 & 0.162 & 0.226 & 0.121 & 0.164 & 0.192 & 0.116 & 0.149 & 0.151 \\
tloen/alpaca-lora-7b &            0.139 & 0.130 & 0.106 & 0.226 & 0.196 & 0.177 & 0.160 & 0.069 & 0.074 & 0.184 & 0.157 & 0.134 & 0.206 & 0.177 & 0.157 \\
\hline
EleutherAI/pythia-1.4b &            0.116 & 0.101 & 0.107 & 0.113 & 0.061 & 0.065 & 0.127 & 0.196 & 0.183 & 0.091 & 0.122 & 0.137 & 0.105 & 0.084 & 0.093 \\
EleutherAI/pythia-2.8b &            0.126 & 0.119 & 0.138 & 0.117 & 0.115 & 0.070 & 0.071 & 0.114 & 0.116 & 0.068 & 0.081 & 0.068 & 0.098 & 0.102 & 0.069 \\
EleutherAI/pythia-6.9b &            0.076 & 0.097 & 0.094 & 0.099 & 0.069 & 0.067 & 0.082 & 0.110 & 0.119 & 0.105 & 0.087 & 0.064 & 0.102 & 0.078 & 0.066 \\
EleutherAI/pythia-12b &            0.104 & 0.100 & 0.107 & 0.099 & 0.084 & 0.092 & 0.111 & 0.053 & 0.100 & 0.074 & 0.099 & 0.093 & 0.087 & 0.091 & 0.093 \\
\hline
EleutherAI/gpt-neox-20b &            0.131 & 0.091 & 0.118 & 0.089 & 0.055 & 0.065 & 0.110 & 0.086 & 0.066 & 0.065 & 0.112 & 0.185 & 0.083 & 0.080 & 0.115 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.071 & 0.049 & 0.033 & 0.082 & 0.048 & 0.073 & 0.074 & 0.088 & 0.107 & 0.121 & 0.058 & 0.063 & 0.101 & 0.053 & 0.069 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.097 & 0.065 & 0.042 & 0.140 & 0.053 & 0.090 & 0.081 & 0.068 & 0.086 & 0.120 & 0.067 & 0.080 & 0.130 & 0.060 & 0.085 \\
\hline
databricks/dolly-v2-3b &            0.087 & 0.075 & 0.065 & 0.070 & 0.046 & 0.064 & 0.076 & 0.076 & 0.078 & 0.093 & 0.062 & 0.056 & 0.081 & 0.054 & 0.061 \\
databricks/dolly-v2-7b &            0.098 & 0.112 & 0.122 & 0.104 & 0.048 & 0.068 & 0.110 & 0.097 & 0.103 & 0.083 & 0.101 & 0.101 & 0.094 & 0.073 & 0.084 \\
databricks/dolly-v2-12b &            0.077 & 0.109 & 0.104 & 0.063 & 0.064 & 0.085 & 0.095 & 0.121 & 0.097 & 0.046 & 0.092 & 0.084 & 0.055 & 0.077 & 0.085 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.100 & 0.085 & 0.082 & 0.078 & 0.103 & 0.078 & 0.072 & 0.086 & 0.058 & 0.050 & 0.071 & 0.095 & 0.065 & 0.088 & 0.086 \\
stabilityai/stablelm-tuned-alpha-7b &            0.072 & 0.111 & 0.116 & 0.180 & 0.108 & 0.096 & 0.100 & 0.127 & 0.079 & 0.143 & 0.077 & 0.089 & 0.162 & 0.094 & 0.093 \\
\hline
tiiuae/falcon-7b &            0.055 & 0.050 & 0.043 & 0.086 & 0.081 & 0.095 & 0.159 & 0.109 & 0.118 & 0.234 & 0.169 & 0.162 & 0.150 & 0.120 & 0.124 \\
tiiuae/falcon-7b-instruct &            0.082 & 0.101 & 0.091 & 0.152 & 0.107 & 0.140 & 0.031 & 0.158 & 0.151 & 0.068 & 0.124 & 0.116 & 0.115 & 0.114 & 0.130 \\
tiiuae/falcon-40b &            0.087 & 0.061 & 0.087 & 0.061 & 0.169 & 0.065 & 0.063 & 0.057 & 0.075 & 0.126 & 0.037 & 0.115 & 0.096 & 0.100 & 0.091 \\
tiiuae/falcon-40b-instruct &            0.077 & 0.070 & 0.092 & 0.118 & 0.144 & 0.066 & 0.052 & 0.152 & 0.059 & 0.066 & 0.109 & 0.063 & 0.096 & 0.128 & 0.065 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.239 & 0.373 & 0.434 & 0.162 & 0.293 & 0.354 & 0.325 & 0.473 & 0.538 & 0.168 & 0.290 & 0.347 & 0.165 & 0.291 & 0.350 \\
gpt4 &            0.378 & 0.418 & 0.479 & 0.383 & 0.428 & 0.490 & 0.438 & 0.477 & 0.542 & 0.451 & 0.482 & 0.548 & 0.417 & 0.455 & 0.519 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.133 & 0.136 & 0.146 & 0.144 & 0.132 & 0.133 & 0.136 & 0.140 & 0.143 & 0.139 & 0.133 & 0.144 & 0.143 & 0.133 & 0.140\\
Performance-Average & 0.061 & 0.072 & 0.092 & 0.070 & 0.070 & 0.085 & 0.081 & 0.091 & 0.102 & 0.089 & 0.081 & 0.091 & 0.075 & 0.071 & 0.085\\
\bottomrule
\end{tabular}
}
\caption{The performance of Literature.}
\end{table}

==> tables/domain_experiments_table/table_man.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.131 & 0.141 & 0.126 & 0.092 & 0.084 & 0.079 & 0.068 & 0.070 & 0.099 & 0.128 & 0.185 & 0.175 & 0.110 & 0.134 & 0.127 \\
bigscience/bloomz-1b1 &            0.112 & 0.109 & 0.098 & 0.120 & 0.110 & 0.105 & 0.081 & 0.075 & 0.064 & 0.156 & 0.131 & 0.160 & 0.138 & 0.120 & 0.132 \\
bigscience/bloomz-1b7 &            0.184 & 0.203 & 0.189 & 0.118 & 0.109 & 0.114 & 0.142 & 0.162 & 0.148 & 0.140 & 0.132 & 0.174 & 0.129 & 0.121 & 0.143 \\
bigscience/bloomz-3b &            0.145 & 0.164 & 0.191 & 0.189 & 0.150 & 0.169 & 0.109 & 0.115 & 0.136 & 0.191 & 0.214 & 0.143 & 0.190 & 0.182 & 0.156 \\
bigscience/bloomz-7b1-mt &            0.140 & 0.148 & 0.152 & 0.139 & 0.112 & 0.209 & 0.132 & 0.168 & 0.137 & 0.187 & 0.221 & 0.238 & 0.162 & 0.166 & 0.224 \\
bigscience/bloomz-7b1 &            0.148 & 0.157 & 0.183 & 0.163 & 0.121 & 0.228 & 0.132 & 0.190 & 0.155 & 0.183 & 0.144 & 0.219 & 0.172 & 0.126 & 0.226 \\
bigscience/bloomz-7b1-p3 &            0.174 & 0.189 & 0.201 & 0.104 & 0.116 & 0.168 & 0.129 & 0.140 & 0.116 & 0.105 & 0.153 & 0.160 & 0.104 & 0.124 & 0.167 \\
bigscience/bloomz &            0.202 & 0.073 & 0.280 & 0.086 & 0.063 & 0.041 & 0.269 & 0.098 & 0.186 & -1.000 & -1.000 & -1.000 & 0.086 & 0.063 & 0.041 \\
bigscience/bloomz-mt &            0.274 & 0.107 & 0.035 & 0.113 & 0.125 & 0.110 & 0.152 & 0.044 & 0.043 & -1.000 & -1.000 & -1.000 & 0.113 & 0.125 & 0.110 \\
bigscience/bloomz-p3 &            0.156 & 0.155 & 0.251 & 0.280 & 0.187 & 0.100 & 0.039 & 0.035 & 0.350 & -1.000 & -1.000 & -1.000 & 0.280 & 0.187 & 0.100 \\
\hline
decapoda-research/llama-7b-hf &            0.139 & 0.150 & 0.108 & 0.244 & 0.215 & 0.257 & 0.070 & 0.055 & 0.060 & 0.203 & 0.208 & 0.276 & 0.226 & 0.212 & 0.265 \\
decapoda-research/llama-13b-hf &            0.147 & 0.188 & 0.245 & 0.199 & 0.268 & 0.380 & 0.305 & 0.207 & 0.224 & 0.235 & 0.272 & 0.439 & 0.215 & 0.270 & 0.396 \\
decapoda-research/llama-30b-hf &            0.154 & 0.241 & 0.236 & 0.206 & 0.325 & 0.198 & 0.051 & 0.088 & 0.075 & 0.081 & -1.000 & -1.000 & 0.175 & 0.325 & 0.198 \\
decapoda-research/llama-65b-hf &            0.133 & 0.095 & 0.044 & 0.255 & 0.283 & 0.186 & 0.037 & 0.035 & 0.087 & -1.000 & -1.000 & -1.000 & 0.255 & 0.283 & 0.186 \\
\hline
project-baize/baize-lora-7B &            0.146 & 0.151 & 0.119 & 0.202 & 0.344 & 0.236 & 0.119 & 0.073 & 0.155 & 0.338 & 0.263 & 0.380 & 0.268 & 0.305 & 0.302 \\
project-baize/baize-healthcare-lora-7B &            0.163 & 0.165 & 0.120 & 0.267 & 0.333 & 0.333 & 0.101 & 0.044 & 0.029 & 0.260 & 0.144 & -1.000 & 0.263 & 0.238 & 0.333 \\
project-baize/baize-lora-13B &            0.179 & 0.212 & 0.316 & 0.172 & 0.254 & 0.228 & 0.196 & 0.130 & 0.126 & 0.230 & 0.194 & 0.448 & 0.199 & 0.226 & 0.329 \\
project-baize/baize-lora-30B &            0.073 & 0.298 & 0.140 & 0.449 & 0.203 & 0.289 & 0.020 & 0.187 & 0.167 & 0.117 & 0.264 & 0.519 & 0.375 & 0.216 & 0.381 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.211 & 0.148 & 0.120 & 0.172 & 0.121 & 0.211 & 0.194 & 0.165 & 0.152 & 0.371 & 0.295 & 0.314 & 0.268 & 0.204 & 0.260 \\
BelleGroup/BELLE-7B-0.6M &            0.156 & 0.169 & 0.212 & 0.182 & 0.200 & 0.328 & 0.187 & 0.193 & 0.171 & 0.298 & 0.249 & 0.370 & 0.238 & 0.223 & 0.348 \\
BelleGroup/BELLE-7B-1M &            0.164 & 0.182 & 0.168 & 0.243 & 0.170 & 0.165 & 0.208 & 0.199 & 0.294 & 0.275 & 0.371 & 0.358 & 0.259 & 0.267 & 0.258 \\
BelleGroup/BELLE-7B-2M &            0.216 & 0.159 & 0.152 & 0.227 & 0.087 & 0.263 & 0.181 & 0.200 & 0.162 & 0.246 & 0.280 & 0.314 & 0.231 & 0.180 & 0.274 \\
\hline
THUDM/chatglm-6b &            0.068 & 0.102 & 0.165 & 0.140 & 0.163 & 0.057 & 0.077 & 0.206 & 0.142 & 0.053 & 0.084 & 0.034 & 0.125 & 0.154 & 0.051 \\
THUDM/doctorglm-6b &            0.038 & 0.033 & 0.030 & 0.074 & 0.051 & 0.033 & 0.022 & 0.024 & 0.038 & -1.000 & -1.000 & -1.000 & 0.074 & 0.051 & 0.033 \\
\hline
fnlp/moss-moon-003-base &            0.074 & 0.068 & 0.030 & 0.111 & 0.091 & 0.127 & 0.083 & 0.072 & 0.047 & 0.128 & 0.042 & 0.064 & 0.119 & 0.067 & 0.101 \\
fnlp/moss-moon-003-sft &            0.042 & 0.059 & 0.058 & 0.050 & 0.062 & 0.053 & -1.000 & 0.102 & 0.100 & 0.062 & 0.113 & 0.076 & 0.056 & 0.086 & 0.064 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.258 & 0.158 & 0.175 & 0.150 & 0.225 & 0.300 & 0.120 & 0.082 & 0.101 & 0.277 & 0.269 & 0.239 & 0.211 & 0.246 & 0.271 \\
lmsys/vicuna-13b-delta-v1.1 &            0.250 & 0.171 & 0.135 & 0.068 & 0.143 & 0.130 & 0.137 & 0.196 & 0.185 & 0.131 & 0.131 & 0.266 & 0.098 & 0.137 & 0.192 \\
tloen/alpaca-lora-7b &            0.176 & 0.139 & 0.120 & 0.238 & 0.198 & 0.153 & 0.134 & 0.107 & 0.101 & 0.282 & 0.072 & 0.090 & 0.258 & 0.142 & 0.125 \\
\hline
EleutherAI/pythia-1.4b &            0.111 & 0.136 & 0.145 & 0.174 & 0.080 & 0.102 & 0.061 & 0.084 & 0.133 & 0.370 & 0.122 & 0.086 & 0.239 & 0.094 & 0.097 \\
EleutherAI/pythia-2.8b &            0.085 & 0.139 & 0.170 & 0.290 & 0.114 & 0.060 & 0.109 & 0.061 & 0.087 & 0.519 & 0.061 & 0.041 & 0.367 & 0.092 & 0.054 \\
EleutherAI/pythia-6.9b &            0.056 & 0.092 & 0.093 & 0.044 & 0.159 & 0.081 & 0.064 & 0.074 & 0.083 & 0.081 & 0.068 & 0.107 & 0.062 & 0.115 & 0.093 \\
EleutherAI/pythia-12b &            0.095 & 0.112 & 0.128 & 0.073 & 0.101 & 0.150 & 0.090 & -1.000 & 0.136 & 0.046 & 0.086 & 0.080 & 0.060 & 0.094 & 0.116 \\
\hline
EleutherAI/gpt-neox-20b &            0.118 & 0.042 & 0.041 & 0.120 & 0.043 & 0.057 & 0.090 & 0.066 & 0.057 & 0.136 & 0.057 & 0.067 & 0.122 & 0.046 & 0.059 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.066 & 0.032 & 0.070 & 0.124 & 0.038 & 0.133 & 0.066 & 0.053 & 0.135 & 0.171 & 0.042 & 0.047 & 0.145 & 0.040 & 0.093 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.083 & 0.090 & 0.039 & 0.081 & 0.039 & 0.082 & 0.041 & 0.062 & 0.095 & 0.082 & 0.052 & 0.158 & 0.082 & 0.045 & 0.117 \\
\hline
databricks/dolly-v2-3b &            0.129 & 0.082 & 0.059 & 0.059 & 0.032 & 0.132 & 0.076 & 0.092 & 0.083 & 0.045 & 0.046 & 0.045 & 0.053 & 0.038 & 0.113 \\
databricks/dolly-v2-7b &            0.084 & 0.058 & 0.078 & 0.077 & 0.062 & 0.071 & 0.133 & 0.097 & 0.129 & 0.215 & 0.064 & 0.072 & 0.141 & 0.063 & 0.071 \\
databricks/dolly-v2-12b &            0.102 & 0.153 & 0.103 & 0.056 & 0.152 & 0.087 & 0.114 & 0.112 & 0.047 & 0.049 & 0.057 & 0.052 & 0.053 & 0.108 & 0.070 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.158 & 0.109 & 0.105 & 0.066 & 0.089 & 0.090 & 0.148 & 0.169 & 0.063 & 0.091 & 0.164 & 0.094 & 0.077 & 0.122 & 0.092 \\
stabilityai/stablelm-tuned-alpha-7b &            0.124 & 0.146 & 0.143 & 0.096 & 0.115 & 0.120 & 0.143 & 0.144 & 0.084 & 0.246 & 0.238 & 0.271 & 0.163 & 0.170 & 0.187 \\
\hline
tiiuae/falcon-7b &            0.070 & 0.090 & 0.106 & 0.093 & 0.088 & 0.089 & 0.081 & 0.081 & 0.080 & 0.024 & 0.026 & 0.260 & 0.074 & 0.070 & 0.138 \\
tiiuae/falcon-7b-instruct &            0.048 & 0.056 & 0.057 & 0.186 & 0.276 & 0.036 & 0.024 & 0.045 & 0.042 & 0.026 & 0.029 & 0.034 & 0.159 & 0.235 & 0.036 \\
tiiuae/falcon-40b &            0.063 & 0.056 & 0.038 & 0.060 & 0.039 & 0.042 & 0.500 & 0.077 & 0.023 & -1.000 & -1.000 & -1.000 & 0.060 & 0.039 & 0.042 \\
tiiuae/falcon-40b-instruct &            0.082 & 0.039 & 0.033 & 0.083 & 0.363 & 0.075 & 0.034 & 0.029 & 0.032 & -1.000 & -1.000 & -1.000 & 0.083 & 0.363 & 0.075 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.100 & 0.199 & 0.246 & 0.048 & 0.208 & 0.287 & 0.078 & 0.280 & 0.379 & 0.088 & 0.212 & 0.272 & 0.068 & 0.210 & 0.279 \\
gpt4 &            0.336 & 0.373 & 0.428 & 0.348 & 0.381 & 0.437 & 0.411 & 0.469 & 0.546 & 0.431 & 0.515 & 0.595 & 0.390 & 0.448 & 0.516 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.135 & 0.135 & 0.138 & 0.152 & 0.155 & 0.157 & 0.101 & 0.095 & 0.129 & 0.006 & -0.037 & -0.027 & 0.166 & 0.161 & 0.171\\
Performance-Average & 0.064 & 0.067 & 0.083 & 0.087 & 0.094 & 0.098 & 0.187 & 0.180 & 0.097 & 0.434 & 0.447 & 0.491 & 0.089 & 0.092 & 0.112\\
\bottomrule
\end{tabular}
}
\caption{The performance of Management.}
\end{table}

==> tables/domain_experiments_table/table_med.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.140 & 0.150 & 0.118 & 0.103 & 0.103 & 0.115 & 0.156 & 0.168 & 0.163 & 0.103 & 0.107 & 0.110 & 0.103 & 0.105 & 0.112 \\
bigscience/bloomz-1b1 &            0.152 & 0.167 & 0.144 & 0.118 & 0.098 & 0.106 & 0.153 & 0.181 & 0.183 & 0.142 & 0.118 & 0.097 & 0.129 & 0.108 & 0.102 \\
bigscience/bloomz-1b7 &            0.151 & 0.147 & 0.160 & 0.102 & 0.132 & 0.151 & 0.173 & 0.237 & 0.201 & 0.154 & 0.144 & 0.185 & 0.127 & 0.138 & 0.167 \\
bigscience/bloomz-3b &            0.195 & 0.196 & 0.190 & 0.187 & 0.146 & 0.151 & 0.180 & 0.204 & 0.227 & 0.192 & 0.187 & 0.138 & 0.190 & 0.166 & 0.145 \\
bigscience/bloomz-7b1-mt &            0.141 & 0.205 & 0.160 & 0.164 & 0.142 & 0.193 & 0.190 & 0.144 & 0.194 & 0.222 & 0.218 & 0.236 & 0.192 & 0.179 & 0.214 \\
bigscience/bloomz-7b1 &            0.144 & 0.198 & 0.173 & 0.184 & 0.140 & 0.227 & 0.194 & 0.213 & 0.206 & 0.223 & 0.198 & 0.223 & 0.203 & 0.153 & 0.226 \\
bigscience/bloomz-7b1-p3 &            0.184 & 0.211 & 0.183 & 0.124 & 0.129 & 0.130 & 0.203 & 0.229 & 0.225 & 0.150 & 0.158 & 0.133 & 0.133 & 0.135 & 0.131 \\
bigscience/bloomz &            0.132 & 0.094 & 0.188 & 0.069 & 0.142 & 0.084 & 0.116 & 0.056 & 0.314 & 0.049 & 0.086 & 0.107 & 0.062 & 0.122 & 0.092 \\
bigscience/bloomz-mt &            0.243 & 0.177 & 0.263 & 0.208 & 0.156 & 0.237 & 0.270 & 0.155 & 0.138 & 0.207 & 0.159 & 0.172 & 0.207 & 0.157 & 0.214 \\
bigscience/bloomz-p3 &            0.123 & 0.146 & 0.067 & 0.231 & 0.068 & 0.126 & 0.067 & 0.071 & 0.093 & 0.189 & 0.090 & 0.022 & 0.212 & 0.078 & 0.117 \\
\hline
decapoda-research/llama-7b-hf &            0.132 & 0.132 & 0.137 & 0.135 & 0.199 & 0.192 & 0.139 & 0.164 & 0.166 & 0.139 & 0.172 & 0.197 & 0.137 & 0.186 & 0.194 \\
decapoda-research/llama-13b-hf &            0.130 & 0.271 & 0.376 & 0.131 & 0.202 & 0.188 & 0.178 & 0.328 & 0.364 & 0.168 & 0.240 & 0.182 & 0.149 & 0.220 & 0.185 \\
decapoda-research/llama-30b-hf &            0.133 & 0.206 & 0.177 & 0.157 & 0.180 & 0.139 & 0.267 & 0.379 & 0.384 & 0.146 & 0.180 & 0.195 & 0.155 & 0.180 & 0.155 \\
decapoda-research/llama-65b-hf &            0.107 & 0.059 & 0.032 & 0.255 & 0.180 & 0.126 & 0.051 & 0.047 & 0.050 & 0.094 & 0.197 & 0.113 & 0.184 & 0.187 & 0.120 \\
\hline
project-baize/baize-lora-7B &            0.219 & 0.135 & 0.115 & 0.167 & 0.200 & 0.212 & 0.208 & 0.148 & 0.210 & 0.193 & 0.160 & 0.187 & 0.180 & 0.180 & 0.200 \\
project-baize/baize-healthcare-lora-7B &            0.257 & 0.131 & 0.116 & 0.196 & 0.228 & 0.187 & 0.339 & 0.220 & 0.300 & 0.108 & 0.286 & 0.335 & 0.148 & 0.251 & 0.256 \\
project-baize/baize-lora-13B &            0.174 & 0.237 & 0.303 & 0.171 & 0.184 & 0.247 & 0.243 & 0.295 & 0.301 & 0.180 & 0.218 & 0.295 & 0.175 & 0.201 & 0.270 \\
project-baize/baize-lora-30B &            0.138 & 0.245 & 0.291 & 0.095 & 0.285 & -1.000 & 0.428 & 0.313 & 0.288 & 0.107 & 0.055 & 0.078 & 0.100 & 0.174 & 0.078 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.159 & 0.152 & 0.154 & 0.193 & 0.183 & 0.161 & 0.216 & 0.214 & 0.156 & 0.229 & 0.161 & 0.187 & 0.211 & 0.172 & 0.174 \\
BelleGroup/BELLE-7B-0.6M &            0.198 & 0.198 & 0.249 & 0.135 & 0.128 & 0.165 & 0.285 & 0.286 & 0.265 & 0.210 & 0.171 & 0.167 & 0.170 & 0.149 & 0.166 \\
BelleGroup/BELLE-7B-1M &            0.155 & 0.182 & 0.156 & 0.200 & 0.141 & 0.156 & 0.231 & 0.237 & 0.237 & 0.219 & 0.147 & 0.157 & 0.209 & 0.144 & 0.156 \\
BelleGroup/BELLE-7B-2M &            0.190 & 0.193 & 0.164 & 0.143 & 0.129 & 0.131 & 0.230 & 0.265 & 0.252 & 0.126 & 0.107 & 0.093 & 0.139 & 0.118 & 0.123 \\
\hline
THUDM/chatglm-6b &            0.080 & 0.090 & 0.138 & 0.088 & 0.094 & 0.150 & 0.130 & 0.076 & 0.164 & 0.101 & 0.039 & 0.056 & 0.091 & 0.082 & 0.115 \\
THUDM/doctorglm-6b &            0.182 & 0.141 & 0.049 & 0.051 & 0.046 & 0.036 & 0.028 & 0.025 & 0.026 & 0.223 & 0.053 & 0.075 & 0.112 & 0.049 & 0.050 \\
\hline
fnlp/moss-moon-003-base &            0.107 & 0.046 & 0.066 & 0.151 & 0.080 & 0.069 & 0.113 & 0.072 & 0.080 & 0.142 & 0.073 & 0.129 & 0.147 & 0.076 & 0.097 \\
fnlp/moss-moon-003-sft &            0.049 & 0.057 & 0.062 & 0.075 & 0.043 & 0.043 & 0.066 & 0.067 & 0.061 & 0.061 & 0.083 & 0.071 & 0.068 & 0.063 & 0.057 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.157 & 0.183 & 0.142 & 0.175 & 0.218 & 0.195 & 0.120 & 0.194 & 0.283 & 0.208 & 0.228 & 0.219 & 0.191 & 0.223 & 0.207 \\
lmsys/vicuna-13b-delta-v1.1 &            0.159 & 0.171 & 0.159 & 0.102 & 0.102 & 0.141 & 0.085 & 0.123 & 0.196 & 0.133 & 0.187 & 0.172 & 0.117 & 0.144 & 0.156 \\
tloen/alpaca-lora-7b &            0.112 & 0.124 & 0.116 & 0.184 & 0.138 & 0.133 & 0.233 & 0.070 & 0.096 & 0.168 & 0.246 & 0.121 & 0.177 & 0.187 & 0.128 \\
\hline
EleutherAI/pythia-1.4b &            0.116 & 0.106 & 0.106 & 0.135 & 0.095 & 0.107 & 0.138 & 0.201 & 0.319 & 0.156 & 0.081 & 0.076 & 0.146 & 0.088 & 0.092 \\
EleutherAI/pythia-2.8b &            0.085 & 0.106 & 0.096 & 0.087 & 0.124 & 0.164 & 0.062 & 0.149 & 0.154 & 0.070 & 0.125 & 0.137 & 0.079 & 0.125 & 0.150 \\
EleutherAI/pythia-6.9b &            0.088 & 0.091 & 0.081 & 0.083 & 0.074 & 0.055 & 0.119 & 0.132 & 0.103 & 0.065 & 0.093 & 0.088 & 0.074 & 0.083 & 0.071 \\
EleutherAI/pythia-12b &            0.096 & 0.125 & 0.159 & 0.055 & 0.077 & 0.059 & 0.156 & -1.000 & 0.164 & 0.107 & 0.097 & 0.086 & 0.081 & 0.087 & 0.072 \\
\hline
EleutherAI/gpt-neox-20b &            0.102 & 0.127 & 0.076 & 0.075 & 0.132 & 0.137 & 0.089 & 0.148 & 0.120 & 0.042 & 0.203 & 0.121 & 0.067 & 0.166 & 0.129 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.053 & 0.038 & 0.051 & 0.050 & 0.042 & 0.048 & 0.113 & 0.116 & 0.117 & 0.083 & 0.038 & 0.039 & 0.066 & 0.040 & 0.044 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.082 & 0.056 & 0.020 & 0.105 & 0.087 & 0.087 & 0.083 & 0.073 & 0.121 & 0.076 & 0.074 & 0.099 & 0.091 & 0.081 & 0.093 \\
\hline
databricks/dolly-v2-3b &            0.078 & 0.070 & 0.069 & 0.077 & 0.034 & 0.056 & 0.081 & 0.080 & 0.074 & 0.048 & 0.081 & 0.081 & 0.063 & 0.058 & 0.063 \\
databricks/dolly-v2-7b &            0.124 & 0.073 & 0.083 & 0.134 & 0.052 & 0.052 & 0.090 & 0.102 & 0.096 & 0.140 & 0.061 & 0.066 & 0.137 & 0.056 & 0.059 \\
databricks/dolly-v2-12b &            0.116 & 0.125 & 0.112 & 0.100 & 0.102 & 0.086 & 0.120 & 0.128 & 0.120 & 0.089 & 0.096 & 0.155 & 0.095 & 0.099 & 0.120 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.093 & 0.056 & 0.060 & 0.063 & 0.101 & 0.092 & 0.056 & 0.077 & 0.039 & 0.063 & 0.059 & 0.051 & 0.063 & 0.081 & 0.073 \\
stabilityai/stablelm-tuned-alpha-7b &            0.068 & 0.097 & 0.107 & 0.093 & 0.090 & 0.073 & 0.112 & 0.105 & 0.090 & 0.131 & 0.150 & 0.094 & 0.111 & 0.118 & 0.083 \\
\hline
tiiuae/falcon-7b &            0.033 & 0.032 & 0.050 & 0.060 & 0.087 & 0.049 & 0.283 & 0.300 & 0.213 & 0.093 & 0.122 & 0.205 & 0.076 & 0.103 & 0.124 \\
tiiuae/falcon-7b-instruct &            0.051 & 0.061 & 0.059 & 0.097 & 0.207 & 0.084 & 0.044 & 0.241 & 0.149 & 0.115 & 0.121 & 0.154 & 0.106 & 0.164 & 0.119 \\
tiiuae/falcon-40b &            0.034 & 0.057 & 0.041 & 0.067 & 0.031 & 0.031 & 0.059 & 0.023 & 0.025 & 0.073 & 0.029 & 0.039 & 0.070 & 0.030 & 0.035 \\
tiiuae/falcon-40b-instruct &            0.146 & 0.048 & 0.134 & 0.141 & 0.133 & 0.178 & 0.294 & 0.055 & 0.108 & 0.111 & 0.067 & 0.172 & 0.128 & 0.105 & 0.175 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.241 & 0.360 & 0.413 & 0.246 & 0.396 & 0.465 & 0.188 & 0.344 & 0.417 & 0.283 & 0.420 & 0.481 & 0.265 & 0.408 & 0.473 \\
gpt4 &            0.459 & 0.489 & 0.549 & 0.472 & 0.500 & 0.561 & 0.457 & 0.506 & 0.580 & 0.466 & 0.512 & 0.587 & 0.469 & 0.506 & 0.574 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.138 & 0.144 & 0.147 & 0.137 & 0.140 & 0.119 & 0.167 & 0.148 & 0.188 & 0.145 & 0.147 & 0.153 & 0.141 & 0.143 & 0.148\\
Performance-Average & 0.071 & 0.085 & 0.103 & 0.073 & 0.086 & 0.191 & 0.096 & 0.198 & 0.111 & 0.075 & 0.092 & 0.104 & 0.070 & 0.085 & 0.097\\
\bottomrule
\end{tabular}
}
\caption{The performance of Medicine.}
\end{table}

==> tables/domain_experiments_table/table_ped.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.124 & 0.144 & 0.136 & 0.108 & 0.109 & 0.107 & 0.120 & 0.174 & 0.178 & 0.119 & 0.133 & 0.138 & 0.113 & 0.120 & 0.121 \\
bigscience/bloomz-1b1 &            0.132 & 0.130 & 0.125 & 0.109 & 0.097 & 0.105 & 0.140 & 0.140 & 0.147 & 0.133 & 0.143 & 0.150 & 0.121 & 0.119 & 0.126 \\
bigscience/bloomz-1b7 &            0.146 & 0.141 & 0.152 & 0.101 & 0.090 & 0.098 & 0.179 & 0.217 & 0.187 & 0.125 & 0.121 & 0.204 & 0.112 & 0.105 & 0.148 \\
bigscience/bloomz-3b &            0.203 & 0.183 & 0.197 & 0.191 & 0.151 & 0.148 & 0.160 & 0.160 & 0.207 & 0.164 & 0.172 & 0.149 & 0.178 & 0.161 & 0.148 \\
bigscience/bloomz-7b1-mt &            0.144 & 0.198 & 0.191 & 0.184 & 0.141 & 0.202 & 0.158 & 0.164 & 0.194 & 0.223 & 0.216 & 0.220 & 0.202 & 0.176 & 0.210 \\
bigscience/bloomz-7b1 &            0.175 & 0.192 & 0.167 & 0.156 & 0.152 & 0.218 & 0.172 & 0.223 & 0.204 & 0.219 & 0.123 & 0.279 & 0.185 & 0.145 & 0.232 \\
bigscience/bloomz-7b1-p3 &            0.164 & 0.215 & 0.174 & 0.129 & 0.104 & 0.156 & 0.210 & 0.205 & 0.200 & 0.171 & 0.090 & 0.108 & 0.143 & 0.101 & 0.146 \\
bigscience/bloomz &            0.206 & 0.121 & 0.378 & 0.040 & 0.038 & 0.035 & 0.341 & 0.256 & 0.184 & 0.046 & 0.042 & 0.047 & 0.044 & 0.041 & 0.043 \\
bigscience/bloomz-mt &            0.211 & 0.105 & 0.196 & 0.677 & 0.148 & 0.055 & 0.148 & 0.290 & 0.259 & 0.302 & 0.128 & 0.094 & 0.442 & 0.136 & 0.079 \\
bigscience/bloomz-p3 &            0.099 & 0.145 & 0.093 & 0.214 & 0.046 & 0.050 & 0.098 & 0.067 & 0.073 & 0.202 & 0.100 & 0.039 & 0.207 & 0.080 & 0.046 \\
\hline
decapoda-research/llama-7b-hf &            0.171 & 0.132 & 0.122 & 0.132 & 0.119 & 0.133 & 0.140 & 0.149 & 0.108 & 0.211 & 0.203 & 0.192 & 0.171 & 0.161 & 0.163 \\
decapoda-research/llama-13b-hf &            0.174 & 0.224 & 0.170 & 0.170 & 0.231 & 0.217 & 0.231 & 0.226 & 0.327 & 0.144 & 0.191 & 0.101 & 0.157 & 0.211 & 0.174 \\
decapoda-research/llama-30b-hf &            0.111 & 0.192 & 0.035 & 0.053 & 0.170 & 0.253 & 0.276 & 0.373 & 0.276 & 0.024 & 0.094 & 0.062 & 0.044 & 0.148 & 0.215 \\
decapoda-research/llama-65b-hf &            0.143 & 0.195 & 0.188 & 0.371 & 0.361 & 0.192 & 0.132 & 0.101 & 0.059 & 0.157 & 0.099 & 0.123 & 0.237 & 0.197 & 0.149 \\
\hline
project-baize/baize-lora-7B &            0.243 & 0.163 & 0.121 & 0.250 & 0.279 & 0.216 & 0.152 & 0.268 & 0.144 & 0.176 & 0.194 & 0.171 & 0.213 & 0.236 & 0.194 \\
project-baize/baize-healthcare-lora-7B &            0.169 & 0.137 & 0.122 & 0.078 & 0.093 & 0.072 & 0.247 & 0.092 & 0.115 & 0.177 & 0.052 & 0.249 & 0.132 & 0.075 & 0.160 \\
project-baize/baize-lora-13B &            0.210 & 0.230 & 0.207 & 0.276 & 0.253 & 0.254 & 0.220 & 0.240 & 0.215 & 0.211 & 0.244 & 0.259 & 0.244 & 0.249 & 0.257 \\
project-baize/baize-lora-30B &            0.064 & 0.146 & 0.256 & 0.222 & 0.277 & -1.000 & 0.051 & 0.210 & 0.150 & 0.038 & 0.090 & 0.035 & 0.161 & 0.218 & 0.035 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.153 & 0.138 & 0.142 & 0.228 & 0.150 & 0.159 & 0.172 & 0.167 & 0.163 & 0.272 & 0.131 & 0.172 & 0.251 & 0.140 & 0.165 \\
BelleGroup/BELLE-7B-0.6M &            0.171 & 0.149 & 0.207 & 0.254 & 0.129 & 0.123 & 0.174 & 0.161 & 0.228 & 0.192 & 0.143 & 0.218 & 0.223 & 0.136 & 0.170 \\
BelleGroup/BELLE-7B-1M &            0.159 & 0.119 & 0.149 & 0.242 & 0.079 & 0.099 & 0.163 & 0.168 & 0.239 & 0.231 & 0.115 & 0.232 & 0.237 & 0.097 & 0.166 \\
BelleGroup/BELLE-7B-2M &            0.133 & 0.166 & 0.153 & 0.143 & 0.106 & 0.176 & 0.146 & 0.163 & 0.186 & 0.200 & 0.193 & 0.147 & 0.157 & 0.150 & 0.170 \\
\hline
THUDM/chatglm-6b &            0.086 & 0.096 & 0.145 & 0.167 & 0.110 & 0.087 & 0.052 & 0.107 & 0.139 & 0.110 & 0.082 & 0.390 & 0.150 & 0.102 & 0.198 \\
THUDM/doctorglm-6b &            0.041 & 0.043 & 0.086 & 0.074 & 0.055 & 0.031 & 0.025 & 0.031 & 0.024 & 0.172 & 0.044 & 0.097 & 0.135 & 0.048 & 0.072 \\
\hline
fnlp/moss-moon-003-base &            0.083 & 0.066 & 0.062 & 0.119 & 0.091 & 0.118 & 0.130 & 0.080 & 0.059 & 0.178 & 0.071 & 0.079 & 0.149 & 0.081 & 0.100 \\
fnlp/moss-moon-003-sft &            0.059 & 0.088 & 0.113 & 0.071 & 0.050 & 0.046 & 0.045 & 0.078 & 0.090 & 0.091 & 0.060 & 0.074 & 0.081 & 0.055 & 0.060 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.143 & 0.144 & 0.122 & 0.161 & 0.252 & 0.229 & 0.137 & 0.266 & 0.220 & 0.208 & 0.208 & 0.150 & 0.185 & 0.230 & 0.189 \\
lmsys/vicuna-13b-delta-v1.1 &            0.150 & 0.148 & 0.136 & 0.080 & 0.083 & 0.115 & 0.098 & 0.115 & 0.174 & 0.138 & 0.157 & 0.139 & 0.109 & 0.120 & 0.127 \\
tloen/alpaca-lora-7b &            0.084 & 0.120 & 0.122 & 0.121 & 0.174 & 0.140 & 0.140 & 0.058 & 0.096 & 0.185 & 0.189 & 0.106 & 0.153 & 0.181 & 0.123 \\
\hline
EleutherAI/pythia-1.4b &            0.136 & 0.148 & 0.132 & 0.217 & 0.264 & 0.182 & 0.038 & 0.065 & 0.044 & 0.269 & 0.194 & 0.170 & 0.241 & 0.232 & 0.176 \\
EleutherAI/pythia-2.8b &            0.091 & 0.097 & 0.087 & 0.046 & 0.104 & 0.127 & 0.106 & 0.163 & 0.183 & 0.219 & 0.211 & 0.115 & 0.141 & 0.153 & 0.122 \\
EleutherAI/pythia-6.9b &            0.090 & 0.086 & 0.074 & 0.116 & 0.052 & 0.076 & 0.068 & 0.098 & 0.097 & 0.129 & 0.148 & 0.158 & 0.122 & 0.101 & 0.117 \\
EleutherAI/pythia-12b &            0.072 & 0.165 & 0.185 & 0.086 & 0.081 & 0.063 & 0.134 & -1.000 & 0.317 & 0.111 & 0.163 & 0.107 & 0.099 & 0.122 & 0.085 \\
\hline
EleutherAI/gpt-neox-20b &            0.193 & 0.124 & 0.188 & 0.115 & 0.159 & 0.180 & 0.113 & 0.132 & 0.108 & 0.320 & 0.298 & 0.382 & 0.175 & 0.226 & 0.277 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.060 & 0.062 & 0.075 & 0.116 & 0.043 & 0.077 & 0.073 & 0.043 & 0.099 & 0.220 & 0.074 & 0.094 & 0.168 & 0.058 & 0.085 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.174 & 0.333 & -1.000 & 0.129 & 0.061 & 0.124 & 0.101 & 0.113 & 0.060 & 0.087 & 0.066 & 0.097 & 0.108 & 0.064 & 0.110 \\
\hline
databricks/dolly-v2-3b &            0.102 & 0.103 & 0.099 & 0.110 & 0.058 & 0.083 & 0.107 & 0.092 & 0.095 & 0.075 & 0.082 & 0.158 & 0.092 & 0.071 & 0.104 \\
databricks/dolly-v2-7b &            0.085 & 0.102 & 0.071 & 0.073 & 0.037 & 0.053 & 0.166 & 0.114 & 0.088 & 0.128 & 0.058 & 0.133 & 0.100 & 0.047 & 0.092 \\
databricks/dolly-v2-12b &            0.087 & 0.123 & 0.102 & 0.113 & 0.087 & 0.168 & 0.108 & 0.131 & 0.148 & 0.074 & 0.108 & 0.154 & 0.094 & 0.097 & 0.161 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.087 & 0.072 & 0.076 & 0.048 & 0.053 & 0.049 & 0.063 & 0.091 & 0.098 & 0.052 & 0.082 & 0.066 & 0.050 & 0.068 & 0.058 \\
stabilityai/stablelm-tuned-alpha-7b &            0.075 & 0.116 & 0.159 & 0.106 & 0.104 & 0.069 & 0.132 & 0.144 & 0.118 & 0.122 & 0.117 & 0.104 & 0.114 & 0.111 & 0.087 \\
\hline
tiiuae/falcon-7b &            0.122 & 0.099 & 0.130 & 0.207 & 0.150 & 0.117 & 0.064 & 0.075 & 0.072 & 0.067 & 0.284 & 0.275 & 0.142 & 0.212 & 0.190 \\
tiiuae/falcon-7b-instruct &            0.141 & 0.094 & 0.099 & 0.064 & 0.092 & 0.049 & 0.088 & 0.112 & 0.040 & 0.119 & 0.142 & 0.065 & 0.092 & 0.119 & 0.058 \\
tiiuae/falcon-40b &            0.044 & 0.026 & 0.034 & 0.026 & 0.025 & 0.037 & 0.039 & 0.058 & 0.042 & 0.071 & 0.038 & 0.228 & 0.054 & 0.033 & 0.157 \\
tiiuae/falcon-40b-instruct &            0.070 & 0.065 & 0.048 & 0.068 & 0.052 & 0.037 & 0.057 & 0.123 & 0.068 & 0.142 & 0.142 & 0.090 & 0.121 & 0.116 & 0.075 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.281 & 0.405 & 0.460 & 0.482 & 0.619 & 0.675 & 0.251 & 0.403 & 0.472 & 0.078 & 0.202 & 0.261 & 0.280 & 0.411 & 0.468 \\
gpt4 &            0.379 & 0.418 & 0.478 & 0.389 & 0.428 & 0.489 & 0.512 & 0.557 & 0.632 & 0.555 & 0.599 & 0.678 & 0.472 & 0.513 & 0.583 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.137 & 0.147 & 0.127 & 0.162 & 0.141 & 0.117 & 0.142 & 0.138 & 0.162 & 0.163 & 0.145 & 0.165 & 0.162 & 0.144 & 0.153\\
Performance-Average & 0.064 & 0.078 & 0.189 & 0.120 & 0.112 & 0.200 & 0.086 & 0.195 & 0.111 & 0.090 & 0.091 & 0.110 & 0.084 & 0.089 & 0.097\\
\bottomrule
\end{tabular}
}
\caption{The performance of Pedagogy.}
\end{table}

==> tables/domain_experiments_table/table_phi.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.101 & 0.124 & 0.121 & 0.119 & 0.134 & 0.100 & 0.114 & 0.123 & 0.134 & 0.159 & 0.140 & 0.173 & 0.137 & 0.137 & 0.132 \\
bigscience/bloomz-1b1 &            0.117 & 0.098 & 0.093 & 0.145 & 0.131 & 0.099 & 0.114 & 0.113 & 0.104 & 0.140 & 0.157 & 0.135 & 0.143 & 0.142 & 0.115 \\
bigscience/bloomz-1b7 &            0.143 & 0.160 & 0.149 & 0.139 & 0.138 & 0.116 & 0.149 & 0.253 & 0.147 & 0.172 & 0.189 & 0.212 & 0.153 & 0.160 & 0.159 \\
bigscience/bloomz-3b &            0.255 & 0.222 & 0.203 & 0.192 & 0.147 & 0.141 & 0.149 & 0.161 & 0.179 & 0.150 & 0.130 & 0.147 & 0.173 & 0.139 & 0.143 \\
bigscience/bloomz-7b1-mt &            0.181 & 0.248 & 0.218 & 0.164 & 0.155 & 0.289 & 0.168 & 0.215 & 0.157 & 0.184 & 0.264 & 0.275 & 0.173 & 0.203 & 0.283 \\
bigscience/bloomz-7b1 &            0.203 & 0.211 & 0.213 & 0.155 & 0.141 & 0.280 & 0.168 & 0.202 & 0.181 & 0.227 & 0.186 & 0.287 & 0.187 & 0.153 & 0.282 \\
bigscience/bloomz-7b1-p3 &            0.199 & 0.235 & 0.165 & 0.139 & 0.132 & 0.213 & 0.197 & 0.159 & 0.163 & 0.108 & 0.126 & 0.123 & 0.130 & 0.130 & 0.189 \\
bigscience/bloomz &            0.256 & 0.172 & 0.385 & 0.027 & 0.025 & 0.022 & 0.270 & 0.081 & 0.177 & 0.040 & 0.031 & 0.030 & 0.035 & 0.029 & 0.027 \\
bigscience/bloomz-mt &            0.343 & 0.166 & 0.256 & 0.469 & 0.183 & 0.268 & 0.121 & 0.083 & 0.069 & 0.442 & 0.089 & 0.148 & 0.453 & 0.128 & 0.198 \\
bigscience/bloomz-p3 &            0.308 & 0.210 & 0.188 & 0.100 & 0.106 & 0.037 & 0.097 & 0.061 & 0.047 & 0.190 & 0.204 & -1.000 & 0.156 & 0.167 & 0.037 \\
\hline
decapoda-research/llama-7b-hf &            0.189 & 0.159 & 0.120 & 0.217 & 0.172 & 0.183 & 0.192 & 0.178 & 0.259 & 0.261 & 0.207 & 0.163 & 0.241 & 0.191 & 0.172 \\
decapoda-research/llama-13b-hf &            0.136 & 0.206 & 0.216 & 0.210 & 0.193 & 0.256 & 0.251 & 0.230 & 0.296 & 0.167 & 0.171 & 0.194 & 0.186 & 0.180 & 0.224 \\
decapoda-research/llama-30b-hf &            0.129 & 0.202 & 0.058 & 0.166 & 0.184 & 0.301 & 0.461 & 0.361 & 0.266 & 0.151 & 0.093 & 0.300 & 0.161 & 0.147 & 0.301 \\
decapoda-research/llama-65b-hf &            0.149 & 0.039 & 0.033 & 0.078 & 0.050 & 0.042 & 0.094 & 0.036 & 0.058 & 0.179 & 0.286 & 0.191 & 0.140 & 0.196 & 0.133 \\
\hline
project-baize/baize-lora-7B &            0.214 & 0.216 & 0.104 & 0.203 & 0.286 & 0.170 & 0.196 & 0.214 & 0.254 & 0.146 & 0.165 & 0.153 & 0.172 & 0.220 & 0.161 \\
project-baize/baize-healthcare-lora-7B &            0.187 & 0.182 & 0.108 & 0.241 & 0.199 & 0.336 & 0.297 & 0.104 & 0.321 & 0.166 & 0.287 & 0.218 & 0.189 & 0.252 & 0.257 \\
project-baize/baize-lora-13B &            0.164 & 0.192 & 0.276 & 0.133 & 0.142 & 0.216 & 0.250 & 0.247 & 0.241 & 0.157 & 0.172 & 0.275 & 0.146 & 0.159 & 0.248 \\
project-baize/baize-lora-30B &            0.088 & 0.164 & 0.174 & 0.286 & 0.249 & -1.000 & 0.335 & 0.282 & 0.157 & 0.075 & 0.127 & 0.372 & 0.176 & 0.178 & 0.372 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.183 & 0.154 & 0.216 & 0.186 & 0.253 & 0.268 & 0.168 & 0.171 & 0.117 & 0.260 & 0.262 & 0.272 & 0.228 & 0.258 & 0.270 \\
BelleGroup/BELLE-7B-0.6M &            0.206 & 0.151 & 0.189 & 0.181 & 0.200 & 0.233 & 0.191 & 0.184 & 0.106 & 0.256 & 0.192 & 0.282 & 0.222 & 0.196 & 0.260 \\
BelleGroup/BELLE-7B-1M &            0.159 & 0.167 & 0.165 & 0.176 & 0.126 & 0.117 & 0.172 & 0.187 & 0.152 & 0.267 & 0.226 & 0.387 & 0.226 & 0.181 & 0.265 \\
BelleGroup/BELLE-7B-2M &            0.155 & 0.175 & 0.123 & 0.179 & 0.078 & 0.164 & 0.143 & 0.172 & 0.112 & 0.286 & 0.303 & 0.314 & 0.210 & 0.202 & 0.204 \\
\hline
THUDM/chatglm-6b &            0.088 & 0.087 & 0.107 & 0.121 & 0.066 & 0.093 & 0.108 & 0.112 & 0.135 & 0.077 & 0.160 & 0.122 & 0.107 & 0.097 & 0.107 \\
THUDM/doctorglm-6b &            0.031 & 0.020 & 0.028 & 0.027 & 0.044 & 0.051 & 0.026 & 0.037 & 0.029 & 0.066 & 0.038 & 0.049 & 0.050 & 0.040 & 0.050 \\
\hline
fnlp/moss-moon-003-base &            0.124 & 0.036 & 0.045 & 0.161 & 0.042 & 0.034 & 0.231 & 0.036 & 0.049 & 0.162 & 0.038 & 0.035 & 0.161 & 0.040 & 0.034 \\
fnlp/moss-moon-003-sft &            0.082 & 0.079 & 0.104 & 0.061 & 0.100 & 0.083 & 0.028 & 0.067 & 0.043 & 0.063 & 0.052 & 0.046 & 0.062 & 0.072 & 0.062 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.208 & 0.204 & 0.229 & 0.250 & 0.301 & 0.257 & 0.134 & 0.188 & 0.084 & 0.200 & 0.193 & 0.155 & 0.222 & 0.240 & 0.200 \\
lmsys/vicuna-13b-delta-v1.1 &            0.203 & 0.176 & 0.176 & 0.255 & 0.248 & 0.177 & 0.051 & 0.051 & 0.026 & 0.197 & 0.184 & 0.142 & 0.223 & 0.213 & 0.157 \\
tloen/alpaca-lora-7b &            0.110 & 0.173 & 0.108 & 0.190 & 0.093 & 0.066 & 0.182 & 0.059 & 0.085 & 0.138 & 0.138 & 0.083 & 0.162 & 0.117 & 0.075 \\
\hline
EleutherAI/pythia-1.4b &            0.136 & 0.141 & 0.154 & 0.320 & 0.143 & 0.194 & 0.187 & 0.065 & 0.044 & 0.321 & 0.140 & 0.097 & 0.321 & 0.141 & 0.141 \\
EleutherAI/pythia-2.8b &            0.095 & 0.101 & 0.091 & 0.086 & 0.155 & 0.057 & 0.052 & 0.102 & 0.051 & 0.077 & 0.167 & 0.137 & 0.081 & 0.161 & 0.103 \\
EleutherAI/pythia-6.9b &            0.120 & 0.106 & 0.095 & 0.161 & 0.068 & 0.069 & 0.089 & 0.055 & 0.071 & 0.129 & 0.190 & 0.169 & 0.143 & 0.136 & 0.124 \\
EleutherAI/pythia-12b &            0.097 & 0.194 & 0.209 & 0.075 & 0.146 & 0.128 & 0.162 & 0.043 & 0.160 & 0.196 & 0.123 & 0.145 & 0.142 & 0.134 & 0.137 \\
\hline
EleutherAI/gpt-neox-20b &            0.226 & 0.071 & 0.121 & 0.159 & 0.198 & 0.114 & 0.144 & 0.048 & 0.082 & 0.187 & 0.194 & 0.145 & 0.169 & 0.196 & 0.131 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.060 & 0.034 & 0.030 & 0.155 & 0.064 & 0.078 & 0.064 & 0.097 & 0.128 & 0.156 & 0.113 & 0.095 & 0.155 & 0.091 & 0.087 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.106 & 0.028 & -1.000 & 0.153 & 0.052 & 0.104 & 0.080 & 0.054 & 0.065 & 0.095 & 0.082 & 0.063 & 0.121 & 0.068 & 0.081 \\
\hline
databricks/dolly-v2-3b &            0.117 & 0.121 & 0.127 & 0.070 & 0.055 & 0.129 & 0.138 & 0.144 & 0.117 & 0.082 & 0.074 & 0.186 & 0.077 & 0.065 & 0.147 \\
databricks/dolly-v2-7b &            0.093 & 0.109 & 0.076 & 0.064 & 0.059 & 0.052 & 0.138 & 0.117 & 0.087 & 0.174 & 0.087 & 0.133 & 0.126 & 0.075 & 0.098 \\
databricks/dolly-v2-12b &            0.091 & 0.121 & 0.108 & 0.131 & 0.116 & 0.156 & 0.148 & 0.172 & 0.078 & 0.103 & 0.169 & 0.137 & 0.116 & 0.145 & 0.146 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.097 & 0.076 & 0.087 & 0.045 & 0.057 & 0.045 & 0.065 & 0.070 & 0.038 & 0.053 & 0.055 & 0.050 & 0.049 & 0.056 & 0.047 \\
stabilityai/stablelm-tuned-alpha-7b &            0.114 & 0.144 & 0.175 & 0.166 & 0.089 & 0.117 & 0.149 & 0.162 & 0.147 & 0.141 & 0.089 & 0.086 & 0.152 & 0.089 & 0.100 \\
\hline
tiiuae/falcon-7b &            0.088 & 0.095 & 0.071 & 0.239 & 0.124 & 0.088 & 0.027 & 0.028 & 0.030 & 0.180 & 0.125 & 0.133 & 0.204 & 0.125 & 0.115 \\
tiiuae/falcon-7b-instruct &            0.064 & 0.039 & 0.068 & 0.210 & 0.104 & 0.228 & 0.027 & 0.158 & 0.049 & 0.066 & 0.125 & 0.118 & 0.120 & 0.118 & 0.155 \\
tiiuae/falcon-40b &            0.065 & 0.080 & 0.061 & 0.024 & 0.027 & 0.029 & 0.027 & 0.025 & 0.025 & 0.083 & 0.045 & 0.046 & 0.060 & 0.039 & 0.039 \\
tiiuae/falcon-40b-instruct &            0.247 & 0.238 & 0.178 & 0.060 & 0.035 & 0.142 & 0.071 & 0.034 & 0.036 & 0.074 & 0.043 & 0.071 & 0.069 & 0.040 & 0.094 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.199 & 0.314 & 0.367 & 0.247 & 0.352 & 0.398 & 0.344 & 0.455 & 0.501 & 0.707 & 0.859 & 0.917 & 0.477 & 0.606 & 0.657 \\
gpt4 &            0.318 & 0.359 & 0.416 & 0.329 & 0.368 & 0.425 & 0.478 & 0.521 & 0.593 & 0.497 & 0.545 & 0.619 & 0.413 & 0.457 & 0.522 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.154 & 0.149 & 0.128 & 0.163 & 0.139 & 0.131 & 0.158 & 0.143 & 0.137 & 0.179 & 0.171 & 0.162 & 0.171 & 0.156 & 0.171\\
Performance-Average & 0.071 & 0.073 & 0.188 & 0.086 & 0.083 & 0.194 & 0.101 & 0.106 & 0.115 & 0.120 & 0.135 & 0.230 & 0.092 & 0.100 & 0.120\\
\bottomrule
\end{tabular}
}
\caption{The performance of Philosophy.}
\end{table}

==> tables/domain_experiments_table/table_sci.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c|}{Xiezhi-Inter.-English} & \multicolumn{3}{|c}{Xiezhi}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                  & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{15}{c}{Generation Probability For Ranking}\\
\hline
bigscience/bloomz-560m &            0.107 & 0.111 & 0.111 & 0.104 & 0.099 & 0.112 & 0.141 & 0.144 & 0.154 & 0.126 & 0.123 & 0.157 & 0.114 & 0.110 & 0.133 \\
bigscience/bloomz-1b1 &            0.133 & 0.096 & 0.096 & 0.117 & 0.110 & 0.117 & 0.134 & 0.143 & 0.136 & 0.152 & 0.123 & 0.153 & 0.133 & 0.116 & 0.134 \\
bigscience/bloomz-1b7 &            0.158 & 0.134 & 0.130 & 0.120 & 0.131 & 0.136 & 0.149 & 0.223 & 0.155 & 0.159 & 0.161 & 0.234 & 0.138 & 0.145 & 0.182 \\
bigscience/bloomz-3b &            0.180 & 0.146 & 0.156 & 0.212 & 0.149 & 0.147 & 0.159 & 0.187 & 0.179 & 0.186 & 0.155 & 0.165 & 0.200 & 0.151 & 0.155 \\
bigscience/bloomz-7b1-mt &            0.150 & 0.184 & 0.166 & 0.159 & 0.138 & 0.203 & 0.146 & 0.161 & 0.149 & 0.203 & 0.194 & 0.196 & 0.179 & 0.164 & 0.200 \\
bigscience/bloomz-7b1 &            0.166 & 0.189 & 0.138 & 0.150 & 0.135 & 0.203 & 0.151 & 0.198 & 0.151 & 0.201 & 0.114 & 0.199 & 0.173 & 0.130 & 0.202 \\
bigscience/bloomz-7b1-p3 &            0.181 & 0.201 & 0.144 & 0.116 & 0.112 & 0.137 & 0.188 & 0.177 & 0.160 & 0.171 & 0.068 & 0.092 & 0.135 & 0.103 & 0.128 \\
bigscience/bloomz &            0.212 & 0.187 & 0.262 & 0.067 & 0.047 & 0.042 & 0.144 & 0.094 & 0.198 & 0.042 & 0.040 & 0.035 & 0.053 & 0.043 & 0.038 \\
bigscience/bloomz-mt &            0.277 & 0.198 & 0.212 & 0.353 & 0.211 & 0.092 & 0.281 & 0.250 & 0.347 & 0.449 & 0.312 & 0.278 & 0.408 & 0.269 & 0.199 \\
bigscience/bloomz-p3 &            0.118 & 0.069 & 0.071 & 0.114 & 0.055 & 0.037 & 0.085 & 0.051 & 0.074 & 0.139 & 0.130 & 0.078 & 0.128 & 0.096 & 0.051 \\
\hline
decapoda-research/llama-7b-hf &            0.138 & 0.126 & 0.115 & 0.108 & 0.152 & 0.166 & 0.137 & 0.100 & 0.135 & 0.173 & 0.170 & 0.160 & 0.139 & 0.161 & 0.163 \\
decapoda-research/llama-13b-hf &            0.120 & 0.221 & 0.261 & 0.134 & 0.153 & 0.221 & 0.187 & 0.182 & 0.302 & 0.127 & 0.172 & 0.196 & 0.130 & 0.162 & 0.211 \\
decapoda-research/llama-30b-hf &            0.140 & 0.208 & 0.159 & 0.086 & 0.169 & 0.162 & 0.198 & 0.199 & 0.227 & 0.058 & 0.156 & 0.218 & 0.077 & 0.165 & 0.180 \\
decapoda-research/llama-65b-hf &            0.146 & 0.140 & 0.073 & 0.112 & 0.154 & 0.135 & 0.113 & 0.073 & 0.099 & 0.135 & 0.196 & 0.154 & 0.125 & 0.178 & 0.145 \\
\hline
project-baize/baize-lora-7B &            0.221 & 0.148 & 0.117 & 0.161 & 0.165 & 0.194 & 0.158 & 0.119 & 0.174 & 0.173 & 0.166 & 0.204 & 0.167 & 0.166 & 0.199 \\
project-baize/baize-healthcare-lora-7B &            0.160 & 0.137 & 0.115 & 0.147 & 0.117 & 0.153 & 0.273 & 0.115 & 0.106 & 0.174 & 0.139 & 0.138 & 0.163 & 0.127 & 0.146 \\
project-baize/baize-lora-13B &            0.149 & 0.199 & 0.241 & 0.200 & 0.195 & 0.267 & 0.202 & 0.166 & 0.195 & 0.159 & 0.167 & 0.297 & 0.180 & 0.181 & 0.281 \\
project-baize/baize-lora-30B &            0.110 & 0.226 & 0.196 & 0.156 & 0.246 & -1.000 & 0.493 & 0.269 & 0.214 & 0.064 & 0.170 & 0.197 & 0.117 & 0.214 & 0.197 \\
\hline
BelleGroup/BELLE-7B-0.2M &            0.164 & 0.110 & 0.144 & 0.195 & 0.144 & 0.141 & 0.161 & 0.162 & 0.156 & 0.187 & 0.135 & 0.194 & 0.191 & 0.140 & 0.167 \\
BelleGroup/BELLE-7B-0.6M &            0.187 & 0.132 & 0.189 & 0.177 & 0.162 & 0.175 & 0.170 & 0.171 & 0.184 & 0.217 & 0.193 & 0.200 & 0.197 & 0.177 & 0.187 \\
BelleGroup/BELLE-7B-1M &            0.163 & 0.144 & 0.131 & 0.188 & 0.116 & 0.130 & 0.162 & 0.166 & 0.175 & 0.234 & 0.142 & 0.204 & 0.210 & 0.129 & 0.166 \\
BelleGroup/BELLE-7B-2M &            0.156 & 0.168 & 0.116 & 0.153 & 0.095 & 0.168 & 0.132 & 0.154 & 0.141 & 0.153 & 0.168 & 0.138 & 0.153 & 0.130 & 0.161 \\
\hline
THUDM/chatglm-6b &            0.074 & 0.092 & 0.132 & 0.119 & 0.135 & 0.125 & 0.087 & 0.089 & 0.117 & 0.089 & 0.092 & 0.128 & 0.111 & 0.123 & 0.126 \\
THUDM/doctorglm-6b &            0.042 & 0.071 & 0.043 & 0.063 & 0.049 & 0.037 & 0.075 & 0.045 & 0.043 & 0.093 & 0.069 & 0.060 & 0.080 & 0.060 & 0.050 \\
\hline
fnlp/moss-moon-003-base &            0.094 & 0.050 & 0.050 & 0.101 & 0.057 & 0.065 & 0.122 & 0.049 & 0.062 & 0.089 & 0.045 & 0.047 & 0.095 & 0.051 & 0.057 \\
fnlp/moss-moon-003-sft &            0.055 & 0.060 & 0.064 & 0.073 & 0.063 & 0.047 & 0.048 & 0.075 & 0.067 & 0.045 & 0.052 & 0.044 & 0.059 & 0.058 & 0.045 \\
\hline
lmsys/vicuna-7b-delta-v1.1 &            0.144 & 0.159 & 0.178 & 0.195 & 0.230 & 0.201 & 0.128 & 0.217 & 0.251 & 0.180 & 0.223 & 0.185 & 0.188 & 0.227 & 0.193 \\
lmsys/vicuna-13b-delta-v1.1 &            0.151 & 0.168 & 0.153 & 0.127 & 0.155 & 0.122 & 0.151 & 0.149 & 0.197 & 0.155 & 0.189 & 0.179 & 0.140 & 0.171 & 0.149 \\
tloen/alpaca-lora-7b &            0.100 & 0.129 & 0.115 & 0.177 & 0.155 & 0.138 & 0.154 & 0.118 & 0.095 & 0.182 & 0.170 & 0.156 & 0.180 & 0.162 & 0.146 \\
\hline
EleutherAI/pythia-1.4b &            0.112 & 0.099 & 0.105 & 0.150 & 0.135 & 0.170 & 0.135 & 0.160 & 0.142 & 0.134 & 0.106 & 0.115 & 0.142 & 0.121 & 0.144 \\
EleutherAI/pythia-2.8b &            0.101 & 0.099 & 0.104 & 0.130 & 0.105 & 0.102 & 0.113 & 0.120 & 0.132 & 0.096 & 0.156 & 0.091 & 0.112 & 0.129 & 0.097 \\
EleutherAI/pythia-6.9b &            0.074 & 0.099 & 0.101 & 0.083 & 0.063 & 0.063 & 0.089 & 0.090 & 0.088 & 0.090 & 0.085 & 0.070 & 0.087 & 0.074 & 0.067 \\
EleutherAI/pythia-12b &            0.104 & 0.129 & 0.137 & 0.080 & 0.089 & 0.110 & 0.130 & -1.000 & 0.195 & 0.093 & 0.121 & 0.121 & 0.086 & 0.105 & 0.115 \\
\hline
EleutherAI/gpt-neox-20b &            0.150 & 0.114 & 0.113 & 0.082 & 0.099 & 0.135 & 0.148 & 0.113 & 0.091 & 0.118 & 0.144 & 0.212 & 0.093 & 0.122 & 0.173 \\
h2oai/h2ogpt-gm-oasst1-en-1024-12b &            0.061 & 0.047 & 0.059 & 0.097 & 0.051 & 0.065 & 0.084 & 0.068 & 0.095 & 0.116 & 0.080 & 0.064 & 0.106 & 0.065 & 0.065 \\
h2oai/h2ogpt-gm-oasst1-en-1024-20b &            0.118 & 0.048 & 0.028 & 0.102 & 0.066 & 0.064 & 0.097 & 0.091 & 0.082 & 0.133 & 0.068 & 0.068 & 0.117 & 0.067 & 0.066 \\
\hline
databricks/dolly-v2-3b &            0.091 & 0.077 & 0.078 & 0.086 & 0.054 & 0.072 & 0.086 & 0.086 & 0.085 & 0.084 & 0.059 & 0.081 & 0.085 & 0.056 & 0.075 \\
databricks/dolly-v2-7b &            0.107 & 0.088 & 0.088 & 0.078 & 0.045 & 0.076 & 0.094 & 0.085 & 0.087 & 0.083 & 0.076 & 0.082 & 0.081 & 0.060 & 0.079 \\
databricks/dolly-v2-12b &            0.107 & 0.102 & 0.102 & 0.099 & 0.073 & 0.102 & 0.108 & 0.105 & 0.121 & 0.076 & 0.100 & 0.134 & 0.088 & 0.086 & 0.117 \\
\hline
stabilityai/stablelm-tuned-alpha-3b &            0.089 & 0.068 & 0.070 & 0.072 & 0.075 & 0.090 & 0.062 & 0.059 & 0.048 & 0.046 & 0.056 & 0.079 & 0.060 & 0.066 & 0.085 \\
stabilityai/stablelm-tuned-alpha-7b &            0.061 & 0.097 & 0.104 & 0.122 & 0.103 & 0.096 & 0.098 & 0.097 & 0.064 & 0.131 & 0.089 & 0.088 & 0.126 & 0.096 & 0.092 \\
\hline
tiiuae/falcon-7b &            0.042 & 0.035 & 0.048 & 0.146 & 0.106 & 0.087 & 0.119 & 0.146 & 0.178 & 0.169 & 0.174 & 0.224 & 0.157 & 0.139 & 0.153 \\
tiiuae/falcon-7b-instruct &            0.054 & 0.061 & 0.089 & 0.143 & 0.159 & 0.103 & 0.040 & 0.105 & 0.138 & 0.155 & 0.213 & 0.196 & 0.149 & 0.186 & 0.149 \\
tiiuae/falcon-40b &            0.038 & 0.033 & 0.053 & 0.060 & 0.047 & 0.062 & 0.061 & 0.089 & 0.051 & 0.084 & 0.035 & 0.041 & 0.074 & 0.040 & 0.050 \\
tiiuae/falcon-40b-instruct &            0.116 & 0.093 & 0.071 & 0.057 & 0.126 & 0.107 & 0.056 & 0.055 & 0.039 & 0.043 & 0.061 & 0.072 & 0.049 & 0.089 & 0.087 \\
\hline
&\multicolumn{15}{c}{Instruction For Ranking}\\
\hline
gpt35 &            0.201 & 0.330 & 0.389 & 0.190 & 0.331 & 0.397 & 0.261 & 0.420 & 0.493 & 0.250 & 0.400 & 0.469 & 0.220 & 0.366 & 0.433 \\
gpt4 &            0.430 & 0.467 & 0.530 & 0.431 & 0.470 & 0.533 & 0.434 & 0.475 & 0.541 & 0.440 & 0.480 & 0.547 & 0.436 & 0.475 & 0.540 \\
\hline
&\multicolumn{15}{c}{Statistic}\\
\hline
Performance-Average & 0.133 & 0.134 & 0.135 & 0.136 & 0.130 & 0.113 & 0.148 & 0.119 & 0.156 & 0.146 & 0.143 & 0.158 & 0.141 & 0.137 & 0.148\\
Performance-Average & 0.067 & 0.077 & 0.088 & 0.068 & 0.077 & 0.186 & 0.085 & 0.185 & 0.100 & 0.081 & 0.085 & 0.098 & 0.074 & 0.079 & 0.090\\
\bottomrule
\end{tabular}
}
\caption{The performance of Science.}
\end{table}

==> tables/tabel_models_rlhf.tex <==
\begin{table}
    \small
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Model}& \textbf{\#Parameter} & \textbf{Base Model} & \textbf{\#Layer} & \textbf{\#Encoder} & \textbf{\#Decoder} & \textbf{\#Pretrain Tokens} & \textbf{\#IFT Sample} & \textbf{RLHF} \\
        \hline
        % T5-Base~\cite{2020t5}~\footnote{https://huggingface.co/t5-base} & 0.22B & - & 12 & 12 & 12 & - & - & - \\
        % BERT-large-uncased~\cite{2018bert}~\footnote{https://huggingface.co/bert-large-uncased} & 0.34B & - & 24 & 24 & - & 3.3B tokens & - & - \\
        % XLNet-large~\cite{2019xlnet}~\footnote{https://huggingface.co/xlnet-large-cased} & 0.34B & - & 24 & - & - & 158GB & - & - \\
        % GPT3-Ada~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 0.35B & - & 24 & - & 24 & - & - & - \\
        % BART-large~\cite{2019bart}~\footnote{https://huggingface.co/facebook/bart-large} & 0.406B & - & 12 & 12 & 12 & 3.2B tokens & - & - \\
        % BLOOM-560m~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-560m} & 0.56B & - & 24 & - & 24 & 350B tokens & - & - \\
        % BLOOMZ-560m~\cite{muennighoff2022crosslingual}~\footnote{https://huggingface.co/bigscience/bloomz-560m} & 0.56B & BLOOM-560m & 24 & - & 24 & - & 3.67B tokens & - \\
        Pythia-1B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-1b} & 1B & - & 16 & - & 16 & 300B tokens & - & - \\
        % GPT3-Babbage~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 1.3B & - & 24 & - & 24 & - & - & - \\
        % GPT2-XL~\cite{radford2019language}~\footnote{https://huggingface.co/gpt2-xl} & 1.5B & - & 48 & - & 48 & 40B tokens & - & - \\
        BLOOM-1b7~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-1b7} & 1.7B & - & 24 & - & 24 & 350B tokens & - & - \\
        BLOOMZ-1b7~\cite{muennighoff2022crosslingual}~\footnote{https://huggingface.co/bigscience/bloomz-1b7} & 1.7B & BLOOM-1b7 & 24 & - & 24 & - & 8.39B tokens & - \\
        Dolly-v2-3b~\cite{2023dolly}~\footnote{https://huggingface.co/databricks/dolly-v2-3b} & 2.8B & Pythia-2.8B & 32 & - & 32 & - & 15K & - \\
        Pythia-2.8B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-2.8b} & 2.8B & - & 32 & - & 32 & 300B tokens & - & - \\
        % BLOOM-3b~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-3b} & 3B & - & 30 & - & 30 & 350B tokens & - & - \\
        BLOOMZ-3b~\cite{muennighoff2022crosslingual}~\footnote{https://huggingface.co/bigscience/bloomz-3b} & 3B & BLOOM-3b & 30 & - & 30 & - & 8.39B tokens & - \\
        % FastChat-T5~\cite{2023fastchat}~\footnote{https://huggingface.co/lmsys/fastchat-t5-3b-v1.0} & 3B & FLAN-T5 XL & 24 & 24 & 24 & - & 70K & - \\
        % FLAN-T5 XL~\cite{chung2022scaling}~\footnote{https://huggingface.co/google/flan-t5-xl} & 3B & T5-XL & 24 & 24 & 24 & - & 1000+ tasks & - \\
        % StableLM-Base-Alpha-3B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-base-alpha-3b} & 3B & - & 16 & - & 16 & 800B tokens & - & - \\
        StableLM-Tuned-Alpha-3B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-tuned-alpha-3b} & 3B & StableLM-Base-Alpha-3B & 16 & - & 16 & - & 632K & - \\
        % T5-XL~\cite{2020t5}~\footnote{https://huggingface.co/t5-3b} & 3B & - & 24 & 24 & 24 & - & - & - \\
        ChatGLM-6B~\cite{zeng2023glm-130b,du2022glm}~\footnote{https://huggingface.co/THUDM/chatglm-6b} & 6B & - & 28 & 28 & 28 & 1T tokens & \checkmark & \checkmark \\
        DoctorGLM~\cite{xiong2023doctorglm}~\footnote{https://github.com/xionghonglin/DoctorGLM} & 6B & ChatGLM-6B & 28 & 28 & 28 & - & 6.38M & - \\
        % ChatGLM-Med~\cite{ChatGLM-Med}~\footnote{https://github.com/SCIR-HI/Med-ChatGLM} & 6B & ChatGLM-6B & 28 & 28 & 28 & - & 8K & - \\
        % GPT3-Curie~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 6.7B & - & 32 & - & 32 & - & - & - \\
        % MPT-7B-Chat~\cite{MosaicML2023Introducing}~\footnote{https://huggingface.co/mosaicml/mpt-7b-chat} & 6.7B & MPT-7B & 32 & - & 32 & - & 360K & - \\
        % MPT-7B-Instruct~\cite{MosaicML2023Introducing}~\footnote{https://huggingface.co/mosaicml/mpt-7b-instruct} & 6.7B & MPT-7B & 32 & - & 32 & - & 59.3K & - \\
        % MPT-7B-StoryWriter-65k+~\cite{MosaicML2023Introducing}~\footnote{https://huggingface.co/mosaicml/mpt-7b-storywriter} & 6.7B & MPT-7B & 32 & - & 32 & - & \checkmark & - \\
        Dolly-v2-7b~\cite{2023dolly}~\footnote{https://huggingface.co/databricks/dolly-v2-7b} & 6.9B & Pythia-6.9B & 32 & - & 32 & - & 15K & - \\
        h2ogpt-oig-oasst1-512-6.9b~\cite{2023h2ogpt}~\footnote{https://huggingface.co/h2oai/h2ogpt-oig-oasst1-512-6.9b} & 6.9B & Pythia-6.9B & 32 & - & 32 & - & 398K & - \\
        Pythia-6.9B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-6.9b} & 6.9B & - & 32 & - & 32 & 300B tokens & - & - \\
        Alpaca-7B~\cite{alpaca}~\footnote{https://huggingface.co/tatsu-lab/alpaca-7b-wdiff} & 7B & LLaMA-7B & 32 & - & 32 & - & 52K & - \\
        Alpaca-LoRA-7B~\cite{2023alpacalora}~\footnote{https://huggingface.co/tloen/alpaca-lora-7b} & 7B & LLaMA-7B & 32 & - & 32 & - & 52K & - \\
        Baize-7B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-lora-7B} & 7B & LLaMA-7B & 32 & - & 32 & - & 263K & - \\
        Baize Healthcare-7B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-healthcare-lora-7B} & 7B & LLaMA-7B & 32 & - & 32 & - & 201K & - \\
        % ChatDoctor~\cite{yunxiang2023chatdoctor}~\footnote{https://github.com/Kent0n-Li/ChatDoctor} & 7B & LLaMA-7B & 32 & - & 32 & - & 167K & - \\
        % HuaTuo~\cite{wang2023huatuo}~\footnote{https://github.com/scir-hi/huatuo-llama-med-chinese} & 7B & LLaMA-7B & 32 & - & 32 & - & 8K & - \\
        % Koala-7B~\cite{koala_blogpost_2023}~\footnote{https://huggingface.co/young-geng/koala} & 7B & LLaMA-7B & 32 & - & 32 & - & 472K & - \\
        LLaMA-7B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-7b-hf} & 7B & - & 32 & - & 32 & 1T tokens & - & - \\
        % Luotuo-lora-7b-0.3~\cite{luotuo}~\footnote{https://huggingface.co/silk-road/luotuo-lora-7b-0.3} & 7B & LLaMA-7B & 32 & - & 32 & - & 152K & - \\
        % PandaLM-7B~\cite{PandaLM}~\footnote{https://github.com/WeOpenML/PandaLM} & 7B & LLaMA-7B & 32 & - & 32 & - & 300K & - \\
        % StableLM-Base-Alpha-7B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-base-alpha-7b} & 7B & - & 16 & - & 16 & 800B tokens & - & - \\
        StableLM-Tuned-Alpha-7B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-tuned-alpha-7b} & 7B & StableLM-Base-Alpha-7B & 16 & - & 16 & - & 632K & - \\
        Vicuna-7b-delta-v1.1~\cite{vicuna2023}~\footnote{https://github.com/lm-sys/FastChat\#vicuna-weights} & 7B & LLaMA-7B & 32 & - & 32 & - & 70K & - \\
        BELLE-7B-0.2M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-0.2M}/0.6M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-0.6M}/1M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-1M}/2M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-2M}~\cite{belle2023exploring} & 7.1B & Bloomz-7b1-mt & 30 & - & 30 & - & 0.2M/0.6M/1M/2M & - \\
        BLOOM-7b1~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-7b1} & 7.1B & - & 30 & - & 30 & 350B tokens & - & - \\
        BLOOMZ-7b1~\footnote{https://huggingface.co/bigscience/bloomz-7b1}/mt~\footnote{https://huggingface.co/bigscience/bloomz-7b1-mt}/p3~\footnote{https://huggingface.co/bigscience/bloomz-7b1-p3}~\cite{muennighoff2022crosslingual} & 7.1B & BLOOM-7b1 & 30 & - & 30 & - & 4.19B tokens & - \\
        % FLAN-T5 XXL~\cite{chung2022scaling}~\footnote{https://huggingface.co/google/flan-t5-xxl} & 11B & T5-XXL & 24 & 24 & 24 & - & 1000+ tasks & - \\
        % T5-XXL~\cite{2020t5}~\footnote{https://huggingface.co/t5-11b} & 11B & - & 24 & 24 & 24 & 1T tokens & - & - \\
        Dolly-v2-12b~\cite{2023dolly}~\footnote{https://huggingface.co/databricks/dolly-v2-12b} & 12B & Pythia-12B & 36 & - & 36 & - & 15K & - \\
        h2ogpt-oasst1-512-12b~\cite{2023h2ogpt}~\footnote{https://huggingface.co/h2oai/h2ogpt-oasst1-512-12b} & 12B & Pythia-12B & 36 & - & 36 & - & 94.6K & - \\
        Open-Assistant-SFT-4-12B~\cite{2023openassistant}~\footnote{https://huggingface.co/OpenAssistant/oasst-sft-4-pythia-12b-epoch-3.5} & 12B & Pythia-12B-deduped & 36 & - & 36 & - & 161K & - \\
        Pythia-12B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-12b} & 12B & - & 36 & - & 36 & 300B tokens & - & - \\
        Baize-13B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-lora-13B} & 13B & LLaMA-13B & 40 & - & 40 & - & 263K & - \\
        % Koala-13B~\cite{koala_blogpost_2023}~\footnote{https://huggingface.co/young-geng/koala} & 13B & LLaMA-13B & 40 & - & 40 & - & 472K & - \\
        LLaMA-13B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-13b-hf} & 13B & - & 40 & - & 40 & 1T tokens & - & - \\
        %mT0-xxl~\footnote{https://huggingface.co/bigscience/mt0-xxl} & 13B & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} \\
        %mT0-xxl-mt~\footnote{https://huggingface.co/bigscience/mt0-xxl-mt} & 13B & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} \\
        %mT5-XXL~\cite{xue-etal-2021-mt5}~\footnote{https://console.cloud.google.com/storage/browser/t5-data/pretrained\_models/mt5/xxl/} & 13B & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} \\
        % StableVicuna-13B~\cite{2023StableLM}~\footnote{https://huggingface.co/CarperAI/stable-vicuna-13b-delta} & 13B & Vicuna-13B v0 & 40 & - & 40 & - & 613K & \checkmark \\
        Vicuna-13b-delta-v1.1~\cite{vicuna2023}~\footnote{https://github.com/lm-sys/FastChat\#vicuna-weights} & 13B & LLaMA-13B & 40 & - & 40 & - & 70K & - \\
        moss-moon-003-sft~\cite{2023moss}~\footnote{https://huggingface.co/fnlp/moss-moon-003-sft} & 16B & moss-moon-003-base & 34 & - & 34 & - & 1.1M & - \\
        moss-moon-003-sft-plugin~\cite{2023moss}~\footnote{https://huggingface.co/fnlp/moss-moon-003-sft-plugin} & 16B & moss-moon-003-base & 34 & - & 34 & - & 1.4M & - \\
        GPT-NeoX-20B~\cite{gptneox}~\footnote{https://huggingface.co/EleutherAI/gpt-neox-20b} & 20B & - & 44 & - & 44 & 825GB & - & - \\
        h2ogpt-oasst1-512-20b~\cite{2023h2ogpt}~\footnote{https://huggingface.co/h2oai/h2ogpt-oasst1-512-20b} & 20B & GPT-NeoX-20B & 44 & - & 44 & - & 94.6K & - \\
        % OPT-IML-30B~\cite{iyer2023optiml}~\footnote{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT-IML} & 30B & OPT-30B & 48 & - & 48 & - & 1500 tasks & - \\
        Baize-30B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-lora-30B} & 33B & LLaMA-30B & 60 & - & 60 & - & 263K & - \\
        LLaMA-30B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-30b-hf} & 33B & - & 60 & - & 60 & 1.4T tokens & - & - \\
        LLaMA-65B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-65b-hf} & 65B & - & 80 & - & 80 & 1.4T tokens & - & - \\
        % GLM-130B~\cite{zeng2023glm-130b}~\footnote{https://github.com/THUDM/GLM-130B} & 130B & - & 70 & 70 & 70 & 400B tokens & - & - \\
        % GPT3-Davinci~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 175B & - & 96 & - & 96 & 300B tokens & - & - \\
        % OPT-IML-175B~\cite{iyer2023optiml}~\footnote{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT-IML} & 175B & OPT-175B & 96 & - & 96 & - & 1500 tasks & - \\
        % BLOOM~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom} & 176B & - & 70 & - & 70 & 366B tokens & - & - \\
        BLOOMZ~\footnote{https://huggingface.co/bigscience/bloomz}/mt~\footnote{https://huggingface.co/bigscience/bloomz-mt}/p3~\footnote{https://huggingface.co/bigscience/bloomz-p3}~\cite{muennighoff2022crosslingual} & 176B & BLOOM & 70 & - & 70 & - & 2.09B tokens & - \\
        ChatGPT~(2023.05.01)~\cite{openaichatgpt}~\footnote{https://platform.openai.com/docs/models/gpt-3-5} & - & GPT-3.5 & - & - & - & - & \checkmark & \checkmark \\
        GPT-4~(2023.05.01)~\cite{openai2023gpt4}~\footnote{https://platform.openai.com/docs/models/gpt-4} & - & - & - & - & - & - & \checkmark & \checkmark \\
        \hline
    \end{tabular}
    }
    \vspace{3mm}
    \caption{The models we evaluted in our experiments.}
    \label{tab:models}
\end{table}

==> tables/table_baselines_comparison.tex <==
\begin{table}[!t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccc}
        \toprule
        Benchmark & Language & #Tasks & #Samples
         \\
        \hline
        MMLU~\cite{hendrycks2021measuring} & En & 57 & 15,908\\
        AGIEval~\cite{zhong2023agieval} & En & 20 & 8,062\\
        MMCU~\cite{zeng2023measuring} & Zh & 51 & 11,900\\
        M3KE~\cite{liu2023m3ke} & Zh & 71 & 20,477 \\
        C-Eval~\cite{huang2023ceval} & Zh & 54 & xxxx\\
        \hline
        \bottomrule
    \end{tabular}
    }
    \caption{Result on Xiezhi-Hard-English}
    \label{tab:detailedModelsPerformance}
\end{table}

% MMLU (Hendrycks et al., 2021) En 57 15,908
% AGIEval (Zhong et al., 2023) En & Zh 20 8,062
% MMCU (Zeng, 2023) Zh 51 11,900
% M3KE Zh 71 20,477

==> tables/table_cute_gpt.tex <==
\begin{table}[h]
    \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|c||ccc|ccc|ccc|ccc}
\toprule
\textbf{Models} & \multicolumn{3}{c|}{MMLU} & \multicolumn{3}{c|}{CEval} & \multicolumn{1}{c||}{M3KE} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c}{Xiezhi-Inter.-English}\\
& 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
\hline
Random-Guess                               & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
\hline
&\multicolumn{19}{c}{Generation Probability For Ranking}\\
\hline
cuteGPT-sft-7b                & 0.146 & 0.105 & 0.125 & 0.122 & 0.117 & 0.136 & 0.121 & 0.123 & 0.158 & 0.166 & 0.150 & 0.177 & 0.188 & 0.132 & 0.127 & 0.124 & \textbf{0.200} & 0.159 & 0.182 \\
cuteGPT-sft-616-13b               & 0.099 & \textbf{0.134} & \textbf{0.179} & 0.100 & 0.136 & 0.146 & 0.099 & 0.115 & 0.141 & 0.183 & 0.104 & 0.142 & 0.199 & 0.097 & 0.094 & 0.109 & 0.115 & 0.104 & 0.113\\
cuteGPT-sft-623-13b           & \textbf{0.154} & 0.092 & 0.051 & 0.143 & \textbf{0.191} & \textbf{0.157} & 0.103 & 0.170 & \textbf{0.204} & 0.143 & 0.180 & 0.221 & \textbf{0.202} & \textbf{0.141} & \textbf{0.189} & \textbf{0.209} & 0.174 & \textbf{0.215} & \textbf{0.255} \\
chatglm2-6B                   & 0.063 & 0.082 & 0.111 & \textbf{0.145} & 0.143 & 0.105 & \textbf{0.182} & \textbf{0.242} & 0.191 & \textbf{0.220} & \textbf{0.259} & \textbf{0.222} & 0.165 & 0.106 & 0.095 & 0.099 & 0.096 & 0.096 & 0.112 \\
chatglm-6B                    & 0.099 & 0.109 & 0.112 & 0.084 & 0.074 & 0.114 & 0.115 & 0.082 & 0.097 & 0.147 & 0.104 & 0.111 & 0.144 & 0.106 & 0.120 & 0.124 & 0.099 & 0.079 & 0.097 \\
doctorglm-6b                  & 0.093 & 0.076 & 0.065 & 0.037 & 0.085 & 0.051 & 0.038 & 0.062 & 0.068 & 0.044 & 0.047 & 0.056 & 0.043 & 0.069 & 0.053 & 0.043 & 0.106 & 0.059 & 0.059 \\
moss-base-16B                 & 0.072 & 0.050 & 0.062 & 0.115 & 0.048 & 0.052 & 0.099 & 0.105 & 0.051 & 0.059 & 0.123 & 0.054 & 0.058 & 0.124 & 0.077 & 0.080 & 0.121 & 0.058 & 0.063 \\
moss-sft-16B                  & 0.064 & 0.065 & 0.051 & 0.063 & 0.062 & 0.072 & 0.075 & 0.072 & 0.067 & 0.068 & 0.073 & 0.081 & 0.066 & 0.071 & 0.070 & 0.059 & 0.074 & 0.084 & 0.075 \\
\hline
ChatGPT                       & 0.240 & 0.298 & 0.371 & 0.286 & 0.289 & 0.360 & 0.290   & 0.218 & 0.352 & 0.414 & 0.266 & 0.418 & 0.487 & 0.217 & 0.361 & 0.428 & 0.305 & 0.452 & 0.517  \\
GPT-4                         & 0.402 & 0.415 & 0.517 & 0.413 & 0.410 & 0.486 & 0.404   & 0.392 & 0.429 & 0.490 & 0.453 & 0.496 & 0.565 & 0.396 & 0.434 & 0.495 & 0.463 & 0.506 & 0.576  \\
\bottomrule
\end{tabular}
}
    \caption{
    The overall performance of all language models are listed in this table. All tested models are divided into broad groups sharing similar character. Bolded font indicates the best performing result within a group, and underlined font indicates the best performing result for the same data set with the same settings.
    }
    \label{tab:all-llm}
\end{table}

==> tables/table_data_statistic.tex <==
\begin{center}
\resizebox{0.8\columnwidth}{!}{%
\begin{supertabular}{|c|c|c|}
\hline
Column 1 & Column 2 & Column 3 \\
\hline
Data 1 & Data 2 & Data 3 \\
\hline
Data 4 & Data 5 & Data 6 \\
\hline
\end{supertabular}
}
\end{center}







\tablehead{%
\hline
\multicolumn{1}{|p{1cm}|}{Column 1} & \multicolumn{1}{p{0.5cm}|}{Column 2} & \multicolumn{1}{p{0.5cm}|}{Column 3} & \multicolumn{1}{p{0.5cm}|}{Column 2} & \multicolumn{1}{p{0.5cm}|}{Column 3} \\
\hline
}

% \begin{supertabular}{|p{3cm}|p{3cm}|p{3cm}|}
\begin{supertabular}{l{1cm}|l{0.5cm}|l{0.5cm}|l{0.5cm}|l{0.5cm}}

Philosophy & 40365 & 102 & 1366 & 45 \\
\qquad Philosophy (Level 1 subject) & 2306 & 48 & 976 & 40 \\
\qquad\qquad Marxist Philosophy & 81 & 0 & 27 & 5 \\
\qquad\qquad Chinese Philosophy & 1102 & 0 & 762 & 5 \\
\qquad\qquad Foreign Philosophy & 40 & 0 & 10 & 5 \\
\qquad\qquad Logic & 105 & 0 & 11 & 5 \\
\qquad\qquad Ethics & 141 & 0 & 44 & 5 \\
\qquad\qquad Aesthetics & 50 & 0 & 5 & 5 \\
\qquad\qquad Religion & 689 & 0 & 156 & 5 \\
\qquad\qquad Philosophy of Science and Technology & 1 & 0 & 0 & 0 \\
Economics & 44449 & 354 & 3545 & 95 \\
\qquad Applied Economics & 1175 & 158 & 265 & 55 \\
\qquad\qquad National Economics & 152 & 2 & 100 & 5 \\
\qquad\qquad Regional Economics & 61 & 0 & 1 & 5 \\
\qquad\qquad Taxation & 39 & 34 & 0 & 5 \\
\qquad\qquad Insurance & 30 & 25 & 0 & 5 \\
\qquad\qquad Industrial Economics & 69 & 0 & 5 & 5 \\
\qquad\qquad International Trade & 71 & 1 & 18 & 5 \\
\qquad\qquad Labour economics & 68 & 48 & 7 & 5 \\
\qquad\qquad Statistics & 147 & 0 & 22 & 5 \\
\qquad\qquad Quantitative Economics & 48 & 0 & 3 & 5 \\
\qquad\qquad Defence Economics & 172 & 0 & 106 & 5 \\
\qquad Theoretical Economics & 4788 & 146 & 3108 & 35 \\
\qquad\qquad Political Economy & 3688 & 50 & 2567 & 5 \\
\qquad\qquad History of Economic Thought & 293 & 0 & 210 & 5 \\
\qquad\qquad Economic history & 667 & 0 & 501 & 5 \\
\qquad\qquad Western economics & 101 & 2 & 54 & 5 \\
\qquad\qquad World Economics & 65 & 0 & 5 & 5 \\
\qquad\qquad Population, Resource and Environmental Economics & 60 & 48 & 0 & 5 \\
Jurisprudence & 52188 & 1189 & 7529 & 170 \\
\qquad Public Security & 125 & 48 & 1 & 5 \\
\qquad Political Science & 36638 & 431 & 6436 & 45 \\
\qquad\qquad Political Science Theory & 6554 & 53 & 4003 & 5 \\
\qquad\qquad Chinese and Foreign Political Systems & 383 & 48 & 229 & 5 \\
\qquad\qquad Scientific Socialism and the International Communist Movement & 45 & 40 & 0 & 5 \\
\qquad\qquad History of the Chinese Communist Party & 59 & 48 & 0 & 5 \\
\qquad\qquad Marxist Theory and Ideological and Political Education & 163 & 48 & 98 & 5 \\
\qquad\qquad International Politics & 1876 & 50 & 1081 & 5 \\
\qquad\qquad International Relations & 1413 & 48 & 691 & 5 \\
\qquad\qquad Diplomacy & 262 & 32 & 138 & 5 \\
\qquad Ethnology & 905 & 271 & 349 & 30 \\
\qquad\qquad Ethnology (Level 2 subject) & 44 & 39 & 0 & 5 \\
\qquad\qquad Marxist Ethnic Theory and Policy & 70 & 41 & 24 & 5 \\
\qquad\qquad Economics of China's Ethnic Minorities & 53 & 47 & 1 & 5 \\
\qquad\qquad History of Ethnic Minorities in China & 95 & 48 & 26 & 5 \\
\qquad\qquad Chinese Ethnic Minority Art & 67 & 48 & 6 & 5 \\
\qquad Law (Level 1 subject) & 874 & 166 & 252 & 55 \\
\qquad\qquad Legal Theory & 222 & 0 & 117 & 5 \\
\qquad\qquad History of Law & 190 & 0 & 125 & 5 \\
\qquad\qquad Constitutional and Administrative Jurisprudence & 51 & 2 & 4 & 5 \\
\qquad\qquad Criminal Law & 54 & 0 & 1 & 5 \\
\qquad\qquad Civil and Commercial Law & 45 & 40 & 0 & 5 \\
\qquad\qquad Litigation Law & 44 & 0 & 0 & 5 \\
\qquad\qquad Economic Law & 44 & 0 & 13 & 5 \\
\qquad\qquad Environmental and Resource Protection Law & 47 & 40 & 2 & 5 \\
\qquad\qquad International Law  & 41 & 36 & 0 & 5 \\
\qquad\qquad Military Law & 58 & 0 & 1 & 5 \\
\qquad Sociology & 4011 & 177 & 982 & 25 \\
\qquad\qquad Sociology (Level 2 discipline) & 45 & 40 & 0 & 5 \\
\qquad\qquad Demography & 137 & 48 & 19 & 5 \\
\qquad\qquad Anthropology & 939 & 0 & 570 & 5 \\
\qquad\qquad Folklore & 44 & 39 & 0 & 5 \\
\qquad Marxist Theory & 1063 & 48 & 740 & 5 \\
Pedagogy & 6984 & 450 & 380 & 95 \\
\qquad Kinesiology & 752 & 218 & 151 & 25 \\
\qquad\qquad Humanities and Sociology of Sport & 62 & 48 & 2 & 5 \\
\qquad\qquad Sports Human Sciences & 37 & 26 & 4 & 5 \\
\qquad\qquad Physical Education and Training & 63 & 48 & 2 & 5 \\
\qquad\qquad Traditional Folk Sports & 171 & 48 & 107 & 5 \\
\qquad Psychology & 755 & 135 & 18 & 15 \\
\qquad\qquad Basic Psychology & 0 & 0 & 0 & 0 \\
\qquad\qquad Developmental and Educational Psychology & 57 & 47 & 5 & 5 \\
\qquad\qquad Applied Psychology & 46 & 40 & 1 & 5 \\
\qquad Pedagogy (Level 1 subject) & 601 & 48 & 151 & 50 \\
\qquad\qquad Principles of Education & 215 & 0 & 125 & 5 \\
\qquad\qquad Curriculum and Pedagogy & 37 & 0 & 0 & 5 \\
\qquad\qquad History of Education & 93 & 0 & 37 & 5 \\
\qquad\qquad Comparative Pedagogy & 37 & 0 & 2 & 5 \\
\qquad\qquad Pre-school Pedagogy & 11 & 0 & 2 & 5 \\
\qquad\qquad Higher Education & 2 & 0 & 0 & 0 \\
\qquad\qquad Adult Education & 38 & 0 & 1 & 5 \\
\qquad\qquad Vocational and Technical Education & 29 & 0 & 1 & 5 \\
\qquad\qquad Special Education & 46 & 0 & 1 & 5 \\
\qquad\qquad Educational Technology & 47 & 0 & 2 & 5 \\
Literature & 26971 & 806 & 1428 & 130 \\
\qquad Chinese Language and Literature & 1763 & 283 & 778 & 45 \\
\qquad\qquad Literary Arts & 671 & 0 & 502 & 5 \\
\qquad\qquad Linguistics and Applied Linguistics & 54 & 42 & 7 & 5 \\
\qquad\qquad Chinese Language and Literature & 80 & 2 & 28 & 5 \\
\qquad\qquad Chinese Classical Literature & 286 & 50 & 124 & 5 \\
\qquad\qquad Ancient Chinese Literature & 296 & 1 & 131 & 5 \\
\qquad\qquad Chinese Modern and Contemporary Literature & 104 & 48 & 40 & 5 \\
\qquad\qquad Chinese Minority Languages and Literatures & 59 & 48 & 0 & 5 \\
\qquad\qquad Comparative Literature and World Literature & 107 & 46 & 55 & 5 \\
\qquad Foreign Languages and Literatures & 764 & 373 & 152 & 60 \\
\qquad\qquad English Language and Literature & 57 & 0 & 11 & 5 \\
\qquad\qquad Russian Language and Literature & 67 & 48 & 7 & 5 \\
\qquad\qquad French Language and Literature & 49 & 40 & 4 & 5 \\
\qquad\qquad German Language and Literature & 47 & 0 & 1 & 5 \\
\qquad\qquad Japanese Language and Literature & 82 & 42 & 33 & 5 \\
\qquad\qquad Indian Languages and Literatures & 76 & 48 & 14 & 5 \\
\qquad\qquad Spanish Language and Literature & 46 & 40 & 1 & 5 \\
\qquad\qquad Arabic Language and Literature & 75 & 41 & 29 & 5 \\
\qquad\qquad European Languages and Literatures & 71 & 1 & 24 & 5 \\
\qquad\qquad Asian and African Languages and Literatures & 63 & 48 & 2 & 5 \\
\qquad\qquad Foreign Languages and Applied Linguistics & 22 & 17 & 0 & 5 \\
\qquad Journalism and Communication & 333 & 48 & 89 & 15 \\
\qquad\qquad Journalism & 143 & 0 & 51 & 5 \\
\qquad\qquad Communication Studies & 64 & 0 & 12 & 5 \\
\qquad Language and Literature & 297 & 49 & 55 & 5 \\
History & 162353 & 248 & 9949 & 60 \\
\qquad World History & 1180 & 0 & 423 & 5 \\
\qquad History of China & 6732 & 10 & 1985 & 5 \\
\qquad History (Level 1 subject) & 11973 & 48 & 7150 & 45 \\
\qquad\qquad Historical theory and history of history & 424 & 0 & 213 & 5 \\
\qquad\qquad Archaeology and Museology & 637 & 0 & 355 & 5 \\
\qquad\qquad Historical Geography & 1177 & 0 & 842 & 5 \\
\qquad\qquad Historical Documentation & 410 & 0 & 257 & 5 \\
\qquad\qquad Specialised History & 61 & 0 & 0 & 5 \\
\qquad\qquad Ancient Chinese History & 5003 & 0 & 3290 & 5 \\
\qquad\qquad Modern Chinese History & 3158 & 0 & 2618 & 5 \\
\qquad\qquad World History & 1180 & 0 & 423 & 5 \\
\qquad Archaeology & 1509 & 1 & 413 & 5 \\
Science & 18563 & 2347 & 1261 & 340 \\
\qquad History of Science and Technology & 306 & 88 & 77 & 10 \\
\qquad\qquad History of Science and Technology (Level 2 subject) & 45 & 40 & 0 & 5 \\
\qquad Chemistry & 399 & 200 & 7 & 30 \\
\qquad\qquad Inorganic chemistry & 46 & 41 & 0 & 5 \\
\qquad\qquad Analytical chemistry & 59 & 48 & 0 & 5 \\
\qquad\qquad Organic chemistry & 46 & 40 & 1 & 5 \\
\qquad\qquad Physical Chemistry & 46 & 40 & 1 & 5 \\
\qquad\qquad Polymer chemistry and physics & 36 & 31 & 0 & 5 \\
\qquad Geophysics & 208 & 128 & 16 & 15 \\
\qquad\qquad Solid State Geophysics & 46 & 40 & 1 & 5 \\
\qquad\qquad Space physics & 45 & 39 & 1 & 5 \\
\qquad Geography & 5537 & 204 & 649 & 20 \\
\qquad\qquad Physical Geography & 89 & 48 & 9 & 5 \\
\qquad\qquad Human Geography & 189 & 48 & 110 & 5 \\
\qquad\qquad Cartography and GIS & 103 & 48 & 46 & 5 \\
\qquad Geology & 941 & 386 & 322 & 45 \\
\qquad\qquad Mineralogy & 50 & 41 & 2 & 5 \\
\qquad\qquad Petrology & 46 & 40 & 1 & 5 \\
\qquad\qquad Ore Deposits & 41 & 36 & 0 & 5 \\
\qquad\qquad Geochemistry & 113 & 47 & 56 & 5 \\
\qquad\qquad Palaeontology and Stratigraphy & 99 & 48 & 33 & 5 \\
\qquad\qquad Palaeoanthropology & 249 & 48 & 153 & 5 \\
\qquad\qquad Tectonic Geology & 46 & 40 & 1 & 5 \\
\qquad\qquad Quaternary Geology & 41 & 36 & 0 & 5 \\
\qquad Atmospheric Sciences & 368 & 70 & 2 & 15 \\
\qquad\qquad Meteorology & 270 & 0 & 1 & 5 \\
\qquad\qquad Atmospheric Physics and Atmospheric Environment & 27 & 22 & 0 & 5 \\
\qquad Astronomy & 170 & 102 & 12 & 15 \\
\qquad\qquad Astrophysics & 31 & 25 & 1 & 5 \\
\qquad\qquad Astrometry and Celestial Mechanics & 33 & 26 & 2 & 5 \\
\qquad Mathematics & 1080 & 171 & 67 & 30 \\
\qquad\qquad Basic Mathematics & 31 & 25 & 1 & 5 \\
\qquad\qquad Computational Mathematics & 29 & 22 & 2 & 5 \\
\qquad\qquad Probability Theory and Mathematical Statistics & 46 & 40 & 1 & 5 \\
\qquad\qquad Applied Mathematics & 45 & 40 & 0 & 5 \\
\qquad\qquad Operations Research and Cybernetics & 31 & 22 & 4 & 5 \\
\qquad Marine Science & 299 & 164 & 24 & 25 \\
\qquad\qquad Physical Oceanography & 42 & 36 & 1 & 5 \\
\qquad\qquad Marine Chemistry & 46 & 40 & 1 & 5 \\
\qquad\qquad Marine Biology & 46 & 40 & 1 & 5 \\
\qquad\qquad Marine Geology & 49 & 0 & 3 & 5 \\
\qquad Physics & 1148 & 301 & 35 & 45 \\
\qquad\qquad Theoretical Physics & 44 & 38 & 1 & 5 \\
\qquad\qquad Particle Physics and Atomic Nucleus Physics & 44 & 39 & 0 & 5 \\
\qquad\qquad Atomic and molecular physics & 60 & 48 & 0 & 5 \\
\qquad\qquad Plasma physics & 44 & 39 & 0 & 5 \\
\qquad\qquad Condensed Matter Physics & 60 & 48 & 1 & 5 \\
\qquad\qquad Acoustics & 46 & 0 & 1 & 5 \\
\qquad\qquad Optics & 65 & 0 & 4 & 5 \\
\qquad\qquad Radio physics & 45 & 40 & 0 & 5 \\
\qquad Ecology & 313 & 8 & 49 & 5 \\
\qquad Biology & 2831 & 420 & 138 & 65 \\
\qquad\qquad Botany & 117 & 48 & 8 & 5 \\
\qquad\qquad Zoology & 414 & 48 & 47 & 5 \\
\qquad\qquad Physiology & 51 & 0 & 2 & 5 \\
\qquad\qquad Aquatic Biology & 45 & 40 & 0 & 5 \\
\qquad\qquad Microbiology & 27 & 22 & 0 & 5 \\
\qquad\qquad Neurobiology & 45 & 40 & 0 & 5 \\
\qquad\qquad Genetics & 37 & 0 & 1 & 5 \\
\qquad\qquad Developmental Biology & 61 & 48 & 2 & 5 \\
\qquad\qquad Cell Biology & 46 & 40 & 1 & 5 \\
\qquad\qquad Biochemistry and Molecular Biology & 45 & 39 & 1 & 5 \\
\qquad\qquad Biophysics & 44 & 39 & 0 & 5 \\
\qquad\qquad Ecology & 313 & 8 & 49 & 5 \\
\qquad Systems Science & 163 & 76 & 0 & 15 \\
\qquad\qquad Systems Theory & 45 & 0 & 0 & 5 \\
\qquad\qquad Systems Analysis and Integration & 33 & 28 & 0 & 5 \\
\qquad Statistics & 147 & 0 & 22 & 5 \\
Engineering & 35917 & 4717 & 562 & 770 \\
\qquad Optical Engineering & 771 & 96 & 0 & 10 \\
\qquad\qquad Optical Engineering (Level 2 discipline) & 60 & 48 & 0 & 5 \\
\qquad Biomedical Engineering & 686 & 86 & 0 & 10 \\
\qquad\qquad Biomedical Engineering (Level 2 discipline) & 43 & 38 & 0 & 5 \\
\qquad Traffic and Transport Engineering & 934 & 208 & 25 & 25 \\
\qquad\qquad Road and Railway Engineering & 30 & 25 & 0 & 5 \\
\qquad\qquad Traffic Information Engineering and Control & 56 & 48 & 0 & 5 \\
\qquad\qquad Transport Planning and Management & 63 & 48 & 9 & 5 \\
\qquad\qquad Vehicle Operation Engineering & 46 & 39 & 2 & 5 \\
\qquad Instrument Science and Technology & 781 & 128 & 1 & 15 \\
\qquad\qquad Precision Instruments and Machinery & 46 & 40 & 1 & 5 \\
\qquad\qquad Test and Measurement Technology and Instrumentation & 45 & 40 & 0 & 5 \\
\qquad Information and Communication Engineering & 809 & 118 & 4 & 15 \\
\qquad\qquad Communication and Information Systems & 28 & 22 & 1 & 5 \\
\qquad\qquad Signal and Information Processing & 55 & 48 & 1 & 5 \\
\qquad Weapons Science and Technology & 944 & 162 & 22 & 25 \\
\qquad\qquad Weapon Systems and Operations Engineering & 47 & 41 & 1 & 5 \\
\qquad\qquad Weapon Launch Theory and Technology & 61 & 48 & 1 & 5 \\
\qquad\qquad Artillery, Automatic Weapons and Ammunition Engineering & 30 & 25 & 0 & 5 \\
\qquad\qquad Military Chemistry and Pyrotechnics & 60 & 0 & 0 & 5 \\
\qquad Agricultural Engineering & 890 & 238 & 51 & 25 \\
\qquad\qquad Agricultural Mechanization Engineering & 66 & 46 & 15 & 5 \\
\qquad\qquad Agricultural Soil and Water Engineering & 60 & 48 & 5 & 5 \\
\qquad\qquad Agricultural Bioenvironmental and Energy Engineering & 59 & 48 & 2 & 5 \\
\qquad\qquad Agricultural Electrification and Automation & 55 & 48 & 1 & 5 \\
\qquad Metallurgical Engineering & 772 & 96 & 14 & 10 \\
\qquad\qquad Metallurgical Physical Chemistry & 64 & 48 & 3 & 5 \\
\qquad Mechanics & 902 & 206 & 6 & 25 \\
\qquad\qquad General Mechanics & 45 & 40 & 0 & 5 \\
\qquad\qquad Solid Mechanics & 46 & 40 & 0 & 5 \\
\qquad\qquad Fluid Mechanics & 44 & 39 & 0 & 5 \\
\qquad\qquad Engineering Mechanics & 47 & 39 & 3 & 5 \\
\qquad Power Engineering and Engineering Thermophysics & 994 & 48 & 7 & 35 \\
\qquad\qquad Engineering Thermophysics & 51 & 0 & 4 & 5 \\
\qquad\qquad Thermal Engineering & 48 & 0 & 2 & 5 \\
\qquad\qquad Power Mechanics and Engineering & 60 & 0 & 0 & 5 \\
\qquad\qquad Fluid Mechanics and Engineering & 46 & 0 & 1 & 5 \\
\qquad\qquad Refrigeration and Cryogenic Engineering & 57 & 0 & 0 & 5 \\
\qquad\qquad Chemical Process Machinery & 59 & 0 & 0 & 5 \\
\qquad Chemical Engineering and Technology & 911 & 48 & 12 & 30 \\
\qquad\qquad Chemical Engineering & 60 & 0 & 0 & 5 \\
\qquad\qquad Chemical Processes & 65 & 0 & 4 & 5 \\
\qquad\qquad Biochemistry & 45 & 0 & 0 & 5 \\
\qquad\qquad Applied Chemistry & 46 & 0 & 0 & 5 \\
\qquad\qquad Industrial Catalysis & 50 & 0 & 9 & 5 \\
\qquad Civil Engineering & 1089 & 184 & 121 & 35 \\
\qquad\qquad Geotechnical Engineering & 45 & 0 & 1 & 5 \\
\qquad\qquad Structural Engineering & 45 & 0 & 0 & 5 \\
\qquad\qquad Municipal Engineering & 45 & 0 & 0 & 5 \\
\qquad\qquad Heating, Gas, Ventilation and Air Conditioning Engineering & 54 & 48 & 0 & 5 \\
\qquad\qquad Disaster Prevention and Mitigation Engineering and Protection Engineering & 172 & 48 & 115 & 5 \\
\qquad\qquad Bridge and Tunnel Engineering & 45 & 40 & 0 & 5 \\
\qquad Geological Resources and Geological Engineering & 759 & 93 & 12 & 20 \\
\qquad\qquad Mineral Census and Exploration & 44 & 0 & 0 & 5 \\
\qquad\qquad Earth Exploration and Information Technology & 58 & 45 & 8 & 5 \\
\qquad\qquad Geological Engineering & 50 & 0 & 4 & 5 \\
\qquad Urban and Rural Planning & 104 & 49 & 14 & 5 \\
\qquad Safety Science and Engineering & 77 & 48 & 0 & 5 \\
\qquad Architecture & 984 & 218 & 107 & 25 \\
\qquad\qquad History and Theory of Architecture & 67 & 41 & 21 & 5 \\
\qquad\qquad Architectural Design and Theory & 135 & 49 & 70 & 5 \\
\qquad\qquad Urban Planning and Design  & 45 & 40 & 0 & 5 \\
\qquad\qquad Building Technology Science & 56 & 40 & 11 & 5 \\
\qquad Control Science and Engineering & 883 & 205 & 1 & 30 \\
\qquad\qquad Control Theory and Control Engineering & 44 & 39 & 0 & 5 \\
\qquad\qquad Testing Technology and Automation & 45 & 40 & 0 & 5 \\
\qquad\qquad Systems Engineering & 46 & 0 & 1 & 5 \\
\qquad\qquad Pattern Recognition and Intelligent Systems & 43 & 38 & 0 & 5 \\
\qquad\qquad Navigation, Guidance and Control & 45 & 40 & 0 & 5 \\
\qquad Mechanical Engineering & 852 & 161 & 22 & 25 \\
\qquad\qquad Mechanical Manufacturing and Automation & 50 & 34 & 11 & 5 \\
\qquad\qquad Mechatronics Engineering & 45 & 40 & 0 & 5 \\
\qquad\qquad Mechanical Design and Theory & 46 & 39 & 2 & 5 \\
\qquad\qquad Vehicle Engineering & 45 & 0 & 0 & 5 \\
\qquad Materials Science and Engineering & 806 & 48 & 37 & 20 \\
\qquad\qquad Materials Physics and Chemistry & 45 & 0 & 0 & 5 \\
\qquad\qquad Materials Science & 72 & 0 & 23 & 5 \\
\qquad\qquad Materials Processing Engineering & 45 & 0 & 0 & 5 \\
\qquad Forestry Engineering & 698 & 128 & 0 & 20 \\
\qquad\qquad Forest Engineering & 45 & 0 & 0 & 5 \\
\qquad\qquad Wood Science and Technology & 45 & 40 & 0 & 5 \\
\qquad\qquad Forestry Chemical Processing Engineering & 45 & 40 & 0 & 5 \\
\qquad Nuclear Science and Technology & 841 & 205 & 2 & 25 \\
\qquad\qquad Nuclear Energy Science and Engineering & 45 & 40 & 0 & 5 \\
\qquad\qquad Nuclear Fuel Cycle and Materials & 45 & 40 & 0 & 5 \\
\qquad\qquad Nuclear Technology and Applications & 45 & 40 & 0 & 5 \\
\qquad\qquad Radiation Protection and Environmental Protection & 42 & 37 & 0 & 5 \\
\qquad Water Resources Engineering & 1057 & 256 & 75 & 30 \\
\qquad\qquad Hydrology and Water Resources & 52 & 40 & 7 & 5 \\
\qquad\qquad Hydraulics and River Dynamics & 45 & 40 & 0 & 5 \\
\qquad\qquad Hydraulic Structural Engineering & 46 & 39 & 2 & 5 \\
\qquad\qquad Hydraulic and Hydroelectric Engineering & 54 & 41 & 8 & 5 \\
\qquad\qquad Port, Coastal and Offshore Engineering & 45 & 40 & 0 & 5 \\
\qquad Mapping Science and Technology & 772 & 118 & 18 & 20 \\
\qquad\qquad Geodesy and Surveying Engineering & 29 & 24 & 0 & 5 \\
\qquad\qquad Photogrammetry and Remote Sensing & 45 & 0 & 1 & 5 \\
\qquad\qquad Cartography and Geographic Information Engineering & 65 & 46 & 14 & 5 \\
\qquad Environmental Science and Engineering & 1086 & 48 & 60 & 15 \\
\qquad\qquad Environmental Science & 394 & 0 & 57 & 5 \\
\qquad\qquad Environmental Engineering & 46 & 0 & 2 & 5 \\
\qquad Bioengineering & 84 & 48 & 0 & 5 \\
\qquad Electronic Science and Technology & 819 & 128 & 1 & 25 \\
\qquad\qquad Physical Electronics & 30 & 0 & 0 & 5 \\
\qquad\qquad Circuits and Systems & 39 & 0 & 0 & 5 \\
\qquad\qquad Microelectronics and Solid State Electronics & 45 & 40 & 0 & 5 \\
\qquad\qquad Electromagnetic Field and Microwave Technology & 45 & 40 & 0 & 5 \\
\qquad Electrical Engineering & 844 & 231 & 3 & 30 \\
\qquad\qquad Electrical Machines and Appliances & 31 & 26 & 0 & 5 \\
\qquad\qquad Power Systems and Automation & 46 & 40 & 1 & 5 \\
\qquad\qquad High Voltage and Insulation Technology & 44 & 39 & 0 & 5 \\
\qquad\qquad Power Electronics and Power Transmission & 43 & 38 & 0 & 5 \\
\qquad\qquad Electrical Engineering Theory and New Technology & 45 & 40 & 0 & 5 \\
\qquad Petroleum and Natural Gas Engineering & 763 & 48 & 0 & 20 \\
\qquad\qquad Oil and Gas Well Engineering & 44 & 0 & 0 & 5 \\
\qquad\qquad Oil and Gas Field Development Engineering & 44 & 0 & 0 & 5 \\
\qquad\qquad Oil and Gas Storage and Transportation Engineering & 45 & 0 & 0 & 5 \\
\qquad Mining Engineering & 729 & 136 & 3 & 20 \\
\qquad\qquad Mining Engineering & 30 & 25 & 0 & 5 \\
\qquad\qquad Mineral Processing Engineering & 44 & 39 & 0 & 5 \\
\qquad\qquad Safety Technology and Engineering & 29 & 24 & 0 & 5 \\
\qquad Textile Science and Engineering & 836 & 114 & 9 & 25 \\
\qquad\qquad Textile Engineering & 49 & 0 & 4 & 5 \\
\qquad\qquad Textile Materials and Textile Design & 31 & 26 & 0 & 5 \\
\qquad\qquad Textile Chemistry and Dyeing and Finishing Engineering & 45 & 40 & 0 & 5 \\
\qquad\qquad Clothing & 48 & 0 & 2 & 5 \\
\qquad Cyberspace Security & 78 & 48 & 0 & 5 \\
\qquad Aerospace Science and Technology & 853 & 88 & 6 & 25 \\
\qquad\qquad Aircraft Design & 36 & 0 & 0 & 5 \\
\qquad\qquad Aerospace Propulsion Theory and Engineering & 46 & 40 & 1 & 5 \\
\qquad\qquad Aerospace Manufacturing Engineering & 45 & 0 & 0 & 5 \\
\qquad\qquad Human-Machine and Environmental Engineering & 56 & 0 & 0 & 5 \\
\qquad Marine and Offshore Engineering & 745 & 86 & 5 & 20 \\
\qquad\qquad Ship and Marine Structures Design and Manufacture & 43 & 38 & 0 & 5 \\
\qquad\qquad Turbine Engineering & 44 & 0 & 0 & 5 \\
\qquad\qquad Hydroacoustic Engineering & 45 & 0 & 0 & 5 \\
\qquad Computer Science and Technology & 787 & 88 & 8 & 20 \\
\qquad\qquad Computer System Architecture & 45 & 0 & 0 & 5 \\
\qquad\qquad Computer Software and Theory & 45 & 40 & 0 & 5 \\
\qquad\qquad Computer Application Technology & 34 & 0 & 5 & 5 \\
\qquad Software Engineering & 91 & 48 & 0 & 5 \\
\qquad Light Industry Technology and Engineering & 869 & 86 & 7 & 25 \\
\qquad\qquad Pulp and Paper Engineering & 67 & 0 & 3 & 5 \\
\qquad\qquad Sugar Engineering & 63 & 0 & 2 & 5 \\
\qquad\qquad Fermentation Engineering & 58 & 0 & 0 & 5 \\
\qquad\qquad Leather Chemistry and Engineering & 43 & 38 & 0 & 5 \\
\qquad Iron and Steel Metallurgy & 117 & 88 & 4 & 10 \\
\qquad\qquad Non-Ferrous Metallurgy & 45 & 40 & 0 & 5 \\
\qquad Landscape Architecture & 84 & 48 & 0 & 5 \\
\qquad Food Science and Engineering & 872 & 176 & 5 & 25 \\
\qquad\qquad Food Science & 69 & 0 & 3 & 5 \\
\qquad\qquad Grain, Oil and Vegetable Protein Engineering & 45 & 40 & 0 & 5 \\
\qquad\qquad Agricultural Products Processing and Storage Engineering & 60 & 48 & 0 & 5 \\
\qquad\qquad Fish Processing and Storage Engineering & 45 & 40 & 0 & 5 \\
Agronomy & 11148 & 1245 & 142 & 185 \\
\qquad Crop Science & 926 & 147 & 44 & 15 \\
\qquad\qquad Crop Cultivation and Farming & 61 & 48 & 2 & 5 \\
\qquad\qquad Crop Genetics and Breeding & 61 & 48 & 0 & 5 \\
\qquad Veterinary Medicine & 852 & 175 & 1 & 20 \\
\qquad\qquad Basic Veterinary Medicine & 45 & 40 & 0 & 5 \\
\qquad\qquad Preventive Veterinary Medicine & 45 & 40 & 0 & 5 \\
\qquad\qquad Clinical Veterinary Medicine & 52 & 47 & 0 & 5 \\
\qquad Agricultural Resource Utilisation & 872 & 48 & 24 & 15 \\
\qquad\qquad Soil Science & 46 & 0 & 2 & 5 \\
\qquad\qquad Plant Nutrition & 44 & 0 & 0 & 5 \\
\qquad Horticulture & 803 & 48 & 11 & 20 \\
\qquad\qquad Fruit Tree Science & 34 & 0 & 0 & 5 \\
\qquad\qquad Vegetable Science & 47 & 0 & 1 & 5 \\
\qquad\qquad Tea & 45 & 0 & 0 & 5 \\
\qquad Forestry & 959 & 306 & 29 & 40 \\
\qquad\qquad Forest Genetic Breeding & 45 & 40 & 0 & 5 \\
\qquad\qquad Forest Breeding & 34 & 29 & 0 & 5 \\
\qquad\qquad Forest Conservation & 43 & 37 & 1 & 5 \\
\qquad\qquad Forest Management & 45 & 40 & 0 & 5 \\
\qquad\qquad Wildlife Conservation and Utilisation & 30 & 25 & 0 & 5 \\
\qquad\qquad Landscape Plants and Ornamental Horticulture & 77 & 48 & 21 & 5 \\
\qquad\qquad Soil and Water Conservation and Desertification Control & 46 & 39 & 2 & 5 \\
\qquad Plant Protection & 793 & 136 & 1 & 20 \\
\qquad\qquad Plant Pathology & 45 & 40 & 0 & 5 \\
\qquad\qquad Agricultural Insects and Pest Control & 60 & 48 & 1 & 5 \\
\qquad\qquad Pesticides & 55 & 0 & 0 & 5 \\
\qquad Aquaculture & 796 & 119 & 2 & 20 \\
\qquad\qquad Aquaculture & 45 & 40 & 0 & 5 \\
\qquad\qquad Capture Science & 49 & 39 & 2 & 5 \\
\qquad\qquad Fishery Resources & 45 & 40 & 0 & 5 \\
\qquad Animal Husbandry & 835 & 218 & 2 & 25 \\
\qquad\qquad Animal Genetic Breeding and Reproduction & 58 & 48 & 0 & 5 \\
\qquad\qquad Animal Nutrition and Feed Science & 59 & 48 & 0 & 5 \\
\qquad\qquad Grassland Science & 40 & 35 & 0 & 5 \\
\qquad\qquad Special economic animal husbandry  & 44 & 39 & 0 & 5 \\
\qquad Herbology & 91 & 0 & 4 & 5 \\
Medicine & 11238 & 2130 & 271 & 325 \\
\qquad Traditional Chinese Medicine & 890 & 96 & 52 & 10 \\
\qquad\qquad Chinese herbal medicine (Level 2 discipline) & 60 & 48 & 0 & 5 \\
\qquad Chinese Medicine & 1726 & 597 & 127 & 70 \\
\qquad\qquad Basic Theory of Chinese Medicine & 148 & 48 & 46 & 5 \\
\qquad\qquad Clinical Foundations of Chinese Medicine & 72 & 48 & 9 & 5 \\
\qquad\qquad Chinese Medical History and Literature & 123 & 48 & 29 & 5 \\
\qquad\qquad Formulary & 44 & 0 & 3 & 5 \\
\qquad\qquad Diagnostics of Chinese Medicine & 73 & 48 & 5 & 5 \\
\qquad\qquad Internal Medicine & 69 & 48 & 7 & 5 \\
\qquad\qquad External Medicine & 66 & 48 & 7 & 5 \\
\qquad\qquad Orthopaedics and Traumatology of Chinese Medicine & 66 & 48 & 6 & 5 \\
\qquad\qquad TCM Gynecology & 70 & 48 & 9 & 5 \\
\qquad\qquad TCM Paediatrics & 66 & 48 & 8 & 5 \\
\qquad\qquad Traditional Chinese Medicine & 72 & 48 & 11 & 5 \\
\qquad\qquad Acupuncture, Moxibustion and Tuina & 34 & 26 & 2 & 5 \\
\qquad\qquad Ethnic Medicine & 45 & 40 & 0 & 5 \\
\qquad Combination of Chinese and Western Medicine & 896 & 144 & 104 & 15 \\
\qquad\qquad Fundamentals of Integrated Chinese and Western Medicine & 109 & 48 & 51 & 5 \\
\qquad\qquad Combined Chinese and Western Medicine Clinical & 65 & 48 & 8 & 5 \\
\qquad Clinical Medicine & 1446 & 436 & 33 & 95 \\
\qquad\qquad Internal Medicine & 60 & 0 & 0 & 5 \\
\qquad\qquad Pediatrics & 61 & 0 & 1 & 5 \\
\qquad\qquad Geriatric Medicine & 35 & 30 & 0 & 5 \\
\qquad\qquad Neurology & 45 & 37 & 3 & 5 \\
\qquad\qquad Psychiatry and Mental Health & 40 & 34 & 1 & 5 \\
\qquad\qquad Dermatology and Venereology & 41 & 34 & 1 & 5 \\
\qquad\qquad Imaging Medicine and Nuclear Medicine & 70 & 44 & 21 & 5 \\
\qquad\qquad Diagnostic Clinical Laboratory Medicine & 60 & 48 & 0 & 5 \\
\qquad\qquad Nursing & 66 & 0 & 1 & 5 \\
\qquad\qquad Surgery & 36 & 0 & 2 & 5 \\
\qquad\qquad Obstetrics and Gynaecology & 30 & 25 & 0 & 5 \\
\qquad\qquad Ophthalmology & 46 & 0 & 1 & 5 \\
\qquad\qquad Otorhinolaryngology & 38 & 33 & 0 & 5 \\
\qquad\qquad Oncology & 45 & 0 & 1 & 5 \\
\qquad\qquad Rehabilitation Medicine and Physiotherapy & 46 & 41 & 0 & 5 \\
\qquad\qquad Sports Medicine & 32 & 23 & 4 & 5 \\
\qquad\qquad Anaesthesiology & 50 & 0 & 1 & 5 \\
\qquad\qquad Emergency Medicine & 44 & 39 & 0 & 5 \\
\qquad Public Health and Preventive Medicine & 989 & 177 & 1 & 35 \\
\qquad\qquad Epidemiology and Health Statistics & 45 & 40 & 0 & 5 \\
\qquad\qquad Labour Hygiene and Environmental Health & 46 & 41 & 0 & 5 \\
\qquad\qquad Nutrition and Food Hygiene & 36 & 0 & 0 & 5 \\
\qquad\qquad Paediatric and Child Health and Maternal and Child Health & 60 & 48 & 0 & 5 \\
\qquad\qquad Health Toxicology & 60 & 0 & 0 & 5 \\
\qquad\qquad Military Preventive Medicine & 52 & 0 & 1 & 5 \\
\qquad Dentistry & 782 & 144 & 2 & 15 \\
\qquad\qquad Basic Dental Medicine & 59 & 48 & 0 & 5 \\
\qquad\qquad Dental Clinical Medicine & 61 & 48 & 1 & 5 \\
\qquad Basic Medicine & 956 & 205 & 2 & 40 \\
\qquad\qquad Human Anatomy and Histoplasty & 59 & 48 & 1 & 5 \\
\qquad\qquad Immunology & 61 & 0 & 1 & 5 \\
\qquad\qquad Pathogenic Biology & 43 & 38 & 0 & 5 \\
\qquad\qquad Pathology and Pathophysiology & 40 & 35 & 0 & 5 \\
\qquad\qquad Forensic Medicine & 23 & 0 & 0 & 5 \\
\qquad\qquad Radiological Medicine & 42 & 0 & 0 & 5 \\
\qquad\qquad Aviation, Aerospace and Maritime Medicine & 41 & 36 & 0 & 5 \\
\qquad Nursing & 66 & 0 & 1 & 5 \\
\qquad Speciality Medicine & 76 & 48 & 0 & 5 \\
\qquad Pharmacy & 926 & 237 & 6 & 35 \\
\qquad\qquad Medicinal Chemistry & 46 & 40 & 1 & 5 \\
\qquad\qquad Pharmacy & 53 & 42 & 5 & 5 \\
\qquad\qquad Biopharmaceutics & 45 & 40 & 0 & 5 \\
\qquad\qquad Pharmaceutical Analysis & 43 & 38 & 0 & 5 \\
\qquad\qquad Microbiology and Biochemical Pharmacy & 45 & 40 & 0 & 5 \\
\qquad\qquad Pharmacology & 42 & 37 & 0 & 5 \\
Military Science & 7510 & 508 & 1082 & 150 \\
\qquad Military Political Work & 161 & 96 & 0 & 10 \\
\qquad\qquad Military Political Work Studies (Level 2 discipline) & 60 & 48 & 0 & 5 \\
\qquad Military Logistics & 112 & 0 & 0 & 5 \\
\qquad Military logistics and military equipment science & 439 & 0 & 0 & 20 \\
\qquad\qquad Military Logistics & 112 & 0 & 0 & 5 \\
\qquad\qquad Rear professional logistics & 60 & 0 & 0 & 5 \\
\qquad\qquad Military Equipment Studies & 152 & 0 & 0 & 5 \\
\qquad Military Thought and Military History & 1237 & 0 & 429 & 15 \\
\qquad\qquad Military Thought & 481 & 0 & 215 & 5 \\
\qquad\qquad Military History & 651 & 0 & 237 & 5 \\
\qquad Military Equipment Studies & 152 & 0 & 0 & 5 \\
\qquad Military Training & 108 & 0 & 1 & 5 \\
\qquad Military Systems & 235 & 36 & 6 & 15 \\
\qquad\qquad Military Organization & 72 & 0 & 5 & 5 \\
\qquad\qquad Military Management & 42 & 36 & 1 & 5 \\
\qquad Military Command & 638 & 74 & 108 & 35 \\
\qquad\qquad Operational Command & 219 & 26 & 101 & 5 \\
\qquad\qquad Military Operations Research & 63 & 0 & 2 & 5 \\
\qquad\qquad Military Communications & 63 & 0 & 2 & 5 \\
\qquad\qquad Military Intelligence & 60 & 0 & 0 & 5 \\
\qquad\qquad Cryptology & 46 & 0 & 1 & 5 \\
\qquad\qquad Military Education and Training & 60 & 0 & 0 & 5 \\
\qquad Campaign Studies & 668 & 156 & 181 & 15 \\
\qquad\qquad Joint Warfare & 45 & 40 & 0 & 5 \\
\qquad\qquad Military Service Campaign Studies & 59 & 48 & 1 & 5 \\
\qquad Tactics & 299 & 100 & 70 & 15 \\
\qquad\qquad Contract Tactics & 90 & 48 & 26 & 5 \\
\qquad\qquad Military tactics & 92 & 48 & 19 & 5 \\
\qquad Strategic Studies & 1136 & 71 & 613 & 15 \\
\qquad\qquad Military Strategy & 70 & 0 & 10 & 5 \\
\qquad\qquad War Mobilisation & 591 & 48 & 377 & 5 \\
Management Studies & 3947 & 835 & 512 & 140 \\
\qquad Management Science and Engineering & 133 & 88 & 2 & 10 \\
\qquad\qquad Management Science and Engineering (Level 2 discipline) & 45 & 40 & 0 & 5 \\
\qquad Public Administration & 327 & 235 & 40 & 30 \\
\qquad\qquad Administrative Management & 57 & 40 & 11 & 5 \\
\qquad\qquad Social Medicine and Health Administration & 33 & 27 & 1 & 5 \\
\qquad\qquad Education Economics and Management & 44 & 34 & 5 & 5 \\
\qquad\qquad Social Security & 63 & 46 & 11 & 5 \\
\qquad\qquad Land Resources Management & 55 & 40 & 10 & 5 \\
\qquad Agricultural and Forestry Economic Management & 426 & 55 & 178 & 15 \\
\qquad\qquad Agricultural Economic Management & 250 & 7 & 169 & 5 \\
\qquad\qquad Forestry Economic Management & 44 & 0 & 0 & 5 \\
\qquad Library, Intelligence and Archives Management & 221 & 48 & 14 & 20 \\
\qquad\qquad Librarianship & 47 & 0 & 12 & 5 \\
\qquad\qquad Intelligence & 36 & 0 & 2 & 5 \\
\qquad\qquad Archival Studies & 50 & 0 & 1 & 5 \\
\qquad Industrial Engineering & 171 & 48 & 61 & 5 \\
\qquad Business Administration & 586 & 169 & 137 & 40 \\
\qquad\qquad Accounting & 60 & 0 & 1 & 5 \\
\qquad\qquad Business Management & 119 & 0 & 48 & 5 \\
\qquad\qquad Financial Management & 57 & 0 & 13 & 5 \\
\qquad\qquad Marketing & 54 & 0 & 9 & 5 \\
\qquad\qquad Human Resource Management & 61 & 48 & 2 & 5 \\
\qquad\qquad Tourism Management & 108 & 48 & 53 & 5 \\
\qquad\qquad Technology Economics and Management & 44 & 25 & 12 & 5 \\
\qquad Tourism Management & 169 & 48 & 66 & 5 \\
\qquad Logistics Management and Engineering & 85 & 48 & 0 & 5 \\
\qquad E-Commerce & 71 & 48 & 0 & 5 \\
Art Studies & 6719 & 367 & 254 & 60 \\
\qquad Theatre and Film Studies & 109 & 48 & 22 & 5 \\
\qquad Fine Art & 122 & 0 & 2 & 5 \\
\qquad Art Theory & 257 & 48 & 78 & 5 \\
\qquad Design & 118 & 0 & 15 & 5 \\
\qquad Music and Dance & 99 & 48 & 2 & 5 \\
\qquad Art Studies (Level 1 subject) & 0 & 0 & 0 & 0 \\
\qquad Musicology & 68 & 48 & 9 & 5 \\
\qquad Design Art & 52 & 41 & 6 & 5 \\
\qquad Theatre and Operatic Studies & 74 & 48 & 19 & 5 \\
\qquad Film Studies & 87 & 0 & 21 & 5 \\
\qquad Radio and Television Arts & 43 & 37 & 0 & 5 \\
\qquad Dance Studies & 45 & 0 & 1 & 5 \\
     

\caption{The overall data statistic of our proposed Benchmark.}
\label{table_data}
\end{supertabular}

==> tables/table_models_2.tex <==
\begin{table}
    \small
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Model}& \textbf{\#Parameter} & \textbf{Base Model} & \textbf{\#Layer} & \textbf{\#Encoder} & \textbf{\#Decoder} & \textbf{\#Pretrain Tokens} & \textbf{\#IFT Sample} & \textbf{RLHF} \\
        \hline
        T5-Base~\cite{2020t5}~\footnote{https://huggingface.co/t5-base} & 0.22B & - & 12 & 12 & 12 & - & - & - \\
        BERT-large-uncased~\cite{2018bert}~\footnote{https://huggingface.co/bert-large-uncased} & 0.34B & - & 24 & 24 & - & 3.3B tokens & - & - \\
        XLNet-large~\cite{2019xlnet}~\footnote{https://huggingface.co/xlnet-large-cased} & 0.34B & - & 24 & - & - & 158GB & - & - \\
        GPT3-Ada~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 0.35B & - & 24 & - & 24 & - & - & - \\
        BART-large~\cite{2019bart}~\footnote{https://huggingface.co/facebook/bart-large} & 0.406B & - & 12 & 12 & 12 & 3.2B tokens & - & - \\
        BLOOM-560m~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-560m} & 0.56B & - & 24 & - & 24 & 350B tokens & - & - \\
        BLOOMZ-560m~\cite{muennighoff2022crosslingual}~\footnote{https://huggingface.co/bigscience/bloomz-560m} & 0.56B & BLOOM-560m & 24 & - & 24 & - & 3.67B tokens & - \\
        Pythia-1B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-1b} & 1B & - & 16 & - & 16 & 300B tokens & - & - \\
        GPT3-Babbage~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 1.3B & - & 24 & - & 24 & - & - & - \\
        GPT2-XL~\cite{radford2019language}~\footnote{https://huggingface.co/gpt2-xl} & 1.5B & - & 48 & - & 48 & 40B tokens & - & - \\
        BLOOM-1b7~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-1b7} & 1.7B & - & 24 & - & 24 & 350B tokens & - & - \\
        BLOOMZ-1b7~\cite{muennighoff2022crosslingual}~\footnote{https://huggingface.co/bigscience/bloomz-1b7} & 1.7B & BLOOM-1b7 & 24 & - & 24 & - & 8.39B tokens & - \\
        Dolly-v2-3b~\cite{2023dolly}~\footnote{https://huggingface.co/databricks/dolly-v2-3b} & 2.8B & Pythia-2.8B & 32 & - & 32 & - & 15K & - \\
        Pythia-2.8B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-2.8b} & 2.8B & - & 32 & - & 32 & 300B tokens & - & - \\
        BLOOM-3b~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-3b} & 3B & - & 30 & - & 30 & 350B tokens & - & - \\
        BLOOMZ-3b~\cite{muennighoff2022crosslingual}~\footnote{https://huggingface.co/bigscience/bloomz-3b} & 3B & BLOOM-3b & 30 & - & 30 & - & 8.39B tokens & - \\
        FastChat-T5~\cite{2023fastchat}~\footnote{https://huggingface.co/lmsys/fastchat-t5-3b-v1.0} & 3B & FLAN-T5 XL & 24 & 24 & 24 & - & 70K & - \\
        FLAN-T5 XL~\cite{chung2022scaling}~\footnote{https://huggingface.co/google/flan-t5-xl} & 3B & T5-XL & 24 & 24 & 24 & - & 1000+ tasks & - \\
        StableLM-Base-Alpha-3B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-base-alpha-3b} & 3B & - & 16 & - & 16 & 800B tokens & - & - \\
        StableLM-Tuned-Alpha-3B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-tuned-alpha-3b} & 3B & StableLM-Base-Alpha-3B & 16 & - & 16 & - & 632K & - \\
        T5-XL~\cite{2020t5}~\footnote{https://huggingface.co/t5-3b} & 3B & - & 24 & 24 & 24 & - & - & - \\
        ChatGLM-6B~\cite{zeng2023glm-130b,du2022glm}~\footnote{https://huggingface.co/THUDM/chatglm-6b} & 6B & - & 28 & 28 & 28 & 1T tokens & \checkmark & \checkmark \\
        DoctorGLM~\cite{xiong2023doctorglm}~\footnote{https://github.com/xionghonglin/DoctorGLM} & 6B & ChatGLM-6B & 28 & 28 & 28 & - & 6.38M & - \\
        ChatGLM-Med~\cite{ChatGLM-Med}~\footnote{https://github.com/SCIR-HI/Med-ChatGLM} & 6B & ChatGLM-6B & 28 & 28 & 28 & - & 8K & - \\
        GPT3-Curie~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 6.7B & - & 32 & - & 32 & - & - & - \\
        MPT-7B-Chat~\cite{MosaicML2023Introducing}~\footnote{https://huggingface.co/mosaicml/mpt-7b-chat} & 6.7B & MPT-7B & 32 & - & 32 & - & 360K & - \\
        MPT-7B-Instruct~\cite{MosaicML2023Introducing}~\footnote{https://huggingface.co/mosaicml/mpt-7b-instruct} & 6.7B & MPT-7B & 32 & - & 32 & - & 59.3K & - \\
        MPT-7B-StoryWriter-65k+~\cite{MosaicML2023Introducing}~\footnote{https://huggingface.co/mosaicml/mpt-7b-storywriter} & 6.7B & MPT-7B & 32 & - & 32 & - & \checkmark & - \\
        Dolly-v2-7b~\cite{2023dolly}~\footnote{https://huggingface.co/databricks/dolly-v2-7b} & 6.9B & Pythia-6.9B & 32 & - & 32 & - & 15K & - \\
        h2ogpt-oig-oasst1-512-6.9b~\cite{2023h2ogpt}~\footnote{https://huggingface.co/h2oai/h2ogpt-oig-oasst1-512-6.9b} & 6.9B & Pythia-6.9B & 32 & - & 32 & - & 398K & - \\
        Pythia-6.9B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-6.9b} & 6.9B & - & 32 & - & 32 & 300B tokens & - & - \\
        Alpaca-7B~\cite{alpaca}~\footnote{https://huggingface.co/tatsu-lab/alpaca-7b-wdiff} & 7B & LLaMA-7B & 32 & - & 32 & - & 52K & - \\
        Alpaca-LoRA-7B~\cite{2023alpacalora}~\footnote{https://huggingface.co/tloen/alpaca-lora-7b} & 7B & LLaMA-7B & 32 & - & 32 & - & 52K & - \\
        Baize-7B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-lora-7B} & 7B & LLaMA-7B & 32 & - & 32 & - & 263K & - \\
        Baize Healthcare-7B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-healthcare-lora-7B} & 7B & LLaMA-7B & 32 & - & 32 & - & 201K & - \\
        ChatDoctor~\cite{yunxiang2023chatdoctor}~\footnote{https://github.com/Kent0n-Li/ChatDoctor} & 7B & LLaMA-7B & 32 & - & 32 & - & 167K & - \\
        HuaTuo~\cite{wang2023huatuo}~\footnote{https://github.com/scir-hi/huatuo-llama-med-chinese} & 7B & LLaMA-7B & 32 & - & 32 & - & 8K & - \\
        Koala-7B~\cite{koala_blogpost_2023}~\footnote{https://huggingface.co/young-geng/koala} & 7B & LLaMA-7B & 32 & - & 32 & - & 472K & - \\
        LLaMA-7B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-7b-hf} & 7B & - & 32 & - & 32 & 1T tokens & - & - \\
        Luotuo-lora-7b-0.3~\cite{luotuo}~\footnote{https://huggingface.co/silk-road/luotuo-lora-7b-0.3} & 7B & LLaMA-7B & 32 & - & 32 & - & 152K & - \\
        PandaLM-7B~\cite{PandaLM}~\footnote{https://github.com/WeOpenML/PandaLM} & 7B & LLaMA-7B & 32 & - & 32 & - & 300K & - \\
        StableLM-Base-Alpha-7B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-base-alpha-7b} & 7B & - & 16 & - & 16 & 800B tokens & - & - \\
        StableLM-Tuned-Alpha-7B~\cite{2023StableLM}~\footnote{https://huggingface.co/stabilityai/stablelm-tuned-alpha-7b} & 7B & StableLM-Base-Alpha-7B & 16 & - & 16 & - & 632K & - \\
        Vicuna-7b-delta-v1.1~\cite{vicuna2023}~\footnote{https://github.com/lm-sys/FastChat\#vicuna-weights} & 7B & LLaMA-7B & 32 & - & 32 & - & 70K & - \\
        BELLE-7B-0.2M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-0.2M}/0.6M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-0.6M}/1M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-1M}/2M~\footnote{https://huggingface.co/BelleGroup/BELLE-7B-2M}~\cite{belle2023exploring} & 7.1B & Bloomz-7b1-mt & 30 & - & 30 & - & 0.2M/0.6M/1M/2M & - \\
        BLOOM-7b1~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom-7b1} & 7.1B & - & 30 & - & 30 & 350B tokens & - & - \\
        BLOOMZ-7b1~\footnote{https://huggingface.co/bigscience/bloomz-7b1}/mt~\footnote{https://huggingface.co/bigscience/bloomz-7b1-mt}/p3~\footnote{https://huggingface.co/bigscience/bloomz-7b1-p3}~\cite{muennighoff2022crosslingual} & 7.1B & BLOOM-7b1 & 30 & - & 30 & - & 4.19B tokens & - \\
        FLAN-T5 XXL~\cite{chung2022scaling}~\footnote{https://huggingface.co/google/flan-t5-xxl} & 11B & T5-XXL & 24 & 24 & 24 & - & 1000+ tasks & - \\
        T5-XXL~\cite{2020t5}~\footnote{https://huggingface.co/t5-11b} & 11B & - & 24 & 24 & 24 & 1T tokens & - & - \\
        Dolly-v2-12b~\cite{2023dolly}~\footnote{https://huggingface.co/databricks/dolly-v2-12b} & 12B & Pythia-12B & 36 & - & 36 & - & 15K & - \\
        h2ogpt-oasst1-512-12b~\cite{2023h2ogpt}~\footnote{https://huggingface.co/h2oai/h2ogpt-oasst1-512-12b} & 12B & Pythia-12B & 36 & - & 36 & - & 94.6K & - \\
        Open-Assistant-SFT-4-12B~\cite{2023openassistant}~\footnote{https://huggingface.co/OpenAssistant/oasst-sft-4-pythia-12b-epoch-3.5} & 12B & Pythia-12B-deduped & 36 & - & 36 & - & 161K & - \\
        Pythia-12B~\cite{biderman2023pythia}~\footnote{https://huggingface.co/EleutherAI/pythia-12b} & 12B & - & 36 & - & 36 & 300B tokens & - & - \\
        Baize-13B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-lora-13B} & 13B & LLaMA-13B & 40 & - & 40 & - & 263K & - \\
        Koala-13B~\cite{koala_blogpost_2023}~\footnote{https://huggingface.co/young-geng/koala} & 13B & LLaMA-13B & 40 & - & 40 & - & 472K & - \\
        LLaMA-13B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-13b-hf} & 13B & - & 40 & - & 40 & 1T tokens & - & - \\
        mT0-xxl~\footnote{https://huggingface.co/bigscience/mt0-xxl} & 13B & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} \\
        mT0-xxl-mt~\footnote{https://huggingface.co/bigscience/mt0-xxl-mt} & 13B & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} \\
        mT5-XXL~\cite{xue-etal-2021-mt5}~\footnote{https://console.cloud.google.com/storage/browser/t5-data/pretrained\_models/mt5/xxl/} & 13B & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} & \red{-} \\
        StableVicuna-13B~\cite{2023StableLM}~\footnote{https://huggingface.co/CarperAI/stable-vicuna-13b-delta} & 13B & Vicuna-13B v0 & 40 & - & 40 & - & 613K & \checkmark \\
        Vicuna-13b-delta-v1.1~\cite{vicuna2023}~\footnote{https://github.com/lm-sys/FastChat\#vicuna-weights} & 13B & LLaMA-13B & 40 & - & 40 & - & 70K & - \\
        moss-moon-003-sft~\cite{2023moss}~\footnote{https://huggingface.co/fnlp/moss-moon-003-sft} & 16B & moss-moon-003-base & 34 & - & 34 & - & 1.1M & - \\
        moss-moon-003-sft-plugin~\cite{2023moss}~\footnote{https://huggingface.co/fnlp/moss-moon-003-sft-plugin} & 16B & moss-moon-003-base & 34 & - & 34 & - & 1.4M & - \\
        GPT-NeoX-20B~\cite{gptneox}~\footnote{https://huggingface.co/EleutherAI/gpt-neox-20b} & 20B & - & 44 & - & 44 & 825GB & - & - \\
        h2ogpt-oasst1-512-20b~\cite{2023h2ogpt}~\footnote{https://huggingface.co/h2oai/h2ogpt-oasst1-512-20b} & 20B & GPT-NeoX-20B & 44 & - & 44 & - & 94.6K & - \\
        OPT-IML-30B~\cite{iyer2023optiml}~\footnote{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT-IML} & 30B & OPT-30B & 48 & - & 48 & - & 1500 tasks & - \\
        Baize-30B~\cite{xu2023baize}~\footnote{https://huggingface.co/project-baize/baize-lora-30B} & 33B & LLaMA-30B & 60 & - & 60 & - & 263K & - \\
        LLaMA-30B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-30b-hf} & 33B & - & 60 & - & 60 & 1.4T tokens & - & - \\
        LLaMA-65B~\cite{touvron2023llama}~\footnote{https://huggingface.co/decapoda-research/llama-65b-hf} & 65B & - & 80 & - & 80 & 1.4T tokens & - & - \\
        GLM-130B~\cite{zeng2023glm-130b}~\footnote{https://github.com/THUDM/GLM-130B} & 130B & - & 70 & 70 & 70 & 400B tokens & - & - \\
        GPT3-Davinci~\cite{brown2020language}~\footnote{https://platform.openai.com/docs/models/gpt-3} & 175B & - & 96 & - & 96 & 300B tokens & - & - \\
        OPT-IML-175B~\cite{iyer2023optiml}~\footnote{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT-IML} & 175B & OPT-175B & 96 & - & 96 & - & 1500 tasks & - \\
        BLOOM~\cite{scao2022bloom}~\footnote{https://huggingface.co/bigscience/bloom} & 176B & - & 70 & - & 70 & 366B tokens & - & - \\
        BLOOMZ~\footnote{https://huggingface.co/bigscience/bloomz}/mt~\footnote{https://huggingface.co/bigscience/bloomz-mt}/p3~\footnote{https://huggingface.co/bigscience/bloomz-p3}~\cite{muennighoff2022crosslingual} & 176B & BLOOM & 70 & - & 70 & - & 2.09B tokens & - \\
        ChatGPT~(2023.05.01)~\cite{openaichatgpt}~\footnote{https://platform.openai.com/docs/models/gpt-3-5} & - & GPT-3.5 & - & - & - & - & \checkmark & \checkmark \\
        GPT-4~(2023.05.01)~\cite{openai2023gpt4}~\footnote{https://platform.openai.com/docs/models/gpt-4} & - & - & - & - & - & - & \checkmark & \checkmark \\
        \hline
    \end{tabular}
    }
    \vspace{3mm}
    \caption{The models we evaluted in our experiments.}
    \label{tab:models}
\end{table}

==> tables/table_red_gpt.tex <==
\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccc|ccc|c||ccc|ccc|ccc|ccc}
        \toprule
         \textbf{Models} & \multicolumn{3}{c|}{MMLU} & \multicolumn{3}{c|}{CEval} & \multicolumn{1}{c||}{M3KE} & \multicolumn{3}{c|}{Xiezhi-Spec.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Inter.-Chinese} & \multicolumn{3}{c|}{Xiezhi-Spec.-English} & \multicolumn{3}{c}{Xiezhi-Inter.-English}\\
         & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot & 0-shot & 1-shot & 3-shot\\
        \hline
        Random-Guess                               & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 & 0.089 \\
        \hline
        &\multicolumn{19}{c}{Generation Probability For Ranking}\\
        \hline
        Bloomz-560m                   & 0.111 & 0.109 & 0.119 & 0.124 & 0.117 & 0.103 & 0.126   & 0.123 & 0.127 & 0.124 & 0.130 & 0.138 & 0.140 & 0.113 & 0.116 & 0.123 & 0.124 & 0.117 & 0.160 \\
        Bloomz-1b1                    & 0.131 & 0.116 & 0.128 & 0.107 & 0.115 & 0.110 & 0.082   & 0.138 & 0.108 & 0.107 & 0.117 & 0.125 & 0.123 & 0.130 & 0.119 & 0.114 & 0.144 & 0.129 & 0.145\\
        Bloomz-1b7                    & 0.107 & 0.117 & 0.164 & 0.054 & 0.058 & 0.103 & 0.102   & 0.165 & 0.151 & 0.159 & 0.152 & \textbf{0.214} & 0.170 & 0.133 & 0.140 & 0.144 & 0.150 & 0.149 & 0.209\\
        Bloomz-3b                     & 0.139 & 0.084 & 0.146 & 0.168 & \textbf{0.182} & 0.194 & 0.063   & 0.186 & 0.154 & 0.168 & 0.151 & 0.180 & 0.182 & 0.201 & 0.155 & 0.156 & 0.175 & 0.164 & 0.158 \\
        Bloomz-7b1                    & 0.167 & 0.160 & 0.205 & 0.074 & 0.072 & 0.073 & 0.073   & 0.154 & 0.178 & 0.162 & 0.148 & 0.160 & 0.156 & 0.176 & 0.153 & 0.207 & 0.217 & 0.204 & 0.229 \\
        Bloomz-7b1-mt                 & 0.189 & 0.196 & 0.210 & 0.077 & 0.078 & 0.158 & 0.072   & 0.163 & 0.175 & 0.154 & 0.155 & 0.195 & 0.164 & 0.180 & 0.146 & 0.219 & 0.228 & 0.171 & 0.232 \\
        Bloomz-7b1-p3                 & 0.066 & 0.059 & 0.075 & 0.071 & 0.070 & 0.072 & 0.081   & 0.177 & 0.198 & 0.158 & 0.183 & 0.173 & 0.170 & 0.130 & 0.130 & 0.162 & 0.157 & 0.132 & 0.134 \\
        Bloomz                        & 0.051 & 0.066 & 0.053 & 0.142 & 0.166 & \underline{\textbf{0.240}} & 0.098   & 0.185 & 0.133 & 0.277 & 0.161 & 0.099 & \textbf{0.224} & 0.069 & 0.082 & 0.056 & 0.058 & 0.055 & 0.049 \\
        Bloomz-mt                     & \underline{\textbf{0.266}} & \underline{\textbf{0.264}} & \underline{\textbf{0.248}} & \textbf{0.204} & 0.164 & 0.151 & \textbf{0.161}   & \underline{\textbf{0.253}} & \textbf{0.198} & \textbf{0.212} & \textbf{0.213} & 0.189 & 0.184 & \underline{\textbf{0.379}} & \underline{\textbf{0.396}} & \underline{\textbf{0.394}} & \underline{\textbf{0.383}} & \underline{\textbf{0.405}} & \underline{\textbf{0.398}} \\
        Bloomz-p3                     & 0.115 & 0.093 & 0.057 & 0.118 & 0.137 & 0.140 & 0.115   & 0.136 & 0.095 & 0.105 & 0.086 & 0.065 & 0.098 & 0.139 & 0.097 & 0.069 & 0.176 & 0.141 & 0.070 \\
        \hline
        llama-7b                      & 0.125 & \textbf{0.132} & 0.093 & 0.133 & 0.106 & 0.110 & \textbf{0.158}   & \textbf{0.152} & 0.141 & 0.117 & 0.142 & 0.135 & 0.128 & 0.159 & 0.165 & 0.161 & \textbf{0.194} & 0.183 & 0.176 \\
        llama-13b                     & \textbf{0.166} & 0.079 & \textbf{0.135} & 0.152 & \textbf{0.181} & \textbf{0.169} & 0.131   & 0.133 & \underline{\textbf{0.241}} & \textbf{0.243} & \textbf{0.211} & \textbf{0.202} & \underline{\textbf{0.303}} & 0.154 & 0.183 & \textbf{0.215} & 0.174 & \textbf{0.216} & \textbf{0.231} \\
        llama-30b                     & 0.076 & 0.107 & 0.073 & 0.079 & 0.119 & 0.082 & 0.079   & 0.140 & 0.206 & 0.162 & 0.186 & \textbf{0.202} & 0.183 & 0.110 & 0.195 & 0.161 & 0.088 & 0.158 & 0.219 \\
        llama-65b                     & 0.143 & 0.121 & 0.100 & \textbf{0.154} & 0.141 & 0.168 & 0.125   & 0.142 & 0.129 & 0.084 & 0.108 & 0.077 & 0.077 & \textbf{0.183} & \textbf{0.204} & 0.172 & 0.133 & 0.191 & 0.157 \\
        \hline
        baize-7b~(lora)               & 0.129 & 0.091 & 0.079 & \textbf{0.194} & 0.180 & \textbf{0.206} & \underline{\textbf{0.231}}   & \textbf{0.216} & 0.148 & 0.123 & 0.173 & 0.158 & 0.198 & \textbf{0.182} & 0.190 & 0.194 & \textbf{0.218} & 0.188 & 0.209 \\
        baize-7b-healthcare~(lora)    & 0.130 & 0.121 & 0.106 & 0.178 & 0.174 & 0.178 & 0.203   & 0.178 & 0.146 & 0.123 & \underline{\textbf{0.266}} & 0.107 & 0.118 & 0.175 & 0.164 & 0.173 & 0.197 & \textbf{0.231} & 0.198 \\
        baize-13b~(lora)              & 0.131 & 0.111 & 0.171 & 0.184 & 0.178 & 0.195 & 0.155   & 0.158 & \textbf{0.221 }& \underline{\textbf{0.256}} & 0.208 & 0.200 & \textbf{0.219} & 0.176 & 0.189 & \textbf{0.239} & 0.187 & 0.185 & \textbf{0.274} \\
        baize-30b~(lora)              & \textbf{0.193} & \textbf{0.216} & \textbf{0.207} & 0.191 & \underline{\textbf{0.196}} & 0.121 & 0.071   & 0.109 & 0.212 & 0.190 & 0.203 & \underline{\textbf{0.256}} & 0.200 & 0.167 & \textbf{0.235} & 0.168 & 0.072 & 0.180 & 0.193 \\
        \hline
        Belle-0.2M                    & 0.127 & \textbf{0.148} & \textbf{0.243} & 0.053 & 0.063 & \textbf{0.136} & \textbf{0.076}   & 0.172 & 0.126 & 0.153 & 0.171 & 0.165 & 0.147 & 0.206 & 0.146 & 0.148 & \textbf{0.217} & 0.150 & 0.173 \\          
        Belle-0.6M                    & 0.091 & 0.114 & 0.180 & \textbf{0.082} & \textbf{0.080} & 0.090 & 0.075   & \textbf{0.188} & 0.149 & \textbf{0.198} & \textbf{0.188} & \textbf{0.188} & 0.175 & 0.173 & \textbf{0.172} & \textbf{0.183} & 0.193 & \textbf{0.184} & \textbf{0.196} \\
        Belle-1M                      & \textbf{0.137} & 0.126 & 0.162 & 0.066 & 0.065 & 0.072 & 0.066   & 0.170 & 0.152 & 0.147 & 0.173 & 0.176 & \textbf{0.197} & \textbf{0.211} & 0.137 & 0.149 & 0.207 & 0.151 & 0.185 \\
        Belle-2M                      & 0.127 & \textbf{0.148} & 0.132 & 0.058 & 0.063 & \textbf{0.136} & 0.057   & 0.163 & \textbf{0.166} & 0.130 & 0.159 & 0.177 & 0.163 & 0.155 & 0.106 & 0.166 & 0.151 & 0.150 & 0.138 \\
        \hline
        % cuteGPT                       & 0.146 & 0.105 & 0.125 & 0.122 & 0.117 & 0.136 & 0.121 & 0.123 & 0.158 & 0.166 & 0.150 & 0.177 & 0.188 & 0.132 & 0.127 & 0.124 & 0.200 & 0.159 & 0.182 \\
        chatglm-6B                    & \textbf{0.099} & \textbf{0.109} & \textbf{0.112} & \textbf{0.084} & 0.074 & \textbf{0.114} & \textbf{0.115}   & \textbf{0.082} & \textbf{0.097} & \textbf{0.147} & \textbf{0.104} & \textbf{0.111} & \textbf{0.144} & \textbf{0.106} & \textbf{0.120} & \textbf{0.124} & 0.099 & \textbf{0.079} & \textbf{0.097} \\
        doctorglm-6b                  & 0.093 & 0.076 & 0.065 & 0.037 & \textbf{0.085} & 0.051 & 0.038   & 0.062 & 0.068 & 0.044 & 0.047 & 0.056 & 0.043 & 0.069 & 0.053 & 0.043 & 0.106 & 0.059 & 0.059 \\
        \hline
        moss-base-16B                 & \textbf{0.072} & 0.050 & \textbf{0.062} & \textbf{0.115} & 0.048 & 0.052 & \textbf{0.099}   & \textbf{0.105} & 0.051 & 0.059 & \textbf{0.123} & 0.054 & 0.058 & \textbf{0.124} & \textbf{0.077} & \textbf{0.080} & \textbf{0.121} & 0.058 & 0.063 \\
        moss-sft-16B                  & 0.064 & \textbf{0.065} & 0.051 & 0.063 & \textbf{0.062} & \textbf{0.072} & 0.075   & 0.072 & \textbf{0.067} & \textbf{0.068} & 0.073 & \textbf{0.081} & \textbf{0.066} & 0.071 & 0.070 & 0.059 & 0.074 & \textbf{0.084} & \textbf{0.075} \\
        \hline
        vicuna-7b                     & 0.051 & 0.051 & 0.029 & 0.063 & 0.071 & 0.064 & 0.059 & 0.169 & \textbf{0.171} & 0.165 & 0.134 & \textbf{0.201} & \textbf{0.213} & 0.182 & \textbf{0.209} & \textbf{0.195} & 0.200 & \textbf{0.214} & 0.182 \\
        vicuna-13b                    & 0.109 & 0.104 & 0.066 & 0.060 & 0.131 & 0.131 & 0.067 & \textbf{0.171} & 0.167 & 0.166 & 0.143 & 0.147 & 0.178 & 0.121 & 0.139 & 0.128 & 0.158 & 0.174 & 0.191 \\
        alpaca-7b                     & 0.135 & \textbf{0.170} & \textbf{0.202} & 0.137 & 0.119 & 0.113 & \textbf{0.142} & 0.129 & 0.139 & 0.123 & \textbf{0.178} & 0.104 & 0.097 & \textbf{0.189} & 0.179 & 0.128 & 0.200 & 0.185 & 0.149 \\
        red002                        & \textbf{0.259} & 0.123 & 0.185 & \underline{\textbf{0.274}} & \textbf{0.173} & \textbf{0.204} & 0.132 & 0.145 & 0.167 & \textbf{0.181} & 0.161 & 0.178 & 0.182 & 0.143 & 0.151 & 0.148 & \textbf{0.221} & 0.177 & \textbf{0.214}  \\
        % minichat-13b-upd              & 0.259 & 0.123 & 0.185 & 0.274 & 0.173 & 0.204 & 0.132 & 0.145 & 0.167 & 0.181 & 0.161 & 0.178 & 0.182 & 0.143 & 0.151 & 0.148 & 0.201 & 0.177 & 0.214  \\
        \hline
        pythia-1.4b                   & \textbf{0.124} & \textbf{0.127} & \textbf{0.121} & \textbf{0.108} & \textbf{0.132} & \textbf{0.138} & 0.083   & \textbf{0.125} & \textbf{0.128} & \textbf{0.135} & 0.111 & 0.146 & 0.135 & \textbf{0.158} & \textbf{0.124} & \textbf{0.124} & \textbf{0.166} & 0.126 & 0.118 \\
        pythia-2.8b                   & 0.103 & 0.110 & 0.066 & 0.064 & 0.089 & 0.122 & 0.086   & 0.114 & 0.120 & 0.131 & 0.091 & 0.113 & 0.112 & 0.126 & 0.118 & 0.112 & 0.110 & \textbf{0.145} & 0.107 \\
        pythia-6.9b                   & 0.115 & 0.070 & 0.084 & 0.078 & 0.073 & 0.094 & 0.073   & 0.086 & 0.094 & 0.092 & 0.097 & 0.098 & 0.085 & 0.091 & 0.088 & 0.083 & 0.099 & 0.099 & 0.096 \\
        pythia-12b                    & 0.075 & 0.059 & 0.066 & 0.077 & 0.097 & 0.078 & \textbf{0.098}   & 0.102 & 0.126 & 0.132 & \textbf{0.125} & \textbf{0.147} & \textbf{0.159} & 0.079 & 0.098 & 0.110 & 0.094 & 0.120 & \textbf{0.120} \\
        \hline
        gpt-neox-20b                  & 0.081 & \textbf{0.132} & 0.086 & 0.086 & \textbf{0.096} & 0.069 & 0.094   & \textbf{0.140} & \textbf{0.103} & \textbf{0.109} & \textbf{0.120} & \textbf{0.098} & 0.085 & 0.088 & \textbf{0.101} & \textbf{0.116} & 0.099 & \textbf{0.113} & \textbf{0.156} \\
        h2ogpt-12b                    & 0.075 & 0.087 & 0.078 & 0.080 & 0.078 & \textbf{0.094} & 0.070   & 0.065 & 0.047 & 0.073 & 0.076 & 0.061 & \textbf{0.091} & 0.088 & 0.050 & 0.065 & 0.105 & 0.063 & 0.067 \\
        h2ogpt-20b                    & \textbf{0.114} & 0.098 & \textbf{0.110} & \textbf{0.094} & 0.084 & 0.061 & \textbf{0.096}   & 0.108 & 0.080 & 0.073 & 0.086 & 0.081 & 0.072 & \textbf{0.108} & 0.068 & 0.086 & \textbf{0.109} & 0.071 & 0.079 \\
        \hline
        dolly-3b                      & 0.066 & 0.060 & 0.055 & 0.079 & \textbf{0.083} & \textbf{0.077} & 0.066   & 0.100 & 0.090 & 0.083 & 0.091 & 0.093 & 0.085 & 0.079 & 0.063 & 0.077 & 0.076 & 0.074 & 0.084 \\
        dolly-7b                      & \textbf{0.095} & \textbf{0.068} & 0.052 & \textbf{0.091} & 0.079 & 0.070 & 0.108 & \textbf{0.108} & 0.089 & 0.092 & \textbf{0.111} & 0.095 & 0.100 & \textbf{0.096} & 0.059 & 0.086 & \textbf{0.123} & 0.085 & 0.090 \\
        dolly-12b                     & \textbf{0.095} & \textbf{0.068} & \textbf{0.093} & 0.085 & 0.071 & 0.073 & \textbf{0.114} & 0.098 & \textbf{0.106} & \textbf{0.103} & 0.094 & \textbf{0.114} & \textbf{0.106} & 0.086 & \textbf{0.088} & \textbf{0.098} & 0.088 & \textbf{0.102} & \textbf{0.116} \\
        \hline
        stablelm-3b                   & 0.070 & 0.085 & 0.071 & 0.086 & 0.082 & \textbf{0.099} & 0.096   & \textbf{0.101} & 0.087 & 0.091 & 0.083 & 0.092 & 0.067 & 0.069 & 0.089 & 0.081 & 0.066 & 0.085 & 0.088 \\
        stablelm-7b                   & \textbf{0.158} & \textbf{0.118} & \textbf{0.093} & \textbf{0.133} & \textbf{0.102} & 0.093 & \textbf{0.140}   & 0.085 & \textbf{0.118} & \textbf{0.122} & \textbf{0.123} & \textbf{0.130} & \textbf{0.095} & \textbf{0.123} & \textbf{0.103} & \textbf{0.100} & \textbf{0.134} & \textbf{0.121} & \textbf{0.105} \\
        \hline
        falcon-7b                     & 0.048 & 0.046 & 0.051 & 0.046 & 0.051 & 0.052 & 0.050   & 0.077 & \textbf{0.096} & \textbf{0.112} & \textbf{0.129} & \textbf{0.141} & \textbf{0.142} & 0.124 & 0.103 & 0.107 & \textbf{0.198} & \textbf{0.200} & \textbf{0.205} \\
        falcon-7b-instruct            & 0.078 & 0.095 & 0.106 & \textbf{0.114} & \textbf{0.095} & 0.079 & 0.104   & 0.075 & 0.083 & 0.087 & 0.060 & 0.133 & 0.123 & \textbf{0.160} & \textbf{0.203} & \textbf{0.156} & 0.141 & 0.167 & 0.152 \\
        falcon-40b                    & 0.038 & 0.043 & 0.077 & 0.085 & 0.090 & \textbf{0.129} & 0.087   & 0.069 & 0.056 & 0.053 & 0.065 & 0.063 & 0.058 & 0.059 & 0.077 & 0.066 & 0.085 & 0.063 & 0.076 \\
        falcon-40b-instruct           & \textbf{0.126} & \textbf{0.123} & \textbf{0.121} & 0.070 & 0.080 & 0.068 & \textbf{0.141} & \textbf{0.103} & 0.085 & 0.079 & 0.115 & 0.082 & 0.081 & 0.118 & 0.143 & 0.124 & 0.083 & 0.108 & 0.104 \\
        \hline
        &\multicolumn{19}{c}{Instruction For Ranking}\\
        \hline
        ChatGPT                       & 0.240 & 0.298 & 0.371 & 0.286 & 0.289 & 0.360 & 0.290   & 0.218 & 0.352 & 0.414 & 0.266 & 0.418 & 0.487 & 0.217 & 0.361 & 0.428 & 0.305 & 0.452 & 0.517  \\
        GPT-4                         & 0.402 & 0.415 & 0.517 & 0.413 & 0.410 & 0.486 & 0.404   & 0.392 & 0.429 & 0.490 & 0.453 & 0.496 & 0.565 & 0.396 & 0.434 & 0.495 & 0.463 & 0.506 & 0.576  \\
        \hline
        &\multicolumn{19}{c}{Statistic}\\
        \hline
        Performance-Average           & 0.120 & 0.117 & 0.125 & 0.113 & 0.114 & 0.124 & 0.111 & 0.140 & 0.140 & 0.145 & 0.144 & 0.148 & 0.152 & 0.145 & 0.145 & 0.150 & 0.156 & 0.157 & 0.166 \\
        Performance-Variance          & 0.062 & 0.068 & 0.087 & 0.067 & 0.065 & 0.078 & 0.064 & 0.058 & 0.070 & 0.082 & 0.067 & 0.082 & 0.095 & 0.067 & 0.080 & 0.090 & 0.078 & 0.092 & 0.104 \\
        \bottomrule
    \end{tabular}
    }
    \caption{
    The overall performance of all language models are listed in this table. All tested models are divided into broad groups sharing similar character. Bolded font indicates the best performing result within a group, and underlined font indicates the best performing result for the same data set with the same settings.
    }
    \label{tab:all-llm}
\end{table}
